Sample Efficient Subspace-based Representations for Nonlinear Meta-Learning

Constructing good representations is critical for learning complex tasks in a sample efficient manner. In the context of meta-learning, representations can be constructed from common patterns of previously seen tasks so that a future task can be learned quickly. While recent works show the benefit of subspace-based representations, such results are limited to linear-regression tasks. This work explores a more general class of nonlinear tasks with applications ranging from binary classification, generalized linear models and neural nets. We prove that subspace-based representations can be learned in a sample-efficient manner and provably benefit future tasks in terms of sample complexity. Numerical results verify the theoretical predictions in classification and neural-network regression tasks.

==> Icassp (3)/Paper/Paper_rebuttal.tex <==
We highly appreciate the comments from all reviewers, and we have updated the paper with proof in https://github.com/sunyue93/RLnonlinear/blob/main/RLnonlinear.pdf

1068

This paper analyzes the theoretical guarantee of nonlinear models in representation learning, specifically, training error of meta-training and generalization of few-shot learning. This is far more general than the papers discussing linear cases such as Kong et al, Tripuraneni et al., and we believe it can be applied in many machine learning tasks. We have mentioned the applications that relate to transfer learning in intro section, such as Deng et al, Bojar et al, Finn et al. In the experiment section we give simulations on image classification, where the same idea can be generalized to large datasets. We are going to run experiment in more complicated settings and illustrate the algorithm's performance. 

Comment for specific questions:
1. We will change the notations in experiment section so that they don't overlap with the theory part. In the experiments, we can treat the coefficients in the bottom layer as $\theta$, and the activations and upper layers provide the nonlinearities.
2. The first experiment is proposed to verify Theorem 3.2, the ability of the moment estimator to find the feature subspace. The reviewer is correct that we do not check the few-shot learning phase. For synthetic example, if the subspace is accurately retrieved and suppose we can find the optimal neural net model, then the few-shot learning is trivially accurate (because we generate the label-feature relevance by randomly picking the neural net coefficient, then we can recover the coefficients if the number of samples is bigger than the degree of freedom in few-shot learning phase). 3. P is mentioned in Assumption 1, which is a $r\times d$ matrix that brings the features from $d$ dimension to $r$ dimension. There are two ways of excecuting the learning: With representation learning, we use our proposed algorithm that computes a moment estimator $\hat M$ and its SVD truncation $\hat M_r$. Then the subspace is used as $\hat U_r$ and we only need to train $\hat f$; Without representation learning, we can go ahead solving $\min_{f,U} L(f,\hat U)$ where both $f$ and $U$ are variables. So the degree of freedom is higher than representation learning case and it requires more data.
Regarding the experiment, when we say "with representation" there is a learned $P$ that we hope is aligned with the underlying subspace $W$. When we say "without representation" we don't project the data onto a low dimensional subspace before few-shot learning, i.e., we keep the features as $d$ dimensional, thus the variable is $d$ dimensional and it's hard to recover with $O(r)$ samples.
4. $W$ and $P$ are different. We assume that $W$ is the function that connects $x$ and $y$. It is the true matrix that comes from nature. $P$ later is the subspace we constructed from our algorithm (which we hope to be close to $W$), and it is used to define the metric $L$. So whatever $P$ is, we can always write the loss with respect to $P$ and $f$.
5. We will correct correspondingly.

1BAA

Comment for specific questions:
1. We have updated the paper with proof at 
https://github.com/sunyue93/RLnonlinear/blob/main/RLnonlinear.pdf
Lemma 3.3 uses well-known Davis-Kahan bound to reveal the connection between error in $W$ and $M$. We will add the lemma to the paper. This is not a substantial change of paper but we agree that it's crucial to point out the connection of error in $M$ and $W$ clear.
2. That is true. Our algorithm is consisted of two phases: meta-training and few-shot learning. In meta-training, we use $O(d)$, more data from meta-training dataset to learn the low dimensional representation. This part by itself requires more data, but we prove that, with the representation learned, we can use $O(r)$, less data for training on the few-shot learning. If we don't run meta-training algorithm and directly learn from scratch on few-shot learning data, to reach the same error it would require $O(d)$ instead of $O(r)$ samples. We only run meta-training once with $O(d)$ samples, and this makes training on every few-shot learning tasks sample-efficient. So the requirement for sample complexity is saved a lot if there are many few-shot learning tasks that share the same low-dimensional subspace to be learned.


==> Icassp (3)/Paper/Paper_review.tex <==
1068

In the context of multi-task learning, the submitted paper offers a theoretical study in the context where all non-linear tasks are expressed in a common low-dimensional space. In this context of subspace-based representation, he explores the problem of few-shot learning. The results on the terminals are promising in the context studied and various simulations come to support the results. The merit of the article is to open the framework of meta-learning under the formal prism of the theory of non-asymptotic estimation. While such a study is interesting, I regret that the application perspective is not mentioned at all. It seems difficult to find application corresponding to work with around 1000 tasks. I also think that parts of the article are difficult to follow. 

1/ It's a bit of a shame to use the same W notation for the layer parameters and the transformation. Also, it is not clear to me the connection with the Theta parameters of the GLM, especially in the experimental phase. All these notations seem a little confusing to me.

2/ In the first set of simulations, it is logical and obvious that increase the number of tasks offer redundancy for observing the subspace. However, I don’t understand what is exactly the new task and where are the associated results? 

3/ Does this sentence « Observe that, without representation learning, one has to search for both f and P . However with representation learning, we fix P = Uˆ r and only search for f. » related to the last simulation (Fig. 3). It is not clear for me, you tell us « with and without the retrieved representations … » What is the matrix P?

4/ In definition 2.5, you start with the matrix W and then continue with P.

5/ In the eq. 2.7 the Log function of the first term is missing.


281E

The paper addresses the important problem of meta-learning and brings relevant contributions. The analyses are discussed with the help of experimental results obtained from synthetic data. I consider the work sound and pertinent. 


1BAA

1. Theorem 3.2 characterizes the error in the moment estimate \hat M, but the
final estimate required is for the subspace W. Where is the error for the 
rank r estimate \hat W characterized? In particular, the result in Theorem 3.4
is stated in terms of \|\hat W-W\| -- can the authors indicate how this
term behaves with respect to the problem dimensions? It can probably be handled
with some additional results from eigenvalue/eigenvector perturbation theory.


2. This is regarding the comment after Theorem 3.4. Although the few-shot 
learning step only requires roughly r samples, isn't the overall
requirement still dominated by the one from Theorem 3.2 (which amounts
to roughly d samples)? That is, even if the initial learning step can be used to 
enable multiple learning tasks in the second step, isn't it
only some constant gain when compared to learning each of them separately
(since the first step always requires d samples)? It would be useful
if the authors clarify this point.

==> Icassp (3)/Paper/notation.tex <==

\usepackage{hyperref,graphicx,amsmath,amsfonts,amssymb,bm,url,breakurl,epsfig,epsf,color,MnSymbol,mathbbol,fmtcount,semtrans,caption,subcaption,multirow,comment, boldline, enumitem}
%\usepackage[]{algorithm2e}
%\usepackage[noend]{algpseudocode}
\usepackage{wrapfig}
\usepackage{amssymb}

\usepackage[utf8]{inputenc} % allow utf-8 input
\usepackage[T1]{fontenc}    % use 8-bit T1 fonts
\usepackage{url}            % simple URL typesetting
\usepackage{booktabs}       % professional-quality tables
\usepackage{amsfonts}       % blackboard math symbols
\usepackage{nicefrac}       % compact symbols for 1/2, etc.
\usepackage{microtype}      % microtypography

\makeatletter
\providecommand*{\boxast}{%
  \mathbin{% as \boxplus and \boxtimes
    \mathpalette\@boxit{*}%
  }%
}
\newcommand*{\@boxit}[2]{%
  % #1: math style (\displaystyle, \textstyle, ...)
  % #2: symbol to be boxed that is centered around the math axis
  \sbox0{$\m@th#1\Box$}%
  % Manual correction for font bounding boxes:
  \ifx#1\displaystyle \ht0=\dimexpr\ht0+.05ex\relax \fi
  \ifx#1\textstyle \ht0=\dimexpr\ht0+.05ex\relax \fi
  \ifx#1\scriptstyle \ht0=\dimexpr\ht0+.04ex\relax \fi
  \ifx#1\scriptscriptstyle \ht0=\dimexpr\ht0+.065ex\relax \fi
  \sbox2{$#1\vcenter{}$}% \ht2 is positionn of math axis
  \rlap{%
    \hbox to \wd0{%
      \hfill
      \raisebox{%
        \dimexpr.5\dimexpr\ht0+\dp0\relax-\ht2\relax
      }{$\m@th#1#2$}%
      \hfill
    }%
  }%
  \Box
}
\makeatother

  \makeatletter
\def\BState{\State\hskip-\ALG@thistlm}
\makeatother


  \usepackage{mathtools}
\DeclarePairedDelimiter{\floor}{\lfloor}{\rfloor}

\usepackage{titlesec}

\usepackage{tikz}
\usepackage{pgfplots}
\usetikzlibrary{pgfplots.groupplots}

\setcounter{secnumdepth}{3}

\titleformat{\paragraph}
{\normalfont\normalsize\bfseries}{\theparagraph}{1em}{}
\titlespacing*{\paragraph}
{0pt}{3.25ex plus 1ex minus .2ex}{1.5ex plus .2ex}

\usepackage{movie15}

%\usepackage{caption}
\usepackage[bottom,hang,flushmargin]{footmisc} 

\setlength{\captionmargin}{30pt}

\newcommand{\tsn}[1]{{\left\vert\kern-0.25ex\left\vert\kern-0.25ex\left\vert #1 
    \right\vert\kern-0.25ex\right\vert\kern-0.25ex\right\vert}}

\definecolor{darkred}{RGB}{150,0,0}
\definecolor{darkgreen}{RGB}{0,150,0}
\definecolor{darkblue}{RGB}{0,0,200}
\hypersetup{colorlinks=true, linkcolor=darkred, citecolor=darkgreen, urlcolor=darkblue}

%--------------
\newtheorem{theorem}{Theorem}[section]
\newtheorem{result}{Result}
\newtheorem{problem}{Problem}
\newtheorem{claim}{Claim}
\newtheorem{assumption}{Assumption}
\newtheorem{question}{Question}
\newtheorem{lemma}[theorem]{Lemma}
\newtheorem{corollary}[theorem]{Corollary}
\newtheorem{propo}[theorem]{Proposition}
\newtheorem{definition}[theorem]{Definition}
\newtheorem{condition}[theorem]{Condition}
\newtheorem{conjecture}[theorem]{Conjecture}

\newtheorem{remark}[subsection]{Remark}
\newtheorem{remarks}[subsection]{Remarks}
\newtheorem{example}[subsection]{Example}

%% TT's definitions
\newcommand\tr{{{\operatorname{trace}}}}
\newcommand{\eps}{\varepsilon}
\newcommand{\epsr}{\varepsilon_R}
\newcommand{\mur}{\mu_R}
\newcommand{\bn}{\alpha}
\newcommand{\pp}{{\text{CL}}}
\newcommand{\distas}{\overset{\text{i.i.d.}}{\sim}}
\newcommand{\np}{{n\wedge p}}
\newcommand{\KB}{\bar{K}}
\newcommand{\bG}{\boldsymbol{\Gamma}}
\newcommand{\xw}{\x_{\w}}
\newcommand{\xv}{\x_{\vb}}
\newcommand{\xu}{\x_{\ub}}
\newcommand{\xvt}[1]{\x_{\vb_{#1}}}
\newcommand{\xvtt}[1]{\x_{\vb,#1}}
\newcommand{\xwt}[1]{\x_{#1,\w}}
\newcommand{\xws}[1]{\x_{#1,\ws}}
\newcommand{\xs}{\x_{\ws}}
\newcommand{\yst}{\hat{\y}}
\newcommand{\st}{\star}
\newcommand{\eig}{\text{eigvec}}
\newcommand{\hu}{h}
\newcommand{\ru}{r}
\newcommand{\pbar}{{{\bar{p}}}}
\newcommand{\pbd}{p}
\newcommand{\lay}[1]{{\vct{k}}^{(#1)}}
\newcommand{\lah}[1]{{\vct{\hat{k}}}^{(#1)}}
\newcommand{\lan}{\vct{k}}
\newcommand{\cmp}{P_{\text{nn}}}
\newcommand{\rest}{{\bf{r}}}
\newcommand{\dcp}{\vct{d}^{\text{cnn}}}
\newcommand{\fcp}{\vct{g}^{\text{CNN}}}
\newcommand{\beq}{\begin{equation}}
\newcommand{\nrest}{\bar{n}}
\newcommand{\eeq}{\end{equation}}
\newcommand{\prox}{{{\text{\bf{prox}}}}}
\newcommand{\cov}{{{\text{\bf{cov}}}}}
\newcommand{\ex}{{{\text{\bf{ex}}}}}
\newcommand{\modu}{{{\text{{mod}}}}}
\newcommand{\map}{{{\text{\bf{map}}}}}
\newcommand{\var}[1]{{{\text{\bf{var}}}}[#1]}
\newcommand{\vrn}{\nu}
\newcommand{\func}[1]{{f_{\text{CNN}}}(#1)}
\newcommand{\funh}[1]{{{\hat{f}}_{\text{CNN}}}(#1)}
\newcommand{\funcp}[1]{{f'_{\text{cnn}}}(#1)}
\newcommand{\funcw}[1]{{{{f}}'_{\text{cnn}}}(#1)}
\newcommand{\dev}{{{\text{\bf{dev}}}}}
\newcommand{\meas}{{{\text{\bf{mean}}(\sigma)}}}
\newcommand{\nn}{\nonumber}
\newcommand{\la}{\lambda}
\newcommand{\K}{{K}}
\newcommand{\A}{{\mtx{A}}}
\newcommand{\sfmx}[1]{\text{sfmx}(#1)}
\newcommand{\cat}[1]{\text{Cat}(#1)}
\newcommand{\amp}{\alpha_{\text{cnn}}}
\newcommand{\bOt}{\bigotimes}
\newcommand{\bt}{\boldsymbol{\theta}}
\newcommand{\Bt}{\boldsymbol{\Theta}}
%\newcommand{\nt}{\boldsymbol{n}}

%\newcommand{\bt}{\times}
\newcommand{\robt}[1]{\bigotimes_{\ell=1}^D{#1}_{\ell}}
\newcommand{\robtu}[1]{\bigotimes_{\ell=1}^D{#1}^{(\ell)}}
\newcommand{\bd}{\bigodot}
\newcommand{\kal}{\prod_{i=1}^{D-1}\tn{\lay{i}}}
%\newcommand{\kall}[1]{\prod_{i=1}^{#1}\tn{\lay{i}}}
\newcommand{\kall}[1]{1_{\lan #1}}
\newcommand{\lall}[1]{{\order{\lip_{\lan #1}}}}%{L^{#1}\prod_{i=1}^{#1}\tn{\lay{i}}}
\newcommand{\lell}[1]{{\lip}_{\lan #1}}
\newcommand{\bell}[1]{{{{\beta}}}_{\lan #1}}
\newcommand{\Ub}{{\mtx{U}}}
\newcommand{\Ubb}{{\mtx{U}}}
\newcommand{\V}{{\mtx{V}}}
\newcommand{\ten}{(\{\vb_\ell\}_{\ell=1}^D)}
\newcommand{\uten}{(\{\ub_\ell\}_{\ell=1}^D)}
\newcommand{\ken}{(\{\lay{i}\}_{i=1}^D)}
\newcommand{\B}{{{\mtx{B}}}}
\newcommand{\alx}{{{\alpha_\X}}}
\newcommand{\aly}[1]{{{\alpha_{\X_{#1}}}}}
\newcommand{\Ib}{{{\mtx{I}}}}
\newcommand{\Xbin}{{{\mtx{B}}}}
\newcommand{\Gbin}{{{\mtx{S}}}}
\newcommand{\xbin}{{{\mtx{b}}}}
\newcommand{\Sb}{{{\mtx{S}}}}
\newcommand{\Gb}{{\mtx{G}}}
\newcommand{\ymean}{{\bar{\y}(\w;\text{avg})}}
\newcommand{\yavg}{{{y}_{\text{avg}}}}
\newcommand{\ravg}[1]{{{r}_{{\text{avg}}}(#1)}}
\newcommand{\fmean}{{\funcw{\w;\text{avg}}}}
\newcommand{\diag}[1]{\text{diag}(#1)}
\newcommand{\out}{\text{out}}
\newcommand{\linest}{\text{lin}}
\newcommand{\inp}{\text{in}}
\newcommand{\inh}{\hat{\text{in}}}
\newcommand{\sexp}{subexponential }
\newcommand{\Lc}{{\cal{L}}}
\newcommand{\Nc}{{\cal{N}}}
\newcommand{\Jc}{{\cal{J}}}
\newcommand{\Jcb}{{\overline{\cal{J}}}}
\newcommand{\Dc}{{\cal{D}}}
\newcommand{\Dcg}[1]{{\cal{D}}^{#1}_{\text{subg}}}
\newcommand{\Dct}{{\tilde{\cal{D}}}}
\newcommand{\Sct}{{\tilde{\cal{S}}}}
%\newcommand{\smn}{\s_{\min}}
\newcommand{\btd}{{\bt_{\ell=1}^D d_\ell}}
\newcommand{\Ro}{{\cal{RO}}}
\newcommand{\PC}{{\cal{PC}}}
\newcommand{\Pb}{{\mtx{P}}}
\newcommand{\Tb}{{\mtx{T}}}
\newcommand{\Kba}{{\vct{k}}_{\text{all}}}
\newcommand{\Qb}{{\mtx{Q}}}
\newcommand{\rng}{\gamma}
\newcommand{\Cb}{{\mtx{C}}}
\newcommand{\Eb}{{\mtx{E}}}
\newcommand{\Hb}{{\mtx{H}}}
\newcommand{\Gc}{{\cal{G}}}
\newcommand{\F}{{\mtx{F}}}
\newcommand{\diff}{{\text{diff}}}
\newcommand{\La}{{\boldsymbol{{\Lambda}}}}
%\newcommand{\noresamp}[1]{{\textcolor{red}{#1}}}
\newcommand{\noresamp}[1]{{\textcolor{red}{#1}}}
\newcommand{\sigmap}{\phi'}
\newcommand{\sigmal}[1]{\sigma^{(#1)}}
\newcommand{\sigmalp}[1]{\sigma'^{(#1)}}
\newcommand{\sigmaa}{\sigma'_{\text{all}}}
\newcommand{\sigmai}[1]{\sigma'_{\text{all},#1}}
\newcommand{\bSi}{{\boldsymbol{{\Sigma}}}}
\newcommand{\bSit}{{\boldsymbol{{\tilde{\Sigma}}}}}
\newcommand{\bSih}{{\boldsymbol{{\hat{\Sigma}}}}}
\newcommand{\bmu}{{\boldsymbol{{\mu}}}}
\newcommand{\Db}{{\mtx{D}}}
\newcommand{\db}{{\vct{d}}}
\newcommand{\oneb}{{\mathbb{1}}}
\newcommand{\onebb}{{\mathbf{1}}}
\newcommand{\Iden}{{\mtx{I}}}
\newcommand{\M}{{\mtx{M}}}
\newcommand{\gm}{\gamma_m}
\newcommand{\order}[1]{{\cal{O}}(#1)}
\newcommand{\rmax}[1]{{\bf{r}_{\max}(#1)}}
\newcommand{\rbmax}[1]{{\bf{\bar{r}}_{\max}(#1)}}
\newcommand{\rmin}[1]{{\bf{r}_{\min}(#1)}}
\newcommand{\smn}[1]{{s_{\min}(#1)}}
\newcommand{\smx}[1]{{s_{\max}(#1)}}
\newcommand{\z}{{\vct{z}}}
\newcommand{\zb}{{\bar{\z}}}
\newcommand{\el}{{\ell}}
\newcommand{\tn}[1]{\|{#1}\|_{\ell_2}}
\newcommand{\tff}[1]{\|{#1}\|_{\ell_4}}
\newcommand{\tin}[1]{\|{#1}\|_{\ell_\infty}}
\newcommand{\trow}[1]{\|{#1}\|_{2,\infty}}
\newcommand{\bad}{{\bar{d}}}
\newcommand{\Dp}{{D^+}}
\newcommand{\tf}[1]{\|{#1}\|_{F}}
\newcommand{\te}[1]{\|{#1}\|_{\psi_1}}
\newcommand{\tsub}[1]{\|{#1}\|_{\psi_2}}
\newcommand{\tsut}[1]{\|{#1}\|_{\psi_{2/3}}}
\newcommand{\tsup}[1]{\|{#1}\|_{\psi_a}}
\newcommand{\dist}[1]{\text{dist}(#1)}
\newcommand{\upp}{{\cal{B}}_{\alpha,\Gamma}}
\newcommand{\upz}{{\cal{B}}_{\alpha_0,\Gamma}}
\newcommand{\dpz}{{\cal{D}}_{\alpha_0,\Gamma}}
\newcommand{\dpp}{{\cal{D}}_{\alpha,\Gamma}}
\newcommand{\mpp}{M_{\alpha,\Gamma}}
%\newcommand{\supp}[1]{\text{supp}(#1)}
\newcommand{\cone}[1]{{\text{cone}(#1)}}
\newcommand{\paf}{\partial f(\x)}
\newcommand{\Cc}{\mathcal{C}}
\newcommand{\Ac}{\mathcal{A}}
\newcommand{\Ccb}{\bar{\mathcal{C}}}
\newcommand{\Xc}{\mathcal{X}}
\newcommand{\xc}{{\text{excess}}}
\newcommand{\Rc}{\mathcal{R}}
\newcommand{\Rcp}{\mathcal{\bar{R}}'}
\newcommand{\Rcb}{\mathcal{N}}
\newcommand{\btrue}{\bbeta_{true}}
\newcommand{\bteta}{\boldsymbol{\theta}}
\newcommand{\bbteta}{\widetilde{\boldsymbol{\theta}}}
\newcommand{\brteta}{\overline{\boldsymbol{\theta}}}
\newcommand{\bbeta}{{\boldsymbol{\beta}}}
\newcommand{\ddelta}{{\boldsymbol{\delta}}}
\newcommand{\babeta}{{\bar{\beta}}}
\newcommand{\balpha}{{\bar{\alpha}}}
\newcommand{\bgamma}{{\bar{\gamma}}}
\newcommand{\Bc}{\mathcal{B}}
\newcommand{\Sc}{\mathcal{S}}
\newcommand{\Mc}{\mathcal{M}}
\newcommand{\pa}{{\partial}}
\newcommand{\Nn}{\mathcal{N}}
\newcommand{\pol}{^\circ}
\newcommand{\vb}{\vct{v}}
\newcommand{\Jb}{\mtx{J}}
\newcommand{\Jt}{\mtx{\tilde{J}}}
\newcommand{\vbl}{\vct{v}^{\text{lin}}}
\newcommand{\fb}{\vct{f}}
\newcommand{\ib}{{\bf{i}}}
\newcommand{\hib}{{\bf{\hat{i}}}}
\newcommand{\Ic}{{\mathcal{I}}}
\newcommand{\all}{{\text{all}}}
\newcommand{\vh}{\vct{\hat{v}}}
\newcommand{\vbb}{\vct{\bar{v}}}
\newcommand{\Xb}{\mtx{\bar{X}}}
\newcommand{\abb}{\mtx{\bar{a}}}
\newcommand{\cb}{\mtx{c}}
\newcommand{\bbb}{\mtx{\bar{b}}}
\newcommand{\w}{\vct{w}}
\newcommand{\err}[1]{\text{Err}_{\Dc}(#1)}
\newcommand{\Wp}{\mtx{W}^\dagger}
\newcommand{\tilW}{\widetilde{\mtx{W}}}
\newcommand{\tilw}{\widetilde{\vct{w}}}
\newcommand{\ob}{\mtx{o}}
\newcommand{\obh}{\mtx{\hat{o}}}
\newcommand{\wh}{{\hat{\mtx{w}}}}
\newcommand{\li}{\left<}
\newcommand{\ri}{\right>}
\newcommand{\s}{\vct{s}}
\newcommand{\sh}{\hat{\vct{s}}}
\newcommand{\ab}{\vct{a}}
\newcommand{\bb}{\vct{b}}
\newcommand{\ub}{{\vct{u}}}
\newcommand{\ubb}{\bar{\vct{u}}}
\newcommand{\h}{\vct{h}}
\newcommand{\hh}{{\vct{h}}}
\newcommand{\g}{{\vct{g}}}
\newcommand{\ii}{{\vct{i}}}
\newcommand{\zm}[1]{{\text{{\bf{zm}}}(#1)}}
\newcommand{\dd}{{\vct{d}}}
\newcommand{\ddt}{{\vct{d}}_\tau}
\newcommand{\Zb}{\mtx{Z}}
\newcommand{\hf}{\hat{f}}
\newcommand{\corrCA}{\rho_\Cc(\M)}
\newcommand{\corr}[1]{{\bf{cor}}(#1)}
\newcommand{\Tc}{\mathcal{T}}
\newcommand{\Fc}{\mathcal{F}}
\newcommand{\Hc}{\mathcal{H}}


%%YP's macros
\newcommand{\qqq}[1]{{\textcolor{red}{?{#1}?}}}
\newcommand{\ihere}{{\textcolor{red}{I AM HERE! }}}
\newcommand{\mat}[1]{{\text{mat}{#1}}}
\newcommand{\gb}{\bar{\g}}
\newcommand{\bs}{\bar{s}}
\newcommand{\cgain}{\alpha_{\text{CNN}}}
\newcommand{\cgainp}{\tn{\E_{\x\sim\Nn(0,\Iden)}[\gcnn{}]}}
\newcommand{\gcnn}[1]{{\vct{g}}_{\text{cnn}#1}}
\newcommand{\ccorr}{\rho_{\text{cnn}}}
\newcommand{\kb}{\vct{k}}
\newcommand{\xh}{\hat{\x}}
\newcommand{\yh}{\hat{\y}}
\newcommand{\xbr}{\bar{\h}}
\newcommand{\xdr}{\tilde{\x}}
\newcommand{\m}{\vct{m}}
\newcommand{\xt}{\tilde{\x}}
\newcommand{\nt}{\tilde{n}}
%\newcommand{\ht}{\tilde{h}}
\newcommand{\rt}{\tilde{r}}
\newcommand{\ft}{\tilde{f}}
\newcommand{\yt}{\tilde{\y}}
\newcommand{\gh}{\hat{\g}}
\newcommand{\gt}{\tilde{\g}}
\newcommand{\wb}{\bar{\w}}
\newcommand{\lip}{L}
\newcommand{\mipp}{L_{\max}}
\newcommand{\mupp}{\bar{\mu}_{\max}}
\newcommand{\mapp}{\mu}
\newcommand{\tcnn}{{\mtx{T}}_{\text{cnn}}}
\newcommand{\lcnn}{{\mtx{L}}_{\text{CNN}}}
\newcommand{\lipa}{{L}}
\newcommand{\smo}{S}
\newcommand{\SM}{{{\bf{S}}}_{L,\kb}}
\newcommand{\SMB}{{{\bf{\bar{S}}}}_{L,\kb}}
\newcommand{\Ws}{\W^\star}
\newcommand{\ws}{{\w^\star}}
\newcommand{\wss}{{\w^\star}}
\newcommand{\yp}[1]{\textcolor{red}{ #1}}
\newcommand{\zeronorm}[1]{\left\|#1 \right\|_0}
\newcommand{\unorm}[1]{\left\|#1 \right\|_u}
\newcommand{\ynorm}[1]{\left\|#1 \right\|_{\bar{y}}}
\newcommand{\onetwonorm}[1]{\left\|#1\right\|_{1,2}}
\newcommand{\opnorm}[1]{\left\|#1\right\|}
\newcommand{\fronorm}[1]{\left\|#1\right\|_{F}}
\newcommand{\onenorm}[1]{\left\|#1\right\|_{\ell_1}}
\newcommand{\twonorm}[1]{\left\|#1\right\|_{\ell_2}}
\newcommand{\wnorm}[2]{\left\|#1\right\|_{#2}}
\newcommand{\Dnorm}[1]{\left\|#1\right\|_{D}}
\newcommand{\oneinfnorm}[1]{\left\|#1\right\|_{1,\infty}}
\newcommand{\infnorm}[1]{\left\|#1\right\|_{\ell_\infty}}
\newcommand{\nucnorm}[1]{\left\|#1\right\|_*}
\newcommand{\abs}[1]{\left|#1\right|}
\newcommand{\avg}[1]{\left< #1 \right>}

\newcommand{\lipp}{\prod_{\ell=1}^D \twonorm{\vct{k}^{(\ell)}}}

\renewcommand{\d}{\mathrm{d}}

\newcommand{\cA}{\mathcal{A}}
\newcommand{\rotd}{\text{R1TD}}
\newcommand{\nntd}{\text{DeepTD}}
\newcommand{\x}{\vct{x}}
\newcommand{\rb}{\vct{r}}
\newcommand{\rbb}{\vct{\widetilde{r}}}
\newcommand{\y}{\vct{y}}
\newcommand{\ybh}{\vct{\hat{y}}}
\newcommand{\W}{\mtx{W}}
\newcommand{\Wc}{{\cal{W}}}
\newcommand{\Vc}{{\cal{V}}}
\newcommand{\bgl}{{~\big |~}}

%--------------

% EJC's macros

\definecolor{emmanuel}{RGB}{255,127,0}
\newcommand{\ejc}[1]{\textcolor{emmanuel}{EJC: #1}}

\newcommand{\p}{{\vct{p}}}
\newcommand{\Kb}{{\mtx{K}}}
\newcommand{\somelog}{16\Kb\log (\Kb)}
\newcommand{\somelg}{\Kb\log (\Kb)}
\newcommand{\pb}{{\vct{p}}}
\newcommand{\qb}{{\vct{q}}}
\newcommand{\R}{\mathbb{R}}
\newcommand{\Pro}{\mathbb{P}}
\newcommand{\C}{\mathbb{C}}
\newcommand{\Z}{\mathbb{Z}}
\newcommand{\<}{\langle}
\renewcommand{\>}{\rangle}
\newcommand{\Var}{\textrm{Var}}
\newcommand{\sgn}[1]{\textrm{sgn}(#1)}
\renewcommand{\P}{\operatorname{\mathbb{P}}}
%\newcommand{\E}{\operatorname{\mathbb{E}}}
\newcommand{\EE}{\operatorname{\mathbb{E}}}
%\newcommand{\var}{\operatorname{\mathbf{var}}}

\newcommand{\todo}[1]{{\bf TODO: #1}}
\newcommand{\grad}[1]{{\nabla\Lc(#1)}}
\newcommand{\gradf}[1]{{\nabla f(#1)}}
\newcommand{\hessf}[1]{{\nabla^2f(#1)}}
\newcommand{\gradw}[1]{{\nabla{\Lc}(#1)}}
\newcommand{\grd}[2]{{\nabla\Lc_{#1}(#2)}}
\newcommand{\e}{\mathrm{e}}
\newcommand{\eb}{\vct{e}}
\renewcommand{\i}{\imath}

\newcommand{\vct}[1]{\bm{#1}}
\newcommand{\mtx}[1]{\bm{#1}}

% MS's macros

\newcommand{\rank}{\operatorname{rank}}
\newcommand{\supp}[1]{\operatorname{supp}(#1)}
\newcommand{\restrict}[1]{\big\vert_{#1}}
\newcommand{\Id}{\text{\em I}}
\newcommand{\OpId}{\mathcal{I}}

\newcommand{\Real}{\operatorname{Re}}
\newcommand{\Imag}{\operatorname{Im}}

\newcommand{\piyp}{\pi'_1(\vct{y})}
\newcommand{\piy}{\pi_1(\vct{y})}
\newcommand{\piar}{\pi_1(\vct{a}_r)}
\newcommand{\piarp}{\pi'_1(\vct{a}_r)}
\newcommand{\set}{{\cal{F}}}
\newcommand{\des}{{\x_0}}

\newcommand{\Pc}{{\cal{P}}}
\newcommand{\X}{{\mtx{X}}}
\newcommand{\Y}{{\mtx{Y}}}
\newcommand{\Vb}{{\mtx{V}}}
\newcommand{\Vh}{\hat{{\mtx{V}}}}
\newcommand{\Vbd}{{\mtx{V}^\dagger}}
\newcommand{\Rb}{{\mtx{R}}}

\newcommand{\calF}{\mathcal{I}}
\newcommand{\calS}{\mathcal{N}}


\newcommand{\MS}[1]{\textcolor{blue}{MS: #1}}
\newcommand{\MST}[1]{\textcolor{red}{#1}}
\newcommand{\SO}[1]{\textcolor{darkgreen}{SO: #1}}


\numberwithin{equation}{section} 

\def \endprf{\hfill {\vrule height6pt width6pt depth0pt}\medskip}
%\newenvironment{proof}{\noindent {\bf Proof} }{\endprf\par}
\newenvironment{proofsk}{\noindent {\bf Proof sketch} }{\endprf\par}


%\newcommand{\qed}{{\unskip\nobreak\hfil\penalty50\hskip2em\vadjust{}
           %\nobreak\hfil$\Box$\parfillskip=0pt\finalhyphendemerits=0\par}}


\newcommand{\note}[1]{{\bf [{\em Note:} #1]}}

\newcommand{\iprod}[2]{\left\langle #1 , #2 \right\rangle}

\newcommand{\red}{\textcolor{red}}
\newcommand{\gi}{\ab_{\gamma_i}}
\newcommand{\ang}{\text{ang}}
\newcommand{\ham}[2]{{\|#1,#2\|_H}}

%\renewcommand{\algorithmicrequire}{\textbf{Input:}}
%\renewcommand{\algorithmicensure}{\textbf{Output:}}

%AJ's macros
\newcommand{\hth}{{\widehat{\boldsymbol{\theta}}}}
\newcommand{\bth}{{\boldsymbol{\theta}}}
\newcommand\cL{\mathcal{L}}
\newcommand\cD{\mathcal{D}}
\newcommand\hcD{\widehat{\cD}}
\newcommand\reals{\mathbb{R}}
\newcommand\bSigma{\boldsymbol{\Sigma}}
\newcommand\normal{{\sf N}}
\newcommand\bdelta{\boldsymbol{\delta}}
\newcommand\sign{{\rm sign}}
\newcommand\sT{{\sf T}}
\newcommand\I{\mtx{I}}
\newcommand\zero{\mtx{0}}
\newcommand\bA{\mtx{A}}
\newcommand\bv{\mtx{v}}
\newcommand\cI{\mathcal{I}}
\newcommand\bz{\boldsymbol{z}}
\newcommand\bg{\boldsymbol{g}}
\newcommand\ba{\boldsymbol{a}}
\def\cC{\mathcal{C}}
\def\de{{\rm d}}
\def\bM{\mtx{M}}
\def\cH{\mathcal{H}}
\def\bu{\boldsymbol{u}}
\def\by{\boldsymbol{y}}
\def\bw{\boldsymbol{w}}
\def\bX{\boldsymbol{X}}
\def\tbX{\tilde{\boldsymbol{X}}}
\def\tbx{\tilde{\boldsymbol{x}}}
\def\tbth{\tilde{\boldsymbol{\theta}}}
\def\hz{\widehat{z}}
\def\ind{\mathbf{1}}
\def\cS{\mathcal{S}}
\def\prob{\mathbb{P}}
\def\tx{\tilde{x}}
\def\reals{\mathbb{R}}
\newcommand{\aj}[1]{\noindent{\textcolor{blue}{\textbf{\#\#\# AJ:} \textsf{#1} \#\#\#}}}

\newcommand{\gauss}{\mathcal{N}(0,I)}
\newcommand{\gausscov}[1]{\mathcal{N}(0,{#1})}
\newcommand{\argmin}{\mathop{\mathrm{argmin}}}
%\newcommand{\cLCE}{\cL_{\mathrm{CE}}}
\newcommand{\cLCE}{\cL}
\newcommand{\mscrU}{{\mathscr{U}}}

==> Icassp (3)/Paper/notation_new.tex <==

\usepackage{hyperref,graphicx,amsmath,amsfonts,amssymb,bm,url,breakurl,epsfig,epsf,color,MnSymbol,mathbbol,fmtcount,semtrans,caption,subcaption,multirow,comment, boldline, enumitem}
%\usepackage[]{algorithm2e}
%\usepackage[noend]{algpseudocode}
\usepackage{wrapfig}
\usepackage{amssymb}


\makeatletter
\providecommand*{\boxast}{%
  \mathbin{% as \boxplus and \boxtimes
    \mathpalette\@boxit{*}%
  }%
}
\newcommand*{\@boxit}[2]{%
  % #1: math style (\displaystyle, \textstyle, ...)
  % #2: symbol to be boxed that is centered around the math axis
  \sbox0{$\m@th#1\Box$}%
  % Manual correction for font bounding boxes:
  \ifx#1\displaystyle \ht0=\dimexpr\ht0+.05ex\relax \fi
  \ifx#1\textstyle \ht0=\dimexpr\ht0+.05ex\relax \fi
  \ifx#1\scriptstyle \ht0=\dimexpr\ht0+.04ex\relax \fi
  \ifx#1\scriptscriptstyle \ht0=\dimexpr\ht0+.065ex\relax \fi
  \sbox2{$#1\vcenter{}$}% \ht2 is positionn of math axis
  \rlap{%
    \hbox to \wd0{%
      \hfill
      \raisebox{%
        \dimexpr.5\dimexpr\ht0+\dp0\relax-\ht2\relax
      }{$\m@th#1#2$}%
      \hfill
    }%
  }%
  \Box
}
\makeatother

  \makeatletter
\def\BState{\State\hskip-\ALG@thistlm}
\makeatother


  \usepackage{mathtools}
\DeclarePairedDelimiter{\floor}{\lfloor}{\rfloor}

%\usepackage{titlesec}

\usepackage{tikz}
\usepackage{pgfplots}
\usetikzlibrary{pgfplots.groupplots}

\setcounter{secnumdepth}{3}


\usepackage{movie15}

%\usepackage{caption}
\usepackage[bottom,hang,flushmargin]{footmisc} 

\setlength{\captionmargin}{30pt}

\newcommand{\tsn}[1]{{\left\vert\kern-0.25ex\left\vert\kern-0.25ex\left\vert #1 
    \right\vert\kern-0.25ex\right\vert\kern-0.25ex\right\vert}}

\definecolor{darkred}{RGB}{150,0,0}
\definecolor{darkgreen}{RGB}{0,150,0}
\definecolor{darkblue}{RGB}{0,0,200}
\hypersetup{colorlinks=true, linkcolor=darkred, citecolor=darkgreen, urlcolor=darkblue}

%--------------

\newtheorem{theorem}{Theorem}[section]
\newtheorem{result}{Result}
\newtheorem{problem}{Problem}
\newtheorem{claim}{Claim}
\newtheorem{assumption}{Assumption}
\newtheorem{question}{Question}
\newtheorem{lemma}[theorem]{Lemma}
\newtheorem{corollary}[theorem]{Corollary}
\newtheorem{propo}[theorem]{Proposition}
\newtheorem{definition}[theorem]{Definition}
\newtheorem{condition}[theorem]{Condition}
\newtheorem{conjecture}[theorem]{Conjecture}

\newtheorem{remark}[subsection]{Remark}
\newtheorem{remarks}[subsection]{Remarks}
\newtheorem{example}[subsection]{Example}

%% TT's definitions
\newcommand\tr{{{\operatorname{trace}}}}
\newcommand{\eps}{\varepsilon}
\newcommand{\epsr}{\varepsilon_R}
\newcommand{\mur}{\mu_R}
\newcommand{\bn}{\alpha}
\newcommand{\pp}{{\text{CL}}}
\newcommand{\distas}{\overset{\text{i.i.d.}}{\sim}}
\newcommand{\np}{{n\wedge p}}
\newcommand{\KB}{\bar{K}}
\newcommand{\bG}{\boldsymbol{\Gamma}}
\newcommand{\xw}{\x_{\w}}
\newcommand{\xv}{\x_{\vb}}
\newcommand{\xu}{\x_{\ub}}
\newcommand{\xvt}[1]{\x_{\vb_{#1}}}
\newcommand{\xvtt}[1]{\x_{\vb,#1}}
\newcommand{\xwt}[1]{\x_{#1,\w}}
\newcommand{\xws}[1]{\x_{#1,\ws}}
\newcommand{\xs}{\x_{\ws}}
\newcommand{\yst}{\hat{\y}}
\newcommand{\st}{\star}
\newcommand{\eig}{\text{eigvec}}
\newcommand{\hu}{h}
\newcommand{\ru}{r}
\newcommand{\pbar}{{{\bar{p}}}}
\newcommand{\pbd}{p}
\newcommand{\lay}[1]{{\vct{k}}^{(#1)}}
\newcommand{\lah}[1]{{\vct{\hat{k}}}^{(#1)}}
\newcommand{\lan}{\vct{k}}
\newcommand{\cmp}{P_{\text{nn}}}
\newcommand{\rest}{{\bf{r}}}
\newcommand{\dcp}{\vct{d}^{\text{cnn}}}
\newcommand{\fcp}{\vct{g}^{\text{CNN}}}
\newcommand{\beq}{\begin{equation}}
\newcommand{\nrest}{\bar{n}}
\newcommand{\eeq}{\end{equation}}
\newcommand{\prox}{{{\text{\bf{prox}}}}}
\newcommand{\cov}{{{\text{\bf{cov}}}}}
\newcommand{\ex}{{{\text{\bf{ex}}}}}
\newcommand{\modu}{{{\text{{mod}}}}}
\newcommand{\map}{{{\text{\bf{map}}}}}
\newcommand{\var}[1]{{{\text{\bf{var}}}}[#1]}
\newcommand{\vrn}{\nu}
\newcommand{\func}[1]{{f_{\text{CNN}}}(#1)}
\newcommand{\funh}[1]{{{\hat{f}}_{\text{CNN}}}(#1)}
\newcommand{\funcp}[1]{{f'_{\text{cnn}}}(#1)}
\newcommand{\funcw}[1]{{{{f}}'_{\text{cnn}}}(#1)}
\newcommand{\dev}{{{\text{\bf{dev}}}}}
\newcommand{\meas}{{{\text{\bf{mean}}(\sigma)}}}
\newcommand{\nn}{\nonumber}
\newcommand{\la}{\lambda}
\newcommand{\K}{{K}}
\newcommand{\A}{{\mtx{A}}}
\newcommand{\sfmx}[1]{\text{sfmx}(#1)}
\newcommand{\cat}[1]{\text{Cat}(#1)}
\newcommand{\amp}{\alpha_{\text{cnn}}}
\newcommand{\bOt}{\bigotimes}
\newcommand{\bt}{\boldsymbol{\theta}}
\newcommand{\Bt}{\boldsymbol{\Theta}}
%\newcommand{\nt}{\boldsymbol{n}}

%\newcommand{\bt}{\times}
\newcommand{\robt}[1]{\bigotimes_{\ell=1}^D{#1}_{\ell}}
\newcommand{\robtu}[1]{\bigotimes_{\ell=1}^D{#1}^{(\ell)}}
\newcommand{\bd}{\bigodot}
\newcommand{\kal}{\prod_{i=1}^{D-1}\tn{\lay{i}}}
%\newcommand{\kall}[1]{\prod_{i=1}^{#1}\tn{\lay{i}}}
\newcommand{\kall}[1]{1_{\lan #1}}
\newcommand{\lall}[1]{{\order{\lip_{\lan #1}}}}%{L^{#1}\prod_{i=1}^{#1}\tn{\lay{i}}}
\newcommand{\lell}[1]{{\lip}_{\lan #1}}
\newcommand{\bell}[1]{{{{\beta}}}_{\lan #1}}
\newcommand{\Ub}{{\mtx{U}}}
\newcommand{\Ubb}{{\mtx{U}}}
\newcommand{\V}{{\mtx{V}}}
\newcommand{\ten}{(\{\vb_\ell\}_{\ell=1}^D)}
\newcommand{\uten}{(\{\ub_\ell\}_{\ell=1}^D)}
\newcommand{\ken}{(\{\lay{i}\}_{i=1}^D)}
\newcommand{\B}{{{\mtx{B}}}}
\newcommand{\alx}{{{\alpha_\X}}}
\newcommand{\aly}[1]{{{\alpha_{\X_{#1}}}}}
\newcommand{\Ib}{{{\mtx{I}}}}
\newcommand{\Xbin}{{{\mtx{B}}}}
\newcommand{\Gbin}{{{\mtx{S}}}}
\newcommand{\xbin}{{{\mtx{b}}}}
\newcommand{\Sb}{{{\mtx{S}}}}
\newcommand{\Gb}{{\mtx{G}}}
\newcommand{\ymean}{{\bar{\y}(\w;\text{avg})}}
\newcommand{\yavg}{{{y}_{\text{avg}}}}
\newcommand{\ravg}[1]{{{r}_{{\text{avg}}}(#1)}}
\newcommand{\fmean}{{\funcw{\w;\text{avg}}}}
\newcommand{\diag}[1]{\text{diag}(#1)}
\newcommand{\out}{\text{out}}
\newcommand{\linest}{\text{lin}}
\newcommand{\inp}{\text{in}}
\newcommand{\inh}{\hat{\text{in}}}
\newcommand{\sexp}{subexponential }
\newcommand{\Lc}{{\cal{L}}}
\newcommand{\Nc}{{\cal{N}}}
\newcommand{\Jc}{{\cal{J}}}
\newcommand{\Jcb}{{\overline{\cal{J}}}}
\newcommand{\Dc}{{\cal{D}}}
\newcommand{\Dcg}[1]{{\cal{D}}^{#1}_{\text{subg}}}
\newcommand{\Dct}{{\tilde{\cal{D}}}}
\newcommand{\Sct}{{\tilde{\cal{S}}}}
%\newcommand{\smn}{\s_{\min}}
\newcommand{\btd}{{\bt_{\ell=1}^D d_\ell}}
\newcommand{\Ro}{{\cal{RO}}}
\newcommand{\PC}{{\cal{PC}}}
\newcommand{\Pb}{{\mtx{P}}}
\newcommand{\Tb}{{\mtx{T}}}
\newcommand{\Kba}{{\vct{k}}_{\text{all}}}
\newcommand{\Qb}{{\mtx{Q}}}
\newcommand{\rng}{\gamma}
\newcommand{\Cb}{{\mtx{C}}}
\newcommand{\Eb}{{\mtx{E}}}
\newcommand{\Hb}{{\mtx{H}}}
\newcommand{\Gc}{{\cal{G}}}
\newcommand{\F}{{\mtx{F}}}
\newcommand{\diff}{{\text{diff}}}
\newcommand{\La}{{\boldsymbol{{\Lambda}}}}
%\newcommand{\noresamp}[1]{{\textcolor{red}{#1}}}
\newcommand{\noresamp}[1]{{\textcolor{red}{#1}}}
\newcommand{\sigmap}{\phi'}
\newcommand{\sigmal}[1]{\sigma^{(#1)}}
\newcommand{\sigmalp}[1]{\sigma'^{(#1)}}
\newcommand{\sigmaa}{\sigma'_{\text{all}}}
\newcommand{\sigmai}[1]{\sigma'_{\text{all},#1}}
\newcommand{\bSi}{{\boldsymbol{{\Sigma}}}}
\newcommand{\bSit}{{\boldsymbol{{\tilde{\Sigma}}}}}
\newcommand{\bSih}{{\boldsymbol{{\hat{\Sigma}}}}}
\newcommand{\bmu}{{\boldsymbol{{\mu}}}}
\newcommand{\Db}{{\mtx{D}}}
\newcommand{\db}{{\vct{d}}}
\newcommand{\oneb}{{\mathbb{1}}}
\newcommand{\onebb}{{\mathbf{1}}}
\newcommand{\Iden}{{\mtx{I}}}
\newcommand{\M}{{\mtx{M}}}
\newcommand{\gm}{\gamma_m}
\newcommand{\order}[1]{{\cal{O}}(#1)}
\newcommand{\rmax}[1]{{\bf{r}_{\max}(#1)}}
\newcommand{\rbmax}[1]{{\bf{\bar{r}}_{\max}(#1)}}
\newcommand{\rmin}[1]{{\bf{r}_{\min}(#1)}}
\newcommand{\smn}[1]{{s_{\min}(#1)}}
\newcommand{\smx}[1]{{s_{\max}(#1)}}
\newcommand{\z}{{\vct{z}}}
\newcommand{\zb}{{\bar{\z}}}
\newcommand{\el}{{\ell}}
\newcommand{\tn}[1]{\|{#1}\|_{\ell_2}}
\newcommand{\tff}[1]{\|{#1}\|_{\ell_4}}
\newcommand{\tin}[1]{\|{#1}\|_{\ell_\infty}}
\newcommand{\trow}[1]{\|{#1}\|_{2,\infty}}
\newcommand{\bad}{{\bar{d}}}
\newcommand{\Dp}{{D^+}}
\newcommand{\tf}[1]{\|{#1}\|_{F}}
\newcommand{\te}[1]{\|{#1}\|_{\psi_1}}
\newcommand{\tsub}[1]{\|{#1}\|_{\psi_2}}
\newcommand{\tsut}[1]{\|{#1}\|_{\psi_{2/3}}}
\newcommand{\tsup}[1]{\|{#1}\|_{\psi_a}}
\newcommand{\dist}[1]{\text{dist}(#1)}
\newcommand{\upp}{{\cal{B}}_{\alpha,\Gamma}}
\newcommand{\upz}{{\cal{B}}_{\alpha_0,\Gamma}}
\newcommand{\dpz}{{\cal{D}}_{\alpha_0,\Gamma}}
\newcommand{\dpp}{{\cal{D}}_{\alpha,\Gamma}}
\newcommand{\mpp}{M_{\alpha,\Gamma}}
%\newcommand{\supp}[1]{\text{supp}(#1)}
\newcommand{\cone}[1]{{\text{cone}(#1)}}
\newcommand{\paf}{\partial f(\x)}
\newcommand{\Cc}{\mathcal{C}}
\newcommand{\Ac}{\mathcal{A}}
\newcommand{\Ccb}{\bar{\mathcal{C}}}
\newcommand{\Xc}{\mathcal{X}}
\newcommand{\xc}{{\text{excess}}}
\newcommand{\Rc}{\mathcal{R}}
\newcommand{\Rcp}{\mathcal{\bar{R}}'}
\newcommand{\Rcb}{\mathcal{N}}
\newcommand{\btrue}{\bbeta_{true}}
\newcommand{\bteta}{\boldsymbol{\theta}}
\newcommand{\bbteta}{\widetilde{\boldsymbol{\theta}}}
\newcommand{\brteta}{\overline{\boldsymbol{\theta}}}
\newcommand{\bbeta}{{\boldsymbol{\beta}}}
\newcommand{\ddelta}{{\boldsymbol{\delta}}}
\newcommand{\babeta}{{\bar{\beta}}}
\newcommand{\balpha}{{\bar{\alpha}}}
\newcommand{\bgamma}{{\bar{\gamma}}}
\newcommand{\Bc}{\mathcal{B}}
\newcommand{\Sc}{\mathcal{S}}
\newcommand{\Mc}{\mathcal{M}}
\newcommand{\pa}{{\partial}}
\newcommand{\Nn}{\mathcal{N}}
\newcommand{\pol}{^\circ}
\newcommand{\vb}{\vct{v}}
\newcommand{\Jb}{\mtx{J}}
\newcommand{\Jt}{\mtx{\tilde{J}}}
\newcommand{\vbl}{\vct{v}^{\text{lin}}}
\newcommand{\fb}{\vct{f}}
\newcommand{\ib}{{\bf{i}}}
\newcommand{\hib}{{\bf{\hat{i}}}}
\newcommand{\Ic}{{\mathcal{I}}}
\newcommand{\all}{{\text{all}}}
\newcommand{\vh}{\vct{\hat{v}}}
\newcommand{\vbb}{\vct{\bar{v}}}
\newcommand{\Xb}{\mtx{\bar{X}}}
\newcommand{\abb}{\mtx{\bar{a}}}
\newcommand{\cb}{\mtx{c}}
\newcommand{\bbb}{\mtx{\bar{b}}}
\newcommand{\w}{\vct{w}}
\newcommand{\err}[1]{\text{Err}_{\Dc}(#1)}
\newcommand{\Wp}{\mtx{W}^\dagger}
\newcommand{\tilW}{\widetilde{\mtx{W}}}
\newcommand{\tilw}{\widetilde{\vct{w}}}
\newcommand{\ob}{\mtx{o}}
\newcommand{\obh}{\mtx{\hat{o}}}
\newcommand{\wh}{{\hat{\mtx{w}}}}
\newcommand{\li}{\left<}
\newcommand{\ri}{\right>}
\newcommand{\s}{\vct{s}}
\newcommand{\sh}{\hat{\vct{s}}}
\newcommand{\ab}{\vct{a}}
\newcommand{\bb}{\vct{b}}
\newcommand{\ub}{{\vct{u}}}
\newcommand{\ubb}{\bar{\vct{u}}}
\newcommand{\h}{\vct{h}}
\newcommand{\hh}{{\vct{h}}}
\newcommand{\g}{{\vct{g}}}
\newcommand{\ii}{{\vct{i}}}
\newcommand{\zm}[1]{{\text{{\bf{zm}}}(#1)}}
\newcommand{\dd}{{\vct{d}}}
\newcommand{\ddt}{{\vct{d}}_\tau}
\newcommand{\Zb}{\mtx{Z}}
\newcommand{\hf}{\hat{f}}
\newcommand{\corrCA}{\rho_\Cc(\M)}
\newcommand{\corr}[1]{{\bf{cor}}(#1)}
\newcommand{\Tc}{\mathcal{T}}
\newcommand{\Fc}{\mathcal{F}}
\newcommand{\Hc}{\mathcal{H}}


%%YP's macros
\newcommand{\qqq}[1]{{\textcolor{red}{?{#1}?}}}
\newcommand{\ihere}{{\textcolor{red}{I AM HERE! }}}
\newcommand{\mat}[1]{{\text{mat}{#1}}}
\newcommand{\gb}{\bar{\g}}
\newcommand{\bs}{\bar{s}}
\newcommand{\cgain}{\alpha_{\text{CNN}}}
\newcommand{\cgainp}{\tn{\E_{\x\sim\Nn(0,\Iden)}[\gcnn{}]}}
\newcommand{\gcnn}[1]{{\vct{g}}_{\text{cnn}#1}}
\newcommand{\ccorr}{\rho_{\text{cnn}}}
\newcommand{\kb}{\vct{k}}
\newcommand{\xh}{\hat{\x}}
\newcommand{\yh}{\hat{\y}}
\newcommand{\xbr}{\bar{\h}}
\newcommand{\xdr}{\tilde{\x}}
\newcommand{\m}{\vct{m}}
\newcommand{\xt}{\tilde{\x}}
\newcommand{\nt}{\tilde{n}}
%\newcommand{\ht}{\tilde{h}}
\newcommand{\rt}{\tilde{r}}
\newcommand{\ft}{\tilde{f}}
\newcommand{\yt}{\tilde{\y}}
\newcommand{\gh}{\hat{\g}}
\newcommand{\gt}{\tilde{\g}}
\newcommand{\wb}{\bar{\w}}
\newcommand{\lip}{L}
\newcommand{\mipp}{L_{\max}}
\newcommand{\mupp}{\bar{\mu}_{\max}}
\newcommand{\mapp}{\mu}
\newcommand{\tcnn}{{\mtx{T}}_{\text{cnn}}}
\newcommand{\lcnn}{{\mtx{L}}_{\text{CNN}}}
\newcommand{\lipa}{{L}}
\newcommand{\smo}{S}
\newcommand{\SM}{{{\bf{S}}}_{L,\kb}}
\newcommand{\SMB}{{{\bf{\bar{S}}}}_{L,\kb}}
\newcommand{\Ws}{\W^\star}
\newcommand{\ws}{{\w^\star}}
\newcommand{\wss}{{\w^\star}}
\newcommand{\yp}[1]{\textcolor{red}{ #1}}
\newcommand{\zeronorm}[1]{\left\|#1 \right\|_0}
\newcommand{\unorm}[1]{\left\|#1 \right\|_u}
\newcommand{\ynorm}[1]{\left\|#1 \right\|_{\bar{y}}}
\newcommand{\onetwonorm}[1]{\left\|#1\right\|_{1,2}}
\newcommand{\opnorm}[1]{\left\|#1\right\|}
\newcommand{\fronorm}[1]{\left\|#1\right\|_{F}}
\newcommand{\onenorm}[1]{\left\|#1\right\|_{\ell_1}}
\newcommand{\twonorm}[1]{\left\|#1\right\|_{\ell_2}}
\newcommand{\wnorm}[2]{\left\|#1\right\|_{#2}}
\newcommand{\Dnorm}[1]{\left\|#1\right\|_{D}}
\newcommand{\oneinfnorm}[1]{\left\|#1\right\|_{1,\infty}}
\newcommand{\infnorm}[1]{\left\|#1\right\|_{\ell_\infty}}
\newcommand{\nucnorm}[1]{\left\|#1\right\|_*}
\newcommand{\abs}[1]{\left|#1\right|}
\newcommand{\avg}[1]{\left< #1 \right>}

\newcommand{\lipp}{\prod_{\ell=1}^D \twonorm{\vct{k}^{(\ell)}}}

\renewcommand{\d}{\mathrm{d}}

\newcommand{\cA}{\mathcal{A}}
\newcommand{\rotd}{\text{R1TD}}
\newcommand{\nntd}{\text{DeepTD}}
\newcommand{\x}{\vct{x}}
\newcommand{\rb}{\vct{r}}
\newcommand{\rbb}{\vct{\widetilde{r}}}
\newcommand{\y}{\vct{y}}
\newcommand{\ybh}{\vct{\hat{y}}}
\newcommand{\W}{\mtx{W}}
\newcommand{\Wc}{{\cal{W}}}
\newcommand{\Vc}{{\cal{V}}}
\newcommand{\bgl}{{~\big |~}}

%--------------

% EJC's macros

\definecolor{emmanuel}{RGB}{255,127,0}
\newcommand{\ejc}[1]{\textcolor{emmanuel}{EJC: #1}}

\newcommand{\p}{{\vct{p}}}
\newcommand{\Kb}{{\mtx{K}}}
\newcommand{\somelog}{16\Kb\log (\Kb)}
\newcommand{\somelg}{\Kb\log (\Kb)}
\newcommand{\pb}{{\vct{p}}}
\newcommand{\qb}{{\vct{q}}}
\newcommand{\R}{\mathbb{R}}
\newcommand{\Pro}{\mathbb{P}}
\newcommand{\C}{\mathbb{C}}
\newcommand{\Z}{\mathbb{Z}}
\newcommand{\<}{\langle}
\renewcommand{\>}{\rangle}
\newcommand{\Var}{\textrm{Var}}
\newcommand{\sgn}[1]{\textrm{sgn}(#1)}
\renewcommand{\P}{\operatorname{\mathbb{P}}}
%\newcommand{\E}{\operatorname{\mathbb{E}}}
\newcommand{\EE}{\operatorname{\mathbb{E}}}
%\newcommand{\var}{\operatorname{\mathbf{var}}}

\newcommand{\todo}[1]{{\bf TODO: #1}}
\newcommand{\grad}[1]{{\nabla\Lc(#1)}}
\newcommand{\gradf}[1]{{\nabla f(#1)}}
\newcommand{\hessf}[1]{{\nabla^2f(#1)}}
\newcommand{\gradw}[1]{{\nabla{\Lc}(#1)}}
\newcommand{\grd}[2]{{\nabla\Lc_{#1}(#2)}}
\newcommand{\e}{\mathrm{e}}
\newcommand{\eb}{\vct{e}}
\renewcommand{\i}{\imath}

\newcommand{\vct}[1]{\bm{#1}}
\newcommand{\mtx}[1]{\bm{#1}}

% MS's macros

\newcommand{\rank}{\operatorname{rank}}
\newcommand{\supp}[1]{\operatorname{supp}(#1)}
\newcommand{\restrict}[1]{\big\vert_{#1}}
\newcommand{\Id}{\text{\em I}}
\newcommand{\OpId}{\mathcal{I}}

\newcommand{\Real}{\operatorname{Re}}
\newcommand{\Imag}{\operatorname{Im}}

\newcommand{\piyp}{\pi'_1(\vct{y})}
\newcommand{\piy}{\pi_1(\vct{y})}
\newcommand{\piar}{\pi_1(\vct{a}_r)}
\newcommand{\piarp}{\pi'_1(\vct{a}_r)}
\newcommand{\set}{{\cal{F}}}
\newcommand{\des}{{\x_0}}

\newcommand{\Pc}{{\cal{P}}}
\newcommand{\X}{{\mtx{X}}}
\newcommand{\Y}{{\mtx{Y}}}
\newcommand{\Vb}{{\mtx{V}}}
\newcommand{\Vh}{\hat{{\mtx{V}}}}
\newcommand{\Vbd}{{\mtx{V}^\dagger}}
\newcommand{\Rb}{{\mtx{R}}}

\newcommand{\calF}{\mathcal{I}}
\newcommand{\calS}{\mathcal{N}}


\newcommand{\MS}[1]{\textcolor{blue}{MS: #1}}
\newcommand{\MST}[1]{\textcolor{red}{#1}}
\newcommand{\SO}[1]{\textcolor{darkgreen}{SO: #1}}


\numberwithin{equation}{section} 

\def \endprf{\hfill {\vrule height6pt width6pt depth0pt}\medskip}
%\newenvironment{proof}{\noindent {\bf Proof} }{\endprf\par}
\newenvironment{proofsk}{\noindent {\bf Proof sketch} }{\endprf\par}


%\newcommand{\qed}{{\unskip\nobreak\hfil\penalty50\hskip2em\vadjust{}
           %\nobreak\hfil$\Box$\parfillskip=0pt\finalhyphendemerits=0\par}}


\newcommand{\note}[1]{{\bf [{\em Note:} #1]}}

\newcommand{\iprod}[2]{\left\langle #1 , #2 \right\rangle}

\newcommand{\red}{\textcolor{red}}
\newcommand{\gi}{\ab_{\gamma_i}}
\newcommand{\ang}{\text{ang}}
\newcommand{\ham}[2]{{\|#1,#2\|_H}}

%\renewcommand{\algorithmicrequire}{\textbf{Input:}}
%\renewcommand{\algorithmicensure}{\textbf{Output:}}

%AJ's macros
\newcommand{\hth}{{\widehat{\boldsymbol{\theta}}}}
\newcommand{\bth}{{\boldsymbol{\theta}}}
\newcommand\cL{\mathcal{L}}
\newcommand\cLoss{\mathrm{loss}}
\newcommand\cD{\mathcal{D}}
\newcommand\hcD{\widehat{\cD}}
\newcommand\reals{\mathbb{R}}
\newcommand\bSigma{\boldsymbol{\Sigma}}
\newcommand\normal{{\sf N}}
\newcommand\bdelta{\boldsymbol{\delta}}
\newcommand\sign{{\rm sign}}
\newcommand\sT{{\sf T}}
\newcommand\I{\mtx{I}}
\newcommand\zero{\mtx{0}}
\newcommand\bA{\mtx{A}}
\newcommand\bv{\mtx{v}}
\newcommand\cI{\mathcal{I}}
\newcommand\bz{\boldsymbol{z}}
\newcommand\bg{\boldsymbol{g}}
\newcommand\ba{\boldsymbol{a}}
\def\cC{\mathcal{C}}
\def\de{{\rm d}}
\def\bM{\mtx{M}}
\def\cH{\mathcal{H}}
\def\bu{\boldsymbol{u}}
\def\by{\boldsymbol{y}}
\def\bw{\boldsymbol{w}}
\def\bX{\boldsymbol{X}}
\def\tbX{\tilde{\boldsymbol{X}}}
\def\tbx{\tilde{\boldsymbol{x}}}
\def\tbth{\tilde{\boldsymbol{\theta}}}
\def\hz{\widehat{z}}
\def\ind{\mathbf{1}}
\def\cS{\mathcal{S}}
\def\prob{\mathbb{P}}
\def\tx{\tilde{x}}
\def\reals{\mathbb{R}}
\newcommand{\aj}[1]{\noindent{\textcolor{blue}{\textbf{\#\#\# AJ:} \textsf{#1} \#\#\#}}}

\newcommand{\gauss}{\mathcal{N}(0,I)}
\newcommand{\gausscov}[1]{\mathcal{N}(0,{#1})}
\newcommand{\argmin}{\mathop{\mathrm{argmin}}}
%\newcommand{\cLCE}{\cL_{\mathrm{CE}}}
\newcommand{\cLCE}{\cL}
\newcommand{\mscrU}{{\mathscr{U}}}

==> Icassp (3)/Paper/s_exp.tex <==
\maketitle
\section{Numerical Experiments}\vspace{-5pt}
\label{s:exp}

% {\color{blue} Leave to Ibrahim}

% {\color{blue} I can roughly see what you did, but I'm not sure about a few details. Maybe I can mark down and talk to you on Mon, I'll have enough time to edit after that.}


We generate synthetic datasets with $k$ different tasks and $n$ samples for all tasks. As dimension of the data and dimension of the subspace we choose $d=50$ and $r=5$, respectively. %In all experiments we choose all $n_j$'s to be same i.e.~$n_j=n$. 

We study two different setups. In the first one data is generated according to Def.~\ref{def:GLM}. For the second setup, there is an underlying 3-layer neural network that fits the data. In both setups our only aim is to retrieve subspace representations of the data using Algorithm \ref{algo:1}.

\begin{figure}[t!]
\centering
\begin{subfigure}[htbp!]{0.23\textwidth}
\centering
\includegraphics[width = \linewidth]{Paper/Figures_in_Paper/11.png}
\subcaption{}\label{fig1a}
\end{subfigure}
\begin{subfigure}[htbp!]{0.23\textwidth}
\centering
\includegraphics[width =\linewidth]{Paper/Figures_in_Paper/21.png}
\subcaption{}\label{fig1b}
\end{subfigure}
\vspace{-0.35cm}
\captionsetup{width=\linewidth}{\caption{Subspace correlations with fixed number of tasks. \hspace{0.4cm}(a) Binary classification (b) Neural network.}  \label{fig1}} 
\end{figure} 

For neural network experiments, we assume that the data are generated from a ground truth neural network which has 3 layers, defined as  
$$ \yij = f^j(\xij) + \epsilon_{i,j} = \mtx{W}_{j3}(\mtx{W}_{j2}(\mtx{W}_{j1}(\mtx{W}\xij))_+)_+ + \epsilon_{i,j}$$ 
where  $\epsilon_{i,j}\sim\Nn(0,1)$ is gaussian noise, $(\cdot)_+$ is the ReLU activation function, $\mtx{W}\in\R^{5\times 50}$ is representation matrix which is same for all $j$'s. The weight matrices $\mtx{W}_{j1},\mtx{W}_{j2}$ and $\vct{W}_{j3}$ are different for each task and they are random gaussian matrices in $\R^{20\times 5},\R^{20\times 20},\R^{20}$ respectively.
\vspace{0cm}
\iffalse
\begin{figure}[htbp!]
\centering
\begin{subfigure}[htbp!]{0.23\textwidth}
\centering
\includegraphics[width = \linewidth]{Paper/Figures_in_Paper/12.png}
\subcaption{}\label{fig2a}
\end{subfigure}
\begin{subfigure}[htbp!]{0.23\textwidth}
\centering
\includegraphics[width =\linewidth]{Paper/Figures_in_Paper/22.png}
\subcaption{}\label{fig2b}
\end{subfigure}
\vspace{-0.2cm}
\captionsetup{width=\linewidth}{\caption{Subspace correlations with fixed number of samples per task and varying number of tasks. (a) Binary classification, (b) Neural network.}  \label{fig2}} 
\end{figure} 
\fi
%{\color{blue} Could you send me the data of the plots? I can work on the figure a bit. It would be better to set ``ylim'' so that the lines span the range of vertical direction. E.g., ylim=[0.4,1] in the first figure. And don't use colors, ICASSP requires grey-scale figures so we can't tell by color.}

In Fig.~\ref{fig1}
%, we apply Algorithm \ref{algo:1} to recover the $r$ dimensional subspace and get $\hat \Ub_r$, and check its distance to the true representation space $\Ub_r$ under different $n$'s and $k$'s. 
we use the subspace correlation as the metric for evaluating the accuracy of subspace recovery, which is defined by  $\frac{\|{\hat{\mtx{U}_r}^\top\mtx{U}_r}\|^2}{\|\mtx{U}_r\|^2}$.
In Fig.~\ref{fig1}, $k=100$ is fixed but $n$'s vary from $20$ to $200$. It can be seen from Fig.~\ref{fig1} that as $nk$ gets bigger, the subspace correlation becomes closer to $1$, which is compatible with Theorem \ref{thm:hatM}

In Fig.~\ref{fig3}(a), the downstream task accuracies for binary classification are depicted. For the new task, a new 1-layer neural network without any activation function is trained with and without the retrieved representations of the earlier tasks. We find the parameters of the neural network by minimizing the cross entropy loss via SGD. For this setup, during meta-training, we set $n=50$ for all tasks and $k=2000$, to have almost perfect representation. We evaluate the test error with $1000$ new samples.
%by generating $1000$ samples from the same task, 

\begin{figure}[t!]
\centering
\begin{subfigure}[htbp!]{0.24\textwidth}
\centering
\includegraphics[width =  \linewidth]{Paper/Figures_in_Paper/colorednewtaskacc.png}
\end{subfigure}
\hspace{-0.2em}
\begin{subfigure}[htbp!]{0.22\textwidth}
\centering
\includegraphics[width =  \linewidth]{Paper/Figures_in_Paper/alltogether.png}
\end{subfigure}
\captionsetup{width=.45\textwidth}{\caption{(a) Accuracy for downstream task, binary classification (b) Accuracy for downstream the task, MNIST} \label{fig3}}
\end{figure}


If the number of few-shot training samples is small, accuracy improves much faster when we use representation learning. This validates that dimension reduction reduces the degrees-of-freedom for few-shot learning, so the optimal model can be learned with fewer samples. As the sample size grows, the relative benefit of representation is smaller but still noticeable.

In Fig. \ref{fig3}(b), Algorithm \ref{algo:1} is also tested in MNIST dataset. $d=784$ and $r$ is not known. We assume that we have different binary classification tasks among pairs of digits such as 0-1;2-3;0-8;8-4 etc. There exist 15 meta-training tasks (i.e., $k=15$). For each task we have 500 samples in each classes. We choose a different pair of classes as few-shot learning task. We choose binary classification among images of 1 and 9, which is not included in the meta-learning phase. We tune the predicted subspace dimensions and number of samples to get Fig. \ref{fig3}(b).
\iffalse
\begin{figure}[htbp!]
\centering
\begin{subfigure}[htbp!]{0.37\textwidth}
\centering
\includegraphics[width =   \linewidth]{Paper/Figures_in_Paper/alltogether.png}
\end{subfigure}
\captionsetup{width=.45\textwidth}{\caption{Accuracy for downstream the task,MNIST} \label{figlast}}
\end{figure}
\vspace{-0.25cm}
\fi
It can be concluded that when $r=20$, 
%it does not serve a good representation 
The downstream task is not learnt well so we need to expand the subspace. For $r=50$ and $r=100$ subspace learning helps for few-shot learning, as when the number of training samples $n$ is between 8-56 they outperform the case without representation. When $r$ gets closer to $d$, the few-shot sample size has to be large to succeeed due to higher degree of freedom.
%When it comes to $r=400$ we deduce that we get results very similar to no representation case, as when $r$ is big and close to $d$, the model has huge degree of freedom so for good test accuracies $n$ must be big.
% \begin{figure}[htbp!]
% \centering
% \begin{subfigure}[htbp!]{0.35\textwidth}
% \centering
% \includegraphics[width =  \linewidth]{Paper/Figures_in_Paper/r15_1vs8_bluered_new_n.png}
% \end{subfigure}
% \captionsetup{width=.45\textwidth}{\caption{Accuracy for downstream task} \label{fig3}}
% \end{figure}
% \vspace{-0.25cm}


% \begin{figure}[htbp!]
% \centering
% \begin{subfigure}[htbp!]{0.35\textwidth}
% \centering
% \includegraphics[width =  \linewidth]{Paper/Figures_in_Paper/r15_1vs8_bluered_new_n.png}
% \end{subfigure}
% \captionsetup{width=.45\textwidth}{\caption{Accuracy for downstream task} \label{fig3}}
% \end{figure}
% \vspace{-0.25cm}
% \section{Conclusion and Future Work}
% In this work we showed that subspace-based representations can be efficiently learned for highly nonlinear tasks including GLMs and neural networks and help reduce sample complexity for future downstream tasks. A drawback of our results is that they are restricted to normally distributed data. It would be desirable to address such limitations by using distributional universality results such as \cite{oymak2018universality,abbasi2019universality}. Another direction is developing a more refined understanding for deep learning by restricting our nonlinear model space to deep neural nets.
%in contrast to more general purpose results developed here.
% {\color{red} YS: The blue curve is about 0.9, I feel it's already very accurate so we don't need this paragraph.}
% Additionally, we generate samples as defined in Def. \ref{def:bin_class}. $y$ conditioned on $\x$ is a random variable, yet not deterministic, so the data is implicitly noisy. Therefore the accuracy cannot reach $1$ empirically on the generated data.
% In Fig. \ref{fig1}, subspace correlations between the actual subspace and the predicted one using Algorithm \ref{algo:1}. Subspace correlations are calculated by  $\frac{\|{\hat{\mtx{U}_r}^\top\mtx{U}_r}\|^2}{\|\mtx{U}_r\|^2}$.It can be deduced that in both nonlinear setup subspace can be learned via moment estimator $t_j$ increases.
% \begin{figure}[htbp!]
% \centering
% \begin{subfigure}[htbp!]{0.4\textwidth}
% \centering
% \includegraphics[width = \linewidth]{Paper/Figures_in_Paper/GrayScale_NN_k100_subspace.png}
% \subcaption{}\label{fig1a}
% \end{subfigure}
% \begin{subfigure}[htbp!]{0.4\textwidth}
% \centering
% \includegraphics[width =\linewidth]{Paper/Figures_in_Paper/GrayScale_NN_nj30_subspace.png}
% \subcaption{}\label{fig1b}
% \end{subfigure}
% \captionsetup{width=.45\textwidth}{\caption{Subspace correlations, (a) for binary classification task whereas (b) stands for 3-layer Neural Net experiment.}  \label{fig1}} 
% \end{figure} 


==> Icassp (3)/Paper/s_gen_loss_proof.tex <==

\section{Proof of main theorems}

\iffalse
\SO{Clearly Theorem \ref{thm:hatM append} is a restatement of Theorem \ref{thm:hatM}. Why don't you say so? Reader is not expected to figure out this by himself. Let us make things clear.}

\SO{Similarly, where is proof of Lemma 3.1? Looks like Lemma \ref{lem:mean nn} is its restatement but again not clear at all for reader. They cannot find proof of Lemma 3.1 in the text.}

\SO{Here is the organization we need: In the appendix, proof of each technical result in the main text is supposed to have its own subsection. Just like this subsection that I added i.e.~Proof of Theorem \ref{thm:hatM}.}
\SO{Maybe briefly describe the outline. Right now, little confusing due to Lemmas within the proof so outline would help i.e.~we first prove Lemma ... which shows ...}
\subsection{Proof of Lemma \ref{lem:M exp} and Theorem \ref{thm:hatM}}
\fi
We sketch the proof at the beginning. First we compute the expectation of $y\x$ in Lemma \ref{lem:mean nn}. That leads to the proof of Lemma \ref{lem:M exp}. Then in Lemma \ref{lem:err_yx} we bound the difference between sum of $y\x$ and its mean using concentration. The concentration of covariance estimator is studied later in Lemma \ref{lem:Zj} and \ref{lem:Zj2}, which leads to Theorem \ref{thm:hatM}.

\subsubsection{Proof of Lemma \ref{lem:M exp}}
We first state Lemma \ref{lem:M exp} below.
\begin{lemma}\label{lem:M exp append}
Let 
\begin{subequations}\label{eq:hatM append}
\begin{align}
\hat\bM &= \mathop{\Scale[1.8]{\sum}}_{j=1}^k \frac{2}{n_j^2}\left[(\sum_{i=1}^{n_j/2} \yij\xij) (\sum_{i=n_j/2+1}^{n_j} \yij\xij)^\top \right.\\
&\quad\quad\quad\quad \left. +  ( \sum_{i=n_j/2+1}^{n_j} \yij\xij) ( \sum_{i=1}^{n_j/2} \yij\xij)^\top\right].\nonumber
\end{align}
\end{subequations}
And
\begin{align*}
    &\mtx{h}^j(\W): \R^{r\times d} \rightarrow \R^d = \mtx{E}_{\x}[f^j(\W \x)\x]\\
    &\bM := \W^\top\W\left(\frac{1}{k}\sum_{j=1}^k \mtx{h}^j(\W)( \mtx{h}^j(\W))^\top\right)\W^\top\W.
\end{align*}
Then $\bM,\hat{\bM}$ satisfies the following. (a) $\text{rank}(\bM)\leq r$. (b) $\text{range-space}(\bM)\subset \text{row-space}(\W)$. (c) $\mtx{E}[\hat{\M}]=\bM$. 
\end{lemma}
\begin{proof}
Part (a) and (b) are easy to see. $\W\in\R^{r\times d}$ so that $\text{rank}(\bM)\leq r$, and since $\bM$ is the product of $\W^\top$ and another matrix, then  $\text{range-space}(\bM)\subset \text{row-space}(\W)$.
Now we will prove Part (c). We first give the lemma for the mean of the random vector $y\x$.

\begin{lemma}\label{lem:mean nn}
We assume that the data is generated as in Def. \ref{def:task}, and we study the $j$-th task whose activation function is $f^j$. 
%{\color{blue} To be finished}
Define
\begin{align*}
    \mtx{h}^j(\W): \R^{r\times d} \rightarrow \R^d = \mtx{E}_{\x\sim\gauss} f^j(\W \x)  \x
\end{align*}
Denote the joint distribution of $(\x,y)$ as $\Pxy$.
Then $\mtx{E}_{(\x,y)\sim\Pxy}(y \x) = \W^\top\W \mtx{h}^j(\W)$.
\end{lemma}

\emph{Proof of Lemma \ref{lem:mean nn}.} The expectation can be expanded as
\begin{align*}
    &\mtx{E}_{(\x,y)\sim\Pxy}(y \x) \\
    &= \mtx{E}_{\x\sim\gauss} f^j(\W \x) \x\\
    &= \mtx{E}_{\x\sim\gauss} \left(f^j(\W \x)  \W^\top\W \x + f^j(\W \x) (I - \W^\top\W)\x \right).
\end{align*}
Note that, because $\x\sim\gauss$ so $\W \x$ and $(I - \W^\top\W)\x$ are Gaussian. $\W\W^\top = I$ implies 
\begin{align*}
    &\quad \Eb (\W \x)\x^\top((I - \W^\top\W))\\
    &= \W(I - \W^\top\W) = 0.
\end{align*}
So $\W \x$ and $(I - \W^\top\W)\x$ are independent, so 
\begin{align*}
    &\quad \mtx{E}_{\x\sim\gauss}  f^j(\W \x) (I - \W^\top\W)\x \\
    &= (\mtx{E}_{\x\sim\gauss}  f^j(\W \x)) (\mtx{E}_{\x\sim\gauss} (I - \W^\top\W)\x) = 0
\end{align*}
Then 
\begin{align*}
    \mtx{E}_{(\x,y)\sim\Pxy}(y \x) &= \W^\top\W(\mtx{E}_{\x\sim\gauss} f^j(\W \x) \x)\\
    &= \W^\top\W \h_j(\W).
\end{align*}

Denote 
\begin{align}\label{eq:Hj def}
    \Hb^j(\W) = \W^\top\W \mtx{h}^j(\W)
\end{align}
Because $\frac{2}{n_j}\sum_{i=1}^{n_j/2} \yij\xij$
and 
$\frac{2}{n_j}\sum_{i={n_j/2}+1}^{n_j} \yij\xij$ 
are independent, and their expectation are both $\Hb^j(\W)$, so that
\begin{align*}
    &\quad \mtx{E}(\frac{2}{n_j}\sum_{i=1}^{n_j/2} \yij\xij)(\frac{2}{n_j}\sum_{i={n_j/2}+1}^{n_j} \yij\xij)^\top \\
    &= \Hb^j(\W)(\Hb^j(\W))^\top.
\end{align*}
At then end
\begin{align*}
    \hat \bM &= \frac{1}{k}\sum_{j=1}^k \mtx{E}(\frac{2}{n_j}\sum_{i=1}^{n_j/2} \yij\xij)(\frac{2}{n_j}\sum_{i={n_j/2}+1}^{n_j} \yij\xij)^\top,\\
    \bM &= \frac{1}{k}\sum_{j=1}^k\Hb^j(\W)(\Hb^j(\W))^\top,
\end{align*}
so we can prove Part (c) that $\mtx{E}(\hat \bM) = \bM$.
\end{proof}


\subsubsection{Proof of Theorem \ref{thm:hatM}}
We restate Theorem \ref{thm:hatM append} below. 
\begin{theorem}\label{thm:hatM append}
Suppose the data is generated as Def. \ref{def:task}. Let $\delta\in(0,1)$, $\epsilon\in(0,1)$. Suppose $y\x$ is a subGaussian random vector with covariance upper bounded by
\begin{align}
   \| \mathbf{Cov}(y \x) \| \le \sigma^2. \label{eq:covyx append}
\end{align} 
Define
\begin{align*}
    \mtx{h}^j(\W): \R^{r\times d} \rightarrow \R^d = \mtx{E}_{\x\sim\gauss} f^j(\W \x)  \x
\end{align*}
And let %$\bM = \mtx{E}_{\theta\sim\mathcal{N}(0,\bSi)} (g(\theta))^2\frac{\theta\theta^\top}{\|\theta\|^2}$, then
\begin{align*}
    \bM = \W^\top\W\left(\frac{1}{k}\sum_{j=1}^k \mtx{h}^j(\W)( \mtx{h}^j(\W))^\top\right)\W^\top\W
\end{align*}
Then there exists a constant $c$, with probability at least $1-\delta$, let 
\begin{align*}
    k = \frac{cd}{n}\log^2(\frac{kd}{\delta}) \max\{\frac{1}{\epsilon^2}, \frac{1}{\epsilon} \log(\frac{kd}{\delta})\}
\end{align*}
we have 
\begin{align*}
    \|\hat \bM - \bM\| \le \epsilon\sigma^2.
\end{align*}
\end{theorem}
\begin{proof}
The following lemmas are similar to \cite{kong2020meta} Section A.1. We extend the concentration inequalities from bounded random vectors to Gaussian random vectors. For completeness we place the lemmas here.

\begin{lemma}\label{lem:err_yx}
(\cite{jin2019short} Cor. 7) 
Let $\|\mathbf{Cov}(y\x)\| \le \sigma^2$, $\delta\in(0,1)$, $t>0$, $\Hb^j(\W)$ be defined in \eqref{eq:Hj def}. With probability $1-\delta$, there exists a constant $c>0$ such that for every $j$,
%\som{Remind the exact assumption on $\sigma$}
\begin{align}
   \|\frac{1}{t}\sum_{i=1}^t \yij\xij - \Hb^j(\W)\| \le c\sigma\sqrt{\frac{d}{t}\log(\frac{kd}{\delta})} \label{eq:gauss_bern}
\end{align}
%\som{Call $\W^\top\W \mtx{h}^j(\W)$ something for simpler notation}
Denote this event as $\mathcal{E}$.
\iffalse
{\it\color{red} for every i,j pairs ? }Denote this event as $\mathcal{E}$.
{\it \color{red} if we dont say "for every i,j pairs" ,k should not appear in an inequality which holds for only one task. Also maybe it is better to  cite [21] A.5, because [28] Cor.7 says only the following
$$\|\frac{1}{t}\sum_{i=1}^t \yij\xij - \W^\top\W \mtx{h}^j(\W)\| \le c\sigma\sqrt{\frac{1}{t}\log(\frac{2d}{\delta})}$$}
\fi
\end{lemma}
With the covariance of $y\x$ being bounded by $\sigma^2$, the following inequalities are true \cite{kong2020meta}.
\begin{align*}
    \Eb\left( (\vb^T\cdot (\frac{1}{t}\sum_{i=1}^t \yij\xij - \theta^j))^2\right) &\le \sigma^2 / t,\mbox{~for~} \|\vb\|=1.\\
    \Eb \left(\|\frac{1}{t}\sum_{i=1}^t \yij\xij - \theta^j \|^2\right) &\le \sigma^2d/t.
\end{align*}


\begin{lemma}\label{lem:Zj}
Define
\begin{align*}
    \Zb_j &= (\frac{2}{n_j}\sum_{i=1}^{n_j/2} \yij\xij)(\frac{2}{n_j}\sum_{i={n_j/2}+1}^{n_j} \yij\xij)^\top \\
    &\quad - \Hb^j(\W)(\Hb^j(\W))^\top,
\end{align*}
Then there exists a constant $c$ such that on the event $\mathcal{E}$ (thus with probability $1-\delta$), for all $j=1,...,k$, 
\begin{align}
    \|\Zb_j \| \le \frac{c\sigma^2d}{n_j} \log(\frac{kd}{\delta}). \label{eq:evt}
\end{align}
\end{lemma}

% {\it \color{red} From my understanding we should have 
% $$\|\Zb_j \| \le (Eq A.1 Bound)(Eq. A.1 bound + 2\|\W^\top\W \mtx{h}^j(\W)\|)$$ choosing $t=\dfrac{n_j}{2}$ then we have $$\|\Zb_j \| \le (c\sigma\sqrt{\frac{2}{n_j}\log(\frac{2d}{\delta})})(c\sigma\sqrt{\frac{2}{n_j}\log(\frac{2d}{\delta})} + 2\|\W^\top\W \mtx{h}^j(\W)\|)$$
% This is more or less what you have found, but the difference is k in $\log$ term and d term }



The proof is almost same as \cite{kong2020meta}, the only difference is that we replace the bound in (\cite{kong2020meta} Prop A.1) by \eqref{eq:gauss_bern}. With the similar replacement, we propose the following lemma. 
\begin{lemma}\label{lem:Zj2}
Let $\delta\in(0,1)$. There exists a constant $c$, such that for any $\epsilon\in(0,1)$, and 
\begin{align}
    k = \frac{cd}{n_j}\log^2(\frac{kd}{\delta}) \max\{\frac{1}{\epsilon^2}, \frac{1}{\epsilon} \log(\frac{kd}{\delta})\}, \label{eq:k lb}
\end{align}
with probability $1-\delta$, 
\begin{align*}
    \|\frac{1}{k} \sum_{j=1}^k \Zb_j\| \le \epsilon \sigma^2.
\end{align*}
\end{lemma}
This means that when \eqref{eq:k lb} is true, with probability $1-\delta$,
\begin{align*}
    \left\|\hat \bM - \W^\top\W\left(\frac{1}{k}\sum_{j=1}^k \mtx{h}^j(\W)( \mtx{h}^j(\W))^\top\right)\W^\top\W\right\| \le \epsilon \sigma^2.
\end{align*}
Note that $\bM$ is defined as \[\bM=\W^\top\W\left(\frac{1}{k}\sum_{j=1}^k \mtx{h}^j(\W)( \mtx{h}^j(\W))^\top\right)\W^\top\W.\] So we have proven that with probability $1-\delta$,
\begin{align*}
    \left\|\hat \bM - \bM\right\| \le \epsilon \sigma^2.
\end{align*}

%\som{Remind that this is $\hat \bM-\bM$ i.e. $\bM=\text{the messy sum}$}
\end{proof}

%\SO{Create a subsection here!!! Reduce the confusion as much as possible, make transitions smooth.}
\subsection{Proof of Theorem \ref{thm:down}}
Now we will prove Theorem \ref{thm:down}. We first review the notations and assumptions mentioned in the theorem.

\subsubsection{Review of Notations and Assumptions}
We define the SVD of $\hat \bM$ as $\hat \Ub \hat\La \hat\Vb^\top$. Let the first $r$ columns of $\hat \Ub$ be $\Ub_r$. 

Let $\hat\W$ be defined as 
\begin{align}
    \hat \W &= \hat \Ub_r \hat \Qb, \label{eq:def W append}\\
    \hat \Qb &= \mathop{\mathrm{argmin}}_{\Qb\in\R^{r\times r}, \Qb\Qb^\top = I}\ \|\hat \Ub_r \Qb - \W\|.
\end{align}
The population cross entropy loss is defined as
\begin{align*}
    &\cLCE(f;\Pb) : \Fc\times \R^{r\times d}\rightarrow \R=\\
    &-\mtx{E}_{\x,y\sim\Pxy} (y\log f(\hat\Pb \x) + (1-y)\log (1 - f(\hat\Pb \x))).
\end{align*}
We will search for a function $f^* \in \Fc$.% that minimizes the population cross entropy loss. 
\begin{assumption}\label{append ass:F}
$\Fc$ is a set of functions satisfying: For any function $f\in\Fc$, any orthonormal matrix $\Qb\in\R^{r\times r}$ and any matrix $\Pb\in\R^{r\times d}$, there exists $g \in \Fc$ such that $f(\Pb \x) = g(\Qb\Pb \x)$.
%\begin{enumerate}
%    \item For any function $f\in\Fc$, any orthonormal matrix $\Qb\in\R^{r\times r}$ and any matrix $\Pb\in\R^{r\times d}$, there exists $g \in \Fc$ such that $f(\Pb \x) = g(\Qb\Pb \x)$.
%    \item $\Fc \subseteq \{f\ |\ \log f,~ \log(1-f)\mathrm{~are~}L\mathrm{~Lipschitz}\}\bigcap \{f\ |\ 0<f(x)<1,\forall x\in\R^r\}$.
%\end{enumerate}
\end{assumption}
Now we define a general loss function $\cL$ and $\cL_e$.
\begin{assumption}\label{append ass:L}
Suppose $\cL$ satisfies the following assumptions:
\begin{enumerate}
    \item %$\cL$ takes $f(\Pb x)$ as the argument, i.e., 
    $\cL$ has the form $\cL(f;\Pb) = \mtx{E}_{\Pxy}\Lcs(f(\Pb \x),y)$. $\cL_e$ has the form $\cL_e(f;\Pb) = \frac{1}{n}\sum_{i=1}^n\Lcs(f(\Pb \x_i),y_i)$.
    \item $\Lcs$ is $L$ Lipschitz in $\Pb \x$.
    \item $\min_{\Pb}\cL(f;\Pb) = \cL(f;\W)$.
\end{enumerate}
\end{assumption}
We solve for $\hat f$, defined as \begin{align}
    \hat f &= \argmin_{f\in\Fc}\ \cLCE(f;\hat \Ub_r^\top). \label{eq:def f append}
\end{align}
\subsubsection{Proof of Theorem \ref{thm:down}}
Now we are ready to restate Theorem \ref{thm:down} and prove it.

\begin{theorem}\label{thm:popu append}
With Assumptions \ref{append ass:F} and \ref{append ass:L}, we have that
    \begin{align*}
        \cLCE(\hat f;\hat \Ub_r^\top)  - \cLCE(f^*;\Ub_r^\top) \lesssim L\sqrt{r}\|\hat \W - \W\|.
    \end{align*}
\end{theorem}

\begin{proof}
We learn the model from the following optimization algorithm.
\begin{align*}
    \hat f &= \argmin_{f\in\Fc}\ \cLCE(f;\hat \Ub_r^\top)
    %\\
    %&= \argmin_{f\in\Fc}\ -\mtx{E}_{\x,y\sim\Pxy} (y\log f(\hat\Ub_r^\top \x) \\
    %&\quad + (1-y)\log (1 - f(\hat\Ub_r^\top \x)))\\
    %&= \argmin_{f\in\Fc}\ -\mtx{E}_{\x\sim\gauss} \left(f^*(\W \x)\log f(\hat \Ub_r^\top \x)\right. \\
    %& \quad \left. + (1-f^*(\W \x))\log (1 - f(\hat \Ub_r^\top \x)) \right).
\end{align*}
Denote $\tilde f\in\Fc$ as the function such that $\tilde f(\hat \W \x) = \hat f(\hat \Ub_r^\top \x)$. So that $\cLCE(\hat f;\hat \Ub_r^\top) = \cLCE(\tilde f;\hat \W)$. Since $\hat f$ minimizes the cross entropy loss, we have that $\cLCE(\tilde f;\hat \W) \le \cLCE(f^*;\hat \W)$. 

Now we have 
\begin{align*}
    &\quad \cLCE (\tilde f;\hat \W) - \cLCE (f^*;\W)\\
    &\le \cLCE (f^*;\hat \W) - \cLCE (f^*;\W)\\
    %&\le -\mtx{E}_{\x\sim\gauss} \left(f^*(\W \x)(\log f^*(\hat\W \x) -\log f^*(\W \x))\right. \\
    %& \quad \left. + (1-f^*(\W \x))(\log (1 - f^*(\hat \W \x)) - \log (1 - f^*(\W \x))) \right)\\
    &\le \mtx{E}_{\x\sim\gauss} L\|(\hat \W - \W)x\|\\
    &\lesssim L\sqrt{r}\|\hat \W - \W\|.
\end{align*}
The last step uses the fact that $\hat \W$ and $\W$ are rank $r$.
\end{proof}

\subsection{Proof of Theorem \ref{thm:rade}}
%Now we prove that the upper bound of the error for few-shot learning with finite samples.
We first state Theorem \ref{thm:rade} below.
\begin{theorem}\label{thm:rade app}
    Suppose we generate $n$ sample data for few shot learning solve for $\hat \theta_e$ from 
    \begin{align}
   	 \hat \bt_e &= \argmin_{\bt}\ \cL_e(\bt;\Ub_r^\top)\quad\text{such~that}\quad\|\bt\|_2\le a.\label{eq:fstar finite theta append}
	\end{align}
   Suppose Assumptions \ref{append ass:F} and \ref{append ass:L} hold.
    There exist constants $c>0$, $\delta\in(0,1)$, with probability at least $1 - n^{-c+1} - \delta$, the solution $\hat\theta_e$ and $\hat\Ub_r$ satisfy
    \begin{align*}
        &\quad \mathcal{L} (\hat\theta_e;\hat\Ub_r^\top) - \mathcal{L} (\theta^*;\W) \\
        &\lesssim \frac{caL(\sqrt{r}+\log(n)) (1+ \sqrt{\log(1/\delta)})}{\sqrt{n}} + L\sqrt{r}\|\hat \W - \W\|. 
    \end{align*}
\end{theorem}
\begin{proof}
We sketch the proof of Theorem \ref{thm:rade app}. After reviewing the notations, we quote a standard generalization bound via Rademacher complexity in Lemma \ref{lem:rade known}. Then we use the smoothness of the loss function to link to the generalization error of linear functions \eqref{eq:lin rade}, and then use Lemma \ref{lemma:chi-sqr} to compute \eqref{eq:lin rade} and finish the proof.

In few-shot learning, the true parameter is $\theta^*$, and the empirical loss function with finite data is 
\begin{align}
    &\cL_e(\theta;\Pb) : \Fc\times \R^{r\times d}\rightarrow \R= \frac{1}{n}\sum_{i=1}^n \Lcs(f(\Pb\x_i), y_i)
    %\notag\\
    %&-\frac{1}{n}\sum_{i=1}^n (y_i\log\phi (\theta^\top\Pb \x_i) + (1-y_i)\log (1 - \phi(\theta^\top\Pb \x_i))) \label{eq:cLCE finite theta app}
\end{align}
Denote each term in the summation as 
\begin{align*}
    &\quad \cL_e^i(\theta;\Pb) : \Fc\times \R^{r\times d}\rightarrow \R = \Lcs(f(\Pb\x_i), y_i).
    %=\notag\\
    %&- (y_i\log \phi (\theta^\top\Pb \x_i) + (1-y_i)\log (1 - \phi(\theta^\top\Pb \x_i)))
\end{align*}
We search for the solution by
\begin{align}
    \hat \theta_e &= \argmin_{\theta}\ \cL_e(\theta;\Ub_r^\top),\mbox{~such~that~} \|\theta\|\le a.\label{eq:fstar finite theta app}
\end{align}
In Theorem \ref{thm:popu append}, we know that
\begin{align*}
    \cLCE(\hat \theta;\hat \Ub_r^\top)  - \cLCE(\theta^*;\Ub_r^\top) \lesssim L\sqrt{r}\|\hat \W - \W\|.
\end{align*}
Denote 
    \begin{align}
        M = \max_{\|\theta\|\le a} |\theta^\top \hat\Ub_r^\top\x_i| \le a \max\|\hat\Ub_r^\top\x_i\|.\label{eq:bound_rade}
    \end{align}
We will bound the difference between $\cL$ and $\cL_e$ by Rademacher complexity theory.
\begin{lemma}\label{lem:rade known}
    \cite{mohri2018foundations}
 
    Let $\mscrU$ be the independent random variables uniformly chosen from $\{-1,1\}$.
    Let $\Rc$ be the Rademacher complexity of the logistic functionals defined on the data,
    \begin{align*}
        \Rc &= \frac{1}{n}\Eb_{\epsilon_i\in\mscrU} \sup_{\|\theta\|\le a} \sum_{i=1}^n\epsilon_i\cL_e^i(\theta;\hat\Ub_r^\top) \\
        %K &= |\log(\phi(-M))|>\max_i\cL_e^i(\theta;\hat\Ub_r^\top)
        K&= \max_i\cL_e^i(\theta;\hat\Ub_r^\top) \le M.
    \end{align*}
    %We know $\cL_e^i(\theta;\hat\Ub_r^\top)<K$ with probability at least $1-n^{-c_1+1}$,
    %then for any $\theta$ such that $\|\theta\|\le a$, with probability $1-\delta-n^{-c_1+1}$, we have that 
    with probability $1-\delta$, we have that 
    \begin{align*}
        |\cL_e(\theta;\Ub_r^\top) - \cL(\theta;\Ub_r^\top)| \le \Rc + \frac{\sqrt{\log(1/\delta)}}{\sqrt{n}}K.
    \end{align*}
\end{lemma}
Thus we have that 
\begin{align*}
    |\mathcal{L} (\hat\theta_e;\hat\Ub_r^\top) - \mathcal{L}_e (\hat\theta_e;\hat\Ub_r^\top)| &\le \Rc + \frac{\sqrt{\log(1/\delta)}}{\sqrt{n}}K,\\
    |\mathcal{L} (\hat\theta;\hat\Ub_r^\top) - \mathcal{L}_e (\hat\theta;\hat\Ub_r^\top)| &\le \Rc + \frac{\sqrt{\log(1/\delta)}}{\sqrt{n}}K.
\end{align*}
Because $\hat\theta_e$ minimizes the empirical loss $\mathcal{L}_e$,
\begin{align*}
    \mathcal{L}_e (\hat\theta_e;\hat\Ub_r^\top) \le \mathcal{L}_e (\hat\theta;\hat\Ub_r^\top).
\end{align*}
Thus 
\begin{align}
    \mathcal{L} (\hat\theta_e;\hat\Ub_r^\top) - \mathcal{L} (\hat\theta;\hat\Ub_r^\top) \le 2\left(\Rc + \frac{\sqrt{\log(1/\delta)}}{\sqrt{n}}K\right).\label{eq:emp loss}
\end{align}
So the remaining target is to bound $\Rc$. 

We first denote $\vb_i = \hat\Ub_r^\top \x_i$, so $\vb_i\in\R^r$ and $\vb_i$ are jointly independent standard normal random variables. %In binary classification, 
$\cL_e^i$ is always $L$ Lipschitz in $\theta^\top\vb_i$, the Rademacher complexity can be upper bounded by
\begin{align}\label{eq:lin rade}
    \Rc \le \tilde\Rc := \frac{L}{n}\Eb_{\epsilon_i\in\mscrU} \sup_{\|\theta\|\le a} \sum_{i=1}^n \epsilon_i\theta^\top\vb_i. 
\end{align}
We first refer to the following lemma.
\begin{lemma}\label{lemma:chi-sqr}
    \cite{laurent2000adaptive} Let $c>0$, $X$ follow $\chi_r^2$ distribution, then
    \begin{align*}
        \Pb(X - r \ge 2\sqrt{cr\log n} + 2c\log n) \le n^{-c}.
    \end{align*}
\end{lemma}

For a constant $c>1$, via union bound we have that $\max{\|\vb_i\|^2} \le r + 2\sqrt{cr\log n} + 2c\log n$ for all $i=1,..,n$ with probability $1 - n^{-c+1}$. We use $\max{\|\vb_i\|} \lesssim c(\sqrt{r} + \log(n))$ for simplicity.

Conditioned on this event, we apply the Rademacher complexity for linear model that 
\begin{align}
   \tilde \Rc &\le \frac{L\max\|\theta\| \cdot \max\|\vb_i\|}{\sqrt{n}}\\
   &\le \frac{caL(\sqrt{r} + \log(n))}{\sqrt{n}}. \label{eq:tilde Rc}
\end{align}
Combining with \eqref{eq:emp loss} and Theorem \ref{thm:popu append} we get the bound in Theorem \ref{thm:rade app}. We can also bound $M$ in \eqref{eq:bound_rade}.

Finally we will use Lemma \ref{lem:M to K} to bound $M$.
\begin{lemma}\label{lem:M to K}
    Let $M$ be defined as in \eqref{eq:bound_rade}.    
    With probability at least $1 - n^{-c+1}$, we have $M<caL(\sqrt{r} + \log(n))$.
\end{lemma}
Let $\vb_i$ be replaced by $\hat \Ub_r^\top\x_i$ in Lemma \ref{lemma:chi-sqr}, then this directly results from Lemma \ref{lemma:chi-sqr}. Lemma \ref{lem:M to K} bounds $M$, thus bounds $K$ (which is $L$ Lipschitz in $M$) in Lemma \ref{lem:rade known}. After we insert \eqref{eq:tilde Rc} together into Lemma \ref{lem:rade known}, we can get the result in  Theorem \ref{thm:rade}.
% By Lemma \ref{lemma:chi-sqr} we know that for a constant $c>2$, we have  $\max{\|\hat\Ub_r^\top\x_i\|} \le c(\sqrt{r} + \log(n))$ for all $i=1,..,n$ with probability $1 - n^{-c+1}$. So with probability at least $1 - n^{-c+1}$, we have $M<ac(\sqrt{r} + \log(n))$.
\end{proof}



==> Icassp (3)/Paper/s_intro.tex <==
\section{Introduction}\label{s:intro}
Meta-learning (and multi-task learning) has proved to be a efficient when available training data is limited. The central idea is exploiting the information (e.g.~training data) provided by earlier related tasks to quickly adapt a new task using few samples.
This idea has a rich history \cite{caruana1997multitask,baxter2000model} and has shown promise in modern machine learning tasks, e.g., in image classification \cite{deng2009imagenet}, machine translation \cite{bojar2014findings} and reinforcement learning \cite{finn2017model}, all of which may involve numerous tasks to be learned with limited data per task.
% between thousands of English and French sentences



 \mf{where? give citation}
  \mf{should we use the term meta-learning or multitask learning? It's better to pick one for consistency}
Modern deep learning algorithms typically exploit the shared information between tasks by learning useful representations \cite{schmidhuber1987evolutionary, thrun2012learning}. The multi-task system was studied by \cite{caruana1997multitask}, and the idea of meta-learning or transfer learning is investigated empirically in modern machine learning framework, showing that the shared representation benefits for training on the new tasks \cite{bengio2013representation, hospedales2020meta, yosinski2014transferable}.  %\cite{bengio2013representation, hospedales2020meta, yosinski2014transferable, raghu2019rapid}. 
An instructive and well-studied problem for meta-learning is mixed linear regression,
for which efficient algorithms and sample complexity bounds are discussed in 
\cite{zhong2016mixed, li2018learning, chen2020learning}. If the tasks lie on a shared low-dimensional subspace, learning this subspace would serve as an efficient representation which helps reduce the search space for future tasks. Once the search space is low dimensional, in order to get the same accuracy, the amount of data required for training is reduced compared to training over the full parameter space. \cite{lounici2011oracle,cavallanti2010linear,maurer2016benefit} propose sample complexity bounds for representation learning for linear multi-task systems. There are study of mixed linear tasks combined with other structures, such as boolean combination of features \cite{balcan2015efficient}, half-spaces \cite{rish2008closed} and sparse representations \cite{argyriou2008convex}.
% \mf{main point: low-dimensional approximation of the feature space makes learning easier in a new task, with fewer samples. Thus in many ML applications one seeks such a representation. can omit 'learned by mixed linear regression'. rewrite parag.}

% The low dimensional subspace of the features, learned by mixed linear regression, is utilized as the search space for training on new tasks.
% \mf{swap the order with next paragraph} 

The recent papers \cite{kong2020meta,kong2020robust} propose meta-learning procedures that involve dimension reduction, clustering and few-shot learning. Here a low-dimensional task subspace is used as the search space for few-shot learning for the new task. 
Another related approach
\cite{du2020few,tripuraneni2020provable}
sets up a nonconvex optimization problem with matrix factors of appropriate sizes, which captures the low dimensional structure. One can apply gradient descent to this nonconvex problem, and studying its behavior requires a nontrivial landscape analysis of the matrix factorization problem.  

However, existing provable algorithms for representation learning are restricted to linear-regression tasks, whereas typical machine learning tasks involve nonlinearity. This can arise from the use of nonlinear models as well as nonlinear label link function (e.g.~generalized linear models).
%. The setup is restrictive compared with the variant types of nonlinear tasks. 
\mf{what does 'objective' mean here? do you mean there are different tasks to be performed with different goals, with the same data?}
A good example is classification problems 
%which represent much of the machine learning applications 
including computer vision and natural language processing \cite{deng2009imagenet, bojar2014findings}. 
In classification tasks, the model is a map from images/text to labels, and the labels are discrete and not linear with respect to the input (i.e.~logistic link function). Another example is the use of nonlinear models such as deep networks
%, which contain many nonlinear activation functions within their layers. 
The existing results for representation learning for the linear-regression setting cannot be easily extended to the nonlinear case. 

\noindent\emph{Can we learn efficient subspace representations for nonlinear tasks such as generalized linear models and neural nets?}
%If one can learn a representation that help classify across several tasks, this representation can be used in this model can be retrieved and transferred to a classifier for other objectives.
%\som{Redundant sentence: In these datasets, there are images of different types of objectives, and the task is to classify which categories each image comes from.}

We consider a realizable setup where the input data is high-dimensional, the \emph{relevant features} lie in a low dimensional subspace and the labels depend only on the \emph{relevant features}. These assumptions are the same as in the existing literature, however we additionally allow for the scenario where labels are possibly an arbitrary nonlinear function of the relevant features. We make the following contributions.

\noindent$\bullet$ \textbf{Efficient representations for nonlinear tasks:} We show that subspace found via method-of-moments (MOM) leads to a consistent estimate of the ground-truth subspace despite arbitrary task nonlinearities, when the data is normally distributed.  We combine this with non-asymptotic learning results to establish sample complexity bounds for representation learning.

% \som{emphasize generalized linear model?}
\noindent$\bullet$ \textbf{Few-shot learning and Applications:} We specialize our results to practical settings with tasks involving binary classification and neural nets. We theoretically and empirically show that subspace-based representation can greatly improve sample efficiency of future tasks.
% \som{More citations are needed! Consider adding a related work (sub)section!}

%that, can we still retrieve the subspace with the same amount of training data?

%{\color{blue}Contribution here}




==> Icassp (3)/Paper/s_main.tex <==
\section{Main Results}
% {\color{red} YS: Commented some text for space limitation}
\vspace{-.1cm}
In this section, we shall establish error bounds for Algorithm \ref{algo:1}. This involves three parts. Theorem \ref{thm:hatM} establishes the quality of the moment estimator $\hat\bM$. %The estimator is then used for few-shot learning, and 
Theorem \ref{thm:down} upper bounds the population cross-entropy risk of $\hat f$ in the few-shot learning stage. Theorem \ref{thm:rade} upper bounds the population risk of the ERM estimator $\hat f_e$, which is learned from finite data.

\subsection{Results on Meta-training}
\begin{lemma}\label{lem:M exp}
$\bM,\hat{\bM}$ satisfies the following. (a) $\text{rank}(\bM)\leq r$. (b) $\text{range-space}(\bM)\subset \text{row-space}(\W)$. (c) $\mtx{E}[\hat{\M}]=\bM$. 
\end{lemma}
In words, $\bM$ returns a consistent estimate of the representation space in the sense that its range is guaranteed to be the subspace of the representation. Observe that to fully recover representation, $\bM$ should contain a diverse set of tasks that can \emph{cover} the representation subspace. For GLM, one needs at least $k\geq r$ tasks to ensure range of $\bM$ is equal to the row-space of $\W$. Additionally, $\hat{\M}$ estimator is also consistent. %All missing proofs can be found in \cite{paperurl}.



% notation (any well-conditioned can be accomplished by estimating the covariance of the inputs and then whitening the data. Such normalization procedures are common e.g.~batch normalization. 
We next present the error on the estimator $\hat \bM$. This theorem applies to standard normal data $\x\sim\Nn(0,\Iden)$. %This is mostly used for notational convenience. In machine learning subGaussian distributions often behave very similar in sufficiently high-dimensions \cite{oymak2018universality,abbasi2019universality}. We leave such generalizations to more general distributions as a future work. 
While this may initially seem restrictive, we remark that identity covariance is mostly used for notational convenience. Additionally, in similar spirit to Central Limit Theorem, machine learning and signal processing algorithms often exhibit distributional universality: For instance, subgaussian distributions often behave very similar or even identical to gaussian distributions in sufficiently high-dimensions \cite{oymak2018universality,abbasi2019universality}. We leave such generalizations to more general distributions as a future work. 
\begin{theorem}[Moment Estimator]\label{thm:hatM}
Suppose the data is generated as in Def.~\ref{def:task}, $n_j\geq N$ for all $j$ and $\xij\distas\Nn(0,\Iden)$. Suppose for some $\sigma>0$ and for all tasks, the label-input product $y\x$ is a subGaussian random vector with covariance upper bounded by $\| \mathbf{Cov}(y \x) \| \le \sigma^2$. (These conditions hold when $|f^j(\x)|<\sigma$.) Let $\delta\in(0,1)$ and $\epsilon\in(0,1)$. Then there exists a constant $c>0$ such that if
\begin{align*}
    k \ge \frac{cd}{N}\log^2(\frac{kd}{\delta}) \max\{\frac{1}{\epsilon^2}, \frac{1}{\epsilon} \log(\frac{kd}{\delta})\},
\end{align*}
$\|\hat \bM - \bM\| \le \epsilon\sigma^2$ with probability at least $1-\delta$.
\end{theorem}
%In essense, this shows that subspace $\M$ can be estimated with $O(kd) samples$
\iffalse
Theorem \ref{thm:hatM} proposes an upper bound for the estimation error of $\bM$. The subspace spanned by $\hat \bM$ is used for few-shot learning. In the context of binary classification, we will show how this error affects the cross entropy loss for the few-shot learning stage. 
\fi
%Downstream task

Recall that $\hat \bM=\hat \Ub \hat\La \hat\Ub^\top$ and $\hat \Ub_r$ is the first $r$ columns of $\hat \Ub$. Denote the estimate of $\W$ via $\hat \W$ given by adjusting $\hat\Ub_r$
\begin{align}
    \hat \W &= (\hat \Ub_r \hat \Qb)^\top,\
    \hat \Qb = \mathop{\mathrm{argmin}}_{\Qb\in\R^{r\times r}, \Qb\Qb^\top = I}\ \|\hat \Ub_r \Qb - \W^\top\|\label{eq:def W}
\end{align}
With the definition of $\hat\W$, $\|\hat \W - \W\|$ defines a distance between the row space of $\W$ and the column space of $\hat \Ub_r$. If the span of the two subspaces are the same, then there exists an orthonormal matrix $\Qb$ such that $\hat \Ub_r \Qb = \W^\top$.

The previous lemma builds upon the assumption that $\|\hat \W - \W\|$ is small. 
%We quote the following lemma first. 
In Theorem \ref{thm:hatM}, we have got $\|\hat \bM - \bM\| \le \epsilon\sigma^2$, then with the extra assumption that $\bM$ is rank $r$, we have the following result from \cite{davis1970rotation}.
\begin{lemma}
If $\|\hat \bM - \bM\| \le \epsilon\sigma^2$, $\lambda_r(\bM) > \epsilon\sigma^2$, then \[\|\hat \W - \W\| \le \epsilon\sigma^2(\lambda_r(\bM) -\epsilon\sigma^2)^{-1}.
%\le \frac{\|\hat \bM - \bM\|}{\lambda_r(\bM) - \|\hat \bM - \bM\|} \le \frac{\epsilon\sigma^2}{\lambda_r(\bM) -\epsilon\sigma^2}.
\]
\end{lemma}



% I think it's better to keep this as \Qb is used in assumption 1 of \Fc

%Another definition of the distance between two subspaces is the difference of projection, defined as 
%\begin{align*}
%    \|\hat \Ub_r\hat \Ub_r^\top - \W^\top\W\|
%\end{align*}
%Note that, with \eqref{eq:def W}, if 

\iffalse
{\color{red} can remove the text, just to keep the assumption on $\Fc$}
Now we use $\hat\Ub_r$ for the downstream task, and we study the population loss of training caused by the error of the estimator $\hat \bM$. We consider the binary classification case, where the data in the new task is generated as Def. \ref{def:bin_class}, with the non-linear function being $f$ and the true subspace being $\W$. The loss we consider, is cross-entropy loss, which is defined as \eqref{eq:cLCE}.
%\begin{align*}
%    &\cLCE(f;\Pb) : \Fc\times \R^{r\times d}\rightarrow \R=\\
%    &-\mtx{E}_{\x,y\sim\Pxy} (y\log f(\hat\Pb \x) + (1-y)\log (1 - f(\hat\Pb \x))) 
%\end{align*}

To train on the data, we need to find the optimal function $f$ that minimizes the population loss. Define the search space of $f$ as $\Fc$. For binary classification, we assume that, 
\begin{enumerate}
    \item For any function $f\in\Fc$, any orthonormal matrix $\Qb\in\R^{r\times r}$ and any matrix $\Pb\in\R^{r\times d}$, there exists $g \in \Fc$ such that $f(\Pb \x) = g(\Qb\Pb \x)$.
    \item $\Fc \subseteq \{f\ |\ \log f,~ \log(1-f)\mathrm{~are~}L\mathrm{~Lipschitz}\}\bigcap \{f\ |\ 0<f(x)<1,\forall x\in\R^r\}$.
\end{enumerate}
We can see that, if we adopt the logistic regression for binary classification example in \eqref{eq:Fcbin}, then both assumptions are true with $L = a$.  

We learn the model from the optimization algorithm \eqref{eq:fstar} (also works for logistic regression in \eqref{eq:fstarbin}). Now we will bound the cross-entropy loss of this model.
\fi

%\so{There is a serious issue here. It seems, we never stated a bound on $\hat{\W}-\W$, we only prove a bound on $\hat{M}-\M$. Thm 3.2 should ideally state bound for the subspace as well. This bound should be in terms of the spectrum of $\M$ i.e. its $r$'th largest singular (e.g.~via davis-kahan thm). If you look at the few-shot learning results, they are in terms of $\|\hat{\W}-\W\|$. This is fine but we should also add an end-to-end learning result where $\|\hat{\W}-\W\|$ is bounded in terms of meta-training sample size. This should be addressed before arXiv submission.}
\subsection{Results on Few-shot Learning}
\vspace{-0.1cm}
In the next step, we will use $\hat\Ub_r$ for few shot learning and find $\hat f$ that minimize the population loss. 
%Recall that the search space for $\hat f$ is $\Fc$. For binary classification, we assume 
%\begin{enumerate}
%Only row-space (representation) matters
%    \item \textbf{Rotation invariance:} For any function $f\in\Fc$, any orthonormal matrix $\Qb\in\R^{r\times r}$ and any matrix $\Pb\in\R^{r\times d}$, there exists $g \in \Fc$ such that $f(\Pb \x) = g(\Qb\Pb \x)$.
%    \item \textbf{Lipschitz:} $\Fc \subseteq \{f\ |\ \log f,~ \log(1-f)\mathrm{~are~}L\mathrm{~Lipschitz}\}$ $~\bigcap~ \{f\ |\ 0<f(x)<1,\forall x\in\R^r\}$.
%\end{enumerate}

\begin{theorem}\label{thm:down}
    Let Assumptions \ref{ass:F} and \ref{ass:L} hold. Let $\hat\W$ be the same as in \eqref{eq:def W} and $\hat f$ be the same as in \eqref{eq:fstar}. Then we have 
    \begin{align*}
        \cLCE(\hat f;\hat \Ub_r^\top) - \cLCE(f^*;\W)\lesssim L\sqrt{r}\|\hat \W - \W\|.
    \end{align*}
\end{theorem}
$\cLCE (f^*;\W)$ assumes the knowledge of the true function $f^*$ and the representation $\W$. This shows that the inaccuracy of the moment estimator $\hat M$ costs us $O(L\sqrt{r}\|\hat \W - \W\|)$. 

Theorem \ref{thm:down} bounds the population risk of $\hat f$, when we use $\hat\Ub_r^\top$ as the representation subspace. Next we discuss the population risk of the finite sample solution $\hat f_e$, which should be worse than $\hat f$ due to the limited samples.
%deviating from true data distribution of the new task. Theorem \ref{thm:rade} bounds the risk in terms of the sample size $n$.

\iffalse
For a concrete example, we apply the logistic regression model for \eqref{eq:cLCE finite}, where $f(\vb) = \phi(\bt^\top\vb)$, $\vb \in \R^r$ and $\phi$ is logistic function. Let the ground truth parameter for generating few-shot learning data be $\bt^*$ and we assume $\|\bt^*\| \le a$. In few-shot learning, we train by solving for $\hat \bt_e$ in the set $\{\bt\ |\ \|\bt\| \le a\}$. The objective is {\color{red} can move this to def 2.6}
\begin{align}
    &\cL_e(\bt;\Pb) : \Fc\times \R^{r\times d}\rightarrow \R= \notag\\
    &-\frac{1}{n}\sum_{i=1}^n (y_i\phi (\bt^\top\Pb \x_i) + (1-y_i)\log (1 - \phi(\bt^\top\Pb \x_i))) \label{eq:cLCE finite theta}
\end{align}
The empirical minimizer is defined by
\begin{align}
    \hat \bt_e &= \argmin_{\bt}\ \cL_e(\bt;\Ub_r^\top),\mbox{~such~that~} \|\bt\|\le a.\label{eq:fstar finite theta}
\end{align}
\fi
\begin{theorem}\label{thm:rade}
    Consider the setup in Def.~\ref{def: test finite} with $n$ i.i.d.~examples with ground-truth model $\bt^*$. Solve for $\hat \bt_e$ via \eqref{eq:fstar finite theta}. There exist constants $c>1$, $\delta\in(0,1)$, with probability at least $1 - n^{-c+1} - \delta$, the solution pair $(\hat\bt_e,\hat\Ub_r)$ satisfies
    \begin{align*}
        \quad \mathcal{L}(&\hat\bt_e;\hat\Ub_r^\top) - \mathcal{L} (\bt^*;\W) \\
        &\leq \frac{caL(\sqrt{r}+\log(n)) (1+ \sqrt{\log(1/\delta)})}{\sqrt{n}} + L\sqrt{r}\|\hat \W - \W\|. 
    \end{align*}
\end{theorem}
Note that the first term grows as $\sqrt{r/n}$. This means the amount of data $n$ we request for few-shot learning is $n\approx r$,  as compared to $n\approx d$ if representation learning is not excecuted. 
%If we do not run representation learning before few-shot learning, the error would instead be proportional to $\sqrt{d/n}$ where $d$ is the ambient dimension and we would need $n\approx d$ examples to learn the new task.
% {\color{red} YS:  No math justification for $n\ge d$ here since I only have upper bound but no lower bound, so it's just an intuition}
%In \eqref{eq:fstar}, we solve for the minimizer of population loss function. Now we will study the finite sample case. In few-shot learning phase, suppose we have the dataset $(\x_i, y_i)$, $i=1,...,n$ and the data is generated as Def. \ref{def: test}. Now we consider the 

==> Icassp (3)/Paper/s_main_nn.tex <==
\begin{lemma}\label{lem:mean nn}
We assume that the data are generated as in Defs. \ref{def:task dis} to \ref{def:data_gen} and Def. \ref{def:nn}, and we study the $j$-th task whose feature matrix is $\Theta^j$. 
%{\color{blue} To be finished}
Define
\begin{align*}
    \mtx{h}(\Theta): \R^{r\times d} \rightarrow \R^r = \mtx{E}_{\x\sim\Px} f(\Theta \x)  \x
\end{align*}
Then $\mtx{E}_{(\x,y)\sim\Pxy}(y \x) = (\Theta^j)^\top(\Theta^j(\Theta^j)^\top)^{-1}\Theta^j\mtx{h}(\Theta^j)$, and $\|y\x\|\le 1$ with probability $1$.
%{\color{blue} To be finished}
\end{lemma}

\noindent\textbf{Proof of Lemma \ref{lem:mean nn}} The boundedness is trivial and we study the expectation.
Denote
\begin{align*}
    \tilde \Theta^j = (\Theta^j)^\top (\Theta^j(\Theta^j)^\top)^{-1}\Theta^j
\end{align*}

We first write the expectation as
\begin{align*}
    &\mtx{E}_{(\x,y)\sim\Pxy}(y \x) \\
    &= \mtx{E}_{\x} f(\Theta^j \x) \x\\
    &= \mtx{E}_{\x\sim\Px} \left(f(\Theta^j \x)  \tilde \Theta^j \x + f(\Theta^j \x) (\x -  \tilde \Theta^j\x) \right).
\end{align*}
Now we prove that 
\begin{align*}
    \mtx{E}_{\x\sim\Px}f(\Theta^j \x) (\x -  \tilde \Theta^j\x) =0
\end{align*}
Denote 
\begin{align*}
    \bar \x &= \tilde \Theta^j\x - (\x -  \tilde \Theta^j\x)\\
    &= 2\tilde \Theta^j\x - \x.
\end{align*}
Then it is easy to see
\begin{align}
    \Theta^j \x  &= \Theta^j \bar \x,\label{eq:easy1 nn} \\
    \x -  \tilde \Theta^j\x &= - \left(\bar \x -  \tilde \Theta^j\bar \x\right),\label{eq:easy2 nn}\\
    \x &=2\tilde \Theta^j\bar \x - \bar \x.
\end{align}


Now we consider the density function of $\bar x$. Let the density of $\x$ be $p_{\x}$, which is uniform on the unit sphere, we have that 
{\color{blue} Need a better notation!}
\begin{align}
    p_{\bar \x} (\bar \x) &= p_{\x}(2\tilde \Theta^j\bar \x - \bar \x) \big|\nabla_{\bar \x} (2\tilde \Theta^j\bar \x - \bar \x \big| \label{eq:den2 nn}\\
    &= p_{\x}(\x) \big|\mathrm{det}(2\tilde \Theta^j - I) \big|\label{eq:den3}\\
    &= p_{\x}(\x).
\end{align}
Here \eqref{eq:den2} uses the fact that the density function $p_{\x}$ is uniform (thus is a constant everywhere), and \eqref{eq:den3} uses that the eigenvalues of $\frac{2\theta^j(\theta^j)^\top}{\|\theta^j\|^2} - I$ only consists of $\pm 1$. Now we can see that the distributions of $\x$ and $\bar \x$ are the same.

So we have that
\begin{align}
    &\quad \mtx{E}_{\x\sim\Px}f(\Theta^j\bar \x) (\bar \x - \tilde \Theta^j\bar \x)\notag\\
    &= \mtx{E}_{\x\sim\Px}f(\Theta^j \x) \left(- (\x -  \tilde \Theta^j\x)\right)\notag\\
    &= - \mtx{E}_{\x\sim\Px}f(\Theta^j \x) (\x -  \tilde \Theta^j\x).\label{eq:mns nn}
\end{align}
which uses \eqref{eq:easy1 nn}, \eqref{eq:easy2 nn}. Since the distributions of $\x$ and $\bar \x$ are the same, we compute via a simple change of variable
\begin{align}
    &\quad \mtx{E}_{\x\sim\Px}f(\Theta^j\bar \x) (\bar \x - \tilde \Theta^j\bar \x) \notag\\
    &= \mtx{E}_{\bar \x\sim\Px}f(\Theta^j\bar \x) (\bar \x - \tilde \Theta^j\bar \x)\notag\\
    &= \mtx{E}_{\x\sim\Px}f(\Theta^j \x) (\x -  \tilde \Theta^j\x).\label{eq:pls nn}
\end{align}

Comparing \eqref{eq:mns nn} and \eqref{eq:pls nn}, we have 
\begin{align*}
    &\quad \mtx{E}_{\x\sim\Px}f(\Theta^j \x) (\x -  \tilde \Theta^j\x)\\
    &= -\mtx{E}_{\x\sim\Px}f(\Theta^j \x) (\x -  \tilde \Theta^j\x)
\end{align*}
so $\mtx{E}_{\x\sim\Px}f(\Theta^j \x) (\x -  \tilde \Theta^j\x)=0$.

Going back to Lemma \ref{lem:mean nn}, we have 
\begin{align*}
    \mtx{E}_{(\x,y)\sim\Pxy}(y \x)
    &= \mtx{E}_{\x\sim\Px} f(\Theta^j \x)  \tilde \Theta^j \x
    \\&= \mtx{E}_{\x\sim\Px} f(\Theta^j \x)  (\Theta^j)^\top (\Theta^j(\Theta^j)^\top)^{-1}\Theta^j \x.
\end{align*}
%\Theta^j

{\color{blue} From here I'll prove using the fact that $y\x$ is subGaussian with $\|\mathbf{Cov}(y\x)\| \le \sigma^2$.}

First we study the concentration of data within the $j$-th class. 
\begin{lemma}
Let $\delta\in(0,1)$, with probability $1-\delta$, there exists a constant $c$ such that
\begin{align*}
    \|\frac{1}{t}\sum_{i=1}^t \yij\xij - \theta^j\| \le c\sigma\sqrt{\frac{d}{t}\log(\frac{kd}{\delta})} 
\end{align*}
for all $j=1,...,k$. 
\end{lemma}
\begin{lemma}
For all $\vb$ such that $\|\vb\| = 1$, there exists a constant $c$ such that
\begin{align*}
    \Eb\left( (\vb^T\cdot (\frac{1}{t}\sum_{i=1}^t \yij\xij - \theta^j))^2\right) \le c\sigma^2 / t. 
\end{align*}
\end{lemma}
\begin{lemma}
There exists a constant $c$ such that \begin{align*}
    \Eb \left(\|\frac{1}{t}\sum_{i=1}^t \yij\xij - \theta^j \|^2\right) \le c\sigma^2d/t. 
\end{align*}
\end{lemma}
\begin{lemma}
Define
\begin{align*}
    \Zb_j = (\frac{1}{t}\sum_{i=1}^t \yij\xij)(\frac{1}{t}\sum_{i=t+1}^{2t} \yij\xij)^\top - \theta^j(\theta^j)^\top,
\end{align*}
Then there exists a constant $c$ such that with probability $1-\delta$, for all $j=1,...,k$, 
\begin{align}
    \|\Zb_j \| \le \frac{c\sigma^2d}{t} \log(\frac{kd}{\delta}). \label{eq:evt}
\end{align}
\end{lemma}

\begin{lemma}
There exists a constant $c$ such that
\begin{align*}
   \|\Eb\sum_{j=1}^k\Zb_j\Zb_j^\top\| \le c\sigma^4dk/t
\end{align*}
\end{lemma}
\begin{lemma}
Let $\delta\in(0,1)$. There exists a constant $c$, such that for any $\epsilon\in(0,1)$, and 
\begin{align}
    k = \frac{cd}{t}\log^2(\frac{kd}{\delta}) \max\{\frac{1}{\epsilon^2}, \frac{1}{\epsilon} \log(\frac{kd}{\delta})\}, \label{eq:k lb}
\end{align}
with probability $1-\delta$, 
\begin{align*}
    \|\frac{1}{k} \sum_{j=1}^k \Zb_j\| \le \epsilon \sigma^2.
\end{align*}
\end{lemma}
This means that when \eqref{eq:k lb}, with probability $1-\delta$,
\begin{align*}
    \left\|\hat \bM - \frac{1}{k}\sum_{j=1}^k\left(\tilde \Theta^j \mtx{h}(\Theta^j)\mtx{h}^\top(\Theta^j)\tilde \Theta^j\right)\right\| \le \epsilon \sigma^2.
\end{align*}


==> Icassp (3)/Paper/s_main_proof.tex <==
\section{Proof of main theorems}
\SO{Clearly Theorem \ref{thm:hatM append} is a restatement of Theorem \ref{thm:hatM}. Why don't you say so? Reader is not expected to figure out this by himself. Let us make things clear.}

\SO{Similarly, where is proof of Lemma 3.1? Looks like Lemma \ref{lem:mean nn} is its restatement but again not clear at all for reader. They cannot find proof of Lemma 3.1 in the text.}

\SO{Here is the organization we need: In the appendix, proof of each technical result in the main text is supposed to have its own subsection. Just like this subsection that I added i.e.~Proof of Theorem \ref{thm:hatM}.}
\SO{Maybe briefly describe the outline. Right now, little confusing due to Lemmas within the proof so outline would help i.e.~we first prove Lemma ... which shows ...}
\subsection{Proof of Lemma \ref{lem:M exp} and Theorem \ref{thm:hatM}}
We sketch the proof at the beginning. First we compute the expectation of $y\x$ in Lemma \ref{lem:mean nn}. That leads to the proof of Lemma \ref{lem:M exp}. Then in Lemma \ref{lem:err_yx} we bound the difference between sum of $y\x$ and its mean using concentration. The concentration of covariance estimator is studied later in Lemma \ref{lem:Zj} and \ref{lem:Zj2}, which leads to Theorem \ref{thm:hatM}.

\subsubsection{Proof of Lemma \ref{lem:M exp}}
We first state Lemma \ref{lem:M exp} below.
\begin{lemma}\label{lem:M exp append}
Let 
\begin{subequations}\label{eq:hatM append}
\begin{align}
\hat\bM &= \mathop{\Scale[1.8]{\sum}}_{j=1}^k \frac{2}{n_j^2}\left[(\sum_{i=1}^{n_j/2} \yij\xij) (\sum_{i=n_j/2+1}^{n_j} \yij\xij)^\top \right.\\
&\quad\quad\quad\quad \left. +  ( \sum_{i=n_j/2+1}^{n_j} \yij\xij) ( \sum_{i=1}^{n_j/2} \yij\xij)^\top\right].\nonumber
\end{align}
\end{subequations}
And
\begin{align*}
    &\mtx{h}^j(\W): \R^{r\times d} \rightarrow \R^d = \mtx{E}_{\x}[f^j(\W \x)\x]\\
    &\bM := \W^\top\W\left(\frac{1}{k}\sum_{j=1}^k \mtx{h}^j(\W)( \mtx{h}^j(\W))^\top\right)\W^\top\W.
\end{align*}
Then $\bM,\hat{\bM}$ satisfies the following. (a) $\text{rank}(\bM)\leq r$. (b) $\text{range-space}(\bM)\subset \text{row-space}(\W)$. (c) $\mtx{E}[\hat{\M}]=\bM$. 
\end{lemma}
\begin{proof}
Part (a) and (b) are easy to see. $\W\in\R^{r\times d}$ so that $\text{rank}(\bM)\leq r$, and since $\bM$ is the product of $\W^\top$ and another matrix, then  $\text{range-space}(\bM)\subset \text{row-space}(\W)$.
Now we will prove Part (c). We first give the lemma for the mean of the random vector $y\x$.

\begin{lemma}\label{lem:mean nn}
We assume that the data is generated as in Def. \ref{def:task}, and we study the $j$-th task whose activation function is $f^j$. 
%{\color{blue} To be finished}
Define
\begin{align*}
    \mtx{h}^j(\W): \R^{r\times d} \rightarrow \R^d = \mtx{E}_{\x\sim\gauss} f^j(\W \x)  \x
\end{align*}
Denote the joint distribution of $(\x,y)$ as $\Pxy$.
Then $\mtx{E}_{(\x,y)\sim\Pxy}(y \x) = \W^\top\W \mtx{h}^j(\W)$.
\end{lemma}

\emph{Proof of Lemma \ref{lem:mean nn}.} The expectation can be expanded as
\begin{align*}
    &\mtx{E}_{(\x,y)\sim\Pxy}(y \x) \\
    &= \mtx{E}_{\x\sim\gauss} f^j(\W \x) \x\\
    &= \mtx{E}_{\x\sim\gauss} \left(f^j(\W \x)  \W^\top\W \x + f^j(\W \x) (I - \W^\top\W)\x \right).
\end{align*}
Note that, because $\x\sim\gauss$ so $\W \x$ and $(I - \W^\top\W)\x$ are Gaussian. $\W\W^\top = I$ implies 
\begin{align*}
    &\quad \Eb (\W \x)\x^\top((I - \W^\top\W))\\
    &= \W(I - \W^\top\W) = 0.
\end{align*}
So $\W \x$ and $(I - \W^\top\W)\x$ are independent, so 
\begin{align*}
    &\quad \mtx{E}_{\x\sim\gauss}  f^j(\W \x) (I - \W^\top\W)\x \\
    &= (\mtx{E}_{\x\sim\gauss}  f^j(\W \x)) (\mtx{E}_{\x\sim\gauss} (I - \W^\top\W)\x) = 0
\end{align*}
Then 
\begin{align*}
    \mtx{E}_{(\x,y)\sim\Pxy}(y \x) &= \W^\top\W(\mtx{E}_{\x\sim\gauss} f^j(\W \x) \x)\\
    &= \W^\top\W \h_j(\W).
\end{align*}

Denote 
\begin{align}\label{eq:Hj def}
    \Hb^j(\W) = \W^\top\W \mtx{h}^j(\W)
\end{align}
Because $\frac{2}{n_j}\sum_{i=1}^{n_j/2} \yij\xij$
and 
$\frac{2}{n_j}\sum_{i={n_j/2}+1}^{n_j} \yij\xij$ 
are independent, and their expectation are both $\Hb^j(\W)$, so that
\begin{align*}
    &\quad \mtx{E}(\frac{2}{n_j}\sum_{i=1}^{n_j/2} \yij\xij)(\frac{2}{n_j}\sum_{i={n_j/2}+1}^{n_j} \yij\xij)^\top \\
    &= \Hb^j(\W)(\Hb^j(\W))^\top.
\end{align*}
At then end
\begin{align*}
    \hat \bM &= \frac{1}{k}\sum_{j=1}^k \mtx{E}(\frac{2}{n_j}\sum_{i=1}^{n_j/2} \yij\xij)(\frac{2}{n_j}\sum_{i={n_j/2}+1}^{n_j} \yij\xij)^\top,\\
    \bM &= \frac{1}{k}\sum_{j=1}^k\Hb^j(\W)(\Hb^j(\W))^\top,
\end{align*}
so we can prove Part (c) that $\mtx{E}(\hat \bM) = \bM$.
\end{proof}


\subsubsection{Proof of Theorem \ref{thm:hatM}}
We restate Theorem \ref{thm:hatM append} below. 
\begin{theorem}\label{thm:hatM append}
Suppose the data is generated as Def. \ref{def:task}. Let $\delta\in(0,1)$, $\epsilon\in(0,1)$. Suppose $y\x$ is a subGaussian random vector with covariance upper bounded by
\begin{align}
   \| \mathbf{Cov}(y \x) \| \le \sigma^2. \label{eq:covyx append}
\end{align} 
Define
\begin{align*}
    \mtx{h}^j(\W): \R^{r\times d} \rightarrow \R^d = \mtx{E}_{\x\sim\gauss} f^j(\W \x)  \x
\end{align*}
And let %$\bM = \mtx{E}_{\theta\sim\mathcal{N}(0,\bSi)} (g(\theta))^2\frac{\theta\theta^\top}{\|\theta\|^2}$, then
\begin{align*}
    \bM = \W^\top\W\left(\frac{1}{k}\sum_{j=1}^k \mtx{h}^j(\W)( \mtx{h}^j(\W))^\top\right)\W^\top\W
\end{align*}
Then there exists a constant $c$, with probability at least $1-\delta$, let 
\begin{align*}
    k = \frac{cd}{n}\log^2(\frac{kd}{\delta}) \max\{\frac{1}{\epsilon^2}, \frac{1}{\epsilon} \log(\frac{kd}{\delta})\}
\end{align*}
we have 
\begin{align*}
    \|\hat \bM - \bM\| \le \epsilon\sigma^2.
\end{align*}
\end{theorem}
\begin{proof}
The following lemmas are similar to \cite{kong2020meta} Section A.1. We extend the concentration inequalities from bounded random vectors to Gaussian random vectors. For completeness we place the lemmas here.

\begin{lemma}\label{lem:err_yx}
(\cite{jin2019short} Cor. 7) 
Let $\|\mathbf{Cov}(y\x)\| \le \sigma^2$, $\delta\in(0,1)$, $t>0$, $\Hb^j(\W)$ be defined in \eqref{eq:Hj def}. With probability $1-\delta$, there exists a constant $c>0$ such that for every $j$,
\som{Remind the exact assumption on $\sigma$}
\begin{align}
   \|\frac{1}{t}\sum_{i=1}^t \yij\xij - \Hb^j(\W)\| \le c\sigma\sqrt{\frac{d}{t}\log(\frac{kd}{\delta})} \label{eq:gauss_bern}
\end{align}
\som{Call $\W^\top\W \mtx{h}^j(\W)$ something for simpler notation}
Denote this event as $\mathcal{E}$.
\iffalse
{\it\color{red} for every i,j pairs ? }Denote this event as $\mathcal{E}$.
{\it \color{red} if we dont say "for every i,j pairs" ,k should not appear in an inequality which holds for only one task. Also maybe it is better to  cite [21] A.5, because [28] Cor.7 says only the following
$$\|\frac{1}{t}\sum_{i=1}^t \yij\xij - \W^\top\W \mtx{h}^j(\W)\| \le c\sigma\sqrt{\frac{1}{t}\log(\frac{2d}{\delta})}$$}
\fi
\end{lemma}
With the covariance of $y\x$ being bounded by $\sigma^2$, the following inequalities are true \cite{kong2020meta}.
\begin{align*}
    \Eb\left( (\vb^T\cdot (\frac{1}{t}\sum_{i=1}^t \yij\xij - \theta^j))^2\right) &\le \sigma^2 / t,\mbox{~for~} \|\vb\|=1.\\
    \Eb \left(\|\frac{1}{t}\sum_{i=1}^t \yij\xij - \theta^j \|^2\right) &\le \sigma^2d/t.
\end{align*}


\begin{lemma}\label{lem:Zj}
Define
\begin{align*}
    \Zb_j &= (\frac{2}{n_j}\sum_{i=1}^{n_j/2} \yij\xij)(\frac{2}{n_j}\sum_{i={n_j/2}+1}^{n_j} \yij\xij)^\top \\
    &\quad - \Hb^j(\W)(\Hb^j(\W))^\top,
\end{align*}
Then there exists a constant $c$ such that on the event $\mathcal{E}$ (thus with probability $1-\delta$), for all $j=1,...,k$, 
\begin{align}
    \|\Zb_j \| \le \frac{c\sigma^2d}{n_j} \log(\frac{kd}{\delta}). \label{eq:evt}
\end{align}
\end{lemma}

% {\it \color{red} From my understanding we should have 
% $$\|\Zb_j \| \le (Eq A.1 Bound)(Eq. A.1 bound + 2\|\W^\top\W \mtx{h}^j(\W)\|)$$ choosing $t=\dfrac{n_j}{2}$ then we have $$\|\Zb_j \| \le (c\sigma\sqrt{\frac{2}{n_j}\log(\frac{2d}{\delta})})(c\sigma\sqrt{\frac{2}{n_j}\log(\frac{2d}{\delta})} + 2\|\W^\top\W \mtx{h}^j(\W)\|)$$
% This is more or less what you have found, but the difference is k in $\log$ term and d term }



The proof is almost same as \cite{kong2020meta}, the only difference is that we replace the bound in (\cite{kong2020meta} Prop A.1) by \eqref{eq:gauss_bern}. With the similar replacement, we propose the following lemma. 
\begin{lemma}\label{lem:Zj2}
Let $\delta\in(0,1)$. There exists a constant $c$, such that for any $\epsilon\in(0,1)$, and 
\begin{align}
    k = \frac{cd}{n_j}\log^2(\frac{kd}{\delta}) \max\{\frac{1}{\epsilon^2}, \frac{1}{\epsilon} \log(\frac{kd}{\delta})\}, \label{eq:k lb}
\end{align}
with probability $1-\delta$, 
\begin{align*}
    \|\frac{1}{k} \sum_{j=1}^k \Zb_j\| \le \epsilon \sigma^2.
\end{align*}
\end{lemma}
This means that when \eqref{eq:k lb} is true, with probability $1-\delta$,
\begin{align*}
    \left\|\hat \bM - \W^\top\W\left(\frac{1}{k}\sum_{j=1}^k \mtx{h}^j(\W)( \mtx{h}^j(\W))^\top\right)\W^\top\W\right\| \le \epsilon \sigma^2.
\end{align*}
Note that $\bM$ is defined as \[\bM=\W^\top\W\left(\frac{1}{k}\sum_{j=1}^k \mtx{h}^j(\W)( \mtx{h}^j(\W))^\top\right)\W^\top\W.\] So we have proven that with probability $1-\delta$,
\begin{align*}
    \left\|\hat \bM - \bM\right\| \le \epsilon \sigma^2.
\end{align*}

\som{Remind that this is $\hat \bM-\bM$ i.e. $\bM=\text{the messy sum}$}
\end{proof}

\SO{Create a subsection here!!! Reduce the confusion as much as possible, make transitions smooth.}
\subsection{Proof of Theorem \ref{thm:down}}
Now we will prove Theorem \ref{thm:down}. We first review the notations and assumptions mentioned in the theorem.

\subsubsection{Review of Notations and Assumptions}
We define the SVD of $\hat \bM$ as $\hat \Ub \hat\La \hat\Vb^\top$. Let the first $r$ columns of $\hat \Ub$ be $\Ub_r$. 

Let $\hat\W$ be defined as 
\begin{align}
    \hat \W &= \hat \Ub_r \hat \Qb, \label{eq:def W append}\\
    \hat \Qb &= \mathop{\mathrm{argmin}}_{\Qb\in\R^{r\times r}, \Qb\Qb^\top = I}\ \|\hat \Ub_r \Qb - \W\|.
\end{align}
The population cross entropy loss is defined as
\begin{align*}
    &\cLCE(f;\Pb) : \Fc\times \R^{r\times d}\rightarrow \R=\\
    &-\mtx{E}_{\x,y\sim\Pxy} (y\log f(\hat\Pb \x) + (1-y)\log (1 - f(\hat\Pb \x))).
\end{align*}
We will search for a function $f^* \in \Fc$ that minimizes the population cross entropy loss. $\Fc$ is a set of functions satisfying
\begin{enumerate}
    \item For any function $f\in\Fc$, any orthonormal matrix $\Qb\in\R^{r\times r}$ and any matrix $\Pb\in\R^{r\times d}$, there exists $g \in \Fc$ such that $f(\Pb \x) = g(\Qb\Pb \x)$.
    \item $\Fc \subseteq \{f\ |\ \log f,~ \log(1-f)\mathrm{~are~}L\mathrm{~Lipschitz}\}\bigcap \{f\ |\ 0<f(x)<1,\forall x\in\R^r\}$.
\end{enumerate}
We solve for $\hat f$, defined as \begin{align}
    \hat f &= \argmin_{f\in\Fc}\ \cLCE(f;\hat \Ub_r^\top). \label{eq:def f append}
\end{align}
\subsubsection{Proof of Theorem \ref{thm:down}}
Now we are ready to restate Theorem \ref{thm:down} and prove it.
\begin{theorem}\label{thm:popu append}
Based on the definition above, we have that
    \begin{align*}
        \cLCE(\hat f;\hat \Ub_r^\top)  - \cLCE(f^*;\Ub_r^\top) \lesssim L\sqrt{r}\|\hat \W - \W\|.
    \end{align*}
\end{theorem}

\begin{proof}
We learn the model from the following optimization algorithm.
\begin{align*}
    \hat f &= \argmin_{f\in\Fc}\ \cLCE(f;\hat \Ub_r^\top)\\
    &= \argmin_{f\in\Fc}\ -\mtx{E}_{\x,y\sim\Pxy} (y\log f(\hat\Ub_r^\top \x) \\
    &\quad + (1-y)\log (1 - f(\hat\Ub_r^\top \x)))\\
    &= \argmin_{f\in\Fc}\ -\mtx{E}_{\x\sim\gauss} \left(f^*(\W \x)\log f(\hat \Ub_r^\top \x)\right. \\
    & \quad \left. + (1-f^*(\W \x))\log (1 - f(\hat \Ub_r^\top \x)) \right).
\end{align*}
Denote $\tilde f\in\Fc$ as the function such that $\tilde f(\hat \W \x) = \hat f(\hat \Ub_r^\top \x)$. So that $\cLCE(\hat f;\hat \Ub_r^\top) = \cLCE(\tilde f;\hat \W)$. Since $\hat f$ minimizes the cross entropy loss, we have that $\cLCE(\tilde f;\hat \W) \le \cLCE(f^*;\hat \W)$. 

Now we have 
\begin{align*}
    &\quad \cLCE (\tilde f;\hat \W) - \cLCE (f;\W)\\
    &\le \cLCE (f^*;\hat \W) - \cLCE (f^*;\W)\\
    &\le -\mtx{E}_{\x\sim\gauss} \left(f^*(\W \x)(\log f^*(\hat\W \x) -\log f^*(\W \x))\right. \\
    & \quad \left. + (1-f^*(\W \x))(\log (1 - f^*(\hat \W \x)) - \log (1 - f^*(\W \x))) \right)\\
    &\le \mtx{E}_{\x\sim\gauss} L\|(\hat \W - \W)x\|\\
    &\lesssim L\sqrt{r}\|\hat \W - \W\|.
\end{align*}
\end{proof}

\subsection{Proof of Theorem \ref{thm:rade}}
%Now we prove that the upper bound of the error for few-shot learning with finite samples.
We first state Theorem \ref{thm:rade} below.
\begin{theorem}\label{thm:rade app}
    Suppose we generate $n$ sample data for few shot learning solve for $\hat \theta_e$ from \eqref{eq:fstar finite theta}. There exist constants $c>0$, $\delta\in(0,1)$, with probability at least $1 - n^{-c+1} - \delta$, the solution $\hat\theta_e$ and $\hat\Ub_r$ satisfy
    \begin{align*}
        &\quad \mathcal{L} (\hat\theta_e;\hat\Ub_r^\top) - \mathcal{L} (\theta^*;\W) \\
        &\lesssim \frac{ac(\sqrt{r}+\log(n)) (1+ \sqrt{\log(1/\delta)})}{\sqrt{n}} + \sqrt{r}\|\hat \W - \W\|. 
    \end{align*}
\end{theorem}
\begin{proof}
We sketch the proof of Theorem \ref{thm:rade app}. After reviewing the notations, we quote a standard generalization bound via Rademacher complexity in Lemma \ref{lem:rade known}. Then we use the smoothness of the loss function to link to the generalization error of linear functions \eqref{eq:lin rade}, and then use Lemma \ref{lemma:chi-sqr} to compute \eqref{eq:lin rade} and finish the proof.

In few-shot learning, the true parameter is $\theta^*$, and the empirical loss function with finite data is 
\begin{align}
    &\cL_e(\theta;\Pb) : \Fc\times \R^{r\times d}\rightarrow \R= \notag\\
    &-\frac{1}{n}\sum_{i=1}^n (y_i\log\phi (\theta^\top\Pb \x_i) + (1-y_i)\log (1 - \phi(\theta^\top\Pb \x_i))) \label{eq:cLCE finite theta app}
\end{align}
Denote each term in the summation as 
\begin{align*}
    &\quad \cL_e^i(\theta;\Pb) : \Fc\times \R^{r\times d}\rightarrow \R=\notag\\
    &- (y_i\log \phi (\theta^\top\Pb \x_i) + (1-y_i)\log (1 - \phi(\theta^\top\Pb \x_i)))
\end{align*}
We search for the solution by
\begin{align}
    \hat \theta_e &= \argmin_{\theta}\ \cL_e(\theta;\Ub_r^\top),\mbox{~such~that~} \|\theta\|\le a.\label{eq:fstar finite theta app}
\end{align}
In Theorem \ref{thm:popu append}, we know that
\begin{align*}
    \cLCE(\hat \theta;\hat \Ub_r^\top)  - \cLCE(\theta^*;\Ub_r^\top) \lesssim L\sqrt{r}\|\hat \W - \W\|.
\end{align*}
Denote 
    \begin{align}
        M = \max_{\|\theta\|\le a} |\theta^\top \hat\Ub_r^\top\x_i| \le a \max\|\hat\Ub_r^\top\x_i\|.\label{eq:bound_rade}
    \end{align}
We will bound the difference between $\cL$ and $\cL_e$ by Rademacher complexity theory.
\begin{lemma}\label{lem:rade known}
    \cite{mohri2018foundations}
 
    Let $\mscrU$ be the independent random variables uniformly chosen from $\{-1,1\}$.
    Let $\Rc$ be the Rademacher complexity of the logistic functionals defined on the data,
    \begin{align*}
        \Rc &= \frac{1}{n}\Eb_{\epsilon_i\in\mscrU} \sup_{\|\theta\|\le a} \sum_{i=1}^n\epsilon_i\cL_e^i(\theta;\hat\Ub_r^\top) \\
        K &= |\log(\phi(-M))|>\max_i\cL_e^i(\theta;\hat\Ub_r^\top)
    \end{align*}
    %We know $\cL_e^i(\theta;\hat\Ub_r^\top)<K$ with probability at least $1-n^{-c_1+1}$,
    %then for any $\theta$ such that $\|\theta\|\le a$, with probability $1-\delta-n^{-c_1+1}$, we have that 
    with probability $1-\delta$, we have that 
    \begin{align*}
        |\cL_e(\theta;\Ub_r^\top) - \cL(\theta;\Ub_r^\top)| \le \Rc + \frac{\sqrt{\log(1/\delta)}}{\sqrt{n}}K.
    \end{align*}
\end{lemma}
Thus we have that 
\begin{align*}
    |\mathcal{L} (\hat\theta_e;\hat\Ub_r^\top) - \mathcal{L}_e (\hat\theta_e;\hat\Ub_r^\top)| &\le \Rc + \frac{\sqrt{\log(1/\delta)}}{\sqrt{n}}K,\\
    |\mathcal{L} (\hat\theta;\hat\Ub_r^\top) - \mathcal{L}_e (\hat\theta;\hat\Ub_r^\top)| &\le \Rc + \frac{\sqrt{\log(1/\delta)}}{\sqrt{n}}K.
\end{align*}
Because $\hat\theta_e$ minimizes the empirical loss $\mathcal{L}_e$,
\begin{align*}
    \mathcal{L}_e (\hat\theta_e;\hat\Ub_r^\top) \le \mathcal{L}_e (\hat\theta;\hat\Ub_r^\top).
\end{align*}
Thus 
\begin{align}
    \mathcal{L} (\hat\theta_e;\hat\Ub_r^\top) - \mathcal{L} (\hat\theta;\hat\Ub_r^\top) \le 2\left(\Rc + \frac{\sqrt{\log(1/\delta)}}{\sqrt{n}}K\right).\label{eq:emp loss}
\end{align}
So the remaining target is to bound $\Rc$. 

We first denote $\vb_i = \hat\Ub_r^\top \x_i$, so $\vb_i\in\R^r$ and $\vb_i$ are jointly independent standard normal random variables. In binary classification, $\cL_e^i$ is always $1$ Lipschitz in $\theta^\top\vb_i$, the Rademacher complexity can be upper bounded by
\begin{align}\label{eq:lin rade}
    \Rc \le \tilde\Rc := \frac{1}{n}\Eb_{\epsilon_i\in\mscrU} \sup_{\|\theta\|\le a} \sum_{i=1}^n \epsilon_i\theta^\top\vb_i. 
\end{align}
We first refer to the following lemma.
\begin{lemma}\label{lemma:chi-sqr}
    \cite{laurent2000adaptive} Let $c>0$, $X$ follow $\chi_r^2$ distribution, then
    \begin{align*}
        \Pb(X - r \ge 2\sqrt{cr\log n} + 2c\log n) \le n^{-c}.
    \end{align*}
\end{lemma}

For a constant $c>1$, via union bound we have that $\max{\|\vb_i\|^2} \le r + 2\sqrt{cr\log n} + 2c\log n$ for all $i=1,..,n$ with probability $1 - n^{-c+1}$. We use $\max{\|\vb_i\|} \lesssim c(\sqrt{r} + \log(n))$ for simplicity.

Conditioned on this event, we apply the Rademacher complexity for linear model that 
\begin{align}
   \tilde \Rc &\le \frac{\max\|\theta\| \cdot \max\|\vb_i\|}{\sqrt{n}}\\
   &\le \frac{ca(\sqrt{r} + \log(n))}{\sqrt{n}}. \label{eq:tilde Rc}
\end{align}
Combining with \eqref{eq:emp loss} and Theorem \ref{thm:popu append} we get the bound in Theorem \ref{thm:rade app}. We can also bound $M$ in \eqref{eq:bound_rade}.

Finally we will use Lemma \ref{lem:M to K} to bound $M$.
\begin{lemma}\label{lem:M to K}
    Let $M$ be defined as in \eqref{eq:bound_rade}.    
    With probability at least $1 - n^{-c+1}$, we have $M<ac(\sqrt{r} + \log(n))$.
\end{lemma}
Let $\vb_i$ be replaced by $\hat \Ub_r^\top\x_i$ in Lemma \ref{lemma:chi-sqr}, then this directly results from Lemma \ref{lemma:chi-sqr}. Lemma \ref{lem:M to K} bounds $M$, thus bounds $K$ (which is $1$ Lipschitz in $M$) in Lemma \ref{lem:rade known}. After we insert \eqref{eq:tilde Rc} together into Lemma \ref{lem:rade known}, we can get the result in  Theorem \ref{thm:rade}.
% By Lemma \ref{lemma:chi-sqr} we know that for a constant $c>2$, we have  $\max{\|\hat\Ub_r^\top\x_i\|} \le c(\sqrt{r} + \log(n))$ for all $i=1,..,n$ with probability $1 - n^{-c+1}$. So with probability at least $1 - n^{-c+1}$, we have $M<ac(\sqrt{r} + \log(n))$.
\end{proof}



==> Icassp (3)/Paper/s_prob.tex <==
\setlength{\topsep}{0.25em}
\newcommand{\xij}{{\x_{i,j}}}
\newcommand{\xijt}{{\x_{i,j}^\top}}
\newcommand{\yij}{{y_{i,j}}}

\section{Problem Formulation}\label{s:prob}
% {\color{red} YS: a paragraph for notation?}
The meta-learning setup that will be considered in this work consists of two phases: (i) meta-training: prior tasks are used to learn a good representation and (ii) few-shot learning: the new task is learned with few samples.
%\som{Is meta-train/test standard and correct phrases?} 
%{\mf better not to use the meta-train and meta-test phrases if we don't need to} 
In the meta-training phase, we learn the low dimensional space spanned by parameters. In the few-shot learning phase, we use the subspace to learn the model of a new task ideally with few samples.

In the first phase, there are multiple tasks to infer from, each with its own distribution. We consider a realizable model where the input and label is associated via a labeling function. One accesses batches of data, each of whom is collected from a task, however we may not know which task it comes from. We make this setup more precise using the following definitions. Below, the ground-truth representation will be denoted by a matrix $\W\in\R^{r\times d}$ row space of which corresponds to the subspace of interest.

%\som{Use $n_j$ for sample size rather than $t_j$ (at least for training)}
\begin{definition} \label{def:task}
\textbf{Meta-training data.} Fix a matrix $\W\in\R^{r\times d}$ satisfying $\W\W^T=\Iden$. The $j$-th task is associated with function $f^j: \R^r\rightarrow \R$. Given input $\x$, the label $y$ is distributed as $p_j(y|\x)=p_j(y|\W\x)$\footnote{In words, the label only depends on the relevant features induced by $\W$.} and the expectation satisfies $\mtx{E}(y) = f^j(\W\x)$.
%{\mf give properties like domain and range of $f$ here, first time it appears.}
Suppose there are $n_j$ samples from the $j$-th task sampled i.i.d.~from this distribution and we denote the dataset $\Sc^j = (\xij, \yij)_{i=1}^{n_j}$. Define the full meta-training dataset to be $\Sc = \bigcup_{j=1}^k\Sc^j$.
\end{definition}
Here, $f^j$ is allowed to be any Lipschitz nonlinear function, i.e., a neural network\footnote{In our theoretical results, we treat $f$ as a general linear function, and in experiments we will use a neural network with a specific structure.}.


%In the multi-task problem, there are a collection of tasks in the meta-training phase, which is defined below.


\iffalse
\begin{definition}\label{def:task dis}\som{I don't think we should use a distribution early on.}
\textbf{Low rank task distribution.} There are in total $k$ tasks. Each training task is associated with a parameter vector $\bt^j\in\R^d$ for $j=1,...,k$.
{\mf right now we're just setting the notation---additional assumptions like definition 2.2 on random features should come later.}
These are generated i.i.d. from a Gaussian distribution $\mathcal{N}(0, \bSi)$. Let $\la_i$ be the $i$-th eigenvalue of $\bSi$ with decreasing order. For low rank parameters, we assume that $\la_{r+1} = 0$. We call $r$ as the effective dimension of parameters.
\end{definition}



\begin{definition} \label{def:task}
\textbf{Meta-training data.} The $j$-th task is associated with parameter $\bt^j\in\R^d$. 
%For any parameter $\bt$, one can collect data from it. 
Suppose there are $n_j$ data from the $j$-th task, we call the dataset $\Sc^j = \{(\xij, \yij)\ |\ i=1,...,n_j\}$. Here $\xij\in\R^d$, $\yij\in\R$. $\xij$, $\yij$ satisfy $\mtx{E}(\yij) = f(\xijt\bt^j)$ for some function $f$. Let the whole meta-training dataset be $\Sc = \bigcup_{j=1,...,k}\Sc^j$. {\mf repeated}
\end{definition}

%\noindent\textbf{:}

\begin{definition} \label{def:data_gen}
\textbf{Data generation.} We assume that there are $k$ binary classification tasks, the $j$-th associated with $\bt^j$. The data $\Sc^j$ is generated by $\xij = \bz / \|\bz\|$ and $\bz \sim \mathcal{N}(0, I)$, $\bz$ is generated independently. Denote the distribution of $\xij$ as $\mathscr{P}_x$.
%The labels $\yij$ satisfy
%$\mtx{E}(\yij|\xij, \bt^j) = f(\xijt\bt^j)$ for some Lipschitz function $f:\R\rightarrow \R$. We propose two examples below.
\end{definition}
%{\color{blue} Do we need to normalize $x$? Just for citing the result in \cite{kong2020meta}, they use Bernstein so they have to use bounded rv. In principle unbounded subGaussian works.}
\fi


\begin{definition} \label{def:bin_class}
\textbf{Binary classification.} Suppose $f^j$ takes values over $[0,1]$,
%{\it\color{red}{Is it [0,1] ?}}. The labels $\yij$ are generated as 
\begin{align*}
    \yij = 
     \begin{cases}
       \text{1,} &{\mbox{with probability } f^j(\W \xij),}\\
       \text{0,} &{\mbox{with probability } 1-f^j(\W\xij).}\\
     \end{cases}
\end{align*}
%Here $f^j(a)\in[0,1]$ for all $a\in[-1,1]$, and the event that $f(a) = 0$ is not true with probability $1$ with respect to Lebesgue measure on $[-1,1]$\footnote{In other words, $f$ is not a constant $0$ function.}.
\end{definition}

\begin{definition}\label{def:GLM}
\noindent\textbf{Generalized linear models (GLM)} (which include logistic/linear regression) can be modeled by choosing $f^j$ to be parameterized by a vector $\bt_j\in\R^r$ and a link function $\phi:\R\rightarrow\R$ as $f^j(\W \xij) := \phi(\bt_j^T\W\xij )$.

\end{definition}
%for $\bt_j\in\R^r$, $\phi$ is a function mapping from $\R$ to $(0,1)$.

% Denote the distribution of $\x,y$ as $\mathscr{P}_{x,y}$.
%\begin{definition}\label{def:nn}
%\textbf{Non-linear regression.} More generally, for $\bt^j\in\R^{r\times d}$, the labels $\yij$ are generated as
%\begin{align*}
%    \yij = f^j(\W\xij) + \epsilon,
%\end{align*}
%$\epsilon$ is a zero mean bounded random variable. 
%\end{definition}

When the dimension of the span of parameters is small, \cite{kong2020meta} performs a dimension reduction algorithm to find the low-dimensional subspace that the parameters span. This is done by selecting the top eigenvectors of the covariance estimate of the cross-correlation between input and labels.
\begin{definition}\label{def:mom}
\textbf{Moment estimator of covariance.} We define the covariance estimator as
\begin{subequations}\label{eq:hatM}
\begin{align}
\hat\bM &= \mathop{\Scale[1.8]{\sum}}_{j=1}^k \frac{2}{n_j^2}\left[(\sum_{i=1}^{n_j/2} \yij\xij) (\sum_{i=n_j/2+1}^{n_j} \yij\xij)^\top \right.\\
&\quad\quad\quad\quad \left. +  ( \sum_{i=n_j/2+1}^{n_j} \yij\xij) ( \sum_{i=1}^{n_j/2} \yij\xij)^\top\right].\nonumber
\end{align}
\end{subequations}
\end{definition}
\noindent\textbf{Subspace estimation.} 
To estimate the subspace $\W$, we use rank-$r$ approximation of $\hat \bM$ to retrieve its principal eigenvector subspace. 
Let $\hat\Ub \hat \La \hat \Ub^\top$ be the eigen-decomposition of $\hat \bM$. Denote $\hat \la_j$ as the $j$th eigenvalue of $\hat \La$. Let $\hat\Ub_r$ be the first $r$ columns of $\hat\Ub$, thus the rank-$r$ approximation is $\hat\bM_r = \hat\Ub_r \mathrm{diag}(\hat \la_{1},...,\hat\la_{r}) \hat \Ub_r^\top$. In the next section, we will prove that the range of $\hat \Ub$ is close to the row space of $\W$.

%{\color{blue} No need to put an algorithm here. If we have a bound for downstream task as well we can fill up the whole procedure.}

%Now we propose the algorithm that accomplishes the subspace retrieval process above. 

In Algorithm \ref{algo:1}, the output $\hat\Ub_r$ is the estimator of the task subspace $\W$. $\hat\Ub_r$ is used as a training step for the few-shot learning phase. For the new task, we search for the function $f^*$ that minimizes the population loss. We shall provide an instructive analysis for the cross-entropy loss, which is usually employed for classification tasks.

\so{Currently, cross-entropy comes out of nowhere. For using cross-ent, label has to be discrete. It cannot be an arbitrary nonlinear function. Overall, we need to do one of the followings:\\
 Option 1: Do the analysis for a Lipschitz loss function for which cross-entropy is a special case.\\
 Option 2: Let us just say that for few-shot phase, we focus on classification and study cross-entropy. Clearly state label is discrete 0-1.}
\begin{definition}\label{def: test}
\textbf{Few-shot classification (Population).} In the few-shot learning phase, suppose $\x,y\sim\Pxy$ satisfy $\mtx{E}(y|\x) = f^*(\W\x)$. Let $\Fc$ be a family of functions as the search space for few-shot learning model. 
Let $\cLCE: \Fc\times \R^{r\times d}\rightarrow \R$ be population cross-entropy loss, defined as 
\begin{align}
    \cLCE(f;\Pb)=-\mtx{E}_{\Pxy} (&y\log f(\Pb \x)\label{eq:cLCE}\\
   &+ (1-y)\log (1 - f(\Pb \x))) \nonumber.
\end{align}
\so{Following my comment above, for cross-ent, clearly $0\leq f\leq 1$. This has to be specified in the definition.}

We search for the solution induced by $\hat{\Ub}_r$ by
\begin{align}
    \hat f &= \argmin_{f\in\Fc}\ \cLCE(f;\hat{\Ub}_r^\top)\label{eq:fstar}
\end{align}
%If $\Pb$ is known, we use $\cLCE(f(\Pb x))$ as an equivalent way of representing $\cLCE(f;\Pb)$.
\end{definition}
Observe that, without representation learning, one has to search for both $f$ and $\Pb$. However with representation learning, we fix $\Pb=\hat{\Ub}_r$ and only search for $f$.
\begin{remark}\label{rem:logistic}
For the GLM Definition \ref{def:GLM}, we can choose $\Fc$ to be the $\ell_2$ norm constrained functions for some $a\leq\infty$% the set of functions $f$ satisfying
% {\color{red} YS: I want to say $\Fc = \phi\circ\bt\circ(\mathrm{variable})$}
\begin{align}
    \Fc = \{\x\rightarrow \phi(\bt^T\x)~\big|~\|\bt\|_2 \le a,~\bt\in\R^r\}, \label{eq:Fcbin}
\end{align}
Let the new data be generated with $f^*(\W\x) = \phi({\bt^*}^\top\W\x)$ for some ground-truth parameter $\bt^*$. We use $\cLCE(\bt;\Pb)$ to denote the cross-entropy loss in this setting. $\hat f$ (parameterized by $\hat{\bt}$) is given by
\begin{align}
    \hat \bt &= \argmin_{\bt}\ \cLCE(\bt;\hat \Ub_r^\top ),\mbox{~such~that~} \|\bt\| \le a. \label{eq:fstarbin}
\end{align}
\end{remark}


\iffalse
\begin{definition}\label{def: test finite}
\textbf{Finite sample few-shot learning.} In the few-shot learning phase, there are in total $n$ samples, and suppose 
$\x_i\in\R^d$ are generated independently, following standard normal distribution, $y_i\in\R$, for $i=1,...,n$. $\x_i$, $y_i$ satisfy $\mtx{E}(y_i|\x_i) = f^*(\W\x_i)$. Lef $\Fc$ be a family of functions as the search space for few-shot activation function. 
Let $\cL_e$ be empirical cross entropy loss, defined as 
\begin{align}
    &\cL_e(f;\Pb) : \Fc\times \R^{r\times d}\rightarrow \R= \notag\\
    &-\frac{1}{n}\sum_{i=1}^n (y_i\log f(\Pb \x_i) + (1-y_i)\log (1 - f(\Pb \x_i))) \label{eq:cLCE finite}
\end{align}
We search for the solution by
\begin{align}
    \hat f_e &= \argmin_{f\in\Fc}\ \cL_e(f;\Ub_r^\top)\label{eq:fstar finite}
\end{align}

\end{definition}
\fi
% and suppose $\x_i\in\R^d$ are generated independently, following standard normal distribution, $y_i\in\R$, for $i=1,...,n$.
\begin{definition}\label{def: test finite}
\textbf{Few-shot learning (Finite sample GLM).} Suppose there are in total $n$ samples for new task $(\x_i,y_i)_{i=1}^n$ and $(\x_i,y_i)$ satisfies $\mtx{E}(y_i|\x_i) = f^*(\W\x_i)$. Lef $\Fc$ be a family of functions for few-shot learning phase. We consider the setup of Remark \ref{rem:logistic}, where $\phi$ is the logistic function. 
%: \Fc\times \R^{r\times d}\rightarrow \R= \notag\\
\begin{align}
    \cL_e(\bt;\Pb)=-\frac{1}{n}\sum_{i=1}^n (&y_i\log(\phi (\bt^\top\Pb \x_i))\label{eq:cLCE finite theta}\\
    &+ (1-y_i)\log (1 - \phi(\bt^\top\Pb \x_i))).\nonumber 
\end{align}
Given an $\ell_2$-norm constraint $a\leq \infty$, the empirical risk minimizer (ERM) is defined as follows
\begin{align}
    \hat \bt_e &= \argmin_{\bt}\ \cL_e(\bt;\Ub_r^\top)\quad\text{such~that}\quad\|\bt\|_2\le a.\label{eq:fstar finite theta}
\end{align}
\end{definition}


\begin{algorithm}[t!]
\caption{Meta-training and Few-shot Learning}\label{algo:1}
\begin{algorithmic}
% with $k$ tasks, the size of data of the $j$-th task has size $n_j$. Dimension $d$. Effective dimension $r$. Set of functions $\Fc$.
\REQUIRE {Dataset $\mathcal{S}$, representation size $r$, function space $\Fc$}
\STATE{Compute $\hat \bM$ via method-of-moments \eqref{eq:hatM}.}
\STATE{Rank $r$ approximation:\\
$\quad\hat\bM_r \leftarrow \hat\Ub_r \mathrm{diag}(\hat \La_{1,1},...,\hat\La_{r,r}) \hat \Ub_r^\top$.}
\STATE{Either~$\hat f \leftarrow \argmin_{f\in\Fc}\ \cLCE(f;\Ub_r^\top) $. $\cLCE$ is defined as \eqref{eq:cLCE}.}
\STATE{Or~~~~~~$\hat f_e \leftarrow \argmin_{f\in\Fc}\ \cL_e(f;\Ub_r^\top) $. $\cL_e$ is defined as \eqref{eq:cLCE finite theta}}
\RETURN{$\hat\Ub_r$ and $\hat f$ or $\hat f_e$.}
\end{algorithmic}
\end{algorithm}%\vspace{-10pt}


==> Icassp (3)/Paper/s_prob_2.tex <==
\setlength{\topsep}{0.25em}
\newcommand{\xij}{{\x_{i,j}}}
\newcommand{\xijt}{{\x_{i,j}^\top}}
\newcommand{\yij}{{y_{i,j}}}

\section{Problem Formulation}\label{s:prob}
% {\color{red} YS: a paragraph for notation?}
\vspace{-0.1cm}
The meta-learning setup that will be considered in this work consists of two phases: (i) meta-training: prior tasks are used to learn a good representation and (ii) few-shot learning: the new task is learned with few samples.
%\som{Is meta-train/test standard and correct phrases?} 
%{\mf better not to use the meta-train and meta-test phrases if we don't need to} 
In the meta-training phase, we learn the low dimensional space spanned by parameters. In the few-shot learning phase, we use the subspace to learn the model of a new task ideally with few samples.

In the first phase, there are multiple task vectors to infer from.%, each with its own distribution. 
We consider a realizable model where the input and label is associated via a labeling function. One accesses batches of data, each of whom is collected from a task.
%, however we may not know which task it comes from. 
%We make this setup more precise using the following definitions. 
Below, we denote the ground-truth representation by a matrix $\W\in\R^{r\times d}$ whose row space corresponds to the subspace of interest.

%\som{Use $n_j$ for sample size rather than $t_j$ (at least for training)}
\begin{definition} \label{def:task}
\textbf{Meta-training data.} Fix a matrix $\W\in\R^{r\times d}$ satisfying $\W\W^T=\Iden$. The $j$-th task is associated with function $f^j: \R^r\rightarrow \R$. Given input $\x\in\R^{d}$, the label $y$ is distributed as $p_j(y|\x)=p_j(y|\W\x)$\footnote{In words, the label only depends on the relevant features induced by $\W$.} and the expectation satisfies $\mtx{E}(y) = f^j(\W\x)$.
%{\mf give properties like domain and range of $f$ here, first time it appears.}
Suppose there are $n_j$ samples from the $j$-th task sampled i.i.d.~from this distribution and we denote the dataset $\Sc^j = (\xij, \yij)_{i=1}^{n_j}$. Define the full meta-training dataset to be $\Sc = \bigcup_{j=1}^k\Sc^j$.
\end{definition}
Here, $f^j$ is allowed to be any Lipschitz nonlinear function, i.e., a neural network\footnote{In our theoretical results, we treat $f$ as a general linear function, and in experiments we will use a neural network with a specific structure.}.


%In the multi-task problem, there are a collection of tasks in the meta-training phase, which is defined below.


\iffalse
\begin{definition}\label{def:task dis}
%\som{I don't think we should use a distribution early on.}
\textbf{Low rank task distribution.} There are in total $k$ tasks. Each training task is associated with a parameter vector $\bt^j\in\R^d$ for $j=1,...,k$.
{\mf right now we're just setting the notation---additional assumptions like definition 2.2 on random features should come later.}
These are generated i.i.d. from a Gaussian distribution $\mathcal{N}(0, \bSi)$. Let $\la_i$ be the $i$-th eigenvalue of $\bSi$ with decreasing order. For low rank parameters, we assume that $\la_{r+1} = 0$. We call $r$ as the effective dimension of parameters.
\end{definition}



\begin{definition} \label{def:task}
\textbf{Meta-training data.} The $j$-th task is associated with parameter $\bt^j\in\R^d$. 
%For any parameter $\bt$, one can collect data from it. 
Suppose there are $n_j$ data from the $j$-th task, we call the dataset $\Sc^j = \{(\xij, \yij)\ |\ i=1,...,n_j\}$. Here $\xij\in\R^d$, $\yij\in\R$. $\xij$, $\yij$ satisfy $\mtx{E}(\yij) = f(\xijt\bt^j)$ for some function $f$. Let the whole meta-training dataset be $\Sc = \bigcup_{j=1,...,k}\Sc^j$. {\mf repeated}
\end{definition}

%\noindent\textbf{:}

\begin{definition} \label{def:data_gen}
\textbf{Data generation.} We assume that there are $k$ binary classification tasks, the $j$-th associated with $\bt^j$. The data $\Sc^j$ is generated by $\xij = \bz / \|\bz\|$ and $\bz \sim \mathcal{N}(0, I)$, $\bz$ is generated independently. Denote the distribution of $\xij$ as $\mathscr{P}_x$.
%The labels $\yij$ satisfy
%$\mtx{E}(\yij|\xij, \bt^j) = f(\xijt\bt^j)$ for some Lipschitz function $f:\R\rightarrow \R$. We propose two examples below.
\end{definition}
%{\color{blue} Do we need to normalize $x$? Just for citing the result in \cite{kong2020meta}, they use Bernstein so they have to use bounded rv. In principle unbounded subGaussian works.}
\fi


\begin{definition} \label{def:bin_class}
\textbf{Binary classification.} Suppose $f^j$ takes values over $[0,1]$,
%{\it\color{red}{Is it [0,1] ?}}. The labels $\yij$ are generated as 
\begin{align*}
    \yij = 
     \begin{cases}
       \text{1,} &{\mbox{with probability } f^j(\W \xij),}\\
       \text{0,} &{\mbox{with probability } 1-f^j(\W\xij).}\\
     \end{cases}
\end{align*}
%Here $f^j(a)\in[0,1]$ for all $a\in[-1,1]$, and the event that $f(a) = 0$ is not true with probability $1$ with respect to Lebesgue measure on $[-1,1]$\footnote{In other words, $f$ is not a constant $0$ function.}.
\end{definition}

\begin{definition}\label{def:GLM}
\noindent\textbf{Generalized linear models (GLM)} (which include logistic/linear regression) can be modeled by choosing $f^j$ to be parameterized by a vector $\bt_j\in\R^r$ and a link function $\phi:\R\rightarrow\R$ as $f^j(\W \xij) := \phi(\bt_j^T\W\xij )$.

\end{definition}
%for $\bt_j\in\R^r$, $\phi$ is a function mapping from $\R$ to $(0,1)$.

% Denote the distribution of $\x,y$ as $\mathscr{P}_{x,y}$.
%\begin{definition}\label{def:nn}
%\textbf{Non-linear regression.} More generally, for $\bt^j\in\R^{r\times d}$, the labels $\yij$ are generated as
%\begin{align*}
%    \yij = f^j(\W\xij) + \epsilon,
%\end{align*}
%$\epsilon$ is a zero mean bounded random variable. 
%\end{definition}

When the dimension of the span of parameters is small, \cite{kong2020meta} performs a dimension reduction algorithm to find the low-dimensional subspace that the parameters span. This is done by selecting the top eigenvectors of the covariance estimate of the cross-correlation between input and labels.
\begin{definition}\label{def:mom}
\textbf{Moment estimator of covariance.} We define the covariance estimator as
\begin{equation}\label{eq:hatM}
\begin{split}
\hat\bM &= \mathop{\Scale[1.8]{\sum}}_{j=1}^k \frac{2}{n_j^2}\left[(\sum_{i=1}^{n_j/2} \yij\xij) (\sum_{i=n_j/2+1}^{n_j} \yij\xij)^\top \right.\\
&\quad\quad\quad\quad \left. +  ( \sum_{i=n_j/2+1}^{n_j} \yij\xij) ( \sum_{i=1}^{n_j/2} \yij\xij)^\top\right].
\end{split}
\end{equation}
Define
\begin{align*}
    &\mtx{h}^j(\W): \R^{r\times d} \rightarrow \R^d = \mtx{E}_{\x}[f^j(\W \x)\x]\\
    &\bM := \W^\top\W\left(\frac{1}{k}\sum_{j=1}^k \mtx{h}^j(\W)( \mtx{h}^j(\W))^\top\right)\W^\top\W.
\end{align*}
\end{definition}
We will prove that $\hat\bM$ is a finite sample estimate of $\bM$.
\noindent\textbf{Subspace estimation.} 
To estimate the subspace $\W$, we use rank-$r$ approximation of $\hat \bM$ to retrieve its principal eigenvector subspace. 
Let $\hat\Ub \hat \La \hat \Ub^\top$ be the eigen-decomposition of $\hat \bM$. Denote $\hat \la_j$ as the $j$th eigenvalue of $\hat \La$. Let $\hat\Ub_r$ be the first $r$ columns of $\hat\Ub$, thus the rank-$r$ approximation is $\hat\bM_r = \hat\Ub_r \mathrm{diag}(\hat \la_{1},...,\hat\la_{r}) \hat \Ub_r^\top$. In the next section, we will prove that the range of $\hat \Ub$ is close to the row space of $\W$.

%{\color{blue} No need to put an algorithm here. If we have a bound for downstream task as well we can fill up the whole procedure.}

%Now we propose the algorithm that accomplishes the subspace retrieval process above. 

In Algorithm \ref{algo:1}, the output $\hat\Ub_r$ is the estimator of the task subspace $\W$. $\hat\Ub_r$ is used as a training step for the few-shot learning phase. For the new task, we search for the function $f^*$ that minimizes the population loss. We shall provide an instructive analysis for a general class of functional family and loss.
\begin{assumption}\label{ass:F}
$\Fc$ is a set of functions satisfying: For any function $f\in\Fc$, any orthonormal matrix $\Qb\in\R^{r\times r}$ and any representation matrix $\Pb\in\R^{r\times d}$, there exists $g \in \Fc$ such that $f(\Pb \x) = g(\Qb\Pb \x)$.
%\begin{enumerate}
%    \item For any function $f\in\Fc$, any orthonormal matrix $\Qb\in\R^{r\times r}$ and any matrix $\Pb\in\R^{r\times d}$, there exists $g \in \Fc$ such that $f(\Pb \x) = g(\Qb\Pb \x)$.
%    \item $\Fc \subseteq \{f\ |\ \log f,~ \log(1-f)\mathrm{~are~}L\mathrm{~Lipschitz}\}\bigcap \{f\ |\ 0<f(x)<1,\forall x\in\R^r\}$.
%\end{enumerate}
\end{assumption}
\ys{In this assumption, we basically mean that the $\Fc$ is invariant with orthonormal rotation $\Qb$. In other words, we only need to find the $r$ dimensional row space $\mathrm{row}(\Pb)$ (to project the features onto it as a low dimensional representation), and don't worry the exact matrix $\Pb$ itself.

Let us introduce population risk $\cL$ and empirical risk $\cL_e$ based on any single loss function between model prediction and true label.}
\begin{align*}
&\cL(f;\Pb) = \mtx{E}_{\Pxy}\cLoss(f(\Pb \x),y)\\
&\cL_e(f;\Pb) = \frac{1}{n}\sum_{i=1}^n\cLoss(f(\Pb \x_i),y_i).
\end{align*}
We make the following assumption on the population risk.
\begin{assumption}\label{ass:L}
Suppose population loss $\cL$ and empirical loss $\cL_e$ satisfy the following assumptions:
\begin{enumerate}[itemsep=-0.1em,topsep=0.3em]
    %\item $\cL$ has the form $\cL(f;\Pb) = \mtx{E}_{\Pxy}\cL(f(\Pb \x),y)$.
    %$\cL_e$ has the form $\cL_e(f;\Pb) = \frac{1}{n}\sum_{i=1}^n\cL(f(\Pb \x_i),y_i)$.
    \item $\cL$ is $L$ Lipschitz in $\Pb \x$.
    \item $\min_{\Pb}\cL(f;\Pb) = \cL(f;\W)$.
\end{enumerate}
\end{assumption}
\noindent\textbf{Example:} Suppose $f$ is an $L$-Lipschitz function with range in $(0,1)$ \ys{and the true labels $y_i$ are from $\{0,1\}$.} The cross entropy function satisfies the assumptions.
\begin{align}
    \cLCE(f;\Pb)=-\mtx{E}_{\Pxy} (&y\log f(\Pb \x)\label{eq:cLCE}\\
   &+ (1-y)\log (1 - f(\Pb \x))) \nonumber.\\
   \cL_e(f;\Pb)=-\frac{1}{n}\sum_{i=1}^n (&y_i\log(f(\Pb \x_i))\label{eq:cLCE finite theta}\\
    &+ (1-y_i)\log (1 - f(\Pb \x_i))).\nonumber 
   %\cL_e(\bt;\Pb)=-\frac{1}{n}\sum_{i=1}^n (&y_i\log(\phi (\bt^\top\Pb \x_i))\label{eq:cLCE finite theta}\\
    %&+ (1-y_i)\log (1 - \phi(\bt^\top\Pb \x_i))).\nonumber 
\end{align}
\ys{With an abuse of notation, we can define the loss with respect to parameterization of the function $f$. For example, if we use the model in Def. \ref{def:GLM}, then we can write the empirical loss as 
\begin{align}
    \cL_e(\bt;\Pb)=-\frac{1}{n}\sum_{i=1}^n (&y_i\log(\phi (\bt^\top\Pb \x_i))\\%\label{eq:cLCE finite theta}\\
    &+ (1-y_i)\log (1 - \phi(\bt^\top\Pb \x_i))).\nonumber
\end{align}
}

% the cross-entropy loss, which is usually employed for classification tasks.
\iffalse
\so{Currently, cross-entropy comes out of nowhere. For using cross-ent, label has to be discrete. It cannot be an arbitrary nonlinear function. Overall, we need to do one of the followings:\\
 Option 1: Do the analysis for a Lipschitz loss function for which cross-entropy is a special case.\\
 Option 2: Let us just say that for few-shot phase, we focus on classification and study cross-entropy. Clearly state label is discrete 0-1.}
 \fi
\begin{definition}\label{def: test}
\textbf{Few-shot classification (Population).} In the few-shot learning phase, suppose $\x,y\sim\Pxy$ satisfy $\mtx{E}[y~|~\x] = f^*(\W\x)$. Let $\Fc$ be a family of functions as the search space for few-shot learning model. 
Let Assumptions \ref{ass:F} and \ref{ass:L} hold. We search for the solution induced by $\hat{\Ub}_r$ by
\begin{align}
    \hat f &= \argmin_{f\in\Fc}\ \cLCE(f;\hat{\Ub}_r^\top)\label{eq:fstar}
\end{align}
%$\cLCE: \Fc\times \R^{r\times d}\rightarrow \R$ be population cross-entropy loss, defined as 
%\begin{align}
%    \cLCE(f;\Pb)=-\mtx{E}_{\Pxy} (&y\log f(\Pb \x)\label{eq:cLCE}\\
%   &+ (1-y)\log (1 - f(\Pb \x))) \nonumber.
%\end{align}

\iffalse
\so{Following my comment above, for cross-ent, clearly $0\leq f\leq 1$. This has to be specified in the definition.}
\fi


%If $\Pb$ is known, we use $\cLCE(f(\Pb x))$ as an equivalent way of representing $\cLCE(f;\Pb)$.
\end{definition}
Observe that, without representation learning, one has to search for both $f$ and $\W$. However with representation learning, we use $\hat{\Ub}_r^\top$ as the representation matrix and only search for $f$.
\begin{remark}\label{rem:logistic}
For the GLM Definition \ref{def:GLM}, we can choose $\Fc$ to be the $\ell_2$ norm constrained functions for some $a\leq\infty$% the set of functions $f$ satisfying
% {\color{red} YS: I want to say $\Fc = \phi\circ\bt\circ(\mathrm{variable})$}
\begin{align}
    \Fc = \{\x\rightarrow \phi(\bt^T\x)~\big|~\|\bt\|_2 \le a,~\bt\in\R^r\}, \label{eq:Fcbin}
\end{align}
Let the new data be generated with $f^*(\W\x) = \phi({\bt^*}^\top\W\x)$ for some ground-truth parameter $\bt^*$. We use $\cLCE(\bt;\Pb)$ to denote the cross-entropy loss in this setting. $\hat f$ (parameterized by $\hat{\bt}$) is given by
\begin{align}
    \hat \bt &= \argmin_{\bt}\ \cLCE(\bt;\hat \Ub_r^\top ),\mbox{~such~that~} \|\bt\| \le a. \label{eq:fstarbin}
\end{align}
\end{remark}


\iffalse
\begin{definition}\label{def: test finite}
\textbf{Finite sample few-shot learning.} In the few-shot learning phase, there are in total $n$ samples, and suppose 
$\x_i\in\R^d$ are generated independently, following standard normal distribution, $y_i\in\R$, for $i=1,...,n$. $\x_i$, $y_i$ satisfy $\mtx{E}(y_i|\x_i) = f^*(\W\x_i)$. Lef $\Fc$ be a family of functions as the search space for few-shot activation function. 
Let $\cL_e$ be empirical loss, satisfying Assumptions \ref{ass:F} and \ref{ass:L}.

%defined as 
%\begin{align}
%    &\cL_e(f;\Pb) : \Fc\times \R^{r\times d}\rightarrow \R= \notag\\
%    &-\frac{1}{n}\sum_{i=1}^n (y_i\log f(\Pb \x_i) + (1-y_i)\log (1 - f(\Pb \x_i))) \label{eq:cLCE finite}
%\end{align}
We search for the solution by
\begin{align}
    \hat f_e &= \argmin_{f\in\Fc}\ \cL_e(f;\Ub_r^\top)\label{eq:fstar finite}
\end{align}

\end{definition}
\fi
% and suppose $\x_i\in\R^d$ are generated independently, following standard normal distribution, $y_i\in\R$, for $i=1,...,n$.
\begin{definition}\label{def: test finite}
\textbf{Few-shot learning (Finite sample GLM).} Suppose there are $n$ samples for new task $(\x_i,y_i)_{i=1}^n$ and $(\x_i,y_i)$ satisfies $\mtx{E}(y_i|\x_i) = f^*(\W\x_i)$. 
%Let $\Fc$ be a family of functions for few-shot learning phase. 
Let $\cL_e$ be empirical loss, satisfying Assumptions \ref{ass:F} and \ref{ass:L}.
%We consider the setup of Remark \ref{rem:logistic}, where $\phi$ is the logistic function. 
%: \Fc\times \R^{r\times d}\rightarrow \R= \notag\\
%\begin{align}
%    \cL_e(\bt;\Pb)=-\frac{1}{n}\sum_{i=1}^n (&y_i\log(\phi (\bt^\top\Pb \x_i))\label{eq:cLCE finite theta}\\
%    &+ (1-y_i)\log (1 - \phi(\bt^\top\Pb \x_i))).\nonumber 
%\end{align}
Given norm constraint $a\leq \infty$, the empirical risk minimizer (ERM) is defined as
\begin{align}
    \hat \bt_e &= \argmin_{\bt}\ \cL_e(\bt;\hat\Ub_r^\top)\quad\text{such~that}\quad\|\bt\|_2\le a.\label{eq:fstar finite theta}
\end{align}
\end{definition}


\setlength{\textfloatsep}{.5em}
\begin{algorithm}[t!]
\caption{Meta-training and Few-shot Learning}\label{algo:1}
\begin{algorithmic}
% with $k$ tasks, the size of data of the $j$-th task has size $n_j$. Dimension $d$. Effective dimension $r$. Set of functions $\Fc$.
\REQUIRE {Dataset $\mathcal{S}$, representation size $r$, function space $\Fc$}
\STATE{Compute $\hat \bM$ via method-of-moments \eqref{eq:hatM}.}
\STATE{Rank $r$ approximation:\\
$\quad\hat\bM_r \leftarrow \hat\Ub_r \mathrm{diag}(\hat \La_{1,1},...,\hat\La_{r,r}) \hat \Ub_r^\top$.}
\STATE{Either~$\hat f \leftarrow \argmin_{f\in\Fc}\ \cLCE(f;\Ub_r^\top) $.
%$\cLCE$ is defined as \eqref{eq:cLCE}.
}
\STATE{Or~~~~~~$\hat f_e \leftarrow \argmin_{f\in\Fc}\ \cL_e(f;\Ub_r^\top) $.
%$\cL_e$ is defined as \eqref{eq:cLCE finite theta}
}
\RETURN{$\hat\Ub_r$ and $\hat f$ or $\hat f_e$.}
\end{algorithmic}
\end{algorithm}%\vspace{-10pt}


==> Icassp (3)/notation.tex <==

\usepackage{hyperref,graphicx,amsmath,amsfonts,amssymb,bm,url,breakurl,epsfig,epsf,color,MnSymbol,mathbbol,fmtcount,semtrans,caption,subcaption,multirow,comment, boldline, enumitem}
%\usepackage[]{algorithm2e}
%\usepackage[noend]{algpseudocode}
\usepackage{wrapfig}
\usepackage{amssymb}

\usepackage[utf8]{inputenc} % allow utf-8 input
\usepackage[T1]{fontenc}    % use 8-bit T1 fonts
\usepackage{url}            % simple URL typesetting
\usepackage{booktabs}       % professional-quality tables
\usepackage{amsfonts}       % blackboard math symbols
\usepackage{nicefrac}       % compact symbols for 1/2, etc.
\usepackage{microtype}      % microtypography

\makeatletter
\providecommand*{\boxast}{%
  \mathbin{% as \boxplus and \boxtimes
    \mathpalette\@boxit{*}%
  }%
}
\newcommand*{\@boxit}[2]{%
  % #1: math style (\displaystyle, \textstyle, ...)
  % #2: symbol to be boxed that is centered around the math axis
  \sbox0{$\m@th#1\Box$}%
  % Manual correction for font bounding boxes:
  \ifx#1\displaystyle \ht0=\dimexpr\ht0+.05ex\relax \fi
  \ifx#1\textstyle \ht0=\dimexpr\ht0+.05ex\relax \fi
  \ifx#1\scriptstyle \ht0=\dimexpr\ht0+.04ex\relax \fi
  \ifx#1\scriptscriptstyle \ht0=\dimexpr\ht0+.065ex\relax \fi
  \sbox2{$#1\vcenter{}$}% \ht2 is positionn of math axis
  \rlap{%
    \hbox to \wd0{%
      \hfill
      \raisebox{%
        \dimexpr.5\dimexpr\ht0+\dp0\relax-\ht2\relax
      }{$\m@th#1#2$}%
      \hfill
    }%
  }%
  \Box
}
\makeatother

  \makeatletter
\def\BState{\State\hskip-\ALG@thistlm}
\makeatother


  \usepackage{mathtools}
\DeclarePairedDelimiter{\floor}{\lfloor}{\rfloor}

\usepackage{titlesec}

\usepackage{tikz}
\usepackage{pgfplots}
\usetikzlibrary{pgfplots.groupplots}

\setcounter{secnumdepth}{3}

\titleformat{\paragraph}
{\normalfont\normalsize\bfseries}{\theparagraph}{1em}{}
\titlespacing*{\paragraph}
{0pt}{3.25ex plus 1ex minus .2ex}{1.5ex plus .2ex}

\usepackage{movie15}

%\usepackage{caption}
\usepackage[bottom,hang,flushmargin]{footmisc} 

\setlength{\captionmargin}{30pt}

\newcommand{\tsn}[1]{{\left\vert\kern-0.25ex\left\vert\kern-0.25ex\left\vert #1 
    \right\vert\kern-0.25ex\right\vert\kern-0.25ex\right\vert}}

\definecolor{darkred}{RGB}{150,0,0}
\definecolor{darkgreen}{RGB}{0,150,0}
\definecolor{darkblue}{RGB}{0,0,200}
\hypersetup{colorlinks=true, linkcolor=darkred, citecolor=darkgreen, urlcolor=darkblue}

%--------------
\newtheorem{theorem}{Theorem}[section]
\newtheorem{result}{Result}
\newtheorem{problem}{Problem}
\newtheorem{claim}{Claim}
\newtheorem{assumption}{Assumption}
\newtheorem{question}{Question}
\newtheorem{lemma}[theorem]{Lemma}
\newtheorem{corollary}[theorem]{Corollary}
\newtheorem{propo}[theorem]{Proposition}
\newtheorem{definition}[theorem]{Definition}
\newtheorem{condition}[theorem]{Condition}
\newtheorem{conjecture}[theorem]{Conjecture}

\newtheorem{remark}[subsection]{Remark}
\newtheorem{remarks}[subsection]{Remarks}
\newtheorem{example}[subsection]{Example}

%% TT's definitions
\newcommand\tr{{{\operatorname{trace}}}}
\newcommand{\eps}{\varepsilon}
\newcommand{\epsr}{\varepsilon_R}
\newcommand{\mur}{\mu_R}
\newcommand{\bn}{\alpha}
\newcommand{\pp}{{\text{CL}}}
\newcommand{\distas}{\overset{\text{i.i.d.}}{\sim}}
\newcommand{\np}{{n\wedge p}}
\newcommand{\KB}{\bar{K}}
\newcommand{\bG}{\boldsymbol{\Gamma}}
\newcommand{\xw}{\x_{\w}}
\newcommand{\xv}{\x_{\vb}}
\newcommand{\xu}{\x_{\ub}}
\newcommand{\xvt}[1]{\x_{\vb_{#1}}}
\newcommand{\xvtt}[1]{\x_{\vb,#1}}
\newcommand{\xwt}[1]{\x_{#1,\w}}
\newcommand{\xws}[1]{\x_{#1,\ws}}
\newcommand{\xs}{\x_{\ws}}
\newcommand{\yst}{\hat{\y}}
\newcommand{\st}{\star}
\newcommand{\eig}{\text{eigvec}}
\newcommand{\hu}{h}
\newcommand{\ru}{r}
\newcommand{\pbar}{{{\bar{p}}}}
\newcommand{\pbd}{p}
\newcommand{\lay}[1]{{\vct{k}}^{(#1)}}
\newcommand{\lah}[1]{{\vct{\hat{k}}}^{(#1)}}
\newcommand{\lan}{\vct{k}}
\newcommand{\cmp}{P_{\text{nn}}}
\newcommand{\rest}{{\bf{r}}}
\newcommand{\dcp}{\vct{d}^{\text{cnn}}}
\newcommand{\fcp}{\vct{g}^{\text{CNN}}}
\newcommand{\beq}{\begin{equation}}
\newcommand{\nrest}{\bar{n}}
\newcommand{\eeq}{\end{equation}}
\newcommand{\prox}{{{\text{\bf{prox}}}}}
\newcommand{\cov}{{{\text{\bf{cov}}}}}
\newcommand{\ex}{{{\text{\bf{ex}}}}}
\newcommand{\modu}{{{\text{{mod}}}}}
\newcommand{\map}{{{\text{\bf{map}}}}}
\newcommand{\var}[1]{{{\text{\bf{var}}}}[#1]}
\newcommand{\vrn}{\nu}
\newcommand{\func}[1]{{f_{\text{CNN}}}(#1)}
\newcommand{\funh}[1]{{{\hat{f}}_{\text{CNN}}}(#1)}
\newcommand{\funcp}[1]{{f'_{\text{cnn}}}(#1)}
\newcommand{\funcw}[1]{{{{f}}'_{\text{cnn}}}(#1)}
\newcommand{\dev}{{{\text{\bf{dev}}}}}
\newcommand{\meas}{{{\text{\bf{mean}}(\sigma)}}}
\newcommand{\nn}{\nonumber}
\newcommand{\la}{\lambda}
\newcommand{\K}{{K}}
\newcommand{\A}{{\mtx{A}}}
\newcommand{\sfmx}[1]{\text{sfmx}(#1)}
\newcommand{\cat}[1]{\text{Cat}(#1)}
\newcommand{\amp}{\alpha_{\text{cnn}}}
\newcommand{\bOt}{\bigotimes}
\newcommand{\bt}{\boldsymbol{\theta}}
\newcommand{\Bt}{\boldsymbol{\Theta}}
%\newcommand{\nt}{\boldsymbol{n}}

%\newcommand{\bt}{\times}
\newcommand{\robt}[1]{\bigotimes_{\ell=1}^D{#1}_{\ell}}
\newcommand{\robtu}[1]{\bigotimes_{\ell=1}^D{#1}^{(\ell)}}
\newcommand{\bd}{\bigodot}
\newcommand{\kal}{\prod_{i=1}^{D-1}\tn{\lay{i}}}
%\newcommand{\kall}[1]{\prod_{i=1}^{#1}\tn{\lay{i}}}
\newcommand{\kall}[1]{1_{\lan #1}}
\newcommand{\lall}[1]{{\order{\lip_{\lan #1}}}}%{L^{#1}\prod_{i=1}^{#1}\tn{\lay{i}}}
\newcommand{\lell}[1]{{\lip}_{\lan #1}}
\newcommand{\bell}[1]{{{{\beta}}}_{\lan #1}}
\newcommand{\Ub}{{\mtx{U}}}
\newcommand{\Ubb}{{\mtx{U}}}
\newcommand{\V}{{\mtx{V}}}
\newcommand{\ten}{(\{\vb_\ell\}_{\ell=1}^D)}
\newcommand{\uten}{(\{\ub_\ell\}_{\ell=1}^D)}
\newcommand{\ken}{(\{\lay{i}\}_{i=1}^D)}
\newcommand{\B}{{{\mtx{B}}}}
\newcommand{\alx}{{{\alpha_\X}}}
\newcommand{\aly}[1]{{{\alpha_{\X_{#1}}}}}
\newcommand{\Ib}{{{\mtx{I}}}}
\newcommand{\Xbin}{{{\mtx{B}}}}
\newcommand{\Gbin}{{{\mtx{S}}}}
\newcommand{\xbin}{{{\mtx{b}}}}
\newcommand{\Sb}{{{\mtx{S}}}}
\newcommand{\Gb}{{\mtx{G}}}
\newcommand{\ymean}{{\bar{\y}(\w;\text{avg})}}
\newcommand{\yavg}{{{y}_{\text{avg}}}}
\newcommand{\ravg}[1]{{{r}_{{\text{avg}}}(#1)}}
\newcommand{\fmean}{{\funcw{\w;\text{avg}}}}
\newcommand{\diag}[1]{\text{diag}(#1)}
\newcommand{\out}{\text{out}}
\newcommand{\linest}{\text{lin}}
\newcommand{\inp}{\text{in}}
\newcommand{\inh}{\hat{\text{in}}}
\newcommand{\sexp}{subexponential }
\newcommand{\Lc}{{\cal{L}}}
\newcommand{\Nc}{{\cal{N}}}
\newcommand{\Jc}{{\cal{J}}}
\newcommand{\Jcb}{{\overline{\cal{J}}}}
\newcommand{\Dc}{{\cal{D}}}
\newcommand{\Dcg}[1]{{\cal{D}}^{#1}_{\text{subg}}}
\newcommand{\Dct}{{\tilde{\cal{D}}}}
\newcommand{\Sct}{{\tilde{\cal{S}}}}
%\newcommand{\smn}{\s_{\min}}
\newcommand{\btd}{{\bt_{\ell=1}^D d_\ell}}
\newcommand{\Ro}{{\cal{RO}}}
\newcommand{\PC}{{\cal{PC}}}
\newcommand{\Pb}{{\mtx{P}}}
\newcommand{\Tb}{{\mtx{T}}}
\newcommand{\Kba}{{\vct{k}}_{\text{all}}}
\newcommand{\Qb}{{\mtx{Q}}}
\newcommand{\rng}{\gamma}
\newcommand{\Cb}{{\mtx{C}}}
\newcommand{\Eb}{{\mtx{E}}}
\newcommand{\Hb}{{\mtx{H}}}
\newcommand{\Gc}{{\cal{G}}}
\newcommand{\F}{{\mtx{F}}}
\newcommand{\diff}{{\text{diff}}}
\newcommand{\La}{{\boldsymbol{{\Lambda}}}}
%\newcommand{\noresamp}[1]{{\textcolor{red}{#1}}}
\newcommand{\noresamp}[1]{{\textcolor{red}{#1}}}
\newcommand{\sigmap}{\phi'}
\newcommand{\sigmal}[1]{\sigma^{(#1)}}
\newcommand{\sigmalp}[1]{\sigma'^{(#1)}}
\newcommand{\sigmaa}{\sigma'_{\text{all}}}
\newcommand{\sigmai}[1]{\sigma'_{\text{all},#1}}
\newcommand{\bSi}{{\boldsymbol{{\Sigma}}}}
\newcommand{\bSit}{{\boldsymbol{{\tilde{\Sigma}}}}}
\newcommand{\bSih}{{\boldsymbol{{\hat{\Sigma}}}}}
\newcommand{\bmu}{{\boldsymbol{{\mu}}}}
\newcommand{\Db}{{\mtx{D}}}
\newcommand{\db}{{\vct{d}}}
\newcommand{\oneb}{{\mathbb{1}}}
\newcommand{\onebb}{{\mathbf{1}}}
\newcommand{\Iden}{{\mtx{I}}}
\newcommand{\M}{{\mtx{M}}}
\newcommand{\gm}{\gamma_m}
\newcommand{\order}[1]{{\cal{O}}(#1)}
\newcommand{\rmax}[1]{{\bf{r}_{\max}(#1)}}
\newcommand{\rbmax}[1]{{\bf{\bar{r}}_{\max}(#1)}}
\newcommand{\rmin}[1]{{\bf{r}_{\min}(#1)}}
\newcommand{\smn}[1]{{s_{\min}(#1)}}
\newcommand{\smx}[1]{{s_{\max}(#1)}}
\newcommand{\z}{{\vct{z}}}
\newcommand{\zb}{{\bar{\z}}}
\newcommand{\el}{{\ell}}
\newcommand{\tn}[1]{\|{#1}\|_{\ell_2}}
\newcommand{\tff}[1]{\|{#1}\|_{\ell_4}}
\newcommand{\tin}[1]{\|{#1}\|_{\ell_\infty}}
\newcommand{\trow}[1]{\|{#1}\|_{2,\infty}}
\newcommand{\bad}{{\bar{d}}}
\newcommand{\Dp}{{D^+}}
\newcommand{\tf}[1]{\|{#1}\|_{F}}
\newcommand{\te}[1]{\|{#1}\|_{\psi_1}}
\newcommand{\tsub}[1]{\|{#1}\|_{\psi_2}}
\newcommand{\tsut}[1]{\|{#1}\|_{\psi_{2/3}}}
\newcommand{\tsup}[1]{\|{#1}\|_{\psi_a}}
\newcommand{\dist}[1]{\text{dist}(#1)}
\newcommand{\upp}{{\cal{B}}_{\alpha,\Gamma}}
\newcommand{\upz}{{\cal{B}}_{\alpha_0,\Gamma}}
\newcommand{\dpz}{{\cal{D}}_{\alpha_0,\Gamma}}
\newcommand{\dpp}{{\cal{D}}_{\alpha,\Gamma}}
\newcommand{\mpp}{M_{\alpha,\Gamma}}
%\newcommand{\supp}[1]{\text{supp}(#1)}
\newcommand{\cone}[1]{{\text{cone}(#1)}}
\newcommand{\paf}{\partial f(\x)}
\newcommand{\Cc}{\mathcal{C}}
\newcommand{\Ac}{\mathcal{A}}
\newcommand{\Ccb}{\bar{\mathcal{C}}}
\newcommand{\Xc}{\mathcal{X}}
\newcommand{\xc}{{\text{excess}}}
\newcommand{\Rc}{\mathcal{R}}
\newcommand{\Rcp}{\mathcal{\bar{R}}'}
\newcommand{\Rcb}{\mathcal{N}}
\newcommand{\btrue}{\bbeta_{true}}
\newcommand{\bteta}{\boldsymbol{\theta}}
\newcommand{\bbteta}{\widetilde{\boldsymbol{\theta}}}
\newcommand{\brteta}{\overline{\boldsymbol{\theta}}}
\newcommand{\bbeta}{{\boldsymbol{\beta}}}
\newcommand{\ddelta}{{\boldsymbol{\delta}}}
\newcommand{\babeta}{{\bar{\beta}}}
\newcommand{\balpha}{{\bar{\alpha}}}
\newcommand{\bgamma}{{\bar{\gamma}}}
\newcommand{\Bc}{\mathcal{B}}
\newcommand{\Sc}{\mathcal{S}}
\newcommand{\Mc}{\mathcal{M}}
\newcommand{\pa}{{\partial}}
\newcommand{\Nn}{\mathcal{N}}
\newcommand{\pol}{^\circ}
\newcommand{\vb}{\vct{v}}
\newcommand{\Jb}{\mtx{J}}
\newcommand{\Jt}{\mtx{\tilde{J}}}
\newcommand{\vbl}{\vct{v}^{\text{lin}}}
\newcommand{\fb}{\vct{f}}
\newcommand{\ib}{{\bf{i}}}
\newcommand{\hib}{{\bf{\hat{i}}}}
\newcommand{\Ic}{{\mathcal{I}}}
\newcommand{\all}{{\text{all}}}
\newcommand{\vh}{\vct{\hat{v}}}
\newcommand{\vbb}{\vct{\bar{v}}}
\newcommand{\Xb}{\mtx{\bar{X}}}
\newcommand{\abb}{\mtx{\bar{a}}}
\newcommand{\cb}{\mtx{c}}
\newcommand{\bbb}{\mtx{\bar{b}}}
\newcommand{\w}{\vct{w}}
\newcommand{\err}[1]{\text{Err}_{\Dc}(#1)}
\newcommand{\Wp}{\mtx{W}^\dagger}
\newcommand{\tilW}{\widetilde{\mtx{W}}}
\newcommand{\tilw}{\widetilde{\vct{w}}}
\newcommand{\ob}{\mtx{o}}
\newcommand{\obh}{\mtx{\hat{o}}}
\newcommand{\wh}{{\hat{\mtx{w}}}}
\newcommand{\li}{\left<}
\newcommand{\ri}{\right>}
\newcommand{\s}{\vct{s}}
\newcommand{\sh}{\hat{\vct{s}}}
\newcommand{\ab}{\vct{a}}
\newcommand{\bb}{\vct{b}}
\newcommand{\ub}{{\vct{u}}}
\newcommand{\ubb}{\bar{\vct{u}}}
\newcommand{\h}{\vct{h}}
\newcommand{\hh}{{\vct{h}}}
\newcommand{\g}{{\vct{g}}}
\newcommand{\ii}{{\vct{i}}}
\newcommand{\zm}[1]{{\text{{\bf{zm}}}(#1)}}
\newcommand{\dd}{{\vct{d}}}
\newcommand{\ddt}{{\vct{d}}_\tau}
\newcommand{\Zb}{\mtx{Z}}
\newcommand{\hf}{\hat{f}}
\newcommand{\corrCA}{\rho_\Cc(\M)}
\newcommand{\corr}[1]{{\bf{cor}}(#1)}
\newcommand{\Tc}{\mathcal{T}}
\newcommand{\Fc}{\mathcal{F}}
\newcommand{\Hc}{\mathcal{H}}


%%YP's macros
\newcommand{\qqq}[1]{{\textcolor{red}{?{#1}?}}}
\newcommand{\ihere}{{\textcolor{red}{I AM HERE! }}}
\newcommand{\mat}[1]{{\text{mat}{#1}}}
\newcommand{\gb}{\bar{\g}}
\newcommand{\bs}{\bar{s}}
\newcommand{\cgain}{\alpha_{\text{CNN}}}
\newcommand{\cgainp}{\tn{\E_{\x\sim\Nn(0,\Iden)}[\gcnn{}]}}
\newcommand{\gcnn}[1]{{\vct{g}}_{\text{cnn}#1}}
\newcommand{\ccorr}{\rho_{\text{cnn}}}
\newcommand{\kb}{\vct{k}}
\newcommand{\xh}{\hat{\x}}
\newcommand{\yh}{\hat{\y}}
\newcommand{\xbr}{\bar{\h}}
\newcommand{\xdr}{\tilde{\x}}
\newcommand{\m}{\vct{m}}
\newcommand{\xt}{\tilde{\x}}
\newcommand{\nt}{\tilde{n}}
%\newcommand{\ht}{\tilde{h}}
\newcommand{\rt}{\tilde{r}}
\newcommand{\ft}{\tilde{f}}
\newcommand{\yt}{\tilde{\y}}
\newcommand{\gh}{\hat{\g}}
\newcommand{\gt}{\tilde{\g}}
\newcommand{\wb}{\bar{\w}}
\newcommand{\lip}{L}
\newcommand{\mipp}{L_{\max}}
\newcommand{\mupp}{\bar{\mu}_{\max}}
\newcommand{\mapp}{\mu}
\newcommand{\tcnn}{{\mtx{T}}_{\text{cnn}}}
\newcommand{\lcnn}{{\mtx{L}}_{\text{CNN}}}
\newcommand{\lipa}{{L}}
\newcommand{\smo}{S}
\newcommand{\SM}{{{\bf{S}}}_{L,\kb}}
\newcommand{\SMB}{{{\bf{\bar{S}}}}_{L,\kb}}
\newcommand{\Ws}{\W^\star}
\newcommand{\ws}{{\w^\star}}
\newcommand{\wss}{{\w^\star}}
\newcommand{\yp}[1]{\textcolor{red}{ #1}}
\newcommand{\zeronorm}[1]{\left\|#1 \right\|_0}
\newcommand{\unorm}[1]{\left\|#1 \right\|_u}
\newcommand{\ynorm}[1]{\left\|#1 \right\|_{\bar{y}}}
\newcommand{\onetwonorm}[1]{\left\|#1\right\|_{1,2}}
\newcommand{\opnorm}[1]{\left\|#1\right\|}
\newcommand{\fronorm}[1]{\left\|#1\right\|_{F}}
\newcommand{\onenorm}[1]{\left\|#1\right\|_{\ell_1}}
\newcommand{\twonorm}[1]{\left\|#1\right\|_{\ell_2}}
\newcommand{\wnorm}[2]{\left\|#1\right\|_{#2}}
\newcommand{\Dnorm}[1]{\left\|#1\right\|_{D}}
\newcommand{\oneinfnorm}[1]{\left\|#1\right\|_{1,\infty}}
\newcommand{\infnorm}[1]{\left\|#1\right\|_{\ell_\infty}}
\newcommand{\nucnorm}[1]{\left\|#1\right\|_*}
\newcommand{\abs}[1]{\left|#1\right|}
\newcommand{\avg}[1]{\left< #1 \right>}

\newcommand{\lipp}{\prod_{\ell=1}^D \twonorm{\vct{k}^{(\ell)}}}

\renewcommand{\d}{\mathrm{d}}

\newcommand{\cA}{\mathcal{A}}
\newcommand{\rotd}{\text{R1TD}}
\newcommand{\nntd}{\text{DeepTD}}
\newcommand{\x}{\vct{x}}
\newcommand{\rb}{\vct{r}}
\newcommand{\rbb}{\vct{\widetilde{r}}}
\newcommand{\y}{\vct{y}}
\newcommand{\ybh}{\vct{\hat{y}}}
\newcommand{\W}{\mtx{W}}
\newcommand{\Wc}{{\cal{W}}}
\newcommand{\Vc}{{\cal{V}}}
\newcommand{\bgl}{{~\big |~}}

%--------------

% EJC's macros

\definecolor{emmanuel}{RGB}{255,127,0}
\newcommand{\ejc}[1]{\textcolor{emmanuel}{EJC: #1}}

\newcommand{\p}{{\vct{p}}}
\newcommand{\Kb}{{\mtx{K}}}
\newcommand{\somelog}{16\Kb\log (\Kb)}
\newcommand{\somelg}{\Kb\log (\Kb)}
\newcommand{\pb}{{\vct{p}}}
\newcommand{\qb}{{\vct{q}}}
\newcommand{\R}{\mathbb{R}}
\newcommand{\Pro}{\mathbb{P}}
\newcommand{\C}{\mathbb{C}}
\newcommand{\Z}{\mathbb{Z}}
\newcommand{\<}{\langle}
\renewcommand{\>}{\rangle}
\newcommand{\Var}{\textrm{Var}}
\newcommand{\sgn}[1]{\textrm{sgn}(#1)}
\renewcommand{\P}{\operatorname{\mathbb{P}}}
%\newcommand{\E}{\operatorname{\mathbb{E}}}
\newcommand{\EE}{\operatorname{\mathbb{E}}}
%\newcommand{\var}{\operatorname{\mathbf{var}}}

\newcommand{\todo}[1]{{\bf TODO: #1}}
\newcommand{\grad}[1]{{\nabla\Lc(#1)}}
\newcommand{\gradf}[1]{{\nabla f(#1)}}
\newcommand{\hessf}[1]{{\nabla^2f(#1)}}
\newcommand{\gradw}[1]{{\nabla{\Lc}(#1)}}
\newcommand{\grd}[2]{{\nabla\Lc_{#1}(#2)}}
\newcommand{\e}{\mathrm{e}}
\newcommand{\eb}{\vct{e}}
\renewcommand{\i}{\imath}

\newcommand{\vct}[1]{\bm{#1}}
\newcommand{\mtx}[1]{\bm{#1}}

% MS's macros

\newcommand{\rank}{\operatorname{rank}}
\newcommand{\supp}[1]{\operatorname{supp}(#1)}
\newcommand{\restrict}[1]{\big\vert_{#1}}
\newcommand{\Id}{\text{\em I}}
\newcommand{\OpId}{\mathcal{I}}

\newcommand{\Real}{\operatorname{Re}}
\newcommand{\Imag}{\operatorname{Im}}

\newcommand{\piyp}{\pi'_1(\vct{y})}
\newcommand{\piy}{\pi_1(\vct{y})}
\newcommand{\piar}{\pi_1(\vct{a}_r)}
\newcommand{\piarp}{\pi'_1(\vct{a}_r)}
\newcommand{\set}{{\cal{F}}}
\newcommand{\des}{{\x_0}}

\newcommand{\Pc}{{\cal{P}}}
\newcommand{\X}{{\mtx{X}}}
\newcommand{\Y}{{\mtx{Y}}}
\newcommand{\Vb}{{\mtx{V}}}
\newcommand{\Vh}{\hat{{\mtx{V}}}}
\newcommand{\Vbd}{{\mtx{V}^\dagger}}
\newcommand{\Rb}{{\mtx{R}}}

\newcommand{\calF}{\mathcal{I}}
\newcommand{\calS}{\mathcal{N}}


\newcommand{\MS}[1]{\textcolor{blue}{MS: #1}}
\newcommand{\MST}[1]{\textcolor{red}{#1}}
\newcommand{\SO}[1]{\textcolor{darkgreen}{SO: #1}}


\numberwithin{equation}{section} 

\def \endprf{\hfill {\vrule height6pt width6pt depth0pt}\medskip}
%\newenvironment{proof}{\noindent {\bf Proof} }{\endprf\par}
\newenvironment{proofsk}{\noindent {\bf Proof sketch} }{\endprf\par}


%\newcommand{\qed}{{\unskip\nobreak\hfil\penalty50\hskip2em\vadjust{}
           %\nobreak\hfil$\Box$\parfillskip=0pt\finalhyphendemerits=0\par}}


\newcommand{\note}[1]{{\bf [{\em Note:} #1]}}

\newcommand{\iprod}[2]{\left\langle #1 , #2 \right\rangle}

\newcommand{\red}{\textcolor{red}}
\newcommand{\gi}{\ab_{\gamma_i}}
\newcommand{\ang}{\text{ang}}
\newcommand{\ham}[2]{{\|#1,#2\|_H}}

%\renewcommand{\algorithmicrequire}{\textbf{Input:}}
%\renewcommand{\algorithmicensure}{\textbf{Output:}}

%AJ's macros
\newcommand{\hth}{{\widehat{\boldsymbol{\theta}}}}
\newcommand{\bth}{{\boldsymbol{\theta}}}
\newcommand\cL{\mathcal{L}}
\newcommand\cD{\mathcal{D}}
\newcommand\hcD{\widehat{\cD}}
\newcommand\reals{\mathbb{R}}
\newcommand\bSigma{\boldsymbol{\Sigma}}
\newcommand\normal{{\sf N}}
\newcommand\bdelta{\boldsymbol{\delta}}
\newcommand\sign{{\rm sign}}
\newcommand\sT{{\sf T}}
\newcommand\I{\mtx{I}}
\newcommand\zero{\mtx{0}}
\newcommand\bA{\mtx{A}}
\newcommand\bv{\mtx{v}}
\newcommand\cI{\mathcal{I}}
\newcommand\bz{\boldsymbol{z}}
\newcommand\bg{\boldsymbol{g}}
\newcommand\ba{\boldsymbol{a}}
\def\cC{\mathcal{C}}
\def\de{{\rm d}}
\def\bM{\mtx{M}}
\def\cH{\mathcal{H}}
\def\bu{\boldsymbol{u}}
\def\by{\boldsymbol{y}}
\def\bw{\boldsymbol{w}}
\def\bX{\boldsymbol{X}}
\def\tbX{\tilde{\boldsymbol{X}}}
\def\tbx{\tilde{\boldsymbol{x}}}
\def\tbth{\tilde{\boldsymbol{\theta}}}
\def\hz{\widehat{z}}
\def\ind{\mathbf{1}}
\def\cS{\mathcal{S}}
\def\prob{\mathbb{P}}
\def\tx{\tilde{x}}
\def\reals{\mathbb{R}}
\newcommand{\aj}[1]{\noindent{\textcolor{blue}{\textbf{\#\#\# AJ:} \textsf{#1} \#\#\#}}}

\newcommand{\gauss}{\mathcal{N}(0,I)}
\newcommand{\gausscov}[1]{\mathcal{N}(0,{#1})}
\newcommand{\argmin}{\mathop{\mathrm{argmin}}}
%\newcommand{\cLCE}{\cL_{\mathrm{CE}}}
\newcommand{\cLCE}{\cL}
\newcommand{\mscrU}{{\mathscr{U}}}

==> Icassp (3)/notation_new.tex <==

\usepackage{hyperref,graphicx,amsmath,amsfonts,amssymb,bm,url,breakurl,epsfig,epsf,color,MnSymbol,mathbbol,fmtcount,semtrans,caption,subcaption,multirow,comment, boldline, enumitem}
%\usepackage[]{algorithm2e}
%\usepackage[noend]{algpseudocode}
\usepackage{wrapfig}
\usepackage{amssymb}


\makeatletter
\providecommand*{\boxast}{%
  \mathbin{% as \boxplus and \boxtimes
    \mathpalette\@boxit{*}%
  }%
}
\newcommand*{\@boxit}[2]{%
  % #1: math style (\displaystyle, \textstyle, ...)
  % #2: symbol to be boxed that is centered around the math axis
  \sbox0{$\m@th#1\Box$}%
  % Manual correction for font bounding boxes:
  \ifx#1\displaystyle \ht0=\dimexpr\ht0+.05ex\relax \fi
  \ifx#1\textstyle \ht0=\dimexpr\ht0+.05ex\relax \fi
  \ifx#1\scriptstyle \ht0=\dimexpr\ht0+.04ex\relax \fi
  \ifx#1\scriptscriptstyle \ht0=\dimexpr\ht0+.065ex\relax \fi
  \sbox2{$#1\vcenter{}$}% \ht2 is positionn of math axis
  \rlap{%
    \hbox to \wd0{%
      \hfill
      \raisebox{%
        \dimexpr.5\dimexpr\ht0+\dp0\relax-\ht2\relax
      }{$\m@th#1#2$}%
      \hfill
    }%
  }%
  \Box
}
\makeatother

  \makeatletter
\def\BState{\State\hskip-\ALG@thistlm}
\makeatother


  \usepackage{mathtools}
\DeclarePairedDelimiter{\floor}{\lfloor}{\rfloor}

%\usepackage{titlesec}

\usepackage{tikz}
\usepackage{pgfplots}
\usetikzlibrary{pgfplots.groupplots}

\setcounter{secnumdepth}{3}


\usepackage{movie15}

%\usepackage{caption}
\usepackage[bottom,hang,flushmargin]{footmisc} 

\setlength{\captionmargin}{30pt}

\newcommand{\tsn}[1]{{\left\vert\kern-0.25ex\left\vert\kern-0.25ex\left\vert #1 
    \right\vert\kern-0.25ex\right\vert\kern-0.25ex\right\vert}}

\definecolor{darkred}{RGB}{150,0,0}
\definecolor{darkgreen}{RGB}{0,150,0}
\definecolor{darkblue}{RGB}{0,0,200}
\hypersetup{colorlinks=true, linkcolor=darkred, citecolor=darkgreen, urlcolor=darkblue}

%--------------

\newtheorem{theorem}{Theorem}[section]
\newtheorem{result}{Result}
\newtheorem{problem}{Problem}
\newtheorem{claim}{Claim}
\newtheorem{assumption}{Assumption}
\newtheorem{question}{Question}
\newtheorem{lemma}[theorem]{Lemma}
\newtheorem{corollary}[theorem]{Corollary}
\newtheorem{propo}[theorem]{Proposition}
\newtheorem{definition}[theorem]{Definition}
\newtheorem{condition}[theorem]{Condition}
\newtheorem{conjecture}[theorem]{Conjecture}

\newtheorem{remark}[subsection]{Remark}
\newtheorem{remarks}[subsection]{Remarks}
\newtheorem{example}[subsection]{Example}

%% TT's definitions
\newcommand\tr{{{\operatorname{trace}}}}
\newcommand{\eps}{\varepsilon}
\newcommand{\epsr}{\varepsilon_R}
\newcommand{\mur}{\mu_R}
\newcommand{\bn}{\alpha}
\newcommand{\pp}{{\text{CL}}}
\newcommand{\distas}{\overset{\text{i.i.d.}}{\sim}}
\newcommand{\np}{{n\wedge p}}
\newcommand{\KB}{\bar{K}}
\newcommand{\bG}{\boldsymbol{\Gamma}}
\newcommand{\xw}{\x_{\w}}
\newcommand{\xv}{\x_{\vb}}
\newcommand{\xu}{\x_{\ub}}
\newcommand{\xvt}[1]{\x_{\vb_{#1}}}
\newcommand{\xvtt}[1]{\x_{\vb,#1}}
\newcommand{\xwt}[1]{\x_{#1,\w}}
\newcommand{\xws}[1]{\x_{#1,\ws}}
\newcommand{\xs}{\x_{\ws}}
\newcommand{\yst}{\hat{\y}}
\newcommand{\st}{\star}
\newcommand{\eig}{\text{eigvec}}
\newcommand{\hu}{h}
\newcommand{\ru}{r}
\newcommand{\pbar}{{{\bar{p}}}}
\newcommand{\pbd}{p}
\newcommand{\lay}[1]{{\vct{k}}^{(#1)}}
\newcommand{\lah}[1]{{\vct{\hat{k}}}^{(#1)}}
\newcommand{\lan}{\vct{k}}
\newcommand{\cmp}{P_{\text{nn}}}
\newcommand{\rest}{{\bf{r}}}
\newcommand{\dcp}{\vct{d}^{\text{cnn}}}
\newcommand{\fcp}{\vct{g}^{\text{CNN}}}
\newcommand{\beq}{\begin{equation}}
\newcommand{\nrest}{\bar{n}}
\newcommand{\eeq}{\end{equation}}
\newcommand{\prox}{{{\text{\bf{prox}}}}}
\newcommand{\cov}{{{\text{\bf{cov}}}}}
\newcommand{\ex}{{{\text{\bf{ex}}}}}
\newcommand{\modu}{{{\text{{mod}}}}}
\newcommand{\map}{{{\text{\bf{map}}}}}
\newcommand{\var}[1]{{{\text{\bf{var}}}}[#1]}
\newcommand{\vrn}{\nu}
\newcommand{\func}[1]{{f_{\text{CNN}}}(#1)}
\newcommand{\funh}[1]{{{\hat{f}}_{\text{CNN}}}(#1)}
\newcommand{\funcp}[1]{{f'_{\text{cnn}}}(#1)}
\newcommand{\funcw}[1]{{{{f}}'_{\text{cnn}}}(#1)}
\newcommand{\dev}{{{\text{\bf{dev}}}}}
\newcommand{\meas}{{{\text{\bf{mean}}(\sigma)}}}
\newcommand{\nn}{\nonumber}
\newcommand{\la}{\lambda}
\newcommand{\K}{{K}}
\newcommand{\A}{{\mtx{A}}}
\newcommand{\sfmx}[1]{\text{sfmx}(#1)}
\newcommand{\cat}[1]{\text{Cat}(#1)}
\newcommand{\amp}{\alpha_{\text{cnn}}}
\newcommand{\bOt}{\bigotimes}
\newcommand{\bt}{\boldsymbol{\theta}}
\newcommand{\Bt}{\boldsymbol{\Theta}}
%\newcommand{\nt}{\boldsymbol{n}}

%\newcommand{\bt}{\times}
\newcommand{\robt}[1]{\bigotimes_{\ell=1}^D{#1}_{\ell}}
\newcommand{\robtu}[1]{\bigotimes_{\ell=1}^D{#1}^{(\ell)}}
\newcommand{\bd}{\bigodot}
\newcommand{\kal}{\prod_{i=1}^{D-1}\tn{\lay{i}}}
%\newcommand{\kall}[1]{\prod_{i=1}^{#1}\tn{\lay{i}}}
\newcommand{\kall}[1]{1_{\lan #1}}
\newcommand{\lall}[1]{{\order{\lip_{\lan #1}}}}%{L^{#1}\prod_{i=1}^{#1}\tn{\lay{i}}}
\newcommand{\lell}[1]{{\lip}_{\lan #1}}
\newcommand{\bell}[1]{{{{\beta}}}_{\lan #1}}
\newcommand{\Ub}{{\mtx{U}}}
\newcommand{\Ubb}{{\mtx{U}}}
\newcommand{\V}{{\mtx{V}}}
\newcommand{\ten}{(\{\vb_\ell\}_{\ell=1}^D)}
\newcommand{\uten}{(\{\ub_\ell\}_{\ell=1}^D)}
\newcommand{\ken}{(\{\lay{i}\}_{i=1}^D)}
\newcommand{\B}{{{\mtx{B}}}}
\newcommand{\alx}{{{\alpha_\X}}}
\newcommand{\aly}[1]{{{\alpha_{\X_{#1}}}}}
\newcommand{\Ib}{{{\mtx{I}}}}
\newcommand{\Xbin}{{{\mtx{B}}}}
\newcommand{\Gbin}{{{\mtx{S}}}}
\newcommand{\xbin}{{{\mtx{b}}}}
\newcommand{\Sb}{{{\mtx{S}}}}
\newcommand{\Gb}{{\mtx{G}}}
\newcommand{\ymean}{{\bar{\y}(\w;\text{avg})}}
\newcommand{\yavg}{{{y}_{\text{avg}}}}
\newcommand{\ravg}[1]{{{r}_{{\text{avg}}}(#1)}}
\newcommand{\fmean}{{\funcw{\w;\text{avg}}}}
\newcommand{\diag}[1]{\text{diag}(#1)}
\newcommand{\out}{\text{out}}
\newcommand{\linest}{\text{lin}}
\newcommand{\inp}{\text{in}}
\newcommand{\inh}{\hat{\text{in}}}
\newcommand{\sexp}{subexponential }
\newcommand{\Lc}{{\cal{L}}}
\newcommand{\Nc}{{\cal{N}}}
\newcommand{\Jc}{{\cal{J}}}
\newcommand{\Jcb}{{\overline{\cal{J}}}}
\newcommand{\Dc}{{\cal{D}}}
\newcommand{\Dcg}[1]{{\cal{D}}^{#1}_{\text{subg}}}
\newcommand{\Dct}{{\tilde{\cal{D}}}}
\newcommand{\Sct}{{\tilde{\cal{S}}}}
%\newcommand{\smn}{\s_{\min}}
\newcommand{\btd}{{\bt_{\ell=1}^D d_\ell}}
\newcommand{\Ro}{{\cal{RO}}}
\newcommand{\PC}{{\cal{PC}}}
\newcommand{\Pb}{{\mtx{P}}}
\newcommand{\Tb}{{\mtx{T}}}
\newcommand{\Kba}{{\vct{k}}_{\text{all}}}
\newcommand{\Qb}{{\mtx{Q}}}
\newcommand{\rng}{\gamma}
\newcommand{\Cb}{{\mtx{C}}}
\newcommand{\Eb}{{\mtx{E}}}
\newcommand{\Hb}{{\mtx{H}}}
\newcommand{\Gc}{{\cal{G}}}
\newcommand{\F}{{\mtx{F}}}
\newcommand{\diff}{{\text{diff}}}
\newcommand{\La}{{\boldsymbol{{\Lambda}}}}
%\newcommand{\noresamp}[1]{{\textcolor{red}{#1}}}
\newcommand{\noresamp}[1]{{\textcolor{red}{#1}}}
\newcommand{\sigmap}{\phi'}
\newcommand{\sigmal}[1]{\sigma^{(#1)}}
\newcommand{\sigmalp}[1]{\sigma'^{(#1)}}
\newcommand{\sigmaa}{\sigma'_{\text{all}}}
\newcommand{\sigmai}[1]{\sigma'_{\text{all},#1}}
\newcommand{\bSi}{{\boldsymbol{{\Sigma}}}}
\newcommand{\bSit}{{\boldsymbol{{\tilde{\Sigma}}}}}
\newcommand{\bSih}{{\boldsymbol{{\hat{\Sigma}}}}}
\newcommand{\bmu}{{\boldsymbol{{\mu}}}}
\newcommand{\Db}{{\mtx{D}}}
\newcommand{\db}{{\vct{d}}}
\newcommand{\oneb}{{\mathbb{1}}}
\newcommand{\onebb}{{\mathbf{1}}}
\newcommand{\Iden}{{\mtx{I}}}
\newcommand{\M}{{\mtx{M}}}
\newcommand{\gm}{\gamma_m}
\newcommand{\order}[1]{{\cal{O}}(#1)}
\newcommand{\rmax}[1]{{\bf{r}_{\max}(#1)}}
\newcommand{\rbmax}[1]{{\bf{\bar{r}}_{\max}(#1)}}
\newcommand{\rmin}[1]{{\bf{r}_{\min}(#1)}}
\newcommand{\smn}[1]{{s_{\min}(#1)}}
\newcommand{\smx}[1]{{s_{\max}(#1)}}
\newcommand{\z}{{\vct{z}}}
\newcommand{\zb}{{\bar{\z}}}
\newcommand{\el}{{\ell}}
\newcommand{\tn}[1]{\|{#1}\|_{\ell_2}}
\newcommand{\tff}[1]{\|{#1}\|_{\ell_4}}
\newcommand{\tin}[1]{\|{#1}\|_{\ell_\infty}}
\newcommand{\trow}[1]{\|{#1}\|_{2,\infty}}
\newcommand{\bad}{{\bar{d}}}
\newcommand{\Dp}{{D^+}}
\newcommand{\tf}[1]{\|{#1}\|_{F}}
\newcommand{\te}[1]{\|{#1}\|_{\psi_1}}
\newcommand{\tsub}[1]{\|{#1}\|_{\psi_2}}
\newcommand{\tsut}[1]{\|{#1}\|_{\psi_{2/3}}}
\newcommand{\tsup}[1]{\|{#1}\|_{\psi_a}}
\newcommand{\dist}[1]{\text{dist}(#1)}
\newcommand{\upp}{{\cal{B}}_{\alpha,\Gamma}}
\newcommand{\upz}{{\cal{B}}_{\alpha_0,\Gamma}}
\newcommand{\dpz}{{\cal{D}}_{\alpha_0,\Gamma}}
\newcommand{\dpp}{{\cal{D}}_{\alpha,\Gamma}}
\newcommand{\mpp}{M_{\alpha,\Gamma}}
%\newcommand{\supp}[1]{\text{supp}(#1)}
\newcommand{\cone}[1]{{\text{cone}(#1)}}
\newcommand{\paf}{\partial f(\x)}
\newcommand{\Cc}{\mathcal{C}}
\newcommand{\Ac}{\mathcal{A}}
\newcommand{\Ccb}{\bar{\mathcal{C}}}
\newcommand{\Xc}{\mathcal{X}}
\newcommand{\xc}{{\text{excess}}}
\newcommand{\Rc}{\mathcal{R}}
\newcommand{\Rcp}{\mathcal{\bar{R}}'}
\newcommand{\Rcb}{\mathcal{N}}
\newcommand{\btrue}{\bbeta_{true}}
\newcommand{\bteta}{\boldsymbol{\theta}}
\newcommand{\bbteta}{\widetilde{\boldsymbol{\theta}}}
\newcommand{\brteta}{\overline{\boldsymbol{\theta}}}
\newcommand{\bbeta}{{\boldsymbol{\beta}}}
\newcommand{\ddelta}{{\boldsymbol{\delta}}}
\newcommand{\babeta}{{\bar{\beta}}}
\newcommand{\balpha}{{\bar{\alpha}}}
\newcommand{\bgamma}{{\bar{\gamma}}}
\newcommand{\Bc}{\mathcal{B}}
\newcommand{\Sc}{\mathcal{S}}
\newcommand{\Mc}{\mathcal{M}}
\newcommand{\pa}{{\partial}}
\newcommand{\Nn}{\mathcal{N}}
\newcommand{\pol}{^\circ}
\newcommand{\vb}{\vct{v}}
\newcommand{\Jb}{\mtx{J}}
\newcommand{\Jt}{\mtx{\tilde{J}}}
\newcommand{\vbl}{\vct{v}^{\text{lin}}}
\newcommand{\fb}{\vct{f}}
\newcommand{\ib}{{\bf{i}}}
\newcommand{\hib}{{\bf{\hat{i}}}}
\newcommand{\Ic}{{\mathcal{I}}}
\newcommand{\all}{{\text{all}}}
\newcommand{\vh}{\vct{\hat{v}}}
\newcommand{\vbb}{\vct{\bar{v}}}
\newcommand{\Xb}{\mtx{\bar{X}}}
\newcommand{\abb}{\mtx{\bar{a}}}
\newcommand{\cb}{\mtx{c}}
\newcommand{\bbb}{\mtx{\bar{b}}}
\newcommand{\w}{\vct{w}}
\newcommand{\err}[1]{\text{Err}_{\Dc}(#1)}
\newcommand{\Wp}{\mtx{W}^\dagger}
\newcommand{\tilW}{\widetilde{\mtx{W}}}
\newcommand{\tilw}{\widetilde{\vct{w}}}
\newcommand{\ob}{\mtx{o}}
\newcommand{\obh}{\mtx{\hat{o}}}
\newcommand{\wh}{{\hat{\mtx{w}}}}
\newcommand{\li}{\left<}
\newcommand{\ri}{\right>}
\newcommand{\s}{\vct{s}}
\newcommand{\sh}{\hat{\vct{s}}}
\newcommand{\ab}{\vct{a}}
\newcommand{\bb}{\vct{b}}
\newcommand{\ub}{{\vct{u}}}
\newcommand{\ubb}{\bar{\vct{u}}}
\newcommand{\h}{\vct{h}}
\newcommand{\hh}{{\vct{h}}}
\newcommand{\g}{{\vct{g}}}
\newcommand{\ii}{{\vct{i}}}
\newcommand{\zm}[1]{{\text{{\bf{zm}}}(#1)}}
\newcommand{\dd}{{\vct{d}}}
\newcommand{\ddt}{{\vct{d}}_\tau}
\newcommand{\Zb}{\mtx{Z}}
\newcommand{\hf}{\hat{f}}
\newcommand{\corrCA}{\rho_\Cc(\M)}
\newcommand{\corr}[1]{{\bf{cor}}(#1)}
\newcommand{\Tc}{\mathcal{T}}
\newcommand{\Fc}{\mathcal{F}}
\newcommand{\Hc}{\mathcal{H}}


%%YP's macros
\newcommand{\qqq}[1]{{\textcolor{red}{?{#1}?}}}
\newcommand{\ihere}{{\textcolor{red}{I AM HERE! }}}
\newcommand{\mat}[1]{{\text{mat}{#1}}}
\newcommand{\gb}{\bar{\g}}
\newcommand{\bs}{\bar{s}}
\newcommand{\cgain}{\alpha_{\text{CNN}}}
\newcommand{\cgainp}{\tn{\E_{\x\sim\Nn(0,\Iden)}[\gcnn{}]}}
\newcommand{\gcnn}[1]{{\vct{g}}_{\text{cnn}#1}}
\newcommand{\ccorr}{\rho_{\text{cnn}}}
\newcommand{\kb}{\vct{k}}
\newcommand{\xh}{\hat{\x}}
\newcommand{\yh}{\hat{\y}}
\newcommand{\xbr}{\bar{\h}}
\newcommand{\xdr}{\tilde{\x}}
\newcommand{\m}{\vct{m}}
\newcommand{\xt}{\tilde{\x}}
\newcommand{\nt}{\tilde{n}}
%\newcommand{\ht}{\tilde{h}}
\newcommand{\rt}{\tilde{r}}
\newcommand{\ft}{\tilde{f}}
\newcommand{\yt}{\tilde{\y}}
\newcommand{\gh}{\hat{\g}}
\newcommand{\gt}{\tilde{\g}}
\newcommand{\wb}{\bar{\w}}
\newcommand{\lip}{L}
\newcommand{\mipp}{L_{\max}}
\newcommand{\mupp}{\bar{\mu}_{\max}}
\newcommand{\mapp}{\mu}
\newcommand{\tcnn}{{\mtx{T}}_{\text{cnn}}}
\newcommand{\lcnn}{{\mtx{L}}_{\text{CNN}}}
\newcommand{\lipa}{{L}}
\newcommand{\smo}{S}
\newcommand{\SM}{{{\bf{S}}}_{L,\kb}}
\newcommand{\SMB}{{{\bf{\bar{S}}}}_{L,\kb}}
\newcommand{\Ws}{\W^\star}
\newcommand{\ws}{{\w^\star}}
\newcommand{\wss}{{\w^\star}}
\newcommand{\yp}[1]{\textcolor{red}{ #1}}
\newcommand{\zeronorm}[1]{\left\|#1 \right\|_0}
\newcommand{\unorm}[1]{\left\|#1 \right\|_u}
\newcommand{\ynorm}[1]{\left\|#1 \right\|_{\bar{y}}}
\newcommand{\onetwonorm}[1]{\left\|#1\right\|_{1,2}}
\newcommand{\opnorm}[1]{\left\|#1\right\|}
\newcommand{\fronorm}[1]{\left\|#1\right\|_{F}}
\newcommand{\onenorm}[1]{\left\|#1\right\|_{\ell_1}}
\newcommand{\twonorm}[1]{\left\|#1\right\|_{\ell_2}}
\newcommand{\wnorm}[2]{\left\|#1\right\|_{#2}}
\newcommand{\Dnorm}[1]{\left\|#1\right\|_{D}}
\newcommand{\oneinfnorm}[1]{\left\|#1\right\|_{1,\infty}}
\newcommand{\infnorm}[1]{\left\|#1\right\|_{\ell_\infty}}
\newcommand{\nucnorm}[1]{\left\|#1\right\|_*}
\newcommand{\abs}[1]{\left|#1\right|}
\newcommand{\avg}[1]{\left< #1 \right>}

\newcommand{\lipp}{\prod_{\ell=1}^D \twonorm{\vct{k}^{(\ell)}}}

\renewcommand{\d}{\mathrm{d}}

\newcommand{\cA}{\mathcal{A}}
\newcommand{\rotd}{\text{R1TD}}
\newcommand{\nntd}{\text{DeepTD}}
\newcommand{\x}{\vct{x}}
\newcommand{\rb}{\vct{r}}
\newcommand{\rbb}{\vct{\widetilde{r}}}
\newcommand{\y}{\vct{y}}
\newcommand{\ybh}{\vct{\hat{y}}}
\newcommand{\W}{\mtx{W}}
\newcommand{\Wc}{{\cal{W}}}
\newcommand{\Vc}{{\cal{V}}}
\newcommand{\bgl}{{~\big |~}}

%--------------

% EJC's macros

\definecolor{emmanuel}{RGB}{255,127,0}
\newcommand{\ejc}[1]{\textcolor{emmanuel}{EJC: #1}}

\newcommand{\p}{{\vct{p}}}
\newcommand{\Kb}{{\mtx{K}}}
\newcommand{\somelog}{16\Kb\log (\Kb)}
\newcommand{\somelg}{\Kb\log (\Kb)}
\newcommand{\pb}{{\vct{p}}}
\newcommand{\qb}{{\vct{q}}}
\newcommand{\R}{\mathbb{R}}
\newcommand{\Pro}{\mathbb{P}}
\newcommand{\C}{\mathbb{C}}
\newcommand{\Z}{\mathbb{Z}}
\newcommand{\<}{\langle}
\renewcommand{\>}{\rangle}
\newcommand{\Var}{\textrm{Var}}
\newcommand{\sgn}[1]{\textrm{sgn}(#1)}
\renewcommand{\P}{\operatorname{\mathbb{P}}}
%\newcommand{\E}{\operatorname{\mathbb{E}}}
\newcommand{\EE}{\operatorname{\mathbb{E}}}
%\newcommand{\var}{\operatorname{\mathbf{var}}}

\newcommand{\todo}[1]{{\bf TODO: #1}}
\newcommand{\grad}[1]{{\nabla\Lc(#1)}}
\newcommand{\gradf}[1]{{\nabla f(#1)}}
\newcommand{\hessf}[1]{{\nabla^2f(#1)}}
\newcommand{\gradw}[1]{{\nabla{\Lc}(#1)}}
\newcommand{\grd}[2]{{\nabla\Lc_{#1}(#2)}}
\newcommand{\e}{\mathrm{e}}
\newcommand{\eb}{\vct{e}}
\renewcommand{\i}{\imath}

\newcommand{\vct}[1]{\bm{#1}}
\newcommand{\mtx}[1]{\bm{#1}}

% MS's macros

\newcommand{\rank}{\operatorname{rank}}
\newcommand{\supp}[1]{\operatorname{supp}(#1)}
\newcommand{\restrict}[1]{\big\vert_{#1}}
\newcommand{\Id}{\text{\em I}}
\newcommand{\OpId}{\mathcal{I}}

\newcommand{\Real}{\operatorname{Re}}
\newcommand{\Imag}{\operatorname{Im}}

\newcommand{\piyp}{\pi'_1(\vct{y})}
\newcommand{\piy}{\pi_1(\vct{y})}
\newcommand{\piar}{\pi_1(\vct{a}_r)}
\newcommand{\piarp}{\pi'_1(\vct{a}_r)}
\newcommand{\set}{{\cal{F}}}
\newcommand{\des}{{\x_0}}

\newcommand{\Pc}{{\cal{P}}}
\newcommand{\X}{{\mtx{X}}}
\newcommand{\Y}{{\mtx{Y}}}
\newcommand{\Vb}{{\mtx{V}}}
\newcommand{\Vh}{\hat{{\mtx{V}}}}
\newcommand{\Vbd}{{\mtx{V}^\dagger}}
\newcommand{\Rb}{{\mtx{R}}}

\newcommand{\calF}{\mathcal{I}}
\newcommand{\calS}{\mathcal{N}}


\newcommand{\MS}[1]{\textcolor{blue}{MS: #1}}
\newcommand{\MST}[1]{\textcolor{red}{#1}}
\newcommand{\SO}[1]{\textcolor{darkgreen}{SO: #1}}


\numberwithin{equation}{section} 

\def \endprf{\hfill {\vrule height6pt width6pt depth0pt}\medskip}
%\newenvironment{proof}{\noindent {\bf Proof} }{\endprf\par}
\newenvironment{proofsk}{\noindent {\bf Proof sketch} }{\endprf\par}


%\newcommand{\qed}{{\unskip\nobreak\hfil\penalty50\hskip2em\vadjust{}
           %\nobreak\hfil$\Box$\parfillskip=0pt\finalhyphendemerits=0\par}}


\newcommand{\note}[1]{{\bf [{\em Note:} #1]}}

\newcommand{\iprod}[2]{\left\langle #1 , #2 \right\rangle}

\newcommand{\red}{\textcolor{red}}
\newcommand{\gi}{\ab_{\gamma_i}}
\newcommand{\ang}{\text{ang}}
\newcommand{\ham}[2]{{\|#1,#2\|_H}}

%\renewcommand{\algorithmicrequire}{\textbf{Input:}}
%\renewcommand{\algorithmicensure}{\textbf{Output:}}

%AJ's macros
\newcommand{\hth}{{\widehat{\boldsymbol{\theta}}}}
\newcommand{\bth}{{\boldsymbol{\theta}}}
\newcommand\cL{\mathcal{L}}
\newcommand\cLoss{\mathrm{loss}}
\newcommand\cD{\mathcal{D}}
\newcommand\hcD{\widehat{\cD}}
\newcommand\reals{\mathbb{R}}
\newcommand\bSigma{\boldsymbol{\Sigma}}
\newcommand\normal{{\sf N}}
\newcommand\bdelta{\boldsymbol{\delta}}
\newcommand\sign{{\rm sign}}
\newcommand\sT{{\sf T}}
\newcommand\I{\mtx{I}}
\newcommand\zero{\mtx{0}}
\newcommand\bA{\mtx{A}}
\newcommand\bv{\mtx{v}}
\newcommand\cI{\mathcal{I}}
\newcommand\bz{\boldsymbol{z}}
\newcommand\bg{\boldsymbol{g}}
\newcommand\ba{\boldsymbol{a}}
\def\cC{\mathcal{C}}
\def\de{{\rm d}}
\def\bM{\mtx{M}}
\def\cH{\mathcal{H}}
\def\bu{\boldsymbol{u}}
\def\by{\boldsymbol{y}}
\def\bw{\boldsymbol{w}}
\def\bX{\boldsymbol{X}}
\def\tbX{\tilde{\boldsymbol{X}}}
\def\tbx{\tilde{\boldsymbol{x}}}
\def\tbth{\tilde{\boldsymbol{\theta}}}
\def\hz{\widehat{z}}
\def\ind{\mathbf{1}}
\def\cS{\mathcal{S}}
\def\prob{\mathbb{P}}
\def\tx{\tilde{x}}
\def\reals{\mathbb{R}}
\newcommand{\aj}[1]{\noindent{\textcolor{blue}{\textbf{\#\#\# AJ:} \textsf{#1} \#\#\#}}}

\newcommand{\gauss}{\mathcal{N}(0,I)}
\newcommand{\gausscov}[1]{\mathcal{N}(0,{#1})}
\newcommand{\argmin}{\mathop{\mathrm{argmin}}}
%\newcommand{\cLCE}{\cL_{\mathrm{CE}}}
\newcommand{\cLCE}{\cL}
\newcommand{\mscrU}{{\mathscr{U}}}

==> Icassp (3)/s_exp.tex <==
\maketitle
\section{Numerical Experiments}\vspace{-5pt}
\label{s:exp}

% {\color{blue} Leave to Ibrahim}

% {\color{blue} I can roughly see what you did, but I'm not sure about a few details. Maybe I can mark down and talk to you on Mon, I'll have enough time to edit after that.}


We generate synthetic datasets with $k$ different tasks and $n$ samples for all tasks. As dimension of the data and dimension of the subspace we choose $d=50$ and $r=5$, respectively. %In all experiments we choose all $n_j$'s to be same i.e.~$n_j=n$. 

We study two different setups. In the first one data is generated according to Def.~\ref{def:GLM}. For the second setup, there is an underlying 3-layer neural network that fits the data. In both setups our only aim is to retrieve subspace representations of the data using Algorithm \ref{algo:1}.

\begin{figure}[t!]
\centering
\begin{subfigure}[htbp!]{0.23\textwidth}
\centering
\includegraphics[width = \linewidth]{Paper/Figures_in_Paper/11.png}
\subcaption{}\label{fig1a}
\end{subfigure}
\begin{subfigure}[htbp!]{0.23\textwidth}
\centering
\includegraphics[width =\linewidth]{Paper/Figures_in_Paper/21.png}
\subcaption{}\label{fig1b}
\end{subfigure}
\vspace{-0.35cm}
\captionsetup{width=\linewidth}{\caption{Subspace correlations with fixed number of tasks. \hspace{0.4cm}(a) Binary classification (b) Neural network.}  \label{fig1}} 
\end{figure} 

For neural network experiments, we assume that the data are generated from a ground truth neural network which has 3 layers, defined as  
$$ \yij = f^j(\xij) + \epsilon_{i,j} = \mtx{W}_{j3}(\mtx{W}_{j2}(\mtx{W}_{j1}(\mtx{W}\xij))_+)_+ + \epsilon_{i,j}$$ 
where  $\epsilon_{i,j}\sim\Nn(0,1)$ is gaussian noise, $(\cdot)_+$ is the ReLU activation function, $\mtx{W}\in\R^{5\times 50}$ is representation matrix which is same for all $j$'s. The weight matrices $\mtx{W}_{j1},\mtx{W}_{j2}$ and $\vct{W}_{j3}$ are different for each task and they are random gaussian matrices in $\R^{20\times 5},\R^{20\times 20},\R^{20}$ respectively.
\vspace{0cm}
\iffalse
\begin{figure}[htbp!]
\centering
\begin{subfigure}[htbp!]{0.23\textwidth}
\centering
\includegraphics[width = \linewidth]{Paper/Figures_in_Paper/12.png}
\subcaption{}\label{fig2a}
\end{subfigure}
\begin{subfigure}[htbp!]{0.23\textwidth}
\centering
\includegraphics[width =\linewidth]{Paper/Figures_in_Paper/22.png}
\subcaption{}\label{fig2b}
\end{subfigure}
\vspace{-0.2cm}
\captionsetup{width=\linewidth}{\caption{Subspace correlations with fixed number of samples per task and varying number of tasks. (a) Binary classification, (b) Neural network.}  \label{fig2}} 
\end{figure} 
\fi
%{\color{blue} Could you send me the data of the plots? I can work on the figure a bit. It would be better to set ``ylim'' so that the lines span the range of vertical direction. E.g., ylim=[0.4,1] in the first figure. And don't use colors, ICASSP requires grey-scale figures so we can't tell by color.}

In Fig.~\ref{fig1}
%, we apply Algorithm \ref{algo:1} to recover the $r$ dimensional subspace and get $\hat \Ub_r$, and check its distance to the true representation space $\Ub_r$ under different $n$'s and $k$'s. 
we use the subspace correlation as the metric for evaluating the accuracy of subspace recovery, which is defined by  $\frac{\|{\hat{\mtx{U}_r}^\top\mtx{U}_r}\|^2}{\|\mtx{U}_r\|^2}$.
In Fig.~\ref{fig1}, $k=100$ is fixed but $n$'s vary from $20$ to $200$. It can be seen from Fig.~\ref{fig1} that as $nk$ gets bigger, the subspace correlation becomes closer to $1$, which is compatible with Theorem \ref{thm:hatM}

In Fig.~\ref{fig3}(a), the downstream task accuracies for binary classification are depicted. For the new task, a new 1-layer neural network without any activation function is trained with and without the retrieved representations of the earlier tasks. We find the parameters of the neural network by minimizing the cross entropy loss via SGD. For this setup, during meta-training, we set $n=50$ for all tasks and $k=2000$, to have almost perfect representation. We evaluate the test error with $1000$ new samples.
%by generating $1000$ samples from the same task, 

\begin{figure}[t!]
\centering
\begin{subfigure}[htbp!]{0.24\textwidth}
\centering
\includegraphics[width =  \linewidth]{Paper/Figures_in_Paper/colorednewtaskacc.png}
\end{subfigure}
\hspace{-0.2em}
\begin{subfigure}[htbp!]{0.22\textwidth}
\centering
\includegraphics[width =  \linewidth]{Paper/Figures_in_Paper/alltogether.png}
\end{subfigure}
\captionsetup{width=.45\textwidth}{\caption{(a) Accuracy for downstream task, binary classification (b) Accuracy for downstream the task, MNIST} \label{fig3}}
\end{figure}


If the number of few-shot training samples is small, accuracy improves much faster when we use representation learning. This validates that dimension reduction reduces the degrees-of-freedom for few-shot learning, so the optimal model can be learned with fewer samples. As the sample size grows, the relative benefit of representation is smaller but still noticeable.

In Fig. \ref{fig3}(b), Algorithm \ref{algo:1} is also tested in MNIST dataset. $d=784$ and $r$ is not known. We assume that we have different binary classification tasks among pairs of digits such as 0-1;2-3;0-8;8-4 etc. There exist 15 meta-training tasks (i.e., $k=15$). For each task we have 500 samples in each classes. We choose a different pair of classes as few-shot learning task. We choose binary classification among images of 1 and 9, which is not included in the meta-learning phase. We tune the predicted subspace dimensions and number of samples to get Fig. \ref{fig3}(b).
\iffalse
\begin{figure}[htbp!]
\centering
\begin{subfigure}[htbp!]{0.37\textwidth}
\centering
\includegraphics[width =   \linewidth]{Paper/Figures_in_Paper/alltogether.png}
\end{subfigure}
\captionsetup{width=.45\textwidth}{\caption{Accuracy for downstream the task,MNIST} \label{figlast}}
\end{figure}
\vspace{-0.25cm}
\fi
It can be concluded that when $r=20$, 
%it does not serve a good representation 
The downstream task is not learnt well so we need to expand the subspace. For $r=50$ and $r=100$ subspace learning helps for few-shot learning, as when the number of training samples $n$ is between 8-56 they outperform the case without representation. When $r$ gets closer to $d$, the few-shot sample size has to be large to succeeed due to higher degree of freedom.
%When it comes to $r=400$ we deduce that we get results very similar to no representation case, as when $r$ is big and close to $d$, the model has huge degree of freedom so for good test accuracies $n$ must be big.
% \begin{figure}[htbp!]
% \centering
% \begin{subfigure}[htbp!]{0.35\textwidth}
% \centering
% \includegraphics[width =  \linewidth]{Paper/Figures_in_Paper/r15_1vs8_bluered_new_n.png}
% \end{subfigure}
% \captionsetup{width=.45\textwidth}{\caption{Accuracy for downstream task} \label{fig3}}
% \end{figure}
% \vspace{-0.25cm}


% \begin{figure}[htbp!]
% \centering
% \begin{subfigure}[htbp!]{0.35\textwidth}
% \centering
% \includegraphics[width =  \linewidth]{Paper/Figures_in_Paper/r15_1vs8_bluered_new_n.png}
% \end{subfigure}
% \captionsetup{width=.45\textwidth}{\caption{Accuracy for downstream task} \label{fig3}}
% \end{figure}
% \vspace{-0.25cm}
% \section{Conclusion and Future Work}
% In this work we showed that subspace-based representations can be efficiently learned for highly nonlinear tasks including GLMs and neural networks and help reduce sample complexity for future downstream tasks. A drawback of our results is that they are restricted to normally distributed data. It would be desirable to address such limitations by using distributional universality results such as \cite{oymak2018universality,abbasi2019universality}. Another direction is developing a more refined understanding for deep learning by restricting our nonlinear model space to deep neural nets.
%in contrast to more general purpose results developed here.
% {\color{red} YS: The blue curve is about 0.9, I feel it's already very accurate so we don't need this paragraph.}
% Additionally, we generate samples as defined in Def. \ref{def:bin_class}. $y$ conditioned on $\x$ is a random variable, yet not deterministic, so the data is implicitly noisy. Therefore the accuracy cannot reach $1$ empirically on the generated data.
% In Fig. \ref{fig1}, subspace correlations between the actual subspace and the predicted one using Algorithm \ref{algo:1}. Subspace correlations are calculated by  $\frac{\|{\hat{\mtx{U}_r}^\top\mtx{U}_r}\|^2}{\|\mtx{U}_r\|^2}$.It can be deduced that in both nonlinear setup subspace can be learned via moment estimator $t_j$ increases.
% \begin{figure}[htbp!]
% \centering
% \begin{subfigure}[htbp!]{0.4\textwidth}
% \centering
% \includegraphics[width = \linewidth]{Paper/Figures_in_Paper/GrayScale_NN_k100_subspace.png}
% \subcaption{}\label{fig1a}
% \end{subfigure}
% \begin{subfigure}[htbp!]{0.4\textwidth}
% \centering
% \includegraphics[width =\linewidth]{Paper/Figures_in_Paper/GrayScale_NN_nj30_subspace.png}
% \subcaption{}\label{fig1b}
% \end{subfigure}
% \captionsetup{width=.45\textwidth}{\caption{Subspace correlations, (a) for binary classification task whereas (b) stands for 3-layer Neural Net experiment.}  \label{fig1}} 
% \end{figure} 


==> Icassp (3)/s_gen_loss_proof.tex <==

\section{Proof of main theorems}

\iffalse
\SO{Clearly Theorem \ref{thm:hatM append} is a restatement of Theorem \ref{thm:hatM}. Why don't you say so? Reader is not expected to figure out this by himself. Let us make things clear.}

\SO{Similarly, where is proof of Lemma 3.1? Looks like Lemma \ref{lem:mean nn} is its restatement but again not clear at all for reader. They cannot find proof of Lemma 3.1 in the text.}

\SO{Here is the organization we need: In the appendix, proof of each technical result in the main text is supposed to have its own subsection. Just like this subsection that I added i.e.~Proof of Theorem \ref{thm:hatM}.}
\SO{Maybe briefly describe the outline. Right now, little confusing due to Lemmas within the proof so outline would help i.e.~we first prove Lemma ... which shows ...}
\subsection{Proof of Lemma \ref{lem:M exp} and Theorem \ref{thm:hatM}}
\fi
We sketch the proof at the beginning. First we compute the expectation of $y\x$ in Lemma \ref{lem:mean nn}. That leads to the proof of Lemma \ref{lem:M exp}. Then in Lemma \ref{lem:err_yx} we bound the difference between sum of $y\x$ and its mean using concentration. The concentration of covariance estimator is studied later in Lemma \ref{lem:Zj} and \ref{lem:Zj2}, which leads to Theorem \ref{thm:hatM}.

\subsubsection{Proof of Lemma \ref{lem:M exp}}
We first state Lemma \ref{lem:M exp} below.
\begin{lemma}\label{lem:M exp append}
Let 
\begin{subequations}\label{eq:hatM append}
\begin{align}
\hat\bM &= \mathop{\Scale[1.8]{\sum}}_{j=1}^k \frac{2}{n_j^2}\left[(\sum_{i=1}^{n_j/2} \yij\xij) (\sum_{i=n_j/2+1}^{n_j} \yij\xij)^\top \right.\\
&\quad\quad\quad\quad \left. +  ( \sum_{i=n_j/2+1}^{n_j} \yij\xij) ( \sum_{i=1}^{n_j/2} \yij\xij)^\top\right].\nonumber
\end{align}
\end{subequations}
And
\begin{align*}
    &\mtx{h}^j(\W): \R^{r\times d} \rightarrow \R^d = \mtx{E}_{\x}[f^j(\W \x)\x]\\
    &\bM := \W^\top\W\left(\frac{1}{k}\sum_{j=1}^k \mtx{h}^j(\W)( \mtx{h}^j(\W))^\top\right)\W^\top\W.
\end{align*}
Then $\bM,\hat{\bM}$ satisfies the following. (a) $\text{rank}(\bM)\leq r$. (b) $\text{range-space}(\bM)\subset \text{row-space}(\W)$. (c) $\mtx{E}[\hat{\M}]=\bM$. 
\end{lemma}
\begin{proof}
Part (a) and (b) are easy to see. $\W\in\R^{r\times d}$ so that $\text{rank}(\bM)\leq r$, and since $\bM$ is the product of $\W^\top$ and another matrix, then  $\text{range-space}(\bM)\subset \text{row-space}(\W)$.
Now we will prove Part (c). We first give the lemma for the mean of the random vector $y\x$.

\begin{lemma}\label{lem:mean nn}
We assume that the data is generated as in Def. \ref{def:task}, and we study the $j$-th task whose activation function is $f^j$. 
%{\color{blue} To be finished}
Define
\begin{align*}
    \mtx{h}^j(\W): \R^{r\times d} \rightarrow \R^d = \mtx{E}_{\x\sim\gauss} f^j(\W \x)  \x
\end{align*}
Denote the joint distribution of $(\x,y)$ as $\Pxy$.
Then $\mtx{E}_{(\x,y)\sim\Pxy}(y \x) = \W^\top\W \mtx{h}^j(\W)$.
\end{lemma}

\emph{Proof of Lemma \ref{lem:mean nn}.} The expectation can be expanded as
\begin{align*}
    &\mtx{E}_{(\x,y)\sim\Pxy}(y \x) \\
    &= \mtx{E}_{\x\sim\gauss} f^j(\W \x) \x\\
    &= \mtx{E}_{\x\sim\gauss} \left(f^j(\W \x)  \W^\top\W \x + f^j(\W \x) (I - \W^\top\W)\x \right).
\end{align*}
Note that, because $\x\sim\gauss$ so $\W \x$ and $(I - \W^\top\W)\x$ are Gaussian. $\W\W^\top = I$ implies 
\begin{align*}
    &\quad \Eb (\W \x)\x^\top((I - \W^\top\W))\\
    &= \W(I - \W^\top\W) = 0.
\end{align*}
So $\W \x$ and $(I - \W^\top\W)\x$ are independent, so 
\begin{align*}
    &\quad \mtx{E}_{\x\sim\gauss}  f^j(\W \x) (I - \W^\top\W)\x \\
    &= (\mtx{E}_{\x\sim\gauss}  f^j(\W \x)) (\mtx{E}_{\x\sim\gauss} (I - \W^\top\W)\x) = 0
\end{align*}
Then 
\begin{align*}
    \mtx{E}_{(\x,y)\sim\Pxy}(y \x) &= \W^\top\W(\mtx{E}_{\x\sim\gauss} f^j(\W \x) \x)\\
    &= \W^\top\W \h_j(\W).
\end{align*}

Denote 
\begin{align}\label{eq:Hj def}
    \Hb^j(\W) = \W^\top\W \mtx{h}^j(\W)
\end{align}
Because $\frac{2}{n_j}\sum_{i=1}^{n_j/2} \yij\xij$
and 
$\frac{2}{n_j}\sum_{i={n_j/2}+1}^{n_j} \yij\xij$ 
are independent, and their expectation are both $\Hb^j(\W)$, so that
\begin{align*}
    &\quad \mtx{E}(\frac{2}{n_j}\sum_{i=1}^{n_j/2} \yij\xij)(\frac{2}{n_j}\sum_{i={n_j/2}+1}^{n_j} \yij\xij)^\top \\
    &= \Hb^j(\W)(\Hb^j(\W))^\top.
\end{align*}
At then end
\begin{align*}
    \hat \bM &= \frac{1}{k}\sum_{j=1}^k \mtx{E}(\frac{2}{n_j}\sum_{i=1}^{n_j/2} \yij\xij)(\frac{2}{n_j}\sum_{i={n_j/2}+1}^{n_j} \yij\xij)^\top,\\
    \bM &= \frac{1}{k}\sum_{j=1}^k\Hb^j(\W)(\Hb^j(\W))^\top,
\end{align*}
so we can prove Part (c) that $\mtx{E}(\hat \bM) = \bM$.
\end{proof}


\subsubsection{Proof of Theorem \ref{thm:hatM}}
We restate Theorem \ref{thm:hatM append} below. 
\begin{theorem}\label{thm:hatM append}
Suppose the data is generated as Def. \ref{def:task}. Let $\delta\in(0,1)$, $\epsilon\in(0,1)$. Suppose $y\x$ is a subGaussian random vector with covariance upper bounded by
\begin{align}
   \| \mathbf{Cov}(y \x) \| \le \sigma^2. \label{eq:covyx append}
\end{align} 
Define
\begin{align*}
    \mtx{h}^j(\W): \R^{r\times d} \rightarrow \R^d = \mtx{E}_{\x\sim\gauss} f^j(\W \x)  \x
\end{align*}
And let %$\bM = \mtx{E}_{\theta\sim\mathcal{N}(0,\bSi)} (g(\theta))^2\frac{\theta\theta^\top}{\|\theta\|^2}$, then
\begin{align*}
    \bM = \W^\top\W\left(\frac{1}{k}\sum_{j=1}^k \mtx{h}^j(\W)( \mtx{h}^j(\W))^\top\right)\W^\top\W
\end{align*}
Then there exists a constant $c$, with probability at least $1-\delta$, let 
\begin{align*}
    k = \frac{cd}{n}\log^2(\frac{kd}{\delta}) \max\{\frac{1}{\epsilon^2}, \frac{1}{\epsilon} \log(\frac{kd}{\delta})\}
\end{align*}
we have 
\begin{align*}
    \|\hat \bM - \bM\| \le \epsilon\sigma^2.
\end{align*}
\end{theorem}
\begin{proof}
The following lemmas are similar to \cite{kong2020meta} Section A.1. We extend the concentration inequalities from bounded random vectors to Gaussian random vectors. For completeness we place the lemmas here.

\begin{lemma}\label{lem:err_yx}
(\cite{jin2019short} Cor. 7) 
Let $\|\mathbf{Cov}(y\x)\| \le \sigma^2$, $\delta\in(0,1)$, $t>0$, $\Hb^j(\W)$ be defined in \eqref{eq:Hj def}. With probability $1-\delta$, there exists a constant $c>0$ such that for every $j$,
%\som{Remind the exact assumption on $\sigma$}
\begin{align}
   \|\frac{1}{t}\sum_{i=1}^t \yij\xij - \Hb^j(\W)\| \le c\sigma\sqrt{\frac{d}{t}\log(\frac{kd}{\delta})} \label{eq:gauss_bern}
\end{align}
%\som{Call $\W^\top\W \mtx{h}^j(\W)$ something for simpler notation}
Denote this event as $\mathcal{E}$.
\iffalse
{\it\color{red} for every i,j pairs ? }Denote this event as $\mathcal{E}$.
{\it \color{red} if we dont say "for every i,j pairs" ,k should not appear in an inequality which holds for only one task. Also maybe it is better to  cite [21] A.5, because [28] Cor.7 says only the following
$$\|\frac{1}{t}\sum_{i=1}^t \yij\xij - \W^\top\W \mtx{h}^j(\W)\| \le c\sigma\sqrt{\frac{1}{t}\log(\frac{2d}{\delta})}$$}
\fi
\end{lemma}
With the covariance of $y\x$ being bounded by $\sigma^2$, the following inequalities are true \cite{kong2020meta}.
\begin{align*}
    \Eb\left( (\vb^T\cdot (\frac{1}{t}\sum_{i=1}^t \yij\xij - \theta^j))^2\right) &\le \sigma^2 / t,\mbox{~for~} \|\vb\|=1.\\
    \Eb \left(\|\frac{1}{t}\sum_{i=1}^t \yij\xij - \theta^j \|^2\right) &\le \sigma^2d/t.
\end{align*}


\begin{lemma}\label{lem:Zj}
Define
\begin{align*}
    \Zb_j &= (\frac{2}{n_j}\sum_{i=1}^{n_j/2} \yij\xij)(\frac{2}{n_j}\sum_{i={n_j/2}+1}^{n_j} \yij\xij)^\top \\
    &\quad - \Hb^j(\W)(\Hb^j(\W))^\top,
\end{align*}
Then there exists a constant $c$ such that on the event $\mathcal{E}$ (thus with probability $1-\delta$), for all $j=1,...,k$, 
\begin{align}
    \|\Zb_j \| \le \frac{c\sigma^2d}{n_j} \log(\frac{kd}{\delta}). \label{eq:evt}
\end{align}
\end{lemma}

% {\it \color{red} From my understanding we should have 
% $$\|\Zb_j \| \le (Eq A.1 Bound)(Eq. A.1 bound + 2\|\W^\top\W \mtx{h}^j(\W)\|)$$ choosing $t=\dfrac{n_j}{2}$ then we have $$\|\Zb_j \| \le (c\sigma\sqrt{\frac{2}{n_j}\log(\frac{2d}{\delta})})(c\sigma\sqrt{\frac{2}{n_j}\log(\frac{2d}{\delta})} + 2\|\W^\top\W \mtx{h}^j(\W)\|)$$
% This is more or less what you have found, but the difference is k in $\log$ term and d term }



The proof is almost same as \cite{kong2020meta}, the only difference is that we replace the bound in (\cite{kong2020meta} Prop A.1) by \eqref{eq:gauss_bern}. With the similar replacement, we propose the following lemma. 
\begin{lemma}\label{lem:Zj2}
Let $\delta\in(0,1)$. There exists a constant $c$, such that for any $\epsilon\in(0,1)$, and 
\begin{align}
    k = \frac{cd}{n_j}\log^2(\frac{kd}{\delta}) \max\{\frac{1}{\epsilon^2}, \frac{1}{\epsilon} \log(\frac{kd}{\delta})\}, \label{eq:k lb}
\end{align}
with probability $1-\delta$, 
\begin{align*}
    \|\frac{1}{k} \sum_{j=1}^k \Zb_j\| \le \epsilon \sigma^2.
\end{align*}
\end{lemma}
This means that when \eqref{eq:k lb} is true, with probability $1-\delta$,
\begin{align*}
    \left\|\hat \bM - \W^\top\W\left(\frac{1}{k}\sum_{j=1}^k \mtx{h}^j(\W)( \mtx{h}^j(\W))^\top\right)\W^\top\W\right\| \le \epsilon \sigma^2.
\end{align*}
Note that $\bM$ is defined as \[\bM=\W^\top\W\left(\frac{1}{k}\sum_{j=1}^k \mtx{h}^j(\W)( \mtx{h}^j(\W))^\top\right)\W^\top\W.\] So we have proven that with probability $1-\delta$,
\begin{align*}
    \left\|\hat \bM - \bM\right\| \le \epsilon \sigma^2.
\end{align*}

%\som{Remind that this is $\hat \bM-\bM$ i.e. $\bM=\text{the messy sum}$}
\end{proof}

%\SO{Create a subsection here!!! Reduce the confusion as much as possible, make transitions smooth.}
\subsection{Proof of Theorem \ref{thm:down}}
Now we will prove Theorem \ref{thm:down}. We first review the notations and assumptions mentioned in the theorem.

\subsubsection{Review of Notations and Assumptions}
We define the SVD of $\hat \bM$ as $\hat \Ub \hat\La \hat\Vb^\top$. Let the first $r$ columns of $\hat \Ub$ be $\Ub_r$. 

Let $\hat\W$ be defined as 
\begin{align}
    \hat \W &= \hat \Ub_r \hat \Qb, \label{eq:def W append}\\
    \hat \Qb &= \mathop{\mathrm{argmin}}_{\Qb\in\R^{r\times r}, \Qb\Qb^\top = I}\ \|\hat \Ub_r \Qb - \W\|.
\end{align}
The population cross entropy loss is defined as
\begin{align*}
    &\cLCE(f;\Pb) : \Fc\times \R^{r\times d}\rightarrow \R=\\
    &-\mtx{E}_{\x,y\sim\Pxy} (y\log f(\hat\Pb \x) + (1-y)\log (1 - f(\hat\Pb \x))).
\end{align*}
We will search for a function $f^* \in \Fc$.% that minimizes the population cross entropy loss. 
\begin{assumption}\label{append ass:F}
$\Fc$ is a set of functions satisfying: For any function $f\in\Fc$, any orthonormal matrix $\Qb\in\R^{r\times r}$ and any matrix $\Pb\in\R^{r\times d}$, there exists $g \in \Fc$ such that $f(\Pb \x) = g(\Qb\Pb \x)$.
%\begin{enumerate}
%    \item For any function $f\in\Fc$, any orthonormal matrix $\Qb\in\R^{r\times r}$ and any matrix $\Pb\in\R^{r\times d}$, there exists $g \in \Fc$ such that $f(\Pb \x) = g(\Qb\Pb \x)$.
%    \item $\Fc \subseteq \{f\ |\ \log f,~ \log(1-f)\mathrm{~are~}L\mathrm{~Lipschitz}\}\bigcap \{f\ |\ 0<f(x)<1,\forall x\in\R^r\}$.
%\end{enumerate}
\end{assumption}
Now we define a general loss function $\cL$ and $\cL_e$.
\begin{assumption}\label{append ass:L}
Suppose $\cL$ satisfies the following assumptions:
\begin{enumerate}
    \item %$\cL$ takes $f(\Pb x)$ as the argument, i.e., 
    $\cL$ has the form $\cL(f;\Pb) = \mtx{E}_{\Pxy}\Lcs(f(\Pb \x),y)$. $\cL_e$ has the form $\cL_e(f;\Pb) = \frac{1}{n}\sum_{i=1}^n\Lcs(f(\Pb \x_i),y_i)$.
    \item $\Lcs$ is $L$ Lipschitz in $\Pb \x$.
    \item $\min_{\Pb}\cL(f;\Pb) = \cL(f;\W)$.
\end{enumerate}
\end{assumption}
We solve for $\hat f$, defined as \begin{align}
    \hat f &= \argmin_{f\in\Fc}\ \cLCE(f;\hat \Ub_r^\top). \label{eq:def f append}
\end{align}
\subsubsection{Proof of Theorem \ref{thm:down}}
Now we are ready to restate Theorem \ref{thm:down} and prove it.

\begin{theorem}\label{thm:popu append}
With Assumptions \ref{append ass:F} and \ref{append ass:L}, we have that
    \begin{align*}
        \cLCE(\hat f;\hat \Ub_r^\top)  - \cLCE(f^*;\Ub_r^\top) \lesssim L\sqrt{r}\|\hat \W - \W\|.
    \end{align*}
\end{theorem}

\begin{proof}
We learn the model from the following optimization algorithm.
\begin{align*}
    \hat f &= \argmin_{f\in\Fc}\ \cLCE(f;\hat \Ub_r^\top)
    %\\
    %&= \argmin_{f\in\Fc}\ -\mtx{E}_{\x,y\sim\Pxy} (y\log f(\hat\Ub_r^\top \x) \\
    %&\quad + (1-y)\log (1 - f(\hat\Ub_r^\top \x)))\\
    %&= \argmin_{f\in\Fc}\ -\mtx{E}_{\x\sim\gauss} \left(f^*(\W \x)\log f(\hat \Ub_r^\top \x)\right. \\
    %& \quad \left. + (1-f^*(\W \x))\log (1 - f(\hat \Ub_r^\top \x)) \right).
\end{align*}
Denote $\tilde f\in\Fc$ as the function such that $\tilde f(\hat \W \x) = \hat f(\hat \Ub_r^\top \x)$. So that $\cLCE(\hat f;\hat \Ub_r^\top) = \cLCE(\tilde f;\hat \W)$. Since $\hat f$ minimizes the cross entropy loss, we have that $\cLCE(\tilde f;\hat \W) \le \cLCE(f^*;\hat \W)$. 

Now we have 
\begin{align*}
    &\quad \cLCE (\tilde f;\hat \W) - \cLCE (f^*;\W)\\
    &\le \cLCE (f^*;\hat \W) - \cLCE (f^*;\W)\\
    %&\le -\mtx{E}_{\x\sim\gauss} \left(f^*(\W \x)(\log f^*(\hat\W \x) -\log f^*(\W \x))\right. \\
    %& \quad \left. + (1-f^*(\W \x))(\log (1 - f^*(\hat \W \x)) - \log (1 - f^*(\W \x))) \right)\\
    &\le \mtx{E}_{\x\sim\gauss} L\|(\hat \W - \W)x\|\\
    &\lesssim L\sqrt{r}\|\hat \W - \W\|.
\end{align*}
The last step uses the fact that $\hat \W$ and $\W$ are rank $r$.
\end{proof}

\subsection{Proof of Theorem \ref{thm:rade}}
%Now we prove that the upper bound of the error for few-shot learning with finite samples.
We first state Theorem \ref{thm:rade} below.
\begin{theorem}\label{thm:rade app}
    Suppose we generate $n$ sample data for few shot learning solve for $\hat \theta_e$ from 
    \begin{align}
   	 \hat \bt_e &= \argmin_{\bt}\ \cL_e(\bt;\Ub_r^\top)\quad\text{such~that}\quad\|\bt\|_2\le a.\label{eq:fstar finite theta append}
	\end{align}
   Suppose Assumptions \ref{append ass:F} and \ref{append ass:L} hold.
    There exist constants $c>0$, $\delta\in(0,1)$, with probability at least $1 - n^{-c+1} - \delta$, the solution $\hat\theta_e$ and $\hat\Ub_r$ satisfy
    \begin{align*}
        &\quad \mathcal{L} (\hat\theta_e;\hat\Ub_r^\top) - \mathcal{L} (\theta^*;\W) \\
        &\lesssim \frac{caL(\sqrt{r}+\log(n)) (1+ \sqrt{\log(1/\delta)})}{\sqrt{n}} + L\sqrt{r}\|\hat \W - \W\|. 
    \end{align*}
\end{theorem}
\begin{proof}
We sketch the proof of Theorem \ref{thm:rade app}. After reviewing the notations, we quote a standard generalization bound via Rademacher complexity in Lemma \ref{lem:rade known}. Then we use the smoothness of the loss function to link to the generalization error of linear functions \eqref{eq:lin rade}, and then use Lemma \ref{lemma:chi-sqr} to compute \eqref{eq:lin rade} and finish the proof.

In few-shot learning, the true parameter is $\theta^*$, and the empirical loss function with finite data is 
\begin{align}
    &\cL_e(\theta;\Pb) : \Fc\times \R^{r\times d}\rightarrow \R= \frac{1}{n}\sum_{i=1}^n \Lcs(f(\Pb\x_i), y_i)
    %\notag\\
    %&-\frac{1}{n}\sum_{i=1}^n (y_i\log\phi (\theta^\top\Pb \x_i) + (1-y_i)\log (1 - \phi(\theta^\top\Pb \x_i))) \label{eq:cLCE finite theta app}
\end{align}
Denote each term in the summation as 
\begin{align*}
    &\quad \cL_e^i(\theta;\Pb) : \Fc\times \R^{r\times d}\rightarrow \R = \Lcs(f(\Pb\x_i), y_i).
    %=\notag\\
    %&- (y_i\log \phi (\theta^\top\Pb \x_i) + (1-y_i)\log (1 - \phi(\theta^\top\Pb \x_i)))
\end{align*}
We search for the solution by
\begin{align}
    \hat \theta_e &= \argmin_{\theta}\ \cL_e(\theta;\Ub_r^\top),\mbox{~such~that~} \|\theta\|\le a.\label{eq:fstar finite theta app}
\end{align}
In Theorem \ref{thm:popu append}, we know that
\begin{align*}
    \cLCE(\hat \theta;\hat \Ub_r^\top)  - \cLCE(\theta^*;\Ub_r^\top) \lesssim L\sqrt{r}\|\hat \W - \W\|.
\end{align*}
Denote 
    \begin{align}
        M = \max_{\|\theta\|\le a} |\theta^\top \hat\Ub_r^\top\x_i| \le a \max\|\hat\Ub_r^\top\x_i\|.\label{eq:bound_rade}
    \end{align}
We will bound the difference between $\cL$ and $\cL_e$ by Rademacher complexity theory.
\begin{lemma}\label{lem:rade known}
    \cite{mohri2018foundations}
 
    Let $\mscrU$ be the independent random variables uniformly chosen from $\{-1,1\}$.
    Let $\Rc$ be the Rademacher complexity of the logistic functionals defined on the data,
    \begin{align*}
        \Rc &= \frac{1}{n}\Eb_{\epsilon_i\in\mscrU} \sup_{\|\theta\|\le a} \sum_{i=1}^n\epsilon_i\cL_e^i(\theta;\hat\Ub_r^\top) \\
        %K &= |\log(\phi(-M))|>\max_i\cL_e^i(\theta;\hat\Ub_r^\top)
        K&= \max_i\cL_e^i(\theta;\hat\Ub_r^\top) \le M.
    \end{align*}
    %We know $\cL_e^i(\theta;\hat\Ub_r^\top)<K$ with probability at least $1-n^{-c_1+1}$,
    %then for any $\theta$ such that $\|\theta\|\le a$, with probability $1-\delta-n^{-c_1+1}$, we have that 
    with probability $1-\delta$, we have that 
    \begin{align*}
        |\cL_e(\theta;\Ub_r^\top) - \cL(\theta;\Ub_r^\top)| \le \Rc + \frac{\sqrt{\log(1/\delta)}}{\sqrt{n}}K.
    \end{align*}
\end{lemma}
Thus we have that 
\begin{align*}
    |\mathcal{L} (\hat\theta_e;\hat\Ub_r^\top) - \mathcal{L}_e (\hat\theta_e;\hat\Ub_r^\top)| &\le \Rc + \frac{\sqrt{\log(1/\delta)}}{\sqrt{n}}K,\\
    |\mathcal{L} (\hat\theta;\hat\Ub_r^\top) - \mathcal{L}_e (\hat\theta;\hat\Ub_r^\top)| &\le \Rc + \frac{\sqrt{\log(1/\delta)}}{\sqrt{n}}K.
\end{align*}
Because $\hat\theta_e$ minimizes the empirical loss $\mathcal{L}_e$,
\begin{align*}
    \mathcal{L}_e (\hat\theta_e;\hat\Ub_r^\top) \le \mathcal{L}_e (\hat\theta;\hat\Ub_r^\top).
\end{align*}
Thus 
\begin{align}
    \mathcal{L} (\hat\theta_e;\hat\Ub_r^\top) - \mathcal{L} (\hat\theta;\hat\Ub_r^\top) \le 2\left(\Rc + \frac{\sqrt{\log(1/\delta)}}{\sqrt{n}}K\right).\label{eq:emp loss}
\end{align}
So the remaining target is to bound $\Rc$. 

We first denote $\vb_i = \hat\Ub_r^\top \x_i$, so $\vb_i\in\R^r$ and $\vb_i$ are jointly independent standard normal random variables. %In binary classification, 
$\cL_e^i$ is always $L$ Lipschitz in $\theta^\top\vb_i$, the Rademacher complexity can be upper bounded by
\begin{align}\label{eq:lin rade}
    \Rc \le \tilde\Rc := \frac{L}{n}\Eb_{\epsilon_i\in\mscrU} \sup_{\|\theta\|\le a} \sum_{i=1}^n \epsilon_i\theta^\top\vb_i. 
\end{align}
We first refer to the following lemma.
\begin{lemma}\label{lemma:chi-sqr}
    \cite{laurent2000adaptive} Let $c>0$, $X$ follow $\chi_r^2$ distribution, then
    \begin{align*}
        \Pb(X - r \ge 2\sqrt{cr\log n} + 2c\log n) \le n^{-c}.
    \end{align*}
\end{lemma}

For a constant $c>1$, via union bound we have that $\max{\|\vb_i\|^2} \le r + 2\sqrt{cr\log n} + 2c\log n$ for all $i=1,..,n$ with probability $1 - n^{-c+1}$. We use $\max{\|\vb_i\|} \lesssim c(\sqrt{r} + \log(n))$ for simplicity.

Conditioned on this event, we apply the Rademacher complexity for linear model that 
\begin{align}
   \tilde \Rc &\le \frac{L\max\|\theta\| \cdot \max\|\vb_i\|}{\sqrt{n}}\\
   &\le \frac{caL(\sqrt{r} + \log(n))}{\sqrt{n}}. \label{eq:tilde Rc}
\end{align}
Combining with \eqref{eq:emp loss} and Theorem \ref{thm:popu append} we get the bound in Theorem \ref{thm:rade app}. We can also bound $M$ in \eqref{eq:bound_rade}.

Finally we will use Lemma \ref{lem:M to K} to bound $M$.
\begin{lemma}\label{lem:M to K}
    Let $M$ be defined as in \eqref{eq:bound_rade}.    
    With probability at least $1 - n^{-c+1}$, we have $M<caL(\sqrt{r} + \log(n))$.
\end{lemma}
Let $\vb_i$ be replaced by $\hat \Ub_r^\top\x_i$ in Lemma \ref{lemma:chi-sqr}, then this directly results from Lemma \ref{lemma:chi-sqr}. Lemma \ref{lem:M to K} bounds $M$, thus bounds $K$ (which is $L$ Lipschitz in $M$) in Lemma \ref{lem:rade known}. After we insert \eqref{eq:tilde Rc} together into Lemma \ref{lem:rade known}, we can get the result in  Theorem \ref{thm:rade}.
% By Lemma \ref{lemma:chi-sqr} we know that for a constant $c>2$, we have  $\max{\|\hat\Ub_r^\top\x_i\|} \le c(\sqrt{r} + \log(n))$ for all $i=1,..,n$ with probability $1 - n^{-c+1}$. So with probability at least $1 - n^{-c+1}$, we have $M<ac(\sqrt{r} + \log(n))$.
\end{proof}



==> Icassp (3)/s_intro.tex <==
\section{Introduction}\label{s:intro}
Meta-learning (and multi-task learning) has proved to be a efficient when available training data is limited. The central idea is exploiting the information (e.g.~training data) provided by earlier related tasks to quickly adapt a new task using few samples.
This idea has a rich history \cite{caruana1997multitask,baxter2000model} and has shown promise in modern machine learning tasks, e.g., in image classification \cite{deng2009imagenet}, machine translation \cite{bojar2014findings} and reinforcement learning \cite{finn2017model}, all of which may involve numerous tasks to be learned with limited data per task.
% between thousands of English and French sentences



 \mf{where? give citation}
  \mf{should we use the term meta-learning or multitask learning? It's better to pick one for consistency}
Modern deep learning algorithms typically exploit the shared information between tasks by learning useful representations \cite{schmidhuber1987evolutionary, thrun2012learning}. The multi-task system was studied by \cite{caruana1997multitask}, and the idea of meta-learning or transfer learning is investigated empirically in modern machine learning framework, showing that the shared representation benefits for training on the new tasks \cite{bengio2013representation, hospedales2020meta, yosinski2014transferable}.  %\cite{bengio2013representation, hospedales2020meta, yosinski2014transferable, raghu2019rapid}. 
An instructive and well-studied problem for meta-learning is mixed linear regression,
for which efficient algorithms and sample complexity bounds are discussed in 
\cite{zhong2016mixed, li2018learning, chen2020learning}. If the tasks lie on a shared low-dimensional subspace, learning this subspace would serve as an efficient representation which helps reduce the search space for future tasks. Once the search space is low dimensional, in order to get the same accuracy, the amount of data required for training is reduced compared to training over the full parameter space. \cite{lounici2011oracle,cavallanti2010linear,maurer2016benefit} propose sample complexity bounds for representation learning for linear multi-task systems. There are study of mixed linear tasks combined with other structures, such as boolean combination of features \cite{balcan2015efficient}, half-spaces \cite{rish2008closed} and sparse representations \cite{argyriou2008convex}.
% \mf{main point: low-dimensional approximation of the feature space makes learning easier in a new task, with fewer samples. Thus in many ML applications one seeks such a representation. can omit 'learned by mixed linear regression'. rewrite parag.}

% The low dimensional subspace of the features, learned by mixed linear regression, is utilized as the search space for training on new tasks.
% \mf{swap the order with next paragraph} 

The recent papers \cite{kong2020meta,kong2020robust} propose meta-learning procedures that involve dimension reduction, clustering and few-shot learning. Here a low-dimensional task subspace is used as the search space for few-shot learning for the new task. 
Another related approach
\cite{du2020few,tripuraneni2020provable}
sets up a nonconvex optimization problem with matrix factors of appropriate sizes, which captures the low dimensional structure. One can apply gradient descent to this nonconvex problem, and studying its behavior requires a nontrivial landscape analysis of the matrix factorization problem.  

However, existing provable algorithms for representation learning are restricted to linear-regression tasks, whereas typical machine learning tasks involve nonlinearity. This can arise from the use of nonlinear models as well as nonlinear label link function (e.g.~generalized linear models).
%. The setup is restrictive compared with the variant types of nonlinear tasks. 
\mf{what does 'objective' mean here? do you mean there are different tasks to be performed with different goals, with the same data?}
A good example is classification problems 
%which represent much of the machine learning applications 
including computer vision and natural language processing \cite{deng2009imagenet, bojar2014findings}. 
In classification tasks, the model is a map from images/text to labels, and the labels are discrete and not linear with respect to the input (i.e.~logistic link function). Another example is the use of nonlinear models such as deep networks
%, which contain many nonlinear activation functions within their layers. 
The existing results for representation learning for the linear-regression setting cannot be easily extended to the nonlinear case. 

\noindent\emph{Can we learn efficient subspace representations for nonlinear tasks such as generalized linear models and neural nets?}
%If one can learn a representation that help classify across several tasks, this representation can be used in this model can be retrieved and transferred to a classifier for other objectives.
%\som{Redundant sentence: In these datasets, there are images of different types of objectives, and the task is to classify which categories each image comes from.}

We consider a realizable setup where the input data is high-dimensional, the \emph{relevant features} lie in a low dimensional subspace and the labels depend only on the \emph{relevant features}. These assumptions are the same as in the existing literature, however we additionally allow for the scenario where labels are possibly an arbitrary nonlinear function of the relevant features. We make the following contributions.

\noindent$\bullet$ \textbf{Efficient representations for nonlinear tasks:} We show that subspace found via method-of-moments (MOM) leads to a consistent estimate of the ground-truth subspace despite arbitrary task nonlinearities, when the data is normally distributed.  We combine this with non-asymptotic learning results to establish sample complexity bounds for representation learning.

% \som{emphasize generalized linear model?}
\noindent$\bullet$ \textbf{Few-shot learning and Applications:} We specialize our results to practical settings with tasks involving binary classification and neural nets. We theoretically and empirically show that subspace-based representation can greatly improve sample efficiency of future tasks.
% \som{More citations are needed! Consider adding a related work (sub)section!}

%that, can we still retrieve the subspace with the same amount of training data?

%{\color{blue}Contribution here}




==> Icassp (3)/s_main.tex <==
\section{Main Results}
% {\color{red} YS: Commented some text for space limitation}
\vspace{-.1cm}
In this section, we shall establish error bounds for Algorithm \ref{algo:1}. This involves three parts. Theorem \ref{thm:hatM} establishes the quality of the moment estimator $\hat\bM$. %The estimator is then used for few-shot learning, and 
Theorem \ref{thm:down} upper bounds the population cross-entropy risk of $\hat f$ in the few-shot learning stage. Theorem \ref{thm:rade} upper bounds the population risk of the ERM estimator $\hat f_e$, which is learned from finite data.

\subsection{Results on Meta-training}
\begin{lemma}\label{lem:M exp}
$\bM,\hat{\bM}$ satisfies the following. (a) $\text{rank}(\bM)\leq r$. (b) $\text{range-space}(\bM)\subset \text{row-space}(\W)$. (c) $\mtx{E}[\hat{\M}]=\bM$. 
\end{lemma}
In words, $\bM$ returns a consistent estimate of the representation space in the sense that its range is guaranteed to be the subspace of the representation. Observe that to fully recover representation, $\bM$ should contain a diverse set of tasks that can \emph{cover} the representation subspace. For GLM, one needs at least $k\geq r$ tasks to ensure range of $\bM$ is equal to the row-space of $\W$. Additionally, $\hat{\M}$ estimator is also consistent. %All missing proofs can be found in \cite{paperurl}.



% notation (any well-conditioned can be accomplished by estimating the covariance of the inputs and then whitening the data. Such normalization procedures are common e.g.~batch normalization. 
We next present the error on the estimator $\hat \bM$. This theorem applies to standard normal data $\x\sim\Nn(0,\Iden)$. %This is mostly used for notational convenience. In machine learning subGaussian distributions often behave very similar in sufficiently high-dimensions \cite{oymak2018universality,abbasi2019universality}. We leave such generalizations to more general distributions as a future work. 
While this may initially seem restrictive, we remark that identity covariance is mostly used for notational convenience. Additionally, in similar spirit to Central Limit Theorem, machine learning and signal processing algorithms often exhibit distributional universality: For instance, subgaussian distributions often behave very similar or even identical to gaussian distributions in sufficiently high-dimensions \cite{oymak2018universality,abbasi2019universality}. We leave such generalizations to more general distributions as a future work. 
\begin{theorem}[Moment Estimator]\label{thm:hatM}
Suppose the data is generated as in Def.~\ref{def:task}, $n_j\geq N$ for all $j$ and $\xij\distas\Nn(0,\Iden)$. Suppose for some $\sigma>0$ and for all tasks, the label-input product $y\x$ is a subGaussian random vector with covariance upper bounded by $\| \mathbf{Cov}(y \x) \| \le \sigma^2$. (These conditions hold when $|f^j(\x)|<\sigma$.) Let $\delta\in(0,1)$ and $\epsilon\in(0,1)$. Then there exists a constant $c>0$ such that if
\begin{align*}
    k \ge \frac{cd}{N}\log^2(\frac{kd}{\delta}) \max\{\frac{1}{\epsilon^2}, \frac{1}{\epsilon} \log(\frac{kd}{\delta})\},
\end{align*}
$\|\hat \bM - \bM\| \le \epsilon\sigma^2$ with probability at least $1-\delta$.
\end{theorem}
%In essense, this shows that subspace $\M$ can be estimated with $O(kd) samples$
\iffalse
Theorem \ref{thm:hatM} proposes an upper bound for the estimation error of $\bM$. The subspace spanned by $\hat \bM$ is used for few-shot learning. In the context of binary classification, we will show how this error affects the cross entropy loss for the few-shot learning stage. 
\fi
%Downstream task

Recall that $\hat \bM=\hat \Ub \hat\La \hat\Ub^\top$ and $\hat \Ub_r$ is the first $r$ columns of $\hat \Ub$. Denote the estimate of $\W$ via $\hat \W$ given by adjusting $\hat\Ub_r$
\begin{align}
    \hat \W &= (\hat \Ub_r \hat \Qb)^\top,\
    \hat \Qb = \mathop{\mathrm{argmin}}_{\Qb\in\R^{r\times r}, \Qb\Qb^\top = I}\ \|\hat \Ub_r \Qb - \W^\top\|\label{eq:def W}
\end{align}
With the definition of $\hat\W$, $\|\hat \W - \W\|$ defines a distance between the row space of $\W$ and the column space of $\hat \Ub_r$. If the span of the two subspaces are the same, then there exists an orthonormal matrix $\Qb$ such that $\hat \Ub_r \Qb = \W^\top$.

The previous lemma builds upon the assumption that $\|\hat \W - \W\|$ is small. 
%We quote the following lemma first. 
In Theorem \ref{thm:hatM}, we have got $\|\hat \bM - \bM\| \le \epsilon\sigma^2$, then with the extra assumption that $\bM$ is rank $r$, we have the following result from \cite{davis1970rotation}.
\begin{lemma}
If $\|\hat \bM - \bM\| \le \epsilon\sigma^2$, $\lambda_r(\bM) > \epsilon\sigma^2$, then \[\|\hat \W - \W\| \le \epsilon\sigma^2(\lambda_r(\bM) -\epsilon\sigma^2)^{-1}.
%\le \frac{\|\hat \bM - \bM\|}{\lambda_r(\bM) - \|\hat \bM - \bM\|} \le \frac{\epsilon\sigma^2}{\lambda_r(\bM) -\epsilon\sigma^2}.
\]
\end{lemma}



% I think it's better to keep this as \Qb is used in assumption 1 of \Fc

%Another definition of the distance between two subspaces is the difference of projection, defined as 
%\begin{align*}
%    \|\hat \Ub_r\hat \Ub_r^\top - \W^\top\W\|
%\end{align*}
%Note that, with \eqref{eq:def W}, if 

\iffalse
{\color{red} can remove the text, just to keep the assumption on $\Fc$}
Now we use $\hat\Ub_r$ for the downstream task, and we study the population loss of training caused by the error of the estimator $\hat \bM$. We consider the binary classification case, where the data in the new task is generated as Def. \ref{def:bin_class}, with the non-linear function being $f$ and the true subspace being $\W$. The loss we consider, is cross-entropy loss, which is defined as \eqref{eq:cLCE}.
%\begin{align*}
%    &\cLCE(f;\Pb) : \Fc\times \R^{r\times d}\rightarrow \R=\\
%    &-\mtx{E}_{\x,y\sim\Pxy} (y\log f(\hat\Pb \x) + (1-y)\log (1 - f(\hat\Pb \x))) 
%\end{align*}

To train on the data, we need to find the optimal function $f$ that minimizes the population loss. Define the search space of $f$ as $\Fc$. For binary classification, we assume that, 
\begin{enumerate}
    \item For any function $f\in\Fc$, any orthonormal matrix $\Qb\in\R^{r\times r}$ and any matrix $\Pb\in\R^{r\times d}$, there exists $g \in \Fc$ such that $f(\Pb \x) = g(\Qb\Pb \x)$.
    \item $\Fc \subseteq \{f\ |\ \log f,~ \log(1-f)\mathrm{~are~}L\mathrm{~Lipschitz}\}\bigcap \{f\ |\ 0<f(x)<1,\forall x\in\R^r\}$.
\end{enumerate}
We can see that, if we adopt the logistic regression for binary classification example in \eqref{eq:Fcbin}, then both assumptions are true with $L = a$.  

We learn the model from the optimization algorithm \eqref{eq:fstar} (also works for logistic regression in \eqref{eq:fstarbin}). Now we will bound the cross-entropy loss of this model.
\fi

%\so{There is a serious issue here. It seems, we never stated a bound on $\hat{\W}-\W$, we only prove a bound on $\hat{M}-\M$. Thm 3.2 should ideally state bound for the subspace as well. This bound should be in terms of the spectrum of $\M$ i.e. its $r$'th largest singular (e.g.~via davis-kahan thm). If you look at the few-shot learning results, they are in terms of $\|\hat{\W}-\W\|$. This is fine but we should also add an end-to-end learning result where $\|\hat{\W}-\W\|$ is bounded in terms of meta-training sample size. This should be addressed before arXiv submission.}
\subsection{Results on Few-shot Learning}
\vspace{-0.1cm}
In the next step, we will use $\hat\Ub_r$ for few shot learning and find $\hat f$ that minimize the population loss. 
%Recall that the search space for $\hat f$ is $\Fc$. For binary classification, we assume 
%\begin{enumerate}
%Only row-space (representation) matters
%    \item \textbf{Rotation invariance:} For any function $f\in\Fc$, any orthonormal matrix $\Qb\in\R^{r\times r}$ and any matrix $\Pb\in\R^{r\times d}$, there exists $g \in \Fc$ such that $f(\Pb \x) = g(\Qb\Pb \x)$.
%    \item \textbf{Lipschitz:} $\Fc \subseteq \{f\ |\ \log f,~ \log(1-f)\mathrm{~are~}L\mathrm{~Lipschitz}\}$ $~\bigcap~ \{f\ |\ 0<f(x)<1,\forall x\in\R^r\}$.
%\end{enumerate}

\begin{theorem}\label{thm:down}
    Let Assumptions \ref{ass:F} and \ref{ass:L} hold. Let $\hat\W$ be the same as in \eqref{eq:def W} and $\hat f$ be the same as in \eqref{eq:fstar}. Then we have 
    \begin{align*}
        \cLCE(\hat f;\hat \Ub_r^\top) - \cLCE(f^*;\W)\lesssim L\sqrt{r}\|\hat \W - \W\|.
    \end{align*}
\end{theorem}
$\cLCE (f^*;\W)$ assumes the knowledge of the true function $f^*$ and the representation $\W$. This shows that the inaccuracy of the moment estimator $\hat M$ costs us $O(L\sqrt{r}\|\hat \W - \W\|)$. 

Theorem \ref{thm:down} bounds the population risk of $\hat f$, when we use $\hat\Ub_r^\top$ as the representation subspace. Next we discuss the population risk of the finite sample solution $\hat f_e$, which should be worse than $\hat f$ due to the limited samples.
%deviating from true data distribution of the new task. Theorem \ref{thm:rade} bounds the risk in terms of the sample size $n$.

\iffalse
For a concrete example, we apply the logistic regression model for \eqref{eq:cLCE finite}, where $f(\vb) = \phi(\bt^\top\vb)$, $\vb \in \R^r$ and $\phi$ is logistic function. Let the ground truth parameter for generating few-shot learning data be $\bt^*$ and we assume $\|\bt^*\| \le a$. In few-shot learning, we train by solving for $\hat \bt_e$ in the set $\{\bt\ |\ \|\bt\| \le a\}$. The objective is {\color{red} can move this to def 2.6}
\begin{align}
    &\cL_e(\bt;\Pb) : \Fc\times \R^{r\times d}\rightarrow \R= \notag\\
    &-\frac{1}{n}\sum_{i=1}^n (y_i\phi (\bt^\top\Pb \x_i) + (1-y_i)\log (1 - \phi(\bt^\top\Pb \x_i))) \label{eq:cLCE finite theta}
\end{align}
The empirical minimizer is defined by
\begin{align}
    \hat \bt_e &= \argmin_{\bt}\ \cL_e(\bt;\Ub_r^\top),\mbox{~such~that~} \|\bt\|\le a.\label{eq:fstar finite theta}
\end{align}
\fi
\begin{theorem}\label{thm:rade}
    Consider the setup in Def.~\ref{def: test finite} with $n$ i.i.d.~examples with ground-truth model $\bt^*$. Solve for $\hat \bt_e$ via \eqref{eq:fstar finite theta}. There exist constants $c>1$, $\delta\in(0,1)$, with probability at least $1 - n^{-c+1} - \delta$, the solution pair $(\hat\bt_e,\hat\Ub_r)$ satisfies
    \begin{align*}
        \quad \mathcal{L}(&\hat\bt_e;\hat\Ub_r^\top) - \mathcal{L} (\bt^*;\W) \\
        &\leq \frac{caL(\sqrt{r}+\log(n)) (1+ \sqrt{\log(1/\delta)})}{\sqrt{n}} + L\sqrt{r}\|\hat \W - \W\|. 
    \end{align*}
\end{theorem}
Note that the first term grows as $\sqrt{r/n}$. This means the amount of data $n$ we request for few-shot learning is $n\approx r$,  as compared to $n\approx d$ if representation learning is not excecuted. 
%If we do not run representation learning before few-shot learning, the error would instead be proportional to $\sqrt{d/n}$ where $d$ is the ambient dimension and we would need $n\approx d$ examples to learn the new task.
% {\color{red} YS:  No math justification for $n\ge d$ here since I only have upper bound but no lower bound, so it's just an intuition}
%In \eqref{eq:fstar}, we solve for the minimizer of population loss function. Now we will study the finite sample case. In few-shot learning phase, suppose we have the dataset $(\x_i, y_i)$, $i=1,...,n$ and the data is generated as Def. \ref{def: test}. Now we consider the 

==> Icassp (3)/s_main_nn.tex <==
\begin{lemma}\label{lem:mean nn}
We assume that the data are generated as in Defs. \ref{def:task dis} to \ref{def:data_gen} and Def. \ref{def:nn}, and we study the $j$-th task whose feature matrix is $\Theta^j$. 
%{\color{blue} To be finished}
Define
\begin{align*}
    \mtx{h}(\Theta): \R^{r\times d} \rightarrow \R^r = \mtx{E}_{\x\sim\Px} f(\Theta \x)  \x
\end{align*}
Then $\mtx{E}_{(\x,y)\sim\Pxy}(y \x) = (\Theta^j)^\top(\Theta^j(\Theta^j)^\top)^{-1}\Theta^j\mtx{h}(\Theta^j)$, and $\|y\x\|\le 1$ with probability $1$.
%{\color{blue} To be finished}
\end{lemma}

\noindent\textbf{Proof of Lemma \ref{lem:mean nn}} The boundedness is trivial and we study the expectation.
Denote
\begin{align*}
    \tilde \Theta^j = (\Theta^j)^\top (\Theta^j(\Theta^j)^\top)^{-1}\Theta^j
\end{align*}

We first write the expectation as
\begin{align*}
    &\mtx{E}_{(\x,y)\sim\Pxy}(y \x) \\
    &= \mtx{E}_{\x} f(\Theta^j \x) \x\\
    &= \mtx{E}_{\x\sim\Px} \left(f(\Theta^j \x)  \tilde \Theta^j \x + f(\Theta^j \x) (\x -  \tilde \Theta^j\x) \right).
\end{align*}
Now we prove that 
\begin{align*}
    \mtx{E}_{\x\sim\Px}f(\Theta^j \x) (\x -  \tilde \Theta^j\x) =0
\end{align*}
Denote 
\begin{align*}
    \bar \x &= \tilde \Theta^j\x - (\x -  \tilde \Theta^j\x)\\
    &= 2\tilde \Theta^j\x - \x.
\end{align*}
Then it is easy to see
\begin{align}
    \Theta^j \x  &= \Theta^j \bar \x,\label{eq:easy1 nn} \\
    \x -  \tilde \Theta^j\x &= - \left(\bar \x -  \tilde \Theta^j\bar \x\right),\label{eq:easy2 nn}\\
    \x &=2\tilde \Theta^j\bar \x - \bar \x.
\end{align}


Now we consider the density function of $\bar x$. Let the density of $\x$ be $p_{\x}$, which is uniform on the unit sphere, we have that 
{\color{blue} Need a better notation!}
\begin{align}
    p_{\bar \x} (\bar \x) &= p_{\x}(2\tilde \Theta^j\bar \x - \bar \x) \big|\nabla_{\bar \x} (2\tilde \Theta^j\bar \x - \bar \x \big| \label{eq:den2 nn}\\
    &= p_{\x}(\x) \big|\mathrm{det}(2\tilde \Theta^j - I) \big|\label{eq:den3}\\
    &= p_{\x}(\x).
\end{align}
Here \eqref{eq:den2} uses the fact that the density function $p_{\x}$ is uniform (thus is a constant everywhere), and \eqref{eq:den3} uses that the eigenvalues of $\frac{2\theta^j(\theta^j)^\top}{\|\theta^j\|^2} - I$ only consists of $\pm 1$. Now we can see that the distributions of $\x$ and $\bar \x$ are the same.

So we have that
\begin{align}
    &\quad \mtx{E}_{\x\sim\Px}f(\Theta^j\bar \x) (\bar \x - \tilde \Theta^j\bar \x)\notag\\
    &= \mtx{E}_{\x\sim\Px}f(\Theta^j \x) \left(- (\x -  \tilde \Theta^j\x)\right)\notag\\
    &= - \mtx{E}_{\x\sim\Px}f(\Theta^j \x) (\x -  \tilde \Theta^j\x).\label{eq:mns nn}
\end{align}
which uses \eqref{eq:easy1 nn}, \eqref{eq:easy2 nn}. Since the distributions of $\x$ and $\bar \x$ are the same, we compute via a simple change of variable
\begin{align}
    &\quad \mtx{E}_{\x\sim\Px}f(\Theta^j\bar \x) (\bar \x - \tilde \Theta^j\bar \x) \notag\\
    &= \mtx{E}_{\bar \x\sim\Px}f(\Theta^j\bar \x) (\bar \x - \tilde \Theta^j\bar \x)\notag\\
    &= \mtx{E}_{\x\sim\Px}f(\Theta^j \x) (\x -  \tilde \Theta^j\x).\label{eq:pls nn}
\end{align}

Comparing \eqref{eq:mns nn} and \eqref{eq:pls nn}, we have 
\begin{align*}
    &\quad \mtx{E}_{\x\sim\Px}f(\Theta^j \x) (\x -  \tilde \Theta^j\x)\\
    &= -\mtx{E}_{\x\sim\Px}f(\Theta^j \x) (\x -  \tilde \Theta^j\x)
\end{align*}
so $\mtx{E}_{\x\sim\Px}f(\Theta^j \x) (\x -  \tilde \Theta^j\x)=0$.

Going back to Lemma \ref{lem:mean nn}, we have 
\begin{align*}
    \mtx{E}_{(\x,y)\sim\Pxy}(y \x)
    &= \mtx{E}_{\x\sim\Px} f(\Theta^j \x)  \tilde \Theta^j \x
    \\&= \mtx{E}_{\x\sim\Px} f(\Theta^j \x)  (\Theta^j)^\top (\Theta^j(\Theta^j)^\top)^{-1}\Theta^j \x.
\end{align*}
%\Theta^j

{\color{blue} From here I'll prove using the fact that $y\x$ is subGaussian with $\|\mathbf{Cov}(y\x)\| \le \sigma^2$.}

First we study the concentration of data within the $j$-th class. 
\begin{lemma}
Let $\delta\in(0,1)$, with probability $1-\delta$, there exists a constant $c$ such that
\begin{align*}
    \|\frac{1}{t}\sum_{i=1}^t \yij\xij - \theta^j\| \le c\sigma\sqrt{\frac{d}{t}\log(\frac{kd}{\delta})} 
\end{align*}
for all $j=1,...,k$. 
\end{lemma}
\begin{lemma}
For all $\vb$ such that $\|\vb\| = 1$, there exists a constant $c$ such that
\begin{align*}
    \Eb\left( (\vb^T\cdot (\frac{1}{t}\sum_{i=1}^t \yij\xij - \theta^j))^2\right) \le c\sigma^2 / t. 
\end{align*}
\end{lemma}
\begin{lemma}
There exists a constant $c$ such that \begin{align*}
    \Eb \left(\|\frac{1}{t}\sum_{i=1}^t \yij\xij - \theta^j \|^2\right) \le c\sigma^2d/t. 
\end{align*}
\end{lemma}
\begin{lemma}
Define
\begin{align*}
    \Zb_j = (\frac{1}{t}\sum_{i=1}^t \yij\xij)(\frac{1}{t}\sum_{i=t+1}^{2t} \yij\xij)^\top - \theta^j(\theta^j)^\top,
\end{align*}
Then there exists a constant $c$ such that with probability $1-\delta$, for all $j=1,...,k$, 
\begin{align}
    \|\Zb_j \| \le \frac{c\sigma^2d}{t} \log(\frac{kd}{\delta}). \label{eq:evt}
\end{align}
\end{lemma}

\begin{lemma}
There exists a constant $c$ such that
\begin{align*}
   \|\Eb\sum_{j=1}^k\Zb_j\Zb_j^\top\| \le c\sigma^4dk/t
\end{align*}
\end{lemma}
\begin{lemma}
Let $\delta\in(0,1)$. There exists a constant $c$, such that for any $\epsilon\in(0,1)$, and 
\begin{align}
    k = \frac{cd}{t}\log^2(\frac{kd}{\delta}) \max\{\frac{1}{\epsilon^2}, \frac{1}{\epsilon} \log(\frac{kd}{\delta})\}, \label{eq:k lb}
\end{align}
with probability $1-\delta$, 
\begin{align*}
    \|\frac{1}{k} \sum_{j=1}^k \Zb_j\| \le \epsilon \sigma^2.
\end{align*}
\end{lemma}
This means that when \eqref{eq:k lb}, with probability $1-\delta$,
\begin{align*}
    \left\|\hat \bM - \frac{1}{k}\sum_{j=1}^k\left(\tilde \Theta^j \mtx{h}(\Theta^j)\mtx{h}^\top(\Theta^j)\tilde \Theta^j\right)\right\| \le \epsilon \sigma^2.
\end{align*}


==> Icassp (3)/s_main_proof.tex <==
\section{Proof of main theorems}
\SO{Clearly Theorem \ref{thm:hatM append} is a restatement of Theorem \ref{thm:hatM}. Why don't you say so? Reader is not expected to figure out this by himself. Let us make things clear.}

\SO{Similarly, where is proof of Lemma 3.1? Looks like Lemma \ref{lem:mean nn} is its restatement but again not clear at all for reader. They cannot find proof of Lemma 3.1 in the text.}

\SO{Here is the organization we need: In the appendix, proof of each technical result in the main text is supposed to have its own subsection. Just like this subsection that I added i.e.~Proof of Theorem \ref{thm:hatM}.}
\SO{Maybe briefly describe the outline. Right now, little confusing due to Lemmas within the proof so outline would help i.e.~we first prove Lemma ... which shows ...}
\subsection{Proof of Lemma \ref{lem:M exp} and Theorem \ref{thm:hatM}}
We sketch the proof at the beginning. First we compute the expectation of $y\x$ in Lemma \ref{lem:mean nn}. That leads to the proof of Lemma \ref{lem:M exp}. Then in Lemma \ref{lem:err_yx} we bound the difference between sum of $y\x$ and its mean using concentration. The concentration of covariance estimator is studied later in Lemma \ref{lem:Zj} and \ref{lem:Zj2}, which leads to Theorem \ref{thm:hatM}.

\subsubsection{Proof of Lemma \ref{lem:M exp}}
We first state Lemma \ref{lem:M exp} below.
\begin{lemma}\label{lem:M exp append}
Let 
\begin{subequations}\label{eq:hatM append}
\begin{align}
\hat\bM &= \mathop{\Scale[1.8]{\sum}}_{j=1}^k \frac{2}{n_j^2}\left[(\sum_{i=1}^{n_j/2} \yij\xij) (\sum_{i=n_j/2+1}^{n_j} \yij\xij)^\top \right.\\
&\quad\quad\quad\quad \left. +  ( \sum_{i=n_j/2+1}^{n_j} \yij\xij) ( \sum_{i=1}^{n_j/2} \yij\xij)^\top\right].\nonumber
\end{align}
\end{subequations}
And
\begin{align*}
    &\mtx{h}^j(\W): \R^{r\times d} \rightarrow \R^d = \mtx{E}_{\x}[f^j(\W \x)\x]\\
    &\bM := \W^\top\W\left(\frac{1}{k}\sum_{j=1}^k \mtx{h}^j(\W)( \mtx{h}^j(\W))^\top\right)\W^\top\W.
\end{align*}
Then $\bM,\hat{\bM}$ satisfies the following. (a) $\text{rank}(\bM)\leq r$. (b) $\text{range-space}(\bM)\subset \text{row-space}(\W)$. (c) $\mtx{E}[\hat{\M}]=\bM$. 
\end{lemma}
\begin{proof}
Part (a) and (b) are easy to see. $\W\in\R^{r\times d}$ so that $\text{rank}(\bM)\leq r$, and since $\bM$ is the product of $\W^\top$ and another matrix, then  $\text{range-space}(\bM)\subset \text{row-space}(\W)$.
Now we will prove Part (c). We first give the lemma for the mean of the random vector $y\x$.

\begin{lemma}\label{lem:mean nn}
We assume that the data is generated as in Def. \ref{def:task}, and we study the $j$-th task whose activation function is $f^j$. 
%{\color{blue} To be finished}
Define
\begin{align*}
    \mtx{h}^j(\W): \R^{r\times d} \rightarrow \R^d = \mtx{E}_{\x\sim\gauss} f^j(\W \x)  \x
\end{align*}
Denote the joint distribution of $(\x,y)$ as $\Pxy$.
Then $\mtx{E}_{(\x,y)\sim\Pxy}(y \x) = \W^\top\W \mtx{h}^j(\W)$.
\end{lemma}

\emph{Proof of Lemma \ref{lem:mean nn}.} The expectation can be expanded as
\begin{align*}
    &\mtx{E}_{(\x,y)\sim\Pxy}(y \x) \\
    &= \mtx{E}_{\x\sim\gauss} f^j(\W \x) \x\\
    &= \mtx{E}_{\x\sim\gauss} \left(f^j(\W \x)  \W^\top\W \x + f^j(\W \x) (I - \W^\top\W)\x \right).
\end{align*}
Note that, because $\x\sim\gauss$ so $\W \x$ and $(I - \W^\top\W)\x$ are Gaussian. $\W\W^\top = I$ implies 
\begin{align*}
    &\quad \Eb (\W \x)\x^\top((I - \W^\top\W))\\
    &= \W(I - \W^\top\W) = 0.
\end{align*}
So $\W \x$ and $(I - \W^\top\W)\x$ are independent, so 
\begin{align*}
    &\quad \mtx{E}_{\x\sim\gauss}  f^j(\W \x) (I - \W^\top\W)\x \\
    &= (\mtx{E}_{\x\sim\gauss}  f^j(\W \x)) (\mtx{E}_{\x\sim\gauss} (I - \W^\top\W)\x) = 0
\end{align*}
Then 
\begin{align*}
    \mtx{E}_{(\x,y)\sim\Pxy}(y \x) &= \W^\top\W(\mtx{E}_{\x\sim\gauss} f^j(\W \x) \x)\\
    &= \W^\top\W \h_j(\W).
\end{align*}

Denote 
\begin{align}\label{eq:Hj def}
    \Hb^j(\W) = \W^\top\W \mtx{h}^j(\W)
\end{align}
Because $\frac{2}{n_j}\sum_{i=1}^{n_j/2} \yij\xij$
and 
$\frac{2}{n_j}\sum_{i={n_j/2}+1}^{n_j} \yij\xij$ 
are independent, and their expectation are both $\Hb^j(\W)$, so that
\begin{align*}
    &\quad \mtx{E}(\frac{2}{n_j}\sum_{i=1}^{n_j/2} \yij\xij)(\frac{2}{n_j}\sum_{i={n_j/2}+1}^{n_j} \yij\xij)^\top \\
    &= \Hb^j(\W)(\Hb^j(\W))^\top.
\end{align*}
At then end
\begin{align*}
    \hat \bM &= \frac{1}{k}\sum_{j=1}^k \mtx{E}(\frac{2}{n_j}\sum_{i=1}^{n_j/2} \yij\xij)(\frac{2}{n_j}\sum_{i={n_j/2}+1}^{n_j} \yij\xij)^\top,\\
    \bM &= \frac{1}{k}\sum_{j=1}^k\Hb^j(\W)(\Hb^j(\W))^\top,
\end{align*}
so we can prove Part (c) that $\mtx{E}(\hat \bM) = \bM$.
\end{proof}


\subsubsection{Proof of Theorem \ref{thm:hatM}}
We restate Theorem \ref{thm:hatM append} below. 
\begin{theorem}\label{thm:hatM append}
Suppose the data is generated as Def. \ref{def:task}. Let $\delta\in(0,1)$, $\epsilon\in(0,1)$. Suppose $y\x$ is a subGaussian random vector with covariance upper bounded by
\begin{align}
   \| \mathbf{Cov}(y \x) \| \le \sigma^2. \label{eq:covyx append}
\end{align} 
Define
\begin{align*}
    \mtx{h}^j(\W): \R^{r\times d} \rightarrow \R^d = \mtx{E}_{\x\sim\gauss} f^j(\W \x)  \x
\end{align*}
And let %$\bM = \mtx{E}_{\theta\sim\mathcal{N}(0,\bSi)} (g(\theta))^2\frac{\theta\theta^\top}{\|\theta\|^2}$, then
\begin{align*}
    \bM = \W^\top\W\left(\frac{1}{k}\sum_{j=1}^k \mtx{h}^j(\W)( \mtx{h}^j(\W))^\top\right)\W^\top\W
\end{align*}
Then there exists a constant $c$, with probability at least $1-\delta$, let 
\begin{align*}
    k = \frac{cd}{n}\log^2(\frac{kd}{\delta}) \max\{\frac{1}{\epsilon^2}, \frac{1}{\epsilon} \log(\frac{kd}{\delta})\}
\end{align*}
we have 
\begin{align*}
    \|\hat \bM - \bM\| \le \epsilon\sigma^2.
\end{align*}
\end{theorem}
\begin{proof}
The following lemmas are similar to \cite{kong2020meta} Section A.1. We extend the concentration inequalities from bounded random vectors to Gaussian random vectors. For completeness we place the lemmas here.

\begin{lemma}\label{lem:err_yx}
(\cite{jin2019short} Cor. 7) 
Let $\|\mathbf{Cov}(y\x)\| \le \sigma^2$, $\delta\in(0,1)$, $t>0$, $\Hb^j(\W)$ be defined in \eqref{eq:Hj def}. With probability $1-\delta$, there exists a constant $c>0$ such that for every $j$,
\som{Remind the exact assumption on $\sigma$}
\begin{align}
   \|\frac{1}{t}\sum_{i=1}^t \yij\xij - \Hb^j(\W)\| \le c\sigma\sqrt{\frac{d}{t}\log(\frac{kd}{\delta})} \label{eq:gauss_bern}
\end{align}
\som{Call $\W^\top\W \mtx{h}^j(\W)$ something for simpler notation}
Denote this event as $\mathcal{E}$.
\iffalse
{\it\color{red} for every i,j pairs ? }Denote this event as $\mathcal{E}$.
{\it \color{red} if we dont say "for every i,j pairs" ,k should not appear in an inequality which holds for only one task. Also maybe it is better to  cite [21] A.5, because [28] Cor.7 says only the following
$$\|\frac{1}{t}\sum_{i=1}^t \yij\xij - \W^\top\W \mtx{h}^j(\W)\| \le c\sigma\sqrt{\frac{1}{t}\log(\frac{2d}{\delta})}$$}
\fi
\end{lemma}
With the covariance of $y\x$ being bounded by $\sigma^2$, the following inequalities are true \cite{kong2020meta}.
\begin{align*}
    \Eb\left( (\vb^T\cdot (\frac{1}{t}\sum_{i=1}^t \yij\xij - \theta^j))^2\right) &\le \sigma^2 / t,\mbox{~for~} \|\vb\|=1.\\
    \Eb \left(\|\frac{1}{t}\sum_{i=1}^t \yij\xij - \theta^j \|^2\right) &\le \sigma^2d/t.
\end{align*}


\begin{lemma}\label{lem:Zj}
Define
\begin{align*}
    \Zb_j &= (\frac{2}{n_j}\sum_{i=1}^{n_j/2} \yij\xij)(\frac{2}{n_j}\sum_{i={n_j/2}+1}^{n_j} \yij\xij)^\top \\
    &\quad - \Hb^j(\W)(\Hb^j(\W))^\top,
\end{align*}
Then there exists a constant $c$ such that on the event $\mathcal{E}$ (thus with probability $1-\delta$), for all $j=1,...,k$, 
\begin{align}
    \|\Zb_j \| \le \frac{c\sigma^2d}{n_j} \log(\frac{kd}{\delta}). \label{eq:evt}
\end{align}
\end{lemma}

% {\it \color{red} From my understanding we should have 
% $$\|\Zb_j \| \le (Eq A.1 Bound)(Eq. A.1 bound + 2\|\W^\top\W \mtx{h}^j(\W)\|)$$ choosing $t=\dfrac{n_j}{2}$ then we have $$\|\Zb_j \| \le (c\sigma\sqrt{\frac{2}{n_j}\log(\frac{2d}{\delta})})(c\sigma\sqrt{\frac{2}{n_j}\log(\frac{2d}{\delta})} + 2\|\W^\top\W \mtx{h}^j(\W)\|)$$
% This is more or less what you have found, but the difference is k in $\log$ term and d term }



The proof is almost same as \cite{kong2020meta}, the only difference is that we replace the bound in (\cite{kong2020meta} Prop A.1) by \eqref{eq:gauss_bern}. With the similar replacement, we propose the following lemma. 
\begin{lemma}\label{lem:Zj2}
Let $\delta\in(0,1)$. There exists a constant $c$, such that for any $\epsilon\in(0,1)$, and 
\begin{align}
    k = \frac{cd}{n_j}\log^2(\frac{kd}{\delta}) \max\{\frac{1}{\epsilon^2}, \frac{1}{\epsilon} \log(\frac{kd}{\delta})\}, \label{eq:k lb}
\end{align}
with probability $1-\delta$, 
\begin{align*}
    \|\frac{1}{k} \sum_{j=1}^k \Zb_j\| \le \epsilon \sigma^2.
\end{align*}
\end{lemma}
This means that when \eqref{eq:k lb} is true, with probability $1-\delta$,
\begin{align*}
    \left\|\hat \bM - \W^\top\W\left(\frac{1}{k}\sum_{j=1}^k \mtx{h}^j(\W)( \mtx{h}^j(\W))^\top\right)\W^\top\W\right\| \le \epsilon \sigma^2.
\end{align*}
Note that $\bM$ is defined as \[\bM=\W^\top\W\left(\frac{1}{k}\sum_{j=1}^k \mtx{h}^j(\W)( \mtx{h}^j(\W))^\top\right)\W^\top\W.\] So we have proven that with probability $1-\delta$,
\begin{align*}
    \left\|\hat \bM - \bM\right\| \le \epsilon \sigma^2.
\end{align*}

\som{Remind that this is $\hat \bM-\bM$ i.e. $\bM=\text{the messy sum}$}
\end{proof}

\SO{Create a subsection here!!! Reduce the confusion as much as possible, make transitions smooth.}
\subsection{Proof of Theorem \ref{thm:down}}
Now we will prove Theorem \ref{thm:down}. We first review the notations and assumptions mentioned in the theorem.

\subsubsection{Review of Notations and Assumptions}
We define the SVD of $\hat \bM$ as $\hat \Ub \hat\La \hat\Vb^\top$. Let the first $r$ columns of $\hat \Ub$ be $\Ub_r$. 

Let $\hat\W$ be defined as 
\begin{align}
    \hat \W &= \hat \Ub_r \hat \Qb, \label{eq:def W append}\\
    \hat \Qb &= \mathop{\mathrm{argmin}}_{\Qb\in\R^{r\times r}, \Qb\Qb^\top = I}\ \|\hat \Ub_r \Qb - \W\|.
\end{align}
The population cross entropy loss is defined as
\begin{align*}
    &\cLCE(f;\Pb) : \Fc\times \R^{r\times d}\rightarrow \R=\\
    &-\mtx{E}_{\x,y\sim\Pxy} (y\log f(\hat\Pb \x) + (1-y)\log (1 - f(\hat\Pb \x))).
\end{align*}
We will search for a function $f^* \in \Fc$ that minimizes the population cross entropy loss. $\Fc$ is a set of functions satisfying
\begin{enumerate}
    \item For any function $f\in\Fc$, any orthonormal matrix $\Qb\in\R^{r\times r}$ and any matrix $\Pb\in\R^{r\times d}$, there exists $g \in \Fc$ such that $f(\Pb \x) = g(\Qb\Pb \x)$.
    \item $\Fc \subseteq \{f\ |\ \log f,~ \log(1-f)\mathrm{~are~}L\mathrm{~Lipschitz}\}\bigcap \{f\ |\ 0<f(x)<1,\forall x\in\R^r\}$.
\end{enumerate}
We solve for $\hat f$, defined as \begin{align}
    \hat f &= \argmin_{f\in\Fc}\ \cLCE(f;\hat \Ub_r^\top). \label{eq:def f append}
\end{align}
\subsubsection{Proof of Theorem \ref{thm:down}}
Now we are ready to restate Theorem \ref{thm:down} and prove it.
\begin{theorem}\label{thm:popu append}
Based on the definition above, we have that
    \begin{align*}
        \cLCE(\hat f;\hat \Ub_r^\top)  - \cLCE(f^*;\Ub_r^\top) \lesssim L\sqrt{r}\|\hat \W - \W\|.
    \end{align*}
\end{theorem}

\begin{proof}
We learn the model from the following optimization algorithm.
\begin{align*}
    \hat f &= \argmin_{f\in\Fc}\ \cLCE(f;\hat \Ub_r^\top)\\
    &= \argmin_{f\in\Fc}\ -\mtx{E}_{\x,y\sim\Pxy} (y\log f(\hat\Ub_r^\top \x) \\
    &\quad + (1-y)\log (1 - f(\hat\Ub_r^\top \x)))\\
    &= \argmin_{f\in\Fc}\ -\mtx{E}_{\x\sim\gauss} \left(f^*(\W \x)\log f(\hat \Ub_r^\top \x)\right. \\
    & \quad \left. + (1-f^*(\W \x))\log (1 - f(\hat \Ub_r^\top \x)) \right).
\end{align*}
Denote $\tilde f\in\Fc$ as the function such that $\tilde f(\hat \W \x) = \hat f(\hat \Ub_r^\top \x)$. So that $\cLCE(\hat f;\hat \Ub_r^\top) = \cLCE(\tilde f;\hat \W)$. Since $\hat f$ minimizes the cross entropy loss, we have that $\cLCE(\tilde f;\hat \W) \le \cLCE(f^*;\hat \W)$. 

Now we have 
\begin{align*}
    &\quad \cLCE (\tilde f;\hat \W) - \cLCE (f;\W)\\
    &\le \cLCE (f^*;\hat \W) - \cLCE (f^*;\W)\\
    &\le -\mtx{E}_{\x\sim\gauss} \left(f^*(\W \x)(\log f^*(\hat\W \x) -\log f^*(\W \x))\right. \\
    & \quad \left. + (1-f^*(\W \x))(\log (1 - f^*(\hat \W \x)) - \log (1 - f^*(\W \x))) \right)\\
    &\le \mtx{E}_{\x\sim\gauss} L\|(\hat \W - \W)x\|\\
    &\lesssim L\sqrt{r}\|\hat \W - \W\|.
\end{align*}
\end{proof}

\subsection{Proof of Theorem \ref{thm:rade}}
%Now we prove that the upper bound of the error for few-shot learning with finite samples.
We first state Theorem \ref{thm:rade} below.
\begin{theorem}\label{thm:rade app}
    Suppose we generate $n$ sample data for few shot learning solve for $\hat \theta_e$ from \eqref{eq:fstar finite theta}. There exist constants $c>0$, $\delta\in(0,1)$, with probability at least $1 - n^{-c+1} - \delta$, the solution $\hat\theta_e$ and $\hat\Ub_r$ satisfy
    \begin{align*}
        &\quad \mathcal{L} (\hat\theta_e;\hat\Ub_r^\top) - \mathcal{L} (\theta^*;\W) \\
        &\lesssim \frac{ac(\sqrt{r}+\log(n)) (1+ \sqrt{\log(1/\delta)})}{\sqrt{n}} + \sqrt{r}\|\hat \W - \W\|. 
    \end{align*}
\end{theorem}
\begin{proof}
We sketch the proof of Theorem \ref{thm:rade app}. After reviewing the notations, we quote a standard generalization bound via Rademacher complexity in Lemma \ref{lem:rade known}. Then we use the smoothness of the loss function to link to the generalization error of linear functions \eqref{eq:lin rade}, and then use Lemma \ref{lemma:chi-sqr} to compute \eqref{eq:lin rade} and finish the proof.

In few-shot learning, the true parameter is $\theta^*$, and the empirical loss function with finite data is 
\begin{align}
    &\cL_e(\theta;\Pb) : \Fc\times \R^{r\times d}\rightarrow \R= \notag\\
    &-\frac{1}{n}\sum_{i=1}^n (y_i\log\phi (\theta^\top\Pb \x_i) + (1-y_i)\log (1 - \phi(\theta^\top\Pb \x_i))) \label{eq:cLCE finite theta app}
\end{align}
Denote each term in the summation as 
\begin{align*}
    &\quad \cL_e^i(\theta;\Pb) : \Fc\times \R^{r\times d}\rightarrow \R=\notag\\
    &- (y_i\log \phi (\theta^\top\Pb \x_i) + (1-y_i)\log (1 - \phi(\theta^\top\Pb \x_i)))
\end{align*}
We search for the solution by
\begin{align}
    \hat \theta_e &= \argmin_{\theta}\ \cL_e(\theta;\Ub_r^\top),\mbox{~such~that~} \|\theta\|\le a.\label{eq:fstar finite theta app}
\end{align}
In Theorem \ref{thm:popu append}, we know that
\begin{align*}
    \cLCE(\hat \theta;\hat \Ub_r^\top)  - \cLCE(\theta^*;\Ub_r^\top) \lesssim L\sqrt{r}\|\hat \W - \W\|.
\end{align*}
Denote 
    \begin{align}
        M = \max_{\|\theta\|\le a} |\theta^\top \hat\Ub_r^\top\x_i| \le a \max\|\hat\Ub_r^\top\x_i\|.\label{eq:bound_rade}
    \end{align}
We will bound the difference between $\cL$ and $\cL_e$ by Rademacher complexity theory.
\begin{lemma}\label{lem:rade known}
    \cite{mohri2018foundations}
 
    Let $\mscrU$ be the independent random variables uniformly chosen from $\{-1,1\}$.
    Let $\Rc$ be the Rademacher complexity of the logistic functionals defined on the data,
    \begin{align*}
        \Rc &= \frac{1}{n}\Eb_{\epsilon_i\in\mscrU} \sup_{\|\theta\|\le a} \sum_{i=1}^n\epsilon_i\cL_e^i(\theta;\hat\Ub_r^\top) \\
        K &= |\log(\phi(-M))|>\max_i\cL_e^i(\theta;\hat\Ub_r^\top)
    \end{align*}
    %We know $\cL_e^i(\theta;\hat\Ub_r^\top)<K$ with probability at least $1-n^{-c_1+1}$,
    %then for any $\theta$ such that $\|\theta\|\le a$, with probability $1-\delta-n^{-c_1+1}$, we have that 
    with probability $1-\delta$, we have that 
    \begin{align*}
        |\cL_e(\theta;\Ub_r^\top) - \cL(\theta;\Ub_r^\top)| \le \Rc + \frac{\sqrt{\log(1/\delta)}}{\sqrt{n}}K.
    \end{align*}
\end{lemma}
Thus we have that 
\begin{align*}
    |\mathcal{L} (\hat\theta_e;\hat\Ub_r^\top) - \mathcal{L}_e (\hat\theta_e;\hat\Ub_r^\top)| &\le \Rc + \frac{\sqrt{\log(1/\delta)}}{\sqrt{n}}K,\\
    |\mathcal{L} (\hat\theta;\hat\Ub_r^\top) - \mathcal{L}_e (\hat\theta;\hat\Ub_r^\top)| &\le \Rc + \frac{\sqrt{\log(1/\delta)}}{\sqrt{n}}K.
\end{align*}
Because $\hat\theta_e$ minimizes the empirical loss $\mathcal{L}_e$,
\begin{align*}
    \mathcal{L}_e (\hat\theta_e;\hat\Ub_r^\top) \le \mathcal{L}_e (\hat\theta;\hat\Ub_r^\top).
\end{align*}
Thus 
\begin{align}
    \mathcal{L} (\hat\theta_e;\hat\Ub_r^\top) - \mathcal{L} (\hat\theta;\hat\Ub_r^\top) \le 2\left(\Rc + \frac{\sqrt{\log(1/\delta)}}{\sqrt{n}}K\right).\label{eq:emp loss}
\end{align}
So the remaining target is to bound $\Rc$. 

We first denote $\vb_i = \hat\Ub_r^\top \x_i$, so $\vb_i\in\R^r$ and $\vb_i$ are jointly independent standard normal random variables. In binary classification, $\cL_e^i$ is always $1$ Lipschitz in $\theta^\top\vb_i$, the Rademacher complexity can be upper bounded by
\begin{align}\label{eq:lin rade}
    \Rc \le \tilde\Rc := \frac{1}{n}\Eb_{\epsilon_i\in\mscrU} \sup_{\|\theta\|\le a} \sum_{i=1}^n \epsilon_i\theta^\top\vb_i. 
\end{align}
We first refer to the following lemma.
\begin{lemma}\label{lemma:chi-sqr}
    \cite{laurent2000adaptive} Let $c>0$, $X$ follow $\chi_r^2$ distribution, then
    \begin{align*}
        \Pb(X - r \ge 2\sqrt{cr\log n} + 2c\log n) \le n^{-c}.
    \end{align*}
\end{lemma}

For a constant $c>1$, via union bound we have that $\max{\|\vb_i\|^2} \le r + 2\sqrt{cr\log n} + 2c\log n$ for all $i=1,..,n$ with probability $1 - n^{-c+1}$. We use $\max{\|\vb_i\|} \lesssim c(\sqrt{r} + \log(n))$ for simplicity.

Conditioned on this event, we apply the Rademacher complexity for linear model that 
\begin{align}
   \tilde \Rc &\le \frac{\max\|\theta\| \cdot \max\|\vb_i\|}{\sqrt{n}}\\
   &\le \frac{ca(\sqrt{r} + \log(n))}{\sqrt{n}}. \label{eq:tilde Rc}
\end{align}
Combining with \eqref{eq:emp loss} and Theorem \ref{thm:popu append} we get the bound in Theorem \ref{thm:rade app}. We can also bound $M$ in \eqref{eq:bound_rade}.

Finally we will use Lemma \ref{lem:M to K} to bound $M$.
\begin{lemma}\label{lem:M to K}
    Let $M$ be defined as in \eqref{eq:bound_rade}.    
    With probability at least $1 - n^{-c+1}$, we have $M<ac(\sqrt{r} + \log(n))$.
\end{lemma}
Let $\vb_i$ be replaced by $\hat \Ub_r^\top\x_i$ in Lemma \ref{lemma:chi-sqr}, then this directly results from Lemma \ref{lemma:chi-sqr}. Lemma \ref{lem:M to K} bounds $M$, thus bounds $K$ (which is $1$ Lipschitz in $M$) in Lemma \ref{lem:rade known}. After we insert \eqref{eq:tilde Rc} together into Lemma \ref{lem:rade known}, we can get the result in  Theorem \ref{thm:rade}.
% By Lemma \ref{lemma:chi-sqr} we know that for a constant $c>2$, we have  $\max{\|\hat\Ub_r^\top\x_i\|} \le c(\sqrt{r} + \log(n))$ for all $i=1,..,n$ with probability $1 - n^{-c+1}$. So with probability at least $1 - n^{-c+1}$, we have $M<ac(\sqrt{r} + \log(n))$.
\end{proof}



==> Icassp (3)/s_prob.tex <==
\setlength{\topsep}{0.25em}
\newcommand{\xij}{{\x_{i,j}}}
\newcommand{\xijt}{{\x_{i,j}^\top}}
\newcommand{\yij}{{y_{i,j}}}

\section{Problem Formulation}\label{s:prob}
% {\color{red} YS: a paragraph for notation?}
The meta-learning setup that will be considered in this work consists of two phases: (i) meta-training: prior tasks are used to learn a good representation and (ii) few-shot learning: the new task is learned with few samples.
%\som{Is meta-train/test standard and correct phrases?} 
%{\mf better not to use the meta-train and meta-test phrases if we don't need to} 
In the meta-training phase, we learn the low dimensional space spanned by parameters. In the few-shot learning phase, we use the subspace to learn the model of a new task ideally with few samples.

In the first phase, there are multiple tasks to infer from, each with its own distribution. We consider a realizable model where the input and label is associated via a labeling function. One accesses batches of data, each of whom is collected from a task, however we may not know which task it comes from. We make this setup more precise using the following definitions. Below, the ground-truth representation will be denoted by a matrix $\W\in\R^{r\times d}$ row space of which corresponds to the subspace of interest.

%\som{Use $n_j$ for sample size rather than $t_j$ (at least for training)}
\begin{definition} \label{def:task}
\textbf{Meta-training data.} Fix a matrix $\W\in\R^{r\times d}$ satisfying $\W\W^T=\Iden$. The $j$-th task is associated with function $f^j: \R^r\rightarrow \R$. Given input $\x$, the label $y$ is distributed as $p_j(y|\x)=p_j(y|\W\x)$\footnote{In words, the label only depends on the relevant features induced by $\W$.} and the expectation satisfies $\mtx{E}(y) = f^j(\W\x)$.
%{\mf give properties like domain and range of $f$ here, first time it appears.}
Suppose there are $n_j$ samples from the $j$-th task sampled i.i.d.~from this distribution and we denote the dataset $\Sc^j = (\xij, \yij)_{i=1}^{n_j}$. Define the full meta-training dataset to be $\Sc = \bigcup_{j=1}^k\Sc^j$.
\end{definition}
Here, $f^j$ is allowed to be any Lipschitz nonlinear function, i.e., a neural network\footnote{In our theoretical results, we treat $f$ as a general linear function, and in experiments we will use a neural network with a specific structure.}.


%In the multi-task problem, there are a collection of tasks in the meta-training phase, which is defined below.


\iffalse
\begin{definition}\label{def:task dis}\som{I don't think we should use a distribution early on.}
\textbf{Low rank task distribution.} There are in total $k$ tasks. Each training task is associated with a parameter vector $\bt^j\in\R^d$ for $j=1,...,k$.
{\mf right now we're just setting the notation---additional assumptions like definition 2.2 on random features should come later.}
These are generated i.i.d. from a Gaussian distribution $\mathcal{N}(0, \bSi)$. Let $\la_i$ be the $i$-th eigenvalue of $\bSi$ with decreasing order. For low rank parameters, we assume that $\la_{r+1} = 0$. We call $r$ as the effective dimension of parameters.
\end{definition}



\begin{definition} \label{def:task}
\textbf{Meta-training data.} The $j$-th task is associated with parameter $\bt^j\in\R^d$. 
%For any parameter $\bt$, one can collect data from it. 
Suppose there are $n_j$ data from the $j$-th task, we call the dataset $\Sc^j = \{(\xij, \yij)\ |\ i=1,...,n_j\}$. Here $\xij\in\R^d$, $\yij\in\R$. $\xij$, $\yij$ satisfy $\mtx{E}(\yij) = f(\xijt\bt^j)$ for some function $f$. Let the whole meta-training dataset be $\Sc = \bigcup_{j=1,...,k}\Sc^j$. {\mf repeated}
\end{definition}

%\noindent\textbf{:}

\begin{definition} \label{def:data_gen}
\textbf{Data generation.} We assume that there are $k$ binary classification tasks, the $j$-th associated with $\bt^j$. The data $\Sc^j$ is generated by $\xij = \bz / \|\bz\|$ and $\bz \sim \mathcal{N}(0, I)$, $\bz$ is generated independently. Denote the distribution of $\xij$ as $\mathscr{P}_x$.
%The labels $\yij$ satisfy
%$\mtx{E}(\yij|\xij, \bt^j) = f(\xijt\bt^j)$ for some Lipschitz function $f:\R\rightarrow \R$. We propose two examples below.
\end{definition}
%{\color{blue} Do we need to normalize $x$? Just for citing the result in \cite{kong2020meta}, they use Bernstein so they have to use bounded rv. In principle unbounded subGaussian works.}
\fi


\begin{definition} \label{def:bin_class}
\textbf{Binary classification.} Suppose $f^j$ takes values over $[0,1]$,
%{\it\color{red}{Is it [0,1] ?}}. The labels $\yij$ are generated as 
\begin{align*}
    \yij = 
     \begin{cases}
       \text{1,} &{\mbox{with probability } f^j(\W \xij),}\\
       \text{0,} &{\mbox{with probability } 1-f^j(\W\xij).}\\
     \end{cases}
\end{align*}
%Here $f^j(a)\in[0,1]$ for all $a\in[-1,1]$, and the event that $f(a) = 0$ is not true with probability $1$ with respect to Lebesgue measure on $[-1,1]$\footnote{In other words, $f$ is not a constant $0$ function.}.
\end{definition}

\begin{definition}\label{def:GLM}
\noindent\textbf{Generalized linear models (GLM)} (which include logistic/linear regression) can be modeled by choosing $f^j$ to be parameterized by a vector $\bt_j\in\R^r$ and a link function $\phi:\R\rightarrow\R$ as $f^j(\W \xij) := \phi(\bt_j^T\W\xij )$.

\end{definition}
%for $\bt_j\in\R^r$, $\phi$ is a function mapping from $\R$ to $(0,1)$.

% Denote the distribution of $\x,y$ as $\mathscr{P}_{x,y}$.
%\begin{definition}\label{def:nn}
%\textbf{Non-linear regression.} More generally, for $\bt^j\in\R^{r\times d}$, the labels $\yij$ are generated as
%\begin{align*}
%    \yij = f^j(\W\xij) + \epsilon,
%\end{align*}
%$\epsilon$ is a zero mean bounded random variable. 
%\end{definition}

When the dimension of the span of parameters is small, \cite{kong2020meta} performs a dimension reduction algorithm to find the low-dimensional subspace that the parameters span. This is done by selecting the top eigenvectors of the covariance estimate of the cross-correlation between input and labels.
\begin{definition}\label{def:mom}
\textbf{Moment estimator of covariance.} We define the covariance estimator as
\begin{subequations}\label{eq:hatM}
\begin{align}
\hat\bM &= \mathop{\Scale[1.8]{\sum}}_{j=1}^k \frac{2}{n_j^2}\left[(\sum_{i=1}^{n_j/2} \yij\xij) (\sum_{i=n_j/2+1}^{n_j} \yij\xij)^\top \right.\\
&\quad\quad\quad\quad \left. +  ( \sum_{i=n_j/2+1}^{n_j} \yij\xij) ( \sum_{i=1}^{n_j/2} \yij\xij)^\top\right].\nonumber
\end{align}
\end{subequations}
\end{definition}
\noindent\textbf{Subspace estimation.} 
To estimate the subspace $\W$, we use rank-$r$ approximation of $\hat \bM$ to retrieve its principal eigenvector subspace. 
Let $\hat\Ub \hat \La \hat \Ub^\top$ be the eigen-decomposition of $\hat \bM$. Denote $\hat \la_j$ as the $j$th eigenvalue of $\hat \La$. Let $\hat\Ub_r$ be the first $r$ columns of $\hat\Ub$, thus the rank-$r$ approximation is $\hat\bM_r = \hat\Ub_r \mathrm{diag}(\hat \la_{1},...,\hat\la_{r}) \hat \Ub_r^\top$. In the next section, we will prove that the range of $\hat \Ub$ is close to the row space of $\W$.

%{\color{blue} No need to put an algorithm here. If we have a bound for downstream task as well we can fill up the whole procedure.}

%Now we propose the algorithm that accomplishes the subspace retrieval process above. 

In Algorithm \ref{algo:1}, the output $\hat\Ub_r$ is the estimator of the task subspace $\W$. $\hat\Ub_r$ is used as a training step for the few-shot learning phase. For the new task, we search for the function $f^*$ that minimizes the population loss. We shall provide an instructive analysis for the cross-entropy loss, which is usually employed for classification tasks.

\so{Currently, cross-entropy comes out of nowhere. For using cross-ent, label has to be discrete. It cannot be an arbitrary nonlinear function. Overall, we need to do one of the followings:\\
 Option 1: Do the analysis for a Lipschitz loss function for which cross-entropy is a special case.\\
 Option 2: Let us just say that for few-shot phase, we focus on classification and study cross-entropy. Clearly state label is discrete 0-1.}
\begin{definition}\label{def: test}
\textbf{Few-shot classification (Population).} In the few-shot learning phase, suppose $\x,y\sim\Pxy$ satisfy $\mtx{E}(y|\x) = f^*(\W\x)$. Let $\Fc$ be a family of functions as the search space for few-shot learning model. 
Let $\cLCE: \Fc\times \R^{r\times d}\rightarrow \R$ be population cross-entropy loss, defined as 
\begin{align}
    \cLCE(f;\Pb)=-\mtx{E}_{\Pxy} (&y\log f(\Pb \x)\label{eq:cLCE}\\
   &+ (1-y)\log (1 - f(\Pb \x))) \nonumber.
\end{align}
\so{Following my comment above, for cross-ent, clearly $0\leq f\leq 1$. This has to be specified in the definition.}

We search for the solution induced by $\hat{\Ub}_r$ by
\begin{align}
    \hat f &= \argmin_{f\in\Fc}\ \cLCE(f;\hat{\Ub}_r^\top)\label{eq:fstar}
\end{align}
%If $\Pb$ is known, we use $\cLCE(f(\Pb x))$ as an equivalent way of representing $\cLCE(f;\Pb)$.
\end{definition}
Observe that, without representation learning, one has to search for both $f$ and $\Pb$. However with representation learning, we fix $\Pb=\hat{\Ub}_r$ and only search for $f$.
\begin{remark}\label{rem:logistic}
For the GLM Definition \ref{def:GLM}, we can choose $\Fc$ to be the $\ell_2$ norm constrained functions for some $a\leq\infty$% the set of functions $f$ satisfying
% {\color{red} YS: I want to say $\Fc = \phi\circ\bt\circ(\mathrm{variable})$}
\begin{align}
    \Fc = \{\x\rightarrow \phi(\bt^T\x)~\big|~\|\bt\|_2 \le a,~\bt\in\R^r\}, \label{eq:Fcbin}
\end{align}
Let the new data be generated with $f^*(\W\x) = \phi({\bt^*}^\top\W\x)$ for some ground-truth parameter $\bt^*$. We use $\cLCE(\bt;\Pb)$ to denote the cross-entropy loss in this setting. $\hat f$ (parameterized by $\hat{\bt}$) is given by
\begin{align}
    \hat \bt &= \argmin_{\bt}\ \cLCE(\bt;\hat \Ub_r^\top ),\mbox{~such~that~} \|\bt\| \le a. \label{eq:fstarbin}
\end{align}
\end{remark}


\iffalse
\begin{definition}\label{def: test finite}
\textbf{Finite sample few-shot learning.} In the few-shot learning phase, there are in total $n$ samples, and suppose 
$\x_i\in\R^d$ are generated independently, following standard normal distribution, $y_i\in\R$, for $i=1,...,n$. $\x_i$, $y_i$ satisfy $\mtx{E}(y_i|\x_i) = f^*(\W\x_i)$. Lef $\Fc$ be a family of functions as the search space for few-shot activation function. 
Let $\cL_e$ be empirical cross entropy loss, defined as 
\begin{align}
    &\cL_e(f;\Pb) : \Fc\times \R^{r\times d}\rightarrow \R= \notag\\
    &-\frac{1}{n}\sum_{i=1}^n (y_i\log f(\Pb \x_i) + (1-y_i)\log (1 - f(\Pb \x_i))) \label{eq:cLCE finite}
\end{align}
We search for the solution by
\begin{align}
    \hat f_e &= \argmin_{f\in\Fc}\ \cL_e(f;\Ub_r^\top)\label{eq:fstar finite}
\end{align}

\end{definition}
\fi
% and suppose $\x_i\in\R^d$ are generated independently, following standard normal distribution, $y_i\in\R$, for $i=1,...,n$.
\begin{definition}\label{def: test finite}
\textbf{Few-shot learning (Finite sample GLM).} Suppose there are in total $n$ samples for new task $(\x_i,y_i)_{i=1}^n$ and $(\x_i,y_i)$ satisfies $\mtx{E}(y_i|\x_i) = f^*(\W\x_i)$. Lef $\Fc$ be a family of functions for few-shot learning phase. We consider the setup of Remark \ref{rem:logistic}, where $\phi$ is the logistic function. 
%: \Fc\times \R^{r\times d}\rightarrow \R= \notag\\
\begin{align}
    \cL_e(\bt;\Pb)=-\frac{1}{n}\sum_{i=1}^n (&y_i\log(\phi (\bt^\top\Pb \x_i))\label{eq:cLCE finite theta}\\
    &+ (1-y_i)\log (1 - \phi(\bt^\top\Pb \x_i))).\nonumber 
\end{align}
Given an $\ell_2$-norm constraint $a\leq \infty$, the empirical risk minimizer (ERM) is defined as follows
\begin{align}
    \hat \bt_e &= \argmin_{\bt}\ \cL_e(\bt;\Ub_r^\top)\quad\text{such~that}\quad\|\bt\|_2\le a.\label{eq:fstar finite theta}
\end{align}
\end{definition}


\begin{algorithm}[t!]
\caption{Meta-training and Few-shot Learning}\label{algo:1}
\begin{algorithmic}
% with $k$ tasks, the size of data of the $j$-th task has size $n_j$. Dimension $d$. Effective dimension $r$. Set of functions $\Fc$.
\REQUIRE {Dataset $\mathcal{S}$, representation size $r$, function space $\Fc$}
\STATE{Compute $\hat \bM$ via method-of-moments \eqref{eq:hatM}.}
\STATE{Rank $r$ approximation:\\
$\quad\hat\bM_r \leftarrow \hat\Ub_r \mathrm{diag}(\hat \La_{1,1},...,\hat\La_{r,r}) \hat \Ub_r^\top$.}
\STATE{Either~$\hat f \leftarrow \argmin_{f\in\Fc}\ \cLCE(f;\Ub_r^\top) $. $\cLCE$ is defined as \eqref{eq:cLCE}.}
\STATE{Or~~~~~~$\hat f_e \leftarrow \argmin_{f\in\Fc}\ \cL_e(f;\Ub_r^\top) $. $\cL_e$ is defined as \eqref{eq:cLCE finite theta}}
\RETURN{$\hat\Ub_r$ and $\hat f$ or $\hat f_e$.}
\end{algorithmic}
\end{algorithm}%\vspace{-10pt}


==> Icassp (3)/s_prob_2.tex <==
\setlength{\topsep}{0.25em}
\newcommand{\xij}{{\x_{i,j}}}
\newcommand{\xijt}{{\x_{i,j}^\top}}
\newcommand{\yij}{{y_{i,j}}}

\section{Problem Formulation}\label{s:prob}
% {\color{red} YS: a paragraph for notation?}
\vspace{-0.1cm}
The meta-learning setup that will be considered in this work consists of two phases: (i) meta-training: prior tasks are used to learn a good representation and (ii) few-shot learning: the new task is learned with few samples.
%\som{Is meta-train/test standard and correct phrases?} 
%{\mf better not to use the meta-train and meta-test phrases if we don't need to} 
In the meta-training phase, we learn the low dimensional space spanned by parameters. In the few-shot learning phase, we use the subspace to learn the model of a new task ideally with few samples.

In the first phase, there are multiple task vectors to infer from.%, each with its own distribution. 
We consider a realizable model where the input and label is associated via a labeling function. One accesses batches of data, each of whom is collected from a task.
%, however we may not know which task it comes from. 
%We make this setup more precise using the following definitions. 
Below, we denote the ground-truth representation by a matrix $\W\in\R^{r\times d}$ whose row space corresponds to the subspace of interest.

%\som{Use $n_j$ for sample size rather than $t_j$ (at least for training)}
\begin{definition} \label{def:task}
\textbf{Meta-training data.} Fix a matrix $\W\in\R^{r\times d}$ satisfying $\W\W^T=\Iden$. The $j$-th task is associated with function $f^j: \R^r\rightarrow \R$. Given input $\x\in\R^{d}$, the label $y$ is distributed as $p_j(y|\x)=p_j(y|\W\x)$\footnote{In words, the label only depends on the relevant features induced by $\W$.} and the expectation satisfies $\mtx{E}(y) = f^j(\W\x)$.
%{\mf give properties like domain and range of $f$ here, first time it appears.}
Suppose there are $n_j$ samples from the $j$-th task sampled i.i.d.~from this distribution and we denote the dataset $\Sc^j = (\xij, \yij)_{i=1}^{n_j}$. Define the full meta-training dataset to be $\Sc = \bigcup_{j=1}^k\Sc^j$.
\end{definition}
Here, $f^j$ is allowed to be any Lipschitz nonlinear function, i.e., a neural network\footnote{In our theoretical results, we treat $f$ as a general linear function, and in experiments we will use a neural network with a specific structure.}.


%In the multi-task problem, there are a collection of tasks in the meta-training phase, which is defined below.


\iffalse
\begin{definition}\label{def:task dis}
%\som{I don't think we should use a distribution early on.}
\textbf{Low rank task distribution.} There are in total $k$ tasks. Each training task is associated with a parameter vector $\bt^j\in\R^d$ for $j=1,...,k$.
{\mf right now we're just setting the notation---additional assumptions like definition 2.2 on random features should come later.}
These are generated i.i.d. from a Gaussian distribution $\mathcal{N}(0, \bSi)$. Let $\la_i$ be the $i$-th eigenvalue of $\bSi$ with decreasing order. For low rank parameters, we assume that $\la_{r+1} = 0$. We call $r$ as the effective dimension of parameters.
\end{definition}



\begin{definition} \label{def:task}
\textbf{Meta-training data.} The $j$-th task is associated with parameter $\bt^j\in\R^d$. 
%For any parameter $\bt$, one can collect data from it. 
Suppose there are $n_j$ data from the $j$-th task, we call the dataset $\Sc^j = \{(\xij, \yij)\ |\ i=1,...,n_j\}$. Here $\xij\in\R^d$, $\yij\in\R$. $\xij$, $\yij$ satisfy $\mtx{E}(\yij) = f(\xijt\bt^j)$ for some function $f$. Let the whole meta-training dataset be $\Sc = \bigcup_{j=1,...,k}\Sc^j$. {\mf repeated}
\end{definition}

%\noindent\textbf{:}

\begin{definition} \label{def:data_gen}
\textbf{Data generation.} We assume that there are $k$ binary classification tasks, the $j$-th associated with $\bt^j$. The data $\Sc^j$ is generated by $\xij = \bz / \|\bz\|$ and $\bz \sim \mathcal{N}(0, I)$, $\bz$ is generated independently. Denote the distribution of $\xij$ as $\mathscr{P}_x$.
%The labels $\yij$ satisfy
%$\mtx{E}(\yij|\xij, \bt^j) = f(\xijt\bt^j)$ for some Lipschitz function $f:\R\rightarrow \R$. We propose two examples below.
\end{definition}
%{\color{blue} Do we need to normalize $x$? Just for citing the result in \cite{kong2020meta}, they use Bernstein so they have to use bounded rv. In principle unbounded subGaussian works.}
\fi


\begin{definition} \label{def:bin_class}
\textbf{Binary classification.} Suppose $f^j$ takes values over $[0,1]$,
%{\it\color{red}{Is it [0,1] ?}}. The labels $\yij$ are generated as 
\begin{align*}
    \yij = 
     \begin{cases}
       \text{1,} &{\mbox{with probability } f^j(\W \xij),}\\
       \text{0,} &{\mbox{with probability } 1-f^j(\W\xij).}\\
     \end{cases}
\end{align*}
%Here $f^j(a)\in[0,1]$ for all $a\in[-1,1]$, and the event that $f(a) = 0$ is not true with probability $1$ with respect to Lebesgue measure on $[-1,1]$\footnote{In other words, $f$ is not a constant $0$ function.}.
\end{definition}

\begin{definition}\label{def:GLM}
\noindent\textbf{Generalized linear models (GLM)} (which include logistic/linear regression) can be modeled by choosing $f^j$ to be parameterized by a vector $\bt_j\in\R^r$ and a link function $\phi:\R\rightarrow\R$ as $f^j(\W \xij) := \phi(\bt_j^T\W\xij )$.

\end{definition}
%for $\bt_j\in\R^r$, $\phi$ is a function mapping from $\R$ to $(0,1)$.

% Denote the distribution of $\x,y$ as $\mathscr{P}_{x,y}$.
%\begin{definition}\label{def:nn}
%\textbf{Non-linear regression.} More generally, for $\bt^j\in\R^{r\times d}$, the labels $\yij$ are generated as
%\begin{align*}
%    \yij = f^j(\W\xij) + \epsilon,
%\end{align*}
%$\epsilon$ is a zero mean bounded random variable. 
%\end{definition}

When the dimension of the span of parameters is small, \cite{kong2020meta} performs a dimension reduction algorithm to find the low-dimensional subspace that the parameters span. This is done by selecting the top eigenvectors of the covariance estimate of the cross-correlation between input and labels.
\begin{definition}\label{def:mom}
\textbf{Moment estimator of covariance.} We define the covariance estimator as
\begin{equation}\label{eq:hatM}
\begin{split}
\hat\bM &= \mathop{\Scale[1.8]{\sum}}_{j=1}^k \frac{2}{n_j^2}\left[(\sum_{i=1}^{n_j/2} \yij\xij) (\sum_{i=n_j/2+1}^{n_j} \yij\xij)^\top \right.\\
&\quad\quad\quad\quad \left. +  ( \sum_{i=n_j/2+1}^{n_j} \yij\xij) ( \sum_{i=1}^{n_j/2} \yij\xij)^\top\right].
\end{split}
\end{equation}
Define
\begin{align*}
    &\mtx{h}^j(\W): \R^{r\times d} \rightarrow \R^d = \mtx{E}_{\x}[f^j(\W \x)\x]\\
    &\bM := \W^\top\W\left(\frac{1}{k}\sum_{j=1}^k \mtx{h}^j(\W)( \mtx{h}^j(\W))^\top\right)\W^\top\W.
\end{align*}
\end{definition}
We will prove that $\hat\bM$ is a finite sample estimate of $\bM$.
\noindent\textbf{Subspace estimation.} 
To estimate the subspace $\W$, we use rank-$r$ approximation of $\hat \bM$ to retrieve its principal eigenvector subspace. 
Let $\hat\Ub \hat \La \hat \Ub^\top$ be the eigen-decomposition of $\hat \bM$. Denote $\hat \la_j$ as the $j$th eigenvalue of $\hat \La$. Let $\hat\Ub_r$ be the first $r$ columns of $\hat\Ub$, thus the rank-$r$ approximation is $\hat\bM_r = \hat\Ub_r \mathrm{diag}(\hat \la_{1},...,\hat\la_{r}) \hat \Ub_r^\top$. In the next section, we will prove that the range of $\hat \Ub$ is close to the row space of $\W$.

%{\color{blue} No need to put an algorithm here. If we have a bound for downstream task as well we can fill up the whole procedure.}

%Now we propose the algorithm that accomplishes the subspace retrieval process above. 

In Algorithm \ref{algo:1}, the output $\hat\Ub_r$ is the estimator of the task subspace $\W$. $\hat\Ub_r$ is used as a training step for the few-shot learning phase. For the new task, we search for the function $f^*$ that minimizes the population loss. We shall provide an instructive analysis for a general class of functional family and loss.
\begin{assumption}\label{ass:F}
$\Fc$ is a set of functions satisfying: For any function $f\in\Fc$, any orthonormal matrix $\Qb\in\R^{r\times r}$ and any representation matrix $\Pb\in\R^{r\times d}$, there exists $g \in \Fc$ such that $f(\Pb \x) = g(\Qb\Pb \x)$.
%\begin{enumerate}
%    \item For any function $f\in\Fc$, any orthonormal matrix $\Qb\in\R^{r\times r}$ and any matrix $\Pb\in\R^{r\times d}$, there exists $g \in \Fc$ such that $f(\Pb \x) = g(\Qb\Pb \x)$.
%    \item $\Fc \subseteq \{f\ |\ \log f,~ \log(1-f)\mathrm{~are~}L\mathrm{~Lipschitz}\}\bigcap \{f\ |\ 0<f(x)<1,\forall x\in\R^r\}$.
%\end{enumerate}
\end{assumption}
\ys{In this assumption, we basically mean that the $\Fc$ is invariant with orthonormal rotation $\Qb$. In other words, we only need to find the $r$ dimensional row space $\mathrm{row}(\Pb)$ (to project the features onto it as a low dimensional representation), and don't worry the exact matrix $\Pb$ itself.

Let us introduce population risk $\cL$ and empirical risk $\cL_e$ based on any single loss function between model prediction and true label.}
\begin{align*}
&\cL(f;\Pb) = \mtx{E}_{\Pxy}\cLoss(f(\Pb \x),y)\\
&\cL_e(f;\Pb) = \frac{1}{n}\sum_{i=1}^n\cLoss(f(\Pb \x_i),y_i).
\end{align*}
We make the following assumption on the population risk.
\begin{assumption}\label{ass:L}
Suppose population loss $\cL$ and empirical loss $\cL_e$ satisfy the following assumptions:
\begin{enumerate}[itemsep=-0.1em,topsep=0.3em]
    %\item $\cL$ has the form $\cL(f;\Pb) = \mtx{E}_{\Pxy}\cL(f(\Pb \x),y)$.
    %$\cL_e$ has the form $\cL_e(f;\Pb) = \frac{1}{n}\sum_{i=1}^n\cL(f(\Pb \x_i),y_i)$.
    \item $\cL$ is $L$ Lipschitz in $\Pb \x$.
    \item $\min_{\Pb}\cL(f;\Pb) = \cL(f;\W)$.
\end{enumerate}
\end{assumption}
\noindent\textbf{Example:} Suppose $f$ is an $L$-Lipschitz function with range in $(0,1)$ \ys{and the true labels $y_i$ are from $\{0,1\}$.} The cross entropy function satisfies the assumptions.
\begin{align}
    \cLCE(f;\Pb)=-\mtx{E}_{\Pxy} (&y\log f(\Pb \x)\label{eq:cLCE}\\
   &+ (1-y)\log (1 - f(\Pb \x))) \nonumber.\\
   \cL_e(f;\Pb)=-\frac{1}{n}\sum_{i=1}^n (&y_i\log(f(\Pb \x_i))\label{eq:cLCE finite theta}\\
    &+ (1-y_i)\log (1 - f(\Pb \x_i))).\nonumber 
   %\cL_e(\bt;\Pb)=-\frac{1}{n}\sum_{i=1}^n (&y_i\log(\phi (\bt^\top\Pb \x_i))\label{eq:cLCE finite theta}\\
    %&+ (1-y_i)\log (1 - \phi(\bt^\top\Pb \x_i))).\nonumber 
\end{align}
\ys{With an abuse of notation, we can define the loss with respect to parameterization of the function $f$. For example, if we use the model in Def. \ref{def:GLM}, then we can write the empirical loss as 
\begin{align}
    \cL_e(\bt;\Pb)=-\frac{1}{n}\sum_{i=1}^n (&y_i\log(\phi (\bt^\top\Pb \x_i))\\%\label{eq:cLCE finite theta}\\
    &+ (1-y_i)\log (1 - \phi(\bt^\top\Pb \x_i))).\nonumber
\end{align}
}

% the cross-entropy loss, which is usually employed for classification tasks.
\iffalse
\so{Currently, cross-entropy comes out of nowhere. For using cross-ent, label has to be discrete. It cannot be an arbitrary nonlinear function. Overall, we need to do one of the followings:\\
 Option 1: Do the analysis for a Lipschitz loss function for which cross-entropy is a special case.\\
 Option 2: Let us just say that for few-shot phase, we focus on classification and study cross-entropy. Clearly state label is discrete 0-1.}
 \fi
\begin{definition}\label{def: test}
\textbf{Few-shot classification (Population).} In the few-shot learning phase, suppose $\x,y\sim\Pxy$ satisfy $\mtx{E}[y~|~\x] = f^*(\W\x)$. Let $\Fc$ be a family of functions as the search space for few-shot learning model. 
Let Assumptions \ref{ass:F} and \ref{ass:L} hold. We search for the solution induced by $\hat{\Ub}_r$ by
\begin{align}
    \hat f &= \argmin_{f\in\Fc}\ \cLCE(f;\hat{\Ub}_r^\top)\label{eq:fstar}
\end{align}
%$\cLCE: \Fc\times \R^{r\times d}\rightarrow \R$ be population cross-entropy loss, defined as 
%\begin{align}
%    \cLCE(f;\Pb)=-\mtx{E}_{\Pxy} (&y\log f(\Pb \x)\label{eq:cLCE}\\
%   &+ (1-y)\log (1 - f(\Pb \x))) \nonumber.
%\end{align}

\iffalse
\so{Following my comment above, for cross-ent, clearly $0\leq f\leq 1$. This has to be specified in the definition.}
\fi


%If $\Pb$ is known, we use $\cLCE(f(\Pb x))$ as an equivalent way of representing $\cLCE(f;\Pb)$.
\end{definition}
Observe that, without representation learning, one has to search for both $f$ and $\W$. However with representation learning, we use $\hat{\Ub}_r^\top$ as the representation matrix and only search for $f$.
\begin{remark}\label{rem:logistic}
For the GLM Definition \ref{def:GLM}, we can choose $\Fc$ to be the $\ell_2$ norm constrained functions for some $a\leq\infty$% the set of functions $f$ satisfying
% {\color{red} YS: I want to say $\Fc = \phi\circ\bt\circ(\mathrm{variable})$}
\begin{align}
    \Fc = \{\x\rightarrow \phi(\bt^T\x)~\big|~\|\bt\|_2 \le a,~\bt\in\R^r\}, \label{eq:Fcbin}
\end{align}
Let the new data be generated with $f^*(\W\x) = \phi({\bt^*}^\top\W\x)$ for some ground-truth parameter $\bt^*$. We use $\cLCE(\bt;\Pb)$ to denote the cross-entropy loss in this setting. $\hat f$ (parameterized by $\hat{\bt}$) is given by
\begin{align}
    \hat \bt &= \argmin_{\bt}\ \cLCE(\bt;\hat \Ub_r^\top ),\mbox{~such~that~} \|\bt\| \le a. \label{eq:fstarbin}
\end{align}
\end{remark}


\iffalse
\begin{definition}\label{def: test finite}
\textbf{Finite sample few-shot learning.} In the few-shot learning phase, there are in total $n$ samples, and suppose 
$\x_i\in\R^d$ are generated independently, following standard normal distribution, $y_i\in\R$, for $i=1,...,n$. $\x_i$, $y_i$ satisfy $\mtx{E}(y_i|\x_i) = f^*(\W\x_i)$. Lef $\Fc$ be a family of functions as the search space for few-shot activation function. 
Let $\cL_e$ be empirical loss, satisfying Assumptions \ref{ass:F} and \ref{ass:L}.

%defined as 
%\begin{align}
%    &\cL_e(f;\Pb) : \Fc\times \R^{r\times d}\rightarrow \R= \notag\\
%    &-\frac{1}{n}\sum_{i=1}^n (y_i\log f(\Pb \x_i) + (1-y_i)\log (1 - f(\Pb \x_i))) \label{eq:cLCE finite}
%\end{align}
We search for the solution by
\begin{align}
    \hat f_e &= \argmin_{f\in\Fc}\ \cL_e(f;\Ub_r^\top)\label{eq:fstar finite}
\end{align}

\end{definition}
\fi
% and suppose $\x_i\in\R^d$ are generated independently, following standard normal distribution, $y_i\in\R$, for $i=1,...,n$.
\begin{definition}\label{def: test finite}
\textbf{Few-shot learning (Finite sample GLM).} Suppose there are $n$ samples for new task $(\x_i,y_i)_{i=1}^n$ and $(\x_i,y_i)$ satisfies $\mtx{E}(y_i|\x_i) = f^*(\W\x_i)$. 
%Let $\Fc$ be a family of functions for few-shot learning phase. 
Let $\cL_e$ be empirical loss, satisfying Assumptions \ref{ass:F} and \ref{ass:L}.
%We consider the setup of Remark \ref{rem:logistic}, where $\phi$ is the logistic function. 
%: \Fc\times \R^{r\times d}\rightarrow \R= \notag\\
%\begin{align}
%    \cL_e(\bt;\Pb)=-\frac{1}{n}\sum_{i=1}^n (&y_i\log(\phi (\bt^\top\Pb \x_i))\label{eq:cLCE finite theta}\\
%    &+ (1-y_i)\log (1 - \phi(\bt^\top\Pb \x_i))).\nonumber 
%\end{align}
Given norm constraint $a\leq \infty$, the empirical risk minimizer (ERM) is defined as
\begin{align}
    \hat \bt_e &= \argmin_{\bt}\ \cL_e(\bt;\hat\Ub_r^\top)\quad\text{such~that}\quad\|\bt\|_2\le a.\label{eq:fstar finite theta}
\end{align}
\end{definition}


\setlength{\textfloatsep}{.5em}
\begin{algorithm}[t!]
\caption{Meta-training and Few-shot Learning}\label{algo:1}
\begin{algorithmic}
% with $k$ tasks, the size of data of the $j$-th task has size $n_j$. Dimension $d$. Effective dimension $r$. Set of functions $\Fc$.
\REQUIRE {Dataset $\mathcal{S}$, representation size $r$, function space $\Fc$}
\STATE{Compute $\hat \bM$ via method-of-moments \eqref{eq:hatM}.}
\STATE{Rank $r$ approximation:\\
$\quad\hat\bM_r \leftarrow \hat\Ub_r \mathrm{diag}(\hat \La_{1,1},...,\hat\La_{r,r}) \hat \Ub_r^\top$.}
\STATE{Either~$\hat f \leftarrow \argmin_{f\in\Fc}\ \cLCE(f;\Ub_r^\top) $.
%$\cLCE$ is defined as \eqref{eq:cLCE}.
}
\STATE{Or~~~~~~$\hat f_e \leftarrow \argmin_{f\in\Fc}\ \cL_e(f;\Ub_r^\top) $.
%$\cL_e$ is defined as \eqref{eq:cLCE finite theta}
}
\RETURN{$\hat\Ub_r$ and $\hat f$ or $\hat f_e$.}
\end{algorithmic}
\end{algorithm}%\vspace{-10pt}


==> Paper/Paper_rebuttal.tex <==
We highly appreciate the comments from all reviewers, and we have updated the paper with proof in https://github.com/sunyue93/RLnonlinear/blob/main/RLnonlinear.pdf

1068

This paper analyzes the theoretical guarantee of nonlinear models in representation learning, specifically, training error of meta-training and generalization of few-shot learning. This is far more general than the papers discussing linear cases such as Kong et al, Tripuraneni et al., and we believe it can be applied in many machine learning tasks. We have mentioned the applications that relate to transfer learning in intro section, such as Deng et al, Bojar et al, Finn et al. In the experiment section we give simulations on image classification, where the same idea can be generalized to large datasets. We are going to run experiment in more complicated settings and illustrate the algorithm's performance. 

Comment for specific questions:
1. We will change the notations in experiment section so that they don't overlap with the theory part. In the experiments, we can treat the coefficients in the bottom layer as $\theta$, and the activations and upper layers provide the nonlinearities.
2. The first experiment is proposed to verify Theorem 3.2, the ability of the moment estimator to find the feature subspace. The reviewer is correct that we do not check the few-shot learning phase. For synthetic example, if the subspace is accurately retrieved and suppose we can find the optimal neural net model, then the few-shot learning is trivially accurate (because we generate the label-feature relevance by randomly picking the neural net coefficient, then we can recover the coefficients if the number of samples is bigger than the degree of freedom in few-shot learning phase). 3. P is mentioned in Assumption 1, which is a $r\times d$ matrix that brings the features from $d$ dimension to $r$ dimension. There are two ways of excecuting the learning: With representation learning, we use our proposed algorithm that computes a moment estimator $\hat M$ and its SVD truncation $\hat M_r$. Then the subspace is used as $\hat U_r$ and we only need to train $\hat f$; Without representation learning, we can go ahead solving $\min_{f,U} L(f,\hat U)$ where both $f$ and $U$ are variables. So the degree of freedom is higher than representation learning case and it requires more data.
Regarding the experiment, when we say "with representation" there is a learned $P$ that we hope is aligned with the underlying subspace $W$. When we say "without representation" we don't project the data onto a low dimensional subspace before few-shot learning, i.e., we keep the features as $d$ dimensional, thus the variable is $d$ dimensional and it's hard to recover with $O(r)$ samples.
4. $W$ and $P$ are different. We assume that $W$ is the function that connects $x$ and $y$. It is the true matrix that comes from nature. $P$ later is the subspace we constructed from our algorithm (which we hope to be close to $W$), and it is used to define the metric $L$. So whatever $P$ is, we can always write the loss with respect to $P$ and $f$.
5. We will correct correspondingly.

1BAA

Comment for specific questions:
1. We have updated the paper with proof at 
https://github.com/sunyue93/RLnonlinear/blob/main/RLnonlinear.pdf
Lemma 3.3 uses well-known Davis-Kahan bound to reveal the connection between error in $W$ and $M$. We will add the lemma to the paper. This is not a substantial change of paper but we agree that it's crucial to point out the connection of error in $M$ and $W$ clear.
2. That is true. Our algorithm is consisted of two phases: meta-training and few-shot learning. In meta-training, we use $O(d)$, more data from meta-training dataset to learn the low dimensional representation. This part by itself requires more data, but we prove that, with the representation learned, we can use $O(r)$, less data for training on the few-shot learning. If we don't run meta-training algorithm and directly learn from scratch on few-shot learning data, to reach the same error it would require $O(d)$ instead of $O(r)$ samples. We only run meta-training once with $O(d)$ samples, and this makes training on every few-shot learning tasks sample-efficient. So the requirement for sample complexity is saved a lot if there are many few-shot learning tasks that share the same low-dimensional subspace to be learned.


==> Paper/Paper_review.tex <==
1068

In the context of multi-task learning, the submitted paper offers a theoretical study in the context where all non-linear tasks are expressed in a common low-dimensional space. In this context of subspace-based representation, he explores the problem of few-shot learning. The results on the terminals are promising in the context studied and various simulations come to support the results. The merit of the article is to open the framework of meta-learning under the formal prism of the theory of non-asymptotic estimation. While such a study is interesting, I regret that the application perspective is not mentioned at all. It seems difficult to find application corresponding to work with around 1000 tasks. I also think that parts of the article are difficult to follow. 

1/ It's a bit of a shame to use the same W notation for the layer parameters and the transformation. Also, it is not clear to me the connection with the Theta parameters of the GLM, especially in the experimental phase. All these notations seem a little confusing to me.

2/ In the first set of simulations, it is logical and obvious that increase the number of tasks offer redundancy for observing the subspace. However, I don’t understand what is exactly the new task and where are the associated results? 

3/ Does this sentence « Observe that, without representation learning, one has to search for both f and P . However with representation learning, we fix P = Uˆ r and only search for f. » related to the last simulation (Fig. 3). It is not clear for me, you tell us « with and without the retrieved representations … » What is the matrix P?

4/ In definition 2.5, you start with the matrix W and then continue with P.

5/ In the eq. 2.7 the Log function of the first term is missing.


281E

The paper addresses the important problem of meta-learning and brings relevant contributions. The analyses are discussed with the help of experimental results obtained from synthetic data. I consider the work sound and pertinent. 


1BAA

1. Theorem 3.2 characterizes the error in the moment estimate \hat M, but the
final estimate required is for the subspace W. Where is the error for the 
rank r estimate \hat W characterized? In particular, the result in Theorem 3.4
is stated in terms of \|\hat W-W\| -- can the authors indicate how this
term behaves with respect to the problem dimensions? It can probably be handled
with some additional results from eigenvalue/eigenvector perturbation theory.


2. This is regarding the comment after Theorem 3.4. Although the few-shot 
learning step only requires roughly r samples, isn't the overall
requirement still dominated by the one from Theorem 3.2 (which amounts
to roughly d samples)? That is, even if the initial learning step can be used to 
enable multiple learning tasks in the second step, isn't it
only some constant gain when compared to learning each of them separately
(since the first step always requires d samples)? It would be useful
if the authors clarify this point.

==> Paper/notation.tex <==

\usepackage{hyperref,graphicx,amsmath,amsfonts,amssymb,bm,url,breakurl,epsfig,epsf,color,MnSymbol,mathbbol,fmtcount,semtrans,caption,subcaption,multirow,comment, boldline, enumitem}
%\usepackage[]{algorithm2e}
%\usepackage[noend]{algpseudocode}
\usepackage{wrapfig}
\usepackage{amssymb}

\usepackage[utf8]{inputenc} % allow utf-8 input
\usepackage[T1]{fontenc}    % use 8-bit T1 fonts
\usepackage{url}            % simple URL typesetting
\usepackage{booktabs}       % professional-quality tables
\usepackage{amsfonts}       % blackboard math symbols
\usepackage{nicefrac}       % compact symbols for 1/2, etc.
\usepackage{microtype}      % microtypography

\makeatletter
\providecommand*{\boxast}{%
  \mathbin{% as \boxplus and \boxtimes
    \mathpalette\@boxit{*}%
  }%
}
\newcommand*{\@boxit}[2]{%
  % #1: math style (\displaystyle, \textstyle, ...)
  % #2: symbol to be boxed that is centered around the math axis
  \sbox0{$\m@th#1\Box$}%
  % Manual correction for font bounding boxes:
  \ifx#1\displaystyle \ht0=\dimexpr\ht0+.05ex\relax \fi
  \ifx#1\textstyle \ht0=\dimexpr\ht0+.05ex\relax \fi
  \ifx#1\scriptstyle \ht0=\dimexpr\ht0+.04ex\relax \fi
  \ifx#1\scriptscriptstyle \ht0=\dimexpr\ht0+.065ex\relax \fi
  \sbox2{$#1\vcenter{}$}% \ht2 is positionn of math axis
  \rlap{%
    \hbox to \wd0{%
      \hfill
      \raisebox{%
        \dimexpr.5\dimexpr\ht0+\dp0\relax-\ht2\relax
      }{$\m@th#1#2$}%
      \hfill
    }%
  }%
  \Box
}
\makeatother

  \makeatletter
\def\BState{\State\hskip-\ALG@thistlm}
\makeatother


  \usepackage{mathtools}
\DeclarePairedDelimiter{\floor}{\lfloor}{\rfloor}

\usepackage{titlesec}

\usepackage{tikz}
\usepackage{pgfplots}
\usetikzlibrary{pgfplots.groupplots}

\setcounter{secnumdepth}{3}

\titleformat{\paragraph}
{\normalfont\normalsize\bfseries}{\theparagraph}{1em}{}
\titlespacing*{\paragraph}
{0pt}{3.25ex plus 1ex minus .2ex}{1.5ex plus .2ex}

\usepackage{movie15}

%\usepackage{caption}
\usepackage[bottom,hang,flushmargin]{footmisc} 

\setlength{\captionmargin}{30pt}

\newcommand{\tsn}[1]{{\left\vert\kern-0.25ex\left\vert\kern-0.25ex\left\vert #1 
    \right\vert\kern-0.25ex\right\vert\kern-0.25ex\right\vert}}

\definecolor{darkred}{RGB}{150,0,0}
\definecolor{darkgreen}{RGB}{0,150,0}
\definecolor{darkblue}{RGB}{0,0,200}
\hypersetup{colorlinks=true, linkcolor=darkred, citecolor=darkgreen, urlcolor=darkblue}

%--------------
\newtheorem{theorem}{Theorem}[section]
\newtheorem{result}{Result}
\newtheorem{problem}{Problem}
\newtheorem{claim}{Claim}
\newtheorem{assumption}{Assumption}
\newtheorem{question}{Question}
\newtheorem{lemma}[theorem]{Lemma}
\newtheorem{corollary}[theorem]{Corollary}
\newtheorem{propo}[theorem]{Proposition}
\newtheorem{definition}[theorem]{Definition}
\newtheorem{condition}[theorem]{Condition}
\newtheorem{conjecture}[theorem]{Conjecture}

\newtheorem{remark}[subsection]{Remark}
\newtheorem{remarks}[subsection]{Remarks}
\newtheorem{example}[subsection]{Example}

%% TT's definitions
\newcommand\tr{{{\operatorname{trace}}}}
\newcommand{\eps}{\varepsilon}
\newcommand{\epsr}{\varepsilon_R}
\newcommand{\mur}{\mu_R}
\newcommand{\bn}{\alpha}
\newcommand{\pp}{{\text{CL}}}
\newcommand{\distas}{\overset{\text{i.i.d.}}{\sim}}
\newcommand{\np}{{n\wedge p}}
\newcommand{\KB}{\bar{K}}
\newcommand{\bG}{\boldsymbol{\Gamma}}
\newcommand{\xw}{\x_{\w}}
\newcommand{\xv}{\x_{\vb}}
\newcommand{\xu}{\x_{\ub}}
\newcommand{\xvt}[1]{\x_{\vb_{#1}}}
\newcommand{\xvtt}[1]{\x_{\vb,#1}}
\newcommand{\xwt}[1]{\x_{#1,\w}}
\newcommand{\xws}[1]{\x_{#1,\ws}}
\newcommand{\xs}{\x_{\ws}}
\newcommand{\yst}{\hat{\y}}
\newcommand{\st}{\star}
\newcommand{\eig}{\text{eigvec}}
\newcommand{\hu}{h}
\newcommand{\ru}{r}
\newcommand{\pbar}{{{\bar{p}}}}
\newcommand{\pbd}{p}
\newcommand{\lay}[1]{{\vct{k}}^{(#1)}}
\newcommand{\lah}[1]{{\vct{\hat{k}}}^{(#1)}}
\newcommand{\lan}{\vct{k}}
\newcommand{\cmp}{P_{\text{nn}}}
\newcommand{\rest}{{\bf{r}}}
\newcommand{\dcp}{\vct{d}^{\text{cnn}}}
\newcommand{\fcp}{\vct{g}^{\text{CNN}}}
\newcommand{\beq}{\begin{equation}}
\newcommand{\nrest}{\bar{n}}
\newcommand{\eeq}{\end{equation}}
\newcommand{\prox}{{{\text{\bf{prox}}}}}
\newcommand{\cov}{{{\text{\bf{cov}}}}}
\newcommand{\ex}{{{\text{\bf{ex}}}}}
\newcommand{\modu}{{{\text{{mod}}}}}
\newcommand{\map}{{{\text{\bf{map}}}}}
\newcommand{\var}[1]{{{\text{\bf{var}}}}[#1]}
\newcommand{\vrn}{\nu}
\newcommand{\func}[1]{{f_{\text{CNN}}}(#1)}
\newcommand{\funh}[1]{{{\hat{f}}_{\text{CNN}}}(#1)}
\newcommand{\funcp}[1]{{f'_{\text{cnn}}}(#1)}
\newcommand{\funcw}[1]{{{{f}}'_{\text{cnn}}}(#1)}
\newcommand{\dev}{{{\text{\bf{dev}}}}}
\newcommand{\meas}{{{\text{\bf{mean}}(\sigma)}}}
\newcommand{\nn}{\nonumber}
\newcommand{\la}{\lambda}
\newcommand{\K}{{K}}
\newcommand{\A}{{\mtx{A}}}
\newcommand{\sfmx}[1]{\text{sfmx}(#1)}
\newcommand{\cat}[1]{\text{Cat}(#1)}
\newcommand{\amp}{\alpha_{\text{cnn}}}
\newcommand{\bOt}{\bigotimes}
\newcommand{\bt}{\boldsymbol{\theta}}
\newcommand{\Bt}{\boldsymbol{\Theta}}
%\newcommand{\nt}{\boldsymbol{n}}

%\newcommand{\bt}{\times}
\newcommand{\robt}[1]{\bigotimes_{\ell=1}^D{#1}_{\ell}}
\newcommand{\robtu}[1]{\bigotimes_{\ell=1}^D{#1}^{(\ell)}}
\newcommand{\bd}{\bigodot}
\newcommand{\kal}{\prod_{i=1}^{D-1}\tn{\lay{i}}}
%\newcommand{\kall}[1]{\prod_{i=1}^{#1}\tn{\lay{i}}}
\newcommand{\kall}[1]{1_{\lan #1}}
\newcommand{\lall}[1]{{\order{\lip_{\lan #1}}}}%{L^{#1}\prod_{i=1}^{#1}\tn{\lay{i}}}
\newcommand{\lell}[1]{{\lip}_{\lan #1}}
\newcommand{\bell}[1]{{{{\beta}}}_{\lan #1}}
\newcommand{\Ub}{{\mtx{U}}}
\newcommand{\Ubb}{{\mtx{U}}}
\newcommand{\V}{{\mtx{V}}}
\newcommand{\ten}{(\{\vb_\ell\}_{\ell=1}^D)}
\newcommand{\uten}{(\{\ub_\ell\}_{\ell=1}^D)}
\newcommand{\ken}{(\{\lay{i}\}_{i=1}^D)}
\newcommand{\B}{{{\mtx{B}}}}
\newcommand{\alx}{{{\alpha_\X}}}
\newcommand{\aly}[1]{{{\alpha_{\X_{#1}}}}}
\newcommand{\Ib}{{{\mtx{I}}}}
\newcommand{\Xbin}{{{\mtx{B}}}}
\newcommand{\Gbin}{{{\mtx{S}}}}
\newcommand{\xbin}{{{\mtx{b}}}}
\newcommand{\Sb}{{{\mtx{S}}}}
\newcommand{\Gb}{{\mtx{G}}}
\newcommand{\ymean}{{\bar{\y}(\w;\text{avg})}}
\newcommand{\yavg}{{{y}_{\text{avg}}}}
\newcommand{\ravg}[1]{{{r}_{{\text{avg}}}(#1)}}
\newcommand{\fmean}{{\funcw{\w;\text{avg}}}}
\newcommand{\diag}[1]{\text{diag}(#1)}
\newcommand{\out}{\text{out}}
\newcommand{\linest}{\text{lin}}
\newcommand{\inp}{\text{in}}
\newcommand{\inh}{\hat{\text{in}}}
\newcommand{\sexp}{subexponential }
\newcommand{\Lc}{{\cal{L}}}
\newcommand{\Nc}{{\cal{N}}}
\newcommand{\Jc}{{\cal{J}}}
\newcommand{\Jcb}{{\overline{\cal{J}}}}
\newcommand{\Dc}{{\cal{D}}}
\newcommand{\Dcg}[1]{{\cal{D}}^{#1}_{\text{subg}}}
\newcommand{\Dct}{{\tilde{\cal{D}}}}
\newcommand{\Sct}{{\tilde{\cal{S}}}}
%\newcommand{\smn}{\s_{\min}}
\newcommand{\btd}{{\bt_{\ell=1}^D d_\ell}}
\newcommand{\Ro}{{\cal{RO}}}
\newcommand{\PC}{{\cal{PC}}}
\newcommand{\Pb}{{\mtx{P}}}
\newcommand{\Tb}{{\mtx{T}}}
\newcommand{\Kba}{{\vct{k}}_{\text{all}}}
\newcommand{\Qb}{{\mtx{Q}}}
\newcommand{\rng}{\gamma}
\newcommand{\Cb}{{\mtx{C}}}
\newcommand{\Eb}{{\mtx{E}}}
\newcommand{\Hb}{{\mtx{H}}}
\newcommand{\Gc}{{\cal{G}}}
\newcommand{\F}{{\mtx{F}}}
\newcommand{\diff}{{\text{diff}}}
\newcommand{\La}{{\boldsymbol{{\Lambda}}}}
%\newcommand{\noresamp}[1]{{\textcolor{red}{#1}}}
\newcommand{\noresamp}[1]{{\textcolor{red}{#1}}}
\newcommand{\sigmap}{\phi'}
\newcommand{\sigmal}[1]{\sigma^{(#1)}}
\newcommand{\sigmalp}[1]{\sigma'^{(#1)}}
\newcommand{\sigmaa}{\sigma'_{\text{all}}}
\newcommand{\sigmai}[1]{\sigma'_{\text{all},#1}}
\newcommand{\bSi}{{\boldsymbol{{\Sigma}}}}
\newcommand{\bSit}{{\boldsymbol{{\tilde{\Sigma}}}}}
\newcommand{\bSih}{{\boldsymbol{{\hat{\Sigma}}}}}
\newcommand{\bmu}{{\boldsymbol{{\mu}}}}
\newcommand{\Db}{{\mtx{D}}}
\newcommand{\db}{{\vct{d}}}
\newcommand{\oneb}{{\mathbb{1}}}
\newcommand{\onebb}{{\mathbf{1}}}
\newcommand{\Iden}{{\mtx{I}}}
\newcommand{\M}{{\mtx{M}}}
\newcommand{\gm}{\gamma_m}
\newcommand{\order}[1]{{\cal{O}}(#1)}
\newcommand{\rmax}[1]{{\bf{r}_{\max}(#1)}}
\newcommand{\rbmax}[1]{{\bf{\bar{r}}_{\max}(#1)}}
\newcommand{\rmin}[1]{{\bf{r}_{\min}(#1)}}
\newcommand{\smn}[1]{{s_{\min}(#1)}}
\newcommand{\smx}[1]{{s_{\max}(#1)}}
\newcommand{\z}{{\vct{z}}}
\newcommand{\zb}{{\bar{\z}}}
\newcommand{\el}{{\ell}}
\newcommand{\tn}[1]{\|{#1}\|_{\ell_2}}
\newcommand{\tff}[1]{\|{#1}\|_{\ell_4}}
\newcommand{\tin}[1]{\|{#1}\|_{\ell_\infty}}
\newcommand{\trow}[1]{\|{#1}\|_{2,\infty}}
\newcommand{\bad}{{\bar{d}}}
\newcommand{\Dp}{{D^+}}
\newcommand{\tf}[1]{\|{#1}\|_{F}}
\newcommand{\te}[1]{\|{#1}\|_{\psi_1}}
\newcommand{\tsub}[1]{\|{#1}\|_{\psi_2}}
\newcommand{\tsut}[1]{\|{#1}\|_{\psi_{2/3}}}
\newcommand{\tsup}[1]{\|{#1}\|_{\psi_a}}
\newcommand{\dist}[1]{\text{dist}(#1)}
\newcommand{\upp}{{\cal{B}}_{\alpha,\Gamma}}
\newcommand{\upz}{{\cal{B}}_{\alpha_0,\Gamma}}
\newcommand{\dpz}{{\cal{D}}_{\alpha_0,\Gamma}}
\newcommand{\dpp}{{\cal{D}}_{\alpha,\Gamma}}
\newcommand{\mpp}{M_{\alpha,\Gamma}}
%\newcommand{\supp}[1]{\text{supp}(#1)}
\newcommand{\cone}[1]{{\text{cone}(#1)}}
\newcommand{\paf}{\partial f(\x)}
\newcommand{\Cc}{\mathcal{C}}
\newcommand{\Ac}{\mathcal{A}}
\newcommand{\Ccb}{\bar{\mathcal{C}}}
\newcommand{\Xc}{\mathcal{X}}
\newcommand{\xc}{{\text{excess}}}
\newcommand{\Rc}{\mathcal{R}}
\newcommand{\Rcp}{\mathcal{\bar{R}}'}
\newcommand{\Rcb}{\mathcal{N}}
\newcommand{\btrue}{\bbeta_{true}}
\newcommand{\bteta}{\boldsymbol{\theta}}
\newcommand{\bbteta}{\widetilde{\boldsymbol{\theta}}}
\newcommand{\brteta}{\overline{\boldsymbol{\theta}}}
\newcommand{\bbeta}{{\boldsymbol{\beta}}}
\newcommand{\ddelta}{{\boldsymbol{\delta}}}
\newcommand{\babeta}{{\bar{\beta}}}
\newcommand{\balpha}{{\bar{\alpha}}}
\newcommand{\bgamma}{{\bar{\gamma}}}
\newcommand{\Bc}{\mathcal{B}}
\newcommand{\Sc}{\mathcal{S}}
\newcommand{\Mc}{\mathcal{M}}
\newcommand{\pa}{{\partial}}
\newcommand{\Nn}{\mathcal{N}}
\newcommand{\pol}{^\circ}
\newcommand{\vb}{\vct{v}}
\newcommand{\Jb}{\mtx{J}}
\newcommand{\Jt}{\mtx{\tilde{J}}}
\newcommand{\vbl}{\vct{v}^{\text{lin}}}
\newcommand{\fb}{\vct{f}}
\newcommand{\ib}{{\bf{i}}}
\newcommand{\hib}{{\bf{\hat{i}}}}
\newcommand{\Ic}{{\mathcal{I}}}
\newcommand{\all}{{\text{all}}}
\newcommand{\vh}{\vct{\hat{v}}}
\newcommand{\vbb}{\vct{\bar{v}}}
\newcommand{\Xb}{\mtx{\bar{X}}}
\newcommand{\abb}{\mtx{\bar{a}}}
\newcommand{\cb}{\mtx{c}}
\newcommand{\bbb}{\mtx{\bar{b}}}
\newcommand{\w}{\vct{w}}
\newcommand{\err}[1]{\text{Err}_{\Dc}(#1)}
\newcommand{\Wp}{\mtx{W}^\dagger}
\newcommand{\tilW}{\widetilde{\mtx{W}}}
\newcommand{\tilw}{\widetilde{\vct{w}}}
\newcommand{\ob}{\mtx{o}}
\newcommand{\obh}{\mtx{\hat{o}}}
\newcommand{\wh}{{\hat{\mtx{w}}}}
\newcommand{\li}{\left<}
\newcommand{\ri}{\right>}
\newcommand{\s}{\vct{s}}
\newcommand{\sh}{\hat{\vct{s}}}
\newcommand{\ab}{\vct{a}}
\newcommand{\bb}{\vct{b}}
\newcommand{\ub}{{\vct{u}}}
\newcommand{\ubb}{\bar{\vct{u}}}
\newcommand{\h}{\vct{h}}
\newcommand{\hh}{{\vct{h}}}
\newcommand{\g}{{\vct{g}}}
\newcommand{\ii}{{\vct{i}}}
\newcommand{\zm}[1]{{\text{{\bf{zm}}}(#1)}}
\newcommand{\dd}{{\vct{d}}}
\newcommand{\ddt}{{\vct{d}}_\tau}
\newcommand{\Zb}{\mtx{Z}}
\newcommand{\hf}{\hat{f}}
\newcommand{\corrCA}{\rho_\Cc(\M)}
\newcommand{\corr}[1]{{\bf{cor}}(#1)}
\newcommand{\Tc}{\mathcal{T}}
\newcommand{\Fc}{\mathcal{F}}
\newcommand{\Hc}{\mathcal{H}}


%%YP's macros
\newcommand{\qqq}[1]{{\textcolor{red}{?{#1}?}}}
\newcommand{\ihere}{{\textcolor{red}{I AM HERE! }}}
\newcommand{\mat}[1]{{\text{mat}{#1}}}
\newcommand{\gb}{\bar{\g}}
\newcommand{\bs}{\bar{s}}
\newcommand{\cgain}{\alpha_{\text{CNN}}}
\newcommand{\cgainp}{\tn{\E_{\x\sim\Nn(0,\Iden)}[\gcnn{}]}}
\newcommand{\gcnn}[1]{{\vct{g}}_{\text{cnn}#1}}
\newcommand{\ccorr}{\rho_{\text{cnn}}}
\newcommand{\kb}{\vct{k}}
\newcommand{\xh}{\hat{\x}}
\newcommand{\yh}{\hat{\y}}
\newcommand{\xbr}{\bar{\h}}
\newcommand{\xdr}{\tilde{\x}}
\newcommand{\m}{\vct{m}}
\newcommand{\xt}{\tilde{\x}}
\newcommand{\nt}{\tilde{n}}
%\newcommand{\ht}{\tilde{h}}
\newcommand{\rt}{\tilde{r}}
\newcommand{\ft}{\tilde{f}}
\newcommand{\yt}{\tilde{\y}}
\newcommand{\gh}{\hat{\g}}
\newcommand{\gt}{\tilde{\g}}
\newcommand{\wb}{\bar{\w}}
\newcommand{\lip}{L}
\newcommand{\mipp}{L_{\max}}
\newcommand{\mupp}{\bar{\mu}_{\max}}
\newcommand{\mapp}{\mu}
\newcommand{\tcnn}{{\mtx{T}}_{\text{cnn}}}
\newcommand{\lcnn}{{\mtx{L}}_{\text{CNN}}}
\newcommand{\lipa}{{L}}
\newcommand{\smo}{S}
\newcommand{\SM}{{{\bf{S}}}_{L,\kb}}
\newcommand{\SMB}{{{\bf{\bar{S}}}}_{L,\kb}}
\newcommand{\Ws}{\W^\star}
\newcommand{\ws}{{\w^\star}}
\newcommand{\wss}{{\w^\star}}
\newcommand{\yp}[1]{\textcolor{red}{ #1}}
\newcommand{\zeronorm}[1]{\left\|#1 \right\|_0}
\newcommand{\unorm}[1]{\left\|#1 \right\|_u}
\newcommand{\ynorm}[1]{\left\|#1 \right\|_{\bar{y}}}
\newcommand{\onetwonorm}[1]{\left\|#1\right\|_{1,2}}
\newcommand{\opnorm}[1]{\left\|#1\right\|}
\newcommand{\fronorm}[1]{\left\|#1\right\|_{F}}
\newcommand{\onenorm}[1]{\left\|#1\right\|_{\ell_1}}
\newcommand{\twonorm}[1]{\left\|#1\right\|_{\ell_2}}
\newcommand{\wnorm}[2]{\left\|#1\right\|_{#2}}
\newcommand{\Dnorm}[1]{\left\|#1\right\|_{D}}
\newcommand{\oneinfnorm}[1]{\left\|#1\right\|_{1,\infty}}
\newcommand{\infnorm}[1]{\left\|#1\right\|_{\ell_\infty}}
\newcommand{\nucnorm}[1]{\left\|#1\right\|_*}
\newcommand{\abs}[1]{\left|#1\right|}
\newcommand{\avg}[1]{\left< #1 \right>}

\newcommand{\lipp}{\prod_{\ell=1}^D \twonorm{\vct{k}^{(\ell)}}}

\renewcommand{\d}{\mathrm{d}}

\newcommand{\cA}{\mathcal{A}}
\newcommand{\rotd}{\text{R1TD}}
\newcommand{\nntd}{\text{DeepTD}}
\newcommand{\x}{\vct{x}}
\newcommand{\rb}{\vct{r}}
\newcommand{\rbb}{\vct{\widetilde{r}}}
\newcommand{\y}{\vct{y}}
\newcommand{\ybh}{\vct{\hat{y}}}
\newcommand{\W}{\mtx{W}}
\newcommand{\Wc}{{\cal{W}}}
\newcommand{\Vc}{{\cal{V}}}
\newcommand{\bgl}{{~\big |~}}

%--------------

% EJC's macros

\definecolor{emmanuel}{RGB}{255,127,0}
\newcommand{\ejc}[1]{\textcolor{emmanuel}{EJC: #1}}

\newcommand{\p}{{\vct{p}}}
\newcommand{\Kb}{{\mtx{K}}}
\newcommand{\somelog}{16\Kb\log (\Kb)}
\newcommand{\somelg}{\Kb\log (\Kb)}
\newcommand{\pb}{{\vct{p}}}
\newcommand{\qb}{{\vct{q}}}
\newcommand{\R}{\mathbb{R}}
\newcommand{\Pro}{\mathbb{P}}
\newcommand{\C}{\mathbb{C}}
\newcommand{\Z}{\mathbb{Z}}
\newcommand{\<}{\langle}
\renewcommand{\>}{\rangle}
\newcommand{\Var}{\textrm{Var}}
\newcommand{\sgn}[1]{\textrm{sgn}(#1)}
\renewcommand{\P}{\operatorname{\mathbb{P}}}
%\newcommand{\E}{\operatorname{\mathbb{E}}}
\newcommand{\EE}{\operatorname{\mathbb{E}}}
%\newcommand{\var}{\operatorname{\mathbf{var}}}

\newcommand{\todo}[1]{{\bf TODO: #1}}
\newcommand{\grad}[1]{{\nabla\Lc(#1)}}
\newcommand{\gradf}[1]{{\nabla f(#1)}}
\newcommand{\hessf}[1]{{\nabla^2f(#1)}}
\newcommand{\gradw}[1]{{\nabla{\Lc}(#1)}}
\newcommand{\grd}[2]{{\nabla\Lc_{#1}(#2)}}
\newcommand{\e}{\mathrm{e}}
\newcommand{\eb}{\vct{e}}
\renewcommand{\i}{\imath}

\newcommand{\vct}[1]{\bm{#1}}
\newcommand{\mtx}[1]{\bm{#1}}

% MS's macros

\newcommand{\rank}{\operatorname{rank}}
\newcommand{\supp}[1]{\operatorname{supp}(#1)}
\newcommand{\restrict}[1]{\big\vert_{#1}}
\newcommand{\Id}{\text{\em I}}
\newcommand{\OpId}{\mathcal{I}}

\newcommand{\Real}{\operatorname{Re}}
\newcommand{\Imag}{\operatorname{Im}}

\newcommand{\piyp}{\pi'_1(\vct{y})}
\newcommand{\piy}{\pi_1(\vct{y})}
\newcommand{\piar}{\pi_1(\vct{a}_r)}
\newcommand{\piarp}{\pi'_1(\vct{a}_r)}
\newcommand{\set}{{\cal{F}}}
\newcommand{\des}{{\x_0}}

\newcommand{\Pc}{{\cal{P}}}
\newcommand{\X}{{\mtx{X}}}
\newcommand{\Y}{{\mtx{Y}}}
\newcommand{\Vb}{{\mtx{V}}}
\newcommand{\Vh}{\hat{{\mtx{V}}}}
\newcommand{\Vbd}{{\mtx{V}^\dagger}}
\newcommand{\Rb}{{\mtx{R}}}

\newcommand{\calF}{\mathcal{I}}
\newcommand{\calS}{\mathcal{N}}


\newcommand{\MS}[1]{\textcolor{blue}{MS: #1}}
\newcommand{\MST}[1]{\textcolor{red}{#1}}
\newcommand{\SO}[1]{\textcolor{darkgreen}{SO: #1}}


\numberwithin{equation}{section} 

\def \endprf{\hfill {\vrule height6pt width6pt depth0pt}\medskip}
%\newenvironment{proof}{\noindent {\bf Proof} }{\endprf\par}
\newenvironment{proofsk}{\noindent {\bf Proof sketch} }{\endprf\par}


%\newcommand{\qed}{{\unskip\nobreak\hfil\penalty50\hskip2em\vadjust{}
           %\nobreak\hfil$\Box$\parfillskip=0pt\finalhyphendemerits=0\par}}


\newcommand{\note}[1]{{\bf [{\em Note:} #1]}}

\newcommand{\iprod}[2]{\left\langle #1 , #2 \right\rangle}

\newcommand{\red}{\textcolor{red}}
\newcommand{\gi}{\ab_{\gamma_i}}
\newcommand{\ang}{\text{ang}}
\newcommand{\ham}[2]{{\|#1,#2\|_H}}

%\renewcommand{\algorithmicrequire}{\textbf{Input:}}
%\renewcommand{\algorithmicensure}{\textbf{Output:}}

%AJ's macros
\newcommand{\hth}{{\widehat{\boldsymbol{\theta}}}}
\newcommand{\bth}{{\boldsymbol{\theta}}}
\newcommand\cL{\mathcal{L}}
\newcommand\cD{\mathcal{D}}
\newcommand\hcD{\widehat{\cD}}
\newcommand\reals{\mathbb{R}}
\newcommand\bSigma{\boldsymbol{\Sigma}}
\newcommand\normal{{\sf N}}
\newcommand\bdelta{\boldsymbol{\delta}}
\newcommand\sign{{\rm sign}}
\newcommand\sT{{\sf T}}
\newcommand\I{\mtx{I}}
\newcommand\zero{\mtx{0}}
\newcommand\bA{\mtx{A}}
\newcommand\bv{\mtx{v}}
\newcommand\cI{\mathcal{I}}
\newcommand\bz{\boldsymbol{z}}
\newcommand\bg{\boldsymbol{g}}
\newcommand\ba{\boldsymbol{a}}
\def\cC{\mathcal{C}}
\def\de{{\rm d}}
\def\bM{\mtx{M}}
\def\cH{\mathcal{H}}
\def\bu{\boldsymbol{u}}
\def\by{\boldsymbol{y}}
\def\bw{\boldsymbol{w}}
\def\bX{\boldsymbol{X}}
\def\tbX{\tilde{\boldsymbol{X}}}
\def\tbx{\tilde{\boldsymbol{x}}}
\def\tbth{\tilde{\boldsymbol{\theta}}}
\def\hz{\widehat{z}}
\def\ind{\mathbf{1}}
\def\cS{\mathcal{S}}
\def\prob{\mathbb{P}}
\def\tx{\tilde{x}}
\def\reals{\mathbb{R}}
\newcommand{\aj}[1]{\noindent{\textcolor{blue}{\textbf{\#\#\# AJ:} \textsf{#1} \#\#\#}}}

\newcommand{\gauss}{\mathcal{N}(0,I)}
\newcommand{\gausscov}[1]{\mathcal{N}(0,{#1})}
\newcommand{\argmin}{\mathop{\mathrm{argmin}}}
%\newcommand{\cLCE}{\cL_{\mathrm{CE}}}
\newcommand{\cLCE}{\cL}
\newcommand{\mscrU}{{\mathscr{U}}}

==> Paper/notation_new.tex <==

\usepackage{hyperref,graphicx,amsmath,amsfonts,amssymb,bm,url,breakurl,epsfig,epsf,color,MnSymbol,mathbbol,fmtcount,semtrans,caption,subcaption,multirow,comment, boldline, enumitem}
%\usepackage[]{algorithm2e}
%\usepackage[noend]{algpseudocode}
\usepackage{wrapfig}
\usepackage{amssymb}


\makeatletter
\providecommand*{\boxast}{%
  \mathbin{% as \boxplus and \boxtimes
    \mathpalette\@boxit{*}%
  }%
}
\newcommand*{\@boxit}[2]{%
  % #1: math style (\displaystyle, \textstyle, ...)
  % #2: symbol to be boxed that is centered around the math axis
  \sbox0{$\m@th#1\Box$}%
  % Manual correction for font bounding boxes:
  \ifx#1\displaystyle \ht0=\dimexpr\ht0+.05ex\relax \fi
  \ifx#1\textstyle \ht0=\dimexpr\ht0+.05ex\relax \fi
  \ifx#1\scriptstyle \ht0=\dimexpr\ht0+.04ex\relax \fi
  \ifx#1\scriptscriptstyle \ht0=\dimexpr\ht0+.065ex\relax \fi
  \sbox2{$#1\vcenter{}$}% \ht2 is positionn of math axis
  \rlap{%
    \hbox to \wd0{%
      \hfill
      \raisebox{%
        \dimexpr.5\dimexpr\ht0+\dp0\relax-\ht2\relax
      }{$\m@th#1#2$}%
      \hfill
    }%
  }%
  \Box
}
\makeatother

  \makeatletter
\def\BState{\State\hskip-\ALG@thistlm}
\makeatother


  \usepackage{mathtools}
\DeclarePairedDelimiter{\floor}{\lfloor}{\rfloor}

%\usepackage{titlesec}

\usepackage{tikz}
\usepackage{pgfplots}
\usetikzlibrary{pgfplots.groupplots}

\setcounter{secnumdepth}{3}


\usepackage{movie15}

%\usepackage{caption}
\usepackage[bottom,hang,flushmargin]{footmisc} 

\setlength{\captionmargin}{30pt}

\newcommand{\tsn}[1]{{\left\vert\kern-0.25ex\left\vert\kern-0.25ex\left\vert #1 
    \right\vert\kern-0.25ex\right\vert\kern-0.25ex\right\vert}}

\definecolor{darkred}{RGB}{150,0,0}
\definecolor{darkgreen}{RGB}{0,150,0}
\definecolor{darkblue}{RGB}{0,0,200}
\hypersetup{colorlinks=true, linkcolor=darkred, citecolor=darkgreen, urlcolor=darkblue}

%--------------

\newtheorem{theorem}{Theorem}[section]
\newtheorem{result}{Result}
\newtheorem{problem}{Problem}
\newtheorem{claim}{Claim}
\newtheorem{assumption}{Assumption}
\newtheorem{question}{Question}
\newtheorem{lemma}[theorem]{Lemma}
\newtheorem{corollary}[theorem]{Corollary}
\newtheorem{propo}[theorem]{Proposition}
\newtheorem{definition}[theorem]{Definition}
\newtheorem{condition}[theorem]{Condition}
\newtheorem{conjecture}[theorem]{Conjecture}

\newtheorem{remark}[subsection]{Remark}
\newtheorem{remarks}[subsection]{Remarks}
\newtheorem{example}[subsection]{Example}

%% TT's definitions
\newcommand\tr{{{\operatorname{trace}}}}
\newcommand{\eps}{\varepsilon}
\newcommand{\epsr}{\varepsilon_R}
\newcommand{\mur}{\mu_R}
\newcommand{\bn}{\alpha}
\newcommand{\pp}{{\text{CL}}}
\newcommand{\distas}{\overset{\text{i.i.d.}}{\sim}}
\newcommand{\np}{{n\wedge p}}
\newcommand{\KB}{\bar{K}}
\newcommand{\bG}{\boldsymbol{\Gamma}}
\newcommand{\xw}{\x_{\w}}
\newcommand{\xv}{\x_{\vb}}
\newcommand{\xu}{\x_{\ub}}
\newcommand{\xvt}[1]{\x_{\vb_{#1}}}
\newcommand{\xvtt}[1]{\x_{\vb,#1}}
\newcommand{\xwt}[1]{\x_{#1,\w}}
\newcommand{\xws}[1]{\x_{#1,\ws}}
\newcommand{\xs}{\x_{\ws}}
\newcommand{\yst}{\hat{\y}}
\newcommand{\st}{\star}
\newcommand{\eig}{\text{eigvec}}
\newcommand{\hu}{h}
\newcommand{\ru}{r}
\newcommand{\pbar}{{{\bar{p}}}}
\newcommand{\pbd}{p}
\newcommand{\lay}[1]{{\vct{k}}^{(#1)}}
\newcommand{\lah}[1]{{\vct{\hat{k}}}^{(#1)}}
\newcommand{\lan}{\vct{k}}
\newcommand{\cmp}{P_{\text{nn}}}
\newcommand{\rest}{{\bf{r}}}
\newcommand{\dcp}{\vct{d}^{\text{cnn}}}
\newcommand{\fcp}{\vct{g}^{\text{CNN}}}
\newcommand{\beq}{\begin{equation}}
\newcommand{\nrest}{\bar{n}}
\newcommand{\eeq}{\end{equation}}
\newcommand{\prox}{{{\text{\bf{prox}}}}}
\newcommand{\cov}{{{\text{\bf{cov}}}}}
\newcommand{\ex}{{{\text{\bf{ex}}}}}
\newcommand{\modu}{{{\text{{mod}}}}}
\newcommand{\map}{{{\text{\bf{map}}}}}
\newcommand{\var}[1]{{{\text{\bf{var}}}}[#1]}
\newcommand{\vrn}{\nu}
\newcommand{\func}[1]{{f_{\text{CNN}}}(#1)}
\newcommand{\funh}[1]{{{\hat{f}}_{\text{CNN}}}(#1)}
\newcommand{\funcp}[1]{{f'_{\text{cnn}}}(#1)}
\newcommand{\funcw}[1]{{{{f}}'_{\text{cnn}}}(#1)}
\newcommand{\dev}{{{\text{\bf{dev}}}}}
\newcommand{\meas}{{{\text{\bf{mean}}(\sigma)}}}
\newcommand{\nn}{\nonumber}
\newcommand{\la}{\lambda}
\newcommand{\K}{{K}}
\newcommand{\A}{{\mtx{A}}}
\newcommand{\sfmx}[1]{\text{sfmx}(#1)}
\newcommand{\cat}[1]{\text{Cat}(#1)}
\newcommand{\amp}{\alpha_{\text{cnn}}}
\newcommand{\bOt}{\bigotimes}
\newcommand{\bt}{\boldsymbol{\theta}}
\newcommand{\Bt}{\boldsymbol{\Theta}}
%\newcommand{\nt}{\boldsymbol{n}}

%\newcommand{\bt}{\times}
\newcommand{\robt}[1]{\bigotimes_{\ell=1}^D{#1}_{\ell}}
\newcommand{\robtu}[1]{\bigotimes_{\ell=1}^D{#1}^{(\ell)}}
\newcommand{\bd}{\bigodot}
\newcommand{\kal}{\prod_{i=1}^{D-1}\tn{\lay{i}}}
%\newcommand{\kall}[1]{\prod_{i=1}^{#1}\tn{\lay{i}}}
\newcommand{\kall}[1]{1_{\lan #1}}
\newcommand{\lall}[1]{{\order{\lip_{\lan #1}}}}%{L^{#1}\prod_{i=1}^{#1}\tn{\lay{i}}}
\newcommand{\lell}[1]{{\lip}_{\lan #1}}
\newcommand{\bell}[1]{{{{\beta}}}_{\lan #1}}
\newcommand{\Ub}{{\mtx{U}}}
\newcommand{\Ubb}{{\mtx{U}}}
\newcommand{\V}{{\mtx{V}}}
\newcommand{\ten}{(\{\vb_\ell\}_{\ell=1}^D)}
\newcommand{\uten}{(\{\ub_\ell\}_{\ell=1}^D)}
\newcommand{\ken}{(\{\lay{i}\}_{i=1}^D)}
\newcommand{\B}{{{\mtx{B}}}}
\newcommand{\alx}{{{\alpha_\X}}}
\newcommand{\aly}[1]{{{\alpha_{\X_{#1}}}}}
\newcommand{\Ib}{{{\mtx{I}}}}
\newcommand{\Xbin}{{{\mtx{B}}}}
\newcommand{\Gbin}{{{\mtx{S}}}}
\newcommand{\xbin}{{{\mtx{b}}}}
\newcommand{\Sb}{{{\mtx{S}}}}
\newcommand{\Gb}{{\mtx{G}}}
\newcommand{\ymean}{{\bar{\y}(\w;\text{avg})}}
\newcommand{\yavg}{{{y}_{\text{avg}}}}
\newcommand{\ravg}[1]{{{r}_{{\text{avg}}}(#1)}}
\newcommand{\fmean}{{\funcw{\w;\text{avg}}}}
\newcommand{\diag}[1]{\text{diag}(#1)}
\newcommand{\out}{\text{out}}
\newcommand{\linest}{\text{lin}}
\newcommand{\inp}{\text{in}}
\newcommand{\inh}{\hat{\text{in}}}
\newcommand{\sexp}{subexponential }
\newcommand{\Lc}{{\cal{L}}}
\newcommand{\Nc}{{\cal{N}}}
\newcommand{\Jc}{{\cal{J}}}
\newcommand{\Jcb}{{\overline{\cal{J}}}}
\newcommand{\Dc}{{\cal{D}}}
\newcommand{\Dcg}[1]{{\cal{D}}^{#1}_{\text{subg}}}
\newcommand{\Dct}{{\tilde{\cal{D}}}}
\newcommand{\Sct}{{\tilde{\cal{S}}}}
%\newcommand{\smn}{\s_{\min}}
\newcommand{\btd}{{\bt_{\ell=1}^D d_\ell}}
\newcommand{\Ro}{{\cal{RO}}}
\newcommand{\PC}{{\cal{PC}}}
\newcommand{\Pb}{{\mtx{P}}}
\newcommand{\Tb}{{\mtx{T}}}
\newcommand{\Kba}{{\vct{k}}_{\text{all}}}
\newcommand{\Qb}{{\mtx{Q}}}
\newcommand{\rng}{\gamma}
\newcommand{\Cb}{{\mtx{C}}}
\newcommand{\Eb}{{\mtx{E}}}
\newcommand{\Hb}{{\mtx{H}}}
\newcommand{\Gc}{{\cal{G}}}
\newcommand{\F}{{\mtx{F}}}
\newcommand{\diff}{{\text{diff}}}
\newcommand{\La}{{\boldsymbol{{\Lambda}}}}
%\newcommand{\noresamp}[1]{{\textcolor{red}{#1}}}
\newcommand{\noresamp}[1]{{\textcolor{red}{#1}}}
\newcommand{\sigmap}{\phi'}
\newcommand{\sigmal}[1]{\sigma^{(#1)}}
\newcommand{\sigmalp}[1]{\sigma'^{(#1)}}
\newcommand{\sigmaa}{\sigma'_{\text{all}}}
\newcommand{\sigmai}[1]{\sigma'_{\text{all},#1}}
\newcommand{\bSi}{{\boldsymbol{{\Sigma}}}}
\newcommand{\bSit}{{\boldsymbol{{\tilde{\Sigma}}}}}
\newcommand{\bSih}{{\boldsymbol{{\hat{\Sigma}}}}}
\newcommand{\bmu}{{\boldsymbol{{\mu}}}}
\newcommand{\Db}{{\mtx{D}}}
\newcommand{\db}{{\vct{d}}}
\newcommand{\oneb}{{\mathbb{1}}}
\newcommand{\onebb}{{\mathbf{1}}}
\newcommand{\Iden}{{\mtx{I}}}
\newcommand{\M}{{\mtx{M}}}
\newcommand{\gm}{\gamma_m}
\newcommand{\order}[1]{{\cal{O}}(#1)}
\newcommand{\rmax}[1]{{\bf{r}_{\max}(#1)}}
\newcommand{\rbmax}[1]{{\bf{\bar{r}}_{\max}(#1)}}
\newcommand{\rmin}[1]{{\bf{r}_{\min}(#1)}}
\newcommand{\smn}[1]{{s_{\min}(#1)}}
\newcommand{\smx}[1]{{s_{\max}(#1)}}
\newcommand{\z}{{\vct{z}}}
\newcommand{\zb}{{\bar{\z}}}
\newcommand{\el}{{\ell}}
\newcommand{\tn}[1]{\|{#1}\|_{\ell_2}}
\newcommand{\tff}[1]{\|{#1}\|_{\ell_4}}
\newcommand{\tin}[1]{\|{#1}\|_{\ell_\infty}}
\newcommand{\trow}[1]{\|{#1}\|_{2,\infty}}
\newcommand{\bad}{{\bar{d}}}
\newcommand{\Dp}{{D^+}}
\newcommand{\tf}[1]{\|{#1}\|_{F}}
\newcommand{\te}[1]{\|{#1}\|_{\psi_1}}
\newcommand{\tsub}[1]{\|{#1}\|_{\psi_2}}
\newcommand{\tsut}[1]{\|{#1}\|_{\psi_{2/3}}}
\newcommand{\tsup}[1]{\|{#1}\|_{\psi_a}}
\newcommand{\dist}[1]{\text{dist}(#1)}
\newcommand{\upp}{{\cal{B}}_{\alpha,\Gamma}}
\newcommand{\upz}{{\cal{B}}_{\alpha_0,\Gamma}}
\newcommand{\dpz}{{\cal{D}}_{\alpha_0,\Gamma}}
\newcommand{\dpp}{{\cal{D}}_{\alpha,\Gamma}}
\newcommand{\mpp}{M_{\alpha,\Gamma}}
%\newcommand{\supp}[1]{\text{supp}(#1)}
\newcommand{\cone}[1]{{\text{cone}(#1)}}
\newcommand{\paf}{\partial f(\x)}
\newcommand{\Cc}{\mathcal{C}}
\newcommand{\Ac}{\mathcal{A}}
\newcommand{\Ccb}{\bar{\mathcal{C}}}
\newcommand{\Xc}{\mathcal{X}}
\newcommand{\xc}{{\text{excess}}}
\newcommand{\Rc}{\mathcal{R}}
\newcommand{\Rcp}{\mathcal{\bar{R}}'}
\newcommand{\Rcb}{\mathcal{N}}
\newcommand{\btrue}{\bbeta_{true}}
\newcommand{\bteta}{\boldsymbol{\theta}}
\newcommand{\bbteta}{\widetilde{\boldsymbol{\theta}}}
\newcommand{\brteta}{\overline{\boldsymbol{\theta}}}
\newcommand{\bbeta}{{\boldsymbol{\beta}}}
\newcommand{\ddelta}{{\boldsymbol{\delta}}}
\newcommand{\babeta}{{\bar{\beta}}}
\newcommand{\balpha}{{\bar{\alpha}}}
\newcommand{\bgamma}{{\bar{\gamma}}}
\newcommand{\Bc}{\mathcal{B}}
\newcommand{\Sc}{\mathcal{S}}
\newcommand{\Mc}{\mathcal{M}}
\newcommand{\pa}{{\partial}}
\newcommand{\Nn}{\mathcal{N}}
\newcommand{\pol}{^\circ}
\newcommand{\vb}{\vct{v}}
\newcommand{\Jb}{\mtx{J}}
\newcommand{\Jt}{\mtx{\tilde{J}}}
\newcommand{\vbl}{\vct{v}^{\text{lin}}}
\newcommand{\fb}{\vct{f}}
\newcommand{\ib}{{\bf{i}}}
\newcommand{\hib}{{\bf{\hat{i}}}}
\newcommand{\Ic}{{\mathcal{I}}}
\newcommand{\all}{{\text{all}}}
\newcommand{\vh}{\vct{\hat{v}}}
\newcommand{\vbb}{\vct{\bar{v}}}
\newcommand{\Xb}{\mtx{\bar{X}}}
\newcommand{\abb}{\mtx{\bar{a}}}
\newcommand{\cb}{\mtx{c}}
\newcommand{\bbb}{\mtx{\bar{b}}}
\newcommand{\w}{\vct{w}}
\newcommand{\err}[1]{\text{Err}_{\Dc}(#1)}
\newcommand{\Wp}{\mtx{W}^\dagger}
\newcommand{\tilW}{\widetilde{\mtx{W}}}
\newcommand{\tilw}{\widetilde{\vct{w}}}
\newcommand{\ob}{\mtx{o}}
\newcommand{\obh}{\mtx{\hat{o}}}
\newcommand{\wh}{{\hat{\mtx{w}}}}
\newcommand{\li}{\left<}
\newcommand{\ri}{\right>}
\newcommand{\s}{\vct{s}}
\newcommand{\sh}{\hat{\vct{s}}}
\newcommand{\ab}{\vct{a}}
\newcommand{\bb}{\vct{b}}
\newcommand{\ub}{{\vct{u}}}
\newcommand{\ubb}{\bar{\vct{u}}}
\newcommand{\h}{\vct{h}}
\newcommand{\hh}{{\vct{h}}}
\newcommand{\g}{{\vct{g}}}
\newcommand{\ii}{{\vct{i}}}
\newcommand{\zm}[1]{{\text{{\bf{zm}}}(#1)}}
\newcommand{\dd}{{\vct{d}}}
\newcommand{\ddt}{{\vct{d}}_\tau}
\newcommand{\Zb}{\mtx{Z}}
\newcommand{\hf}{\hat{f}}
\newcommand{\corrCA}{\rho_\Cc(\M)}
\newcommand{\corr}[1]{{\bf{cor}}(#1)}
\newcommand{\Tc}{\mathcal{T}}
\newcommand{\Fc}{\mathcal{F}}
\newcommand{\Hc}{\mathcal{H}}


%%YP's macros
\newcommand{\qqq}[1]{{\textcolor{red}{?{#1}?}}}
\newcommand{\ihere}{{\textcolor{red}{I AM HERE! }}}
\newcommand{\mat}[1]{{\text{mat}{#1}}}
\newcommand{\gb}{\bar{\g}}
\newcommand{\bs}{\bar{s}}
\newcommand{\cgain}{\alpha_{\text{CNN}}}
\newcommand{\cgainp}{\tn{\E_{\x\sim\Nn(0,\Iden)}[\gcnn{}]}}
\newcommand{\gcnn}[1]{{\vct{g}}_{\text{cnn}#1}}
\newcommand{\ccorr}{\rho_{\text{cnn}}}
\newcommand{\kb}{\vct{k}}
\newcommand{\xh}{\hat{\x}}
\newcommand{\yh}{\hat{\y}}
\newcommand{\xbr}{\bar{\h}}
\newcommand{\xdr}{\tilde{\x}}
\newcommand{\m}{\vct{m}}
\newcommand{\xt}{\tilde{\x}}
\newcommand{\nt}{\tilde{n}}
%\newcommand{\ht}{\tilde{h}}
\newcommand{\rt}{\tilde{r}}
\newcommand{\ft}{\tilde{f}}
\newcommand{\yt}{\tilde{\y}}
\newcommand{\gh}{\hat{\g}}
\newcommand{\gt}{\tilde{\g}}
\newcommand{\wb}{\bar{\w}}
\newcommand{\lip}{L}
\newcommand{\mipp}{L_{\max}}
\newcommand{\mupp}{\bar{\mu}_{\max}}
\newcommand{\mapp}{\mu}
\newcommand{\tcnn}{{\mtx{T}}_{\text{cnn}}}
\newcommand{\lcnn}{{\mtx{L}}_{\text{CNN}}}
\newcommand{\lipa}{{L}}
\newcommand{\smo}{S}
\newcommand{\SM}{{{\bf{S}}}_{L,\kb}}
\newcommand{\SMB}{{{\bf{\bar{S}}}}_{L,\kb}}
\newcommand{\Ws}{\W^\star}
\newcommand{\ws}{{\w^\star}}
\newcommand{\wss}{{\w^\star}}
\newcommand{\yp}[1]{\textcolor{red}{ #1}}
\newcommand{\zeronorm}[1]{\left\|#1 \right\|_0}
\newcommand{\unorm}[1]{\left\|#1 \right\|_u}
\newcommand{\ynorm}[1]{\left\|#1 \right\|_{\bar{y}}}
\newcommand{\onetwonorm}[1]{\left\|#1\right\|_{1,2}}
\newcommand{\opnorm}[1]{\left\|#1\right\|}
\newcommand{\fronorm}[1]{\left\|#1\right\|_{F}}
\newcommand{\onenorm}[1]{\left\|#1\right\|_{\ell_1}}
\newcommand{\twonorm}[1]{\left\|#1\right\|_{\ell_2}}
\newcommand{\wnorm}[2]{\left\|#1\right\|_{#2}}
\newcommand{\Dnorm}[1]{\left\|#1\right\|_{D}}
\newcommand{\oneinfnorm}[1]{\left\|#1\right\|_{1,\infty}}
\newcommand{\infnorm}[1]{\left\|#1\right\|_{\ell_\infty}}
\newcommand{\nucnorm}[1]{\left\|#1\right\|_*}
\newcommand{\abs}[1]{\left|#1\right|}
\newcommand{\avg}[1]{\left< #1 \right>}

\newcommand{\lipp}{\prod_{\ell=1}^D \twonorm{\vct{k}^{(\ell)}}}

\renewcommand{\d}{\mathrm{d}}

\newcommand{\cA}{\mathcal{A}}
\newcommand{\rotd}{\text{R1TD}}
\newcommand{\nntd}{\text{DeepTD}}
\newcommand{\x}{\vct{x}}
\newcommand{\rb}{\vct{r}}
\newcommand{\rbb}{\vct{\widetilde{r}}}
\newcommand{\y}{\vct{y}}
\newcommand{\ybh}{\vct{\hat{y}}}
\newcommand{\W}{\mtx{W}}
\newcommand{\Wc}{{\cal{W}}}
\newcommand{\Vc}{{\cal{V}}}
\newcommand{\bgl}{{~\big |~}}

%--------------

% EJC's macros

\definecolor{emmanuel}{RGB}{255,127,0}
\newcommand{\ejc}[1]{\textcolor{emmanuel}{EJC: #1}}

\newcommand{\p}{{\vct{p}}}
\newcommand{\Kb}{{\mtx{K}}}
\newcommand{\somelog}{16\Kb\log (\Kb)}
\newcommand{\somelg}{\Kb\log (\Kb)}
\newcommand{\pb}{{\vct{p}}}
\newcommand{\qb}{{\vct{q}}}
\newcommand{\R}{\mathbb{R}}
\newcommand{\Pro}{\mathbb{P}}
\newcommand{\C}{\mathbb{C}}
\newcommand{\Z}{\mathbb{Z}}
\newcommand{\<}{\langle}
\renewcommand{\>}{\rangle}
\newcommand{\Var}{\textrm{Var}}
\newcommand{\sgn}[1]{\textrm{sgn}(#1)}
\renewcommand{\P}{\operatorname{\mathbb{P}}}
%\newcommand{\E}{\operatorname{\mathbb{E}}}
\newcommand{\EE}{\operatorname{\mathbb{E}}}
%\newcommand{\var}{\operatorname{\mathbf{var}}}

\newcommand{\todo}[1]{{\bf TODO: #1}}
\newcommand{\grad}[1]{{\nabla\Lc(#1)}}
\newcommand{\gradf}[1]{{\nabla f(#1)}}
\newcommand{\hessf}[1]{{\nabla^2f(#1)}}
\newcommand{\gradw}[1]{{\nabla{\Lc}(#1)}}
\newcommand{\grd}[2]{{\nabla\Lc_{#1}(#2)}}
\newcommand{\e}{\mathrm{e}}
\newcommand{\eb}{\vct{e}}
\renewcommand{\i}{\imath}

\newcommand{\vct}[1]{\bm{#1}}
\newcommand{\mtx}[1]{\bm{#1}}

% MS's macros

\newcommand{\rank}{\operatorname{rank}}
\newcommand{\supp}[1]{\operatorname{supp}(#1)}
\newcommand{\restrict}[1]{\big\vert_{#1}}
\newcommand{\Id}{\text{\em I}}
\newcommand{\OpId}{\mathcal{I}}

\newcommand{\Real}{\operatorname{Re}}
\newcommand{\Imag}{\operatorname{Im}}

\newcommand{\piyp}{\pi'_1(\vct{y})}
\newcommand{\piy}{\pi_1(\vct{y})}
\newcommand{\piar}{\pi_1(\vct{a}_r)}
\newcommand{\piarp}{\pi'_1(\vct{a}_r)}
\newcommand{\set}{{\cal{F}}}
\newcommand{\des}{{\x_0}}

\newcommand{\Pc}{{\cal{P}}}
\newcommand{\X}{{\mtx{X}}}
\newcommand{\Y}{{\mtx{Y}}}
\newcommand{\Vb}{{\mtx{V}}}
\newcommand{\Vh}{\hat{{\mtx{V}}}}
\newcommand{\Vbd}{{\mtx{V}^\dagger}}
\newcommand{\Rb}{{\mtx{R}}}

\newcommand{\calF}{\mathcal{I}}
\newcommand{\calS}{\mathcal{N}}


\newcommand{\MS}[1]{\textcolor{blue}{MS: #1}}
\newcommand{\MST}[1]{\textcolor{red}{#1}}
\newcommand{\SO}[1]{\textcolor{darkgreen}{SO: #1}}


\numberwithin{equation}{section} 

\def \endprf{\hfill {\vrule height6pt width6pt depth0pt}\medskip}
%\newenvironment{proof}{\noindent {\bf Proof} }{\endprf\par}
\newenvironment{proofsk}{\noindent {\bf Proof sketch} }{\endprf\par}


%\newcommand{\qed}{{\unskip\nobreak\hfil\penalty50\hskip2em\vadjust{}
           %\nobreak\hfil$\Box$\parfillskip=0pt\finalhyphendemerits=0\par}}


\newcommand{\note}[1]{{\bf [{\em Note:} #1]}}

\newcommand{\iprod}[2]{\left\langle #1 , #2 \right\rangle}

\newcommand{\red}{\textcolor{red}}
\newcommand{\gi}{\ab_{\gamma_i}}
\newcommand{\ang}{\text{ang}}
\newcommand{\ham}[2]{{\|#1,#2\|_H}}

%\renewcommand{\algorithmicrequire}{\textbf{Input:}}
%\renewcommand{\algorithmicensure}{\textbf{Output:}}

%AJ's macros
\newcommand{\hth}{{\widehat{\boldsymbol{\theta}}}}
\newcommand{\bth}{{\boldsymbol{\theta}}}
\newcommand\cL{\mathcal{L}}
\newcommand\cLoss{\mathrm{loss}}
\newcommand\cD{\mathcal{D}}
\newcommand\hcD{\widehat{\cD}}
\newcommand\reals{\mathbb{R}}
\newcommand\bSigma{\boldsymbol{\Sigma}}
\newcommand\normal{{\sf N}}
\newcommand\bdelta{\boldsymbol{\delta}}
\newcommand\sign{{\rm sign}}
\newcommand\sT{{\sf T}}
\newcommand\I{\mtx{I}}
\newcommand\zero{\mtx{0}}
\newcommand\bA{\mtx{A}}
\newcommand\bv{\mtx{v}}
\newcommand\cI{\mathcal{I}}
\newcommand\bz{\boldsymbol{z}}
\newcommand\bg{\boldsymbol{g}}
\newcommand\ba{\boldsymbol{a}}
\def\cC{\mathcal{C}}
\def\de{{\rm d}}
\def\bM{\mtx{M}}
\def\cH{\mathcal{H}}
\def\bu{\boldsymbol{u}}
\def\by{\boldsymbol{y}}
\def\bw{\boldsymbol{w}}
\def\bX{\boldsymbol{X}}
\def\tbX{\tilde{\boldsymbol{X}}}
\def\tbx{\tilde{\boldsymbol{x}}}
\def\tbth{\tilde{\boldsymbol{\theta}}}
\def\hz{\widehat{z}}
\def\ind{\mathbf{1}}
\def\cS{\mathcal{S}}
\def\prob{\mathbb{P}}
\def\tx{\tilde{x}}
\def\reals{\mathbb{R}}
\newcommand{\aj}[1]{\noindent{\textcolor{blue}{\textbf{\#\#\# AJ:} \textsf{#1} \#\#\#}}}

\newcommand{\gauss}{\mathcal{N}(0,I)}
\newcommand{\gausscov}[1]{\mathcal{N}(0,{#1})}
\newcommand{\argmin}{\mathop{\mathrm{argmin}}}
%\newcommand{\cLCE}{\cL_{\mathrm{CE}}}
\newcommand{\cLCE}{\cL}
\newcommand{\mscrU}{{\mathscr{U}}}

==> Paper/s_gen_loss_proof.tex <==

\section{Proof of main theorems}

\iffalse
\SO{Clearly Theorem \ref{thm:hatM append} is a restatement of Theorem \ref{thm:hatM}. Why don't you say so? Reader is not expected to figure out this by himself. Let us make things clear.}

\SO{Similarly, where is proof of Lemma 3.1? Looks like Lemma \ref{lem:mean nn} is its restatement but again not clear at all for reader. They cannot find proof of Lemma 3.1 in the text.}

\SO{Here is the organization we need: In the appendix, proof of each technical result in the main text is supposed to have its own subsection. Just like this subsection that I added i.e.~Proof of Theorem \ref{thm:hatM}.}
\SO{Maybe briefly describe the outline. Right now, little confusing due to Lemmas within the proof so outline would help i.e.~we first prove Lemma ... which shows ...}
\subsection{Proof of Lemma \ref{lem:M exp} and Theorem \ref{thm:hatM}}
\fi
We sketch the proof at the beginning. First we compute the expectation of $y\x$ in Lemma \ref{lem:mean nn}. That leads to the proof of Lemma \ref{lem:M exp}. Then in Lemma \ref{lem:err_yx} we bound the difference between sum of $y\x$ and its mean using concentration. The concentration of covariance estimator is studied later in Lemma \ref{lem:Zj} and \ref{lem:Zj2}, which leads to Theorem \ref{thm:hatM}.

\subsubsection{Proof of Lemma \ref{lem:M exp}}
We first state Lemma \ref{lem:M exp} below.
\begin{lemma}\label{lem:M exp append}
Let 
\begin{subequations}\label{eq:hatM append}
\begin{align}
\hat\bM &= \mathop{\Scale[1.8]{\sum}}_{j=1}^k \frac{2}{n_j^2}\left[(\sum_{i=1}^{n_j/2} \yij\xij) (\sum_{i=n_j/2+1}^{n_j} \yij\xij)^\top \right.\\
&\quad\quad\quad\quad \left. +  ( \sum_{i=n_j/2+1}^{n_j} \yij\xij) ( \sum_{i=1}^{n_j/2} \yij\xij)^\top\right].\nonumber
\end{align}
\end{subequations}
And
\begin{align*}
    &\mtx{h}^j(\W): \R^{r\times d} \rightarrow \R^d = \mtx{E}_{\x}[f^j(\W \x)\x]\\
    &\bM := \W^\top\W\left(\frac{1}{k}\sum_{j=1}^k \mtx{h}^j(\W)( \mtx{h}^j(\W))^\top\right)\W^\top\W.
\end{align*}
Then $\bM,\hat{\bM}$ satisfies the following. (a) $\text{rank}(\bM)\leq r$. (b) $\text{range-space}(\bM)\subset \text{row-space}(\W)$. (c) $\mtx{E}[\hat{\M}]=\bM$. 
\end{lemma}
\begin{proof}
Part (a) and (b) are easy to see. $\W\in\R^{r\times d}$ so that $\text{rank}(\bM)\leq r$, and since $\bM$ is the product of $\W^\top$ and another matrix, then  $\text{range-space}(\bM)\subset \text{row-space}(\W)$.
Now we will prove Part (c). We first give the lemma for the mean of the random vector $y\x$.

\begin{lemma}\label{lem:mean nn}
We assume that the data is generated as in Def. \ref{def:task}, and we study the $j$-th task whose activation function is $f^j$. 
%{\color{blue} To be finished}
Define
\begin{align*}
    \mtx{h}^j(\W): \R^{r\times d} \rightarrow \R^d = \mtx{E}_{\x\sim\gauss} f^j(\W \x)  \x
\end{align*}
Denote the joint distribution of $(\x,y)$ as $\Pxy$.
Then $\mtx{E}_{(\x,y)\sim\Pxy}(y \x) = \W^\top\W \mtx{h}^j(\W)$.
\end{lemma}

\emph{Proof of Lemma \ref{lem:mean nn}.} The expectation can be expanded as
\begin{align*}
    &\mtx{E}_{(\x,y)\sim\Pxy}(y \x) \\
    &= \mtx{E}_{\x\sim\gauss} f^j(\W \x) \x\\
    &= \mtx{E}_{\x\sim\gauss} \left(f^j(\W \x)  \W^\top\W \x + f^j(\W \x) (I - \W^\top\W)\x \right).
\end{align*}
Note that, because $\x\sim\gauss$ so $\W \x$ and $(I - \W^\top\W)\x$ are Gaussian. $\W\W^\top = I$ implies 
\begin{align*}
    &\quad \Eb (\W \x)\x^\top((I - \W^\top\W))\\
    &= \W(I - \W^\top\W) = 0.
\end{align*}
So $\W \x$ and $(I - \W^\top\W)\x$ are independent, so 
\begin{align*}
    &\quad \mtx{E}_{\x\sim\gauss}  f^j(\W \x) (I - \W^\top\W)\x \\
    &= (\mtx{E}_{\x\sim\gauss}  f^j(\W \x)) (\mtx{E}_{\x\sim\gauss} (I - \W^\top\W)\x) = 0
\end{align*}
Then 
\begin{align*}
    \mtx{E}_{(\x,y)\sim\Pxy}(y \x) &= \W^\top\W(\mtx{E}_{\x\sim\gauss} f^j(\W \x) \x)\\
    &= \W^\top\W \h_j(\W).
\end{align*}

Denote 
\begin{align}\label{eq:Hj def}
    \Hb^j(\W) = \W^\top\W \mtx{h}^j(\W)
\end{align}
Because $\frac{2}{n_j}\sum_{i=1}^{n_j/2} \yij\xij$
and 
$\frac{2}{n_j}\sum_{i={n_j/2}+1}^{n_j} \yij\xij$ 
are independent, and their expectation are both $\Hb^j(\W)$, so that
\begin{align*}
    &\quad \mtx{E}(\frac{2}{n_j}\sum_{i=1}^{n_j/2} \yij\xij)(\frac{2}{n_j}\sum_{i={n_j/2}+1}^{n_j} \yij\xij)^\top \\
    &= \Hb^j(\W)(\Hb^j(\W))^\top.
\end{align*}
At then end
\begin{align*}
    \hat \bM &= \frac{1}{k}\sum_{j=1}^k \mtx{E}(\frac{2}{n_j}\sum_{i=1}^{n_j/2} \yij\xij)(\frac{2}{n_j}\sum_{i={n_j/2}+1}^{n_j} \yij\xij)^\top,\\
    \bM &= \frac{1}{k}\sum_{j=1}^k\Hb^j(\W)(\Hb^j(\W))^\top,
\end{align*}
so we can prove Part (c) that $\mtx{E}(\hat \bM) = \bM$.
\end{proof}


\subsubsection{Proof of Theorem \ref{thm:hatM}}
We restate Theorem \ref{thm:hatM append} below. 
\begin{theorem}\label{thm:hatM append}
Suppose the data is generated as Def. \ref{def:task}. Let $\delta\in(0,1)$, $\epsilon\in(0,1)$. Suppose $y\x$ is a subGaussian random vector with covariance upper bounded by
\begin{align}
   \| \mathbf{Cov}(y \x) \| \le \sigma^2. \label{eq:covyx append}
\end{align} 
Define
\begin{align*}
    \mtx{h}^j(\W): \R^{r\times d} \rightarrow \R^d = \mtx{E}_{\x\sim\gauss} f^j(\W \x)  \x
\end{align*}
And let %$\bM = \mtx{E}_{\theta\sim\mathcal{N}(0,\bSi)} (g(\theta))^2\frac{\theta\theta^\top}{\|\theta\|^2}$, then
\begin{align*}
    \bM = \W^\top\W\left(\frac{1}{k}\sum_{j=1}^k \mtx{h}^j(\W)( \mtx{h}^j(\W))^\top\right)\W^\top\W
\end{align*}
Then there exists a constant $c$, with probability at least $1-\delta$, let 
\begin{align*}
    k = \frac{cd}{n}\log^2(\frac{kd}{\delta}) \max\{\frac{1}{\epsilon^2}, \frac{1}{\epsilon} \log(\frac{kd}{\delta})\}
\end{align*}
we have 
\begin{align*}
    \|\hat \bM - \bM\| \le \epsilon\sigma^2.
\end{align*}
\end{theorem}
\begin{proof}
The following lemmas are similar to \cite{kong2020meta} Section A.1. We extend the concentration inequalities from bounded random vectors to Gaussian random vectors. For completeness we place the lemmas here.

\begin{lemma}\label{lem:err_yx}
(\cite{jin2019short} Cor. 7) 
Let $\|\mathbf{Cov}(y\x)\| \le \sigma^2$, $\delta\in(0,1)$, $t>0$, $\Hb^j(\W)$ be defined in \eqref{eq:Hj def}. With probability $1-\delta$, there exists a constant $c>0$ such that for every $j$,
%\som{Remind the exact assumption on $\sigma$}
\begin{align}
   \|\frac{1}{t}\sum_{i=1}^t \yij\xij - \Hb^j(\W)\| \le c\sigma\sqrt{\frac{d}{t}\log(\frac{kd}{\delta})} \label{eq:gauss_bern}
\end{align}
%\som{Call $\W^\top\W \mtx{h}^j(\W)$ something for simpler notation}
Denote this event as $\mathcal{E}$.
\iffalse
{\it\color{red} for every i,j pairs ? }Denote this event as $\mathcal{E}$.
{\it \color{red} if we dont say "for every i,j pairs" ,k should not appear in an inequality which holds for only one task. Also maybe it is better to  cite [21] A.5, because [28] Cor.7 says only the following
$$\|\frac{1}{t}\sum_{i=1}^t \yij\xij - \W^\top\W \mtx{h}^j(\W)\| \le c\sigma\sqrt{\frac{1}{t}\log(\frac{2d}{\delta})}$$}
\fi
\end{lemma}
With the covariance of $y\x$ being bounded by $\sigma^2$, the following inequalities are true \cite{kong2020meta}.
\begin{align*}
    \Eb\left( (\vb^T\cdot (\frac{1}{t}\sum_{i=1}^t \yij\xij - \theta^j))^2\right) &\le \sigma^2 / t,\mbox{~for~} \|\vb\|=1.\\
    \Eb \left(\|\frac{1}{t}\sum_{i=1}^t \yij\xij - \theta^j \|^2\right) &\le \sigma^2d/t.
\end{align*}


\begin{lemma}\label{lem:Zj}
Define
\begin{align*}
    \Zb_j &= (\frac{2}{n_j}\sum_{i=1}^{n_j/2} \yij\xij)(\frac{2}{n_j}\sum_{i={n_j/2}+1}^{n_j} \yij\xij)^\top \\
    &\quad - \Hb^j(\W)(\Hb^j(\W))^\top,
\end{align*}
Then there exists a constant $c$ such that on the event $\mathcal{E}$ (thus with probability $1-\delta$), for all $j=1,...,k$, 
\begin{align}
    \|\Zb_j \| \le \frac{c\sigma^2d}{n_j} \log(\frac{kd}{\delta}). \label{eq:evt}
\end{align}
\end{lemma}

% {\it \color{red} From my understanding we should have 
% $$\|\Zb_j \| \le (Eq A.1 Bound)(Eq. A.1 bound + 2\|\W^\top\W \mtx{h}^j(\W)\|)$$ choosing $t=\dfrac{n_j}{2}$ then we have $$\|\Zb_j \| \le (c\sigma\sqrt{\frac{2}{n_j}\log(\frac{2d}{\delta})})(c\sigma\sqrt{\frac{2}{n_j}\log(\frac{2d}{\delta})} + 2\|\W^\top\W \mtx{h}^j(\W)\|)$$
% This is more or less what you have found, but the difference is k in $\log$ term and d term }



The proof is almost same as \cite{kong2020meta}, the only difference is that we replace the bound in (\cite{kong2020meta} Prop A.1) by \eqref{eq:gauss_bern}. With the similar replacement, we propose the following lemma. 
\begin{lemma}\label{lem:Zj2}
Let $\delta\in(0,1)$. There exists a constant $c$, such that for any $\epsilon\in(0,1)$, and 
\begin{align}
    k = \frac{cd}{n_j}\log^2(\frac{kd}{\delta}) \max\{\frac{1}{\epsilon^2}, \frac{1}{\epsilon} \log(\frac{kd}{\delta})\}, \label{eq:k lb}
\end{align}
with probability $1-\delta$, 
\begin{align*}
    \|\frac{1}{k} \sum_{j=1}^k \Zb_j\| \le \epsilon \sigma^2.
\end{align*}
\end{lemma}
This means that when \eqref{eq:k lb} is true, with probability $1-\delta$,
\begin{align*}
    \left\|\hat \bM - \W^\top\W\left(\frac{1}{k}\sum_{j=1}^k \mtx{h}^j(\W)( \mtx{h}^j(\W))^\top\right)\W^\top\W\right\| \le \epsilon \sigma^2.
\end{align*}
Note that $\bM$ is defined as \[\bM=\W^\top\W\left(\frac{1}{k}\sum_{j=1}^k \mtx{h}^j(\W)( \mtx{h}^j(\W))^\top\right)\W^\top\W.\] So we have proven that with probability $1-\delta$,
\begin{align*}
    \left\|\hat \bM - \bM\right\| \le \epsilon \sigma^2.
\end{align*}

%\som{Remind that this is $\hat \bM-\bM$ i.e. $\bM=\text{the messy sum}$}
\end{proof}

%\SO{Create a subsection here!!! Reduce the confusion as much as possible, make transitions smooth.}
\subsection{Proof of Theorem \ref{thm:down}}
Now we will prove Theorem \ref{thm:down}. We first review the notations and assumptions mentioned in the theorem.

\subsubsection{Review of Notations and Assumptions}
We define the SVD of $\hat \bM$ as $\hat \Ub \hat\La \hat\Vb^\top$. Let the first $r$ columns of $\hat \Ub$ be $\Ub_r$. 

Let $\hat\W$ be defined as 
\begin{align}
    \hat \W &= \hat \Ub_r \hat \Qb, \label{eq:def W append}\\
    \hat \Qb &= \mathop{\mathrm{argmin}}_{\Qb\in\R^{r\times r}, \Qb\Qb^\top = I}\ \|\hat \Ub_r \Qb - \W\|.
\end{align}
The population cross entropy loss is defined as
\begin{align*}
    &\cLCE(f;\Pb) : \Fc\times \R^{r\times d}\rightarrow \R=\\
    &-\mtx{E}_{\x,y\sim\Pxy} (y\log f(\hat\Pb \x) + (1-y)\log (1 - f(\hat\Pb \x))).
\end{align*}
We will search for a function $f^* \in \Fc$.% that minimizes the population cross entropy loss. 
\begin{assumption}\label{append ass:F}
$\Fc$ is a set of functions satisfying: For any function $f\in\Fc$, any orthonormal matrix $\Qb\in\R^{r\times r}$ and any matrix $\Pb\in\R^{r\times d}$, there exists $g \in \Fc$ such that $f(\Pb \x) = g(\Qb\Pb \x)$.
%\begin{enumerate}
%    \item For any function $f\in\Fc$, any orthonormal matrix $\Qb\in\R^{r\times r}$ and any matrix $\Pb\in\R^{r\times d}$, there exists $g \in \Fc$ such that $f(\Pb \x) = g(\Qb\Pb \x)$.
%    \item $\Fc \subseteq \{f\ |\ \log f,~ \log(1-f)\mathrm{~are~}L\mathrm{~Lipschitz}\}\bigcap \{f\ |\ 0<f(x)<1,\forall x\in\R^r\}$.
%\end{enumerate}
\end{assumption}
Now we define a general loss function $\cL$ and $\cL_e$.
\begin{assumption}\label{append ass:L}
Suppose $\cL$ satisfies the following assumptions:
\begin{enumerate}
    \item %$\cL$ takes $f(\Pb x)$ as the argument, i.e., 
    $\cL$ has the form $\cL(f;\Pb) = \mtx{E}_{\Pxy}\Lcs(f(\Pb \x),y)$. $\cL_e$ has the form $\cL_e(f;\Pb) = \frac{1}{n}\sum_{i=1}^n\Lcs(f(\Pb \x_i),y_i)$.
    \item $\Lcs$ is $L$ Lipschitz in $\Pb \x$.
    \item $\min_{\Pb}\cL(f;\Pb) = \cL(f;\W)$.
\end{enumerate}
\end{assumption}
We solve for $\hat f$, defined as \begin{align}
    \hat f &= \argmin_{f\in\Fc}\ \cLCE(f;\hat \Ub_r^\top). \label{eq:def f append}
\end{align}
\subsubsection{Proof of Theorem \ref{thm:down}}
Now we are ready to restate Theorem \ref{thm:down} and prove it.

\begin{theorem}\label{thm:popu append}
With Assumptions \ref{append ass:F} and \ref{append ass:L}, we have that
    \begin{align*}
        \cLCE(\hat f;\hat \Ub_r^\top)  - \cLCE(f^*;\Ub_r^\top) \lesssim L\sqrt{r}\|\hat \W - \W\|.
    \end{align*}
\end{theorem}

\begin{proof}
We learn the model from the following optimization algorithm.
\begin{align*}
    \hat f &= \argmin_{f\in\Fc}\ \cLCE(f;\hat \Ub_r^\top)
    %\\
    %&= \argmin_{f\in\Fc}\ -\mtx{E}_{\x,y\sim\Pxy} (y\log f(\hat\Ub_r^\top \x) \\
    %&\quad + (1-y)\log (1 - f(\hat\Ub_r^\top \x)))\\
    %&= \argmin_{f\in\Fc}\ -\mtx{E}_{\x\sim\gauss} \left(f^*(\W \x)\log f(\hat \Ub_r^\top \x)\right. \\
    %& \quad \left. + (1-f^*(\W \x))\log (1 - f(\hat \Ub_r^\top \x)) \right).
\end{align*}
Denote $\tilde f\in\Fc$ as the function such that $\tilde f(\hat \W \x) = \hat f(\hat \Ub_r^\top \x)$. So that $\cLCE(\hat f;\hat \Ub_r^\top) = \cLCE(\tilde f;\hat \W)$. Since $\hat f$ minimizes the cross entropy loss, we have that $\cLCE(\tilde f;\hat \W) \le \cLCE(f^*;\hat \W)$. 

Now we have 
\begin{align*}
    &\quad \cLCE (\tilde f;\hat \W) - \cLCE (f^*;\W)\\
    &\le \cLCE (f^*;\hat \W) - \cLCE (f^*;\W)\\
    %&\le -\mtx{E}_{\x\sim\gauss} \left(f^*(\W \x)(\log f^*(\hat\W \x) -\log f^*(\W \x))\right. \\
    %& \quad \left. + (1-f^*(\W \x))(\log (1 - f^*(\hat \W \x)) - \log (1 - f^*(\W \x))) \right)\\
    &\le \mtx{E}_{\x\sim\gauss} L\|(\hat \W - \W)x\|\\
    &\lesssim L\sqrt{r}\|\hat \W - \W\|.
\end{align*}
The last step uses the fact that $\hat \W$ and $\W$ are rank $r$.
\end{proof}

\subsection{Proof of Theorem \ref{thm:rade}}
%Now we prove that the upper bound of the error for few-shot learning with finite samples.
We first state Theorem \ref{thm:rade} below.
\begin{theorem}\label{thm:rade app}
    Suppose we generate $n$ sample data for few shot learning solve for $\hat \theta_e$ from 
    \begin{align}
   	 \hat \bt_e &= \argmin_{\bt}\ \cL_e(\bt;\Ub_r^\top)\quad\text{such~that}\quad\|\bt\|_2\le a.\label{eq:fstar finite theta append}
	\end{align}
   Suppose Assumptions \ref{append ass:F} and \ref{append ass:L} hold.
    There exist constants $c>0$, $\delta\in(0,1)$, with probability at least $1 - n^{-c+1} - \delta$, the solution $\hat\theta_e$ and $\hat\Ub_r$ satisfy
    \begin{align*}
        &\quad \mathcal{L} (\hat\theta_e;\hat\Ub_r^\top) - \mathcal{L} (\theta^*;\W) \\
        &\lesssim \frac{caL(\sqrt{r}+\log(n)) (1+ \sqrt{\log(1/\delta)})}{\sqrt{n}} + L\sqrt{r}\|\hat \W - \W\|. 
    \end{align*}
\end{theorem}
\begin{proof}
We sketch the proof of Theorem \ref{thm:rade app}. After reviewing the notations, we quote a standard generalization bound via Rademacher complexity in Lemma \ref{lem:rade known}. Then we use the smoothness of the loss function to link to the generalization error of linear functions \eqref{eq:lin rade}, and then use Lemma \ref{lemma:chi-sqr} to compute \eqref{eq:lin rade} and finish the proof.

In few-shot learning, the true parameter is $\theta^*$, and the empirical loss function with finite data is 
\begin{align}
    &\cL_e(\theta;\Pb) : \Fc\times \R^{r\times d}\rightarrow \R= \frac{1}{n}\sum_{i=1}^n \Lcs(f(\Pb\x_i), y_i)
    %\notag\\
    %&-\frac{1}{n}\sum_{i=1}^n (y_i\log\phi (\theta^\top\Pb \x_i) + (1-y_i)\log (1 - \phi(\theta^\top\Pb \x_i))) \label{eq:cLCE finite theta app}
\end{align}
Denote each term in the summation as 
\begin{align*}
    &\quad \cL_e^i(\theta;\Pb) : \Fc\times \R^{r\times d}\rightarrow \R = \Lcs(f(\Pb\x_i), y_i).
    %=\notag\\
    %&- (y_i\log \phi (\theta^\top\Pb \x_i) + (1-y_i)\log (1 - \phi(\theta^\top\Pb \x_i)))
\end{align*}
We search for the solution by
\begin{align}
    \hat \theta_e &= \argmin_{\theta}\ \cL_e(\theta;\Ub_r^\top),\mbox{~such~that~} \|\theta\|\le a.\label{eq:fstar finite theta app}
\end{align}
In Theorem \ref{thm:popu append}, we know that
\begin{align*}
    \cLCE(\hat \theta;\hat \Ub_r^\top)  - \cLCE(\theta^*;\Ub_r^\top) \lesssim L\sqrt{r}\|\hat \W - \W\|.
\end{align*}
Denote 
    \begin{align}
        M = \max_{\|\theta\|\le a} |\theta^\top \hat\Ub_r^\top\x_i| \le a \max\|\hat\Ub_r^\top\x_i\|.\label{eq:bound_rade}
    \end{align}
We will bound the difference between $\cL$ and $\cL_e$ by Rademacher complexity theory.
\begin{lemma}\label{lem:rade known}
    \cite{mohri2018foundations}
 
    Let $\mscrU$ be the independent random variables uniformly chosen from $\{-1,1\}$.
    Let $\Rc$ be the Rademacher complexity of the logistic functionals defined on the data,
    \begin{align*}
        \Rc &= \frac{1}{n}\Eb_{\epsilon_i\in\mscrU} \sup_{\|\theta\|\le a} \sum_{i=1}^n\epsilon_i\cL_e^i(\theta;\hat\Ub_r^\top) \\
        %K &= |\log(\phi(-M))|>\max_i\cL_e^i(\theta;\hat\Ub_r^\top)
        K&= \max_i\cL_e^i(\theta;\hat\Ub_r^\top) \le M.
    \end{align*}
    %We know $\cL_e^i(\theta;\hat\Ub_r^\top)<K$ with probability at least $1-n^{-c_1+1}$,
    %then for any $\theta$ such that $\|\theta\|\le a$, with probability $1-\delta-n^{-c_1+1}$, we have that 
    with probability $1-\delta$, we have that 
    \begin{align*}
        |\cL_e(\theta;\Ub_r^\top) - \cL(\theta;\Ub_r^\top)| \le \Rc + \frac{\sqrt{\log(1/\delta)}}{\sqrt{n}}K.
    \end{align*}
\end{lemma}
Thus we have that 
\begin{align*}
    |\mathcal{L} (\hat\theta_e;\hat\Ub_r^\top) - \mathcal{L}_e (\hat\theta_e;\hat\Ub_r^\top)| &\le \Rc + \frac{\sqrt{\log(1/\delta)}}{\sqrt{n}}K,\\
    |\mathcal{L} (\hat\theta;\hat\Ub_r^\top) - \mathcal{L}_e (\hat\theta;\hat\Ub_r^\top)| &\le \Rc + \frac{\sqrt{\log(1/\delta)}}{\sqrt{n}}K.
\end{align*}
Because $\hat\theta_e$ minimizes the empirical loss $\mathcal{L}_e$,
\begin{align*}
    \mathcal{L}_e (\hat\theta_e;\hat\Ub_r^\top) \le \mathcal{L}_e (\hat\theta;\hat\Ub_r^\top).
\end{align*}
Thus 
\begin{align}
    \mathcal{L} (\hat\theta_e;\hat\Ub_r^\top) - \mathcal{L} (\hat\theta;\hat\Ub_r^\top) \le 2\left(\Rc + \frac{\sqrt{\log(1/\delta)}}{\sqrt{n}}K\right).\label{eq:emp loss}
\end{align}
So the remaining target is to bound $\Rc$. 

We first denote $\vb_i = \hat\Ub_r^\top \x_i$, so $\vb_i\in\R^r$ and $\vb_i$ are jointly independent standard normal random variables. %In binary classification, 
$\cL_e^i$ is always $L$ Lipschitz in $\theta^\top\vb_i$, the Rademacher complexity can be upper bounded by
\begin{align}\label{eq:lin rade}
    \Rc \le \tilde\Rc := \frac{L}{n}\Eb_{\epsilon_i\in\mscrU} \sup_{\|\theta\|\le a} \sum_{i=1}^n \epsilon_i\theta^\top\vb_i. 
\end{align}
We first refer to the following lemma.
\begin{lemma}\label{lemma:chi-sqr}
    \cite{laurent2000adaptive} Let $c>0$, $X$ follow $\chi_r^2$ distribution, then
    \begin{align*}
        \Pb(X - r \ge 2\sqrt{cr\log n} + 2c\log n) \le n^{-c}.
    \end{align*}
\end{lemma}

For a constant $c>1$, via union bound we have that $\max{\|\vb_i\|^2} \le r + 2\sqrt{cr\log n} + 2c\log n$ for all $i=1,..,n$ with probability $1 - n^{-c+1}$. We use $\max{\|\vb_i\|} \lesssim c(\sqrt{r} + \log(n))$ for simplicity.

Conditioned on this event, we apply the Rademacher complexity for linear model that 
\begin{align}
   \tilde \Rc &\le \frac{L\max\|\theta\| \cdot \max\|\vb_i\|}{\sqrt{n}}\\
   &\le \frac{caL(\sqrt{r} + \log(n))}{\sqrt{n}}. \label{eq:tilde Rc}
\end{align}
Combining with \eqref{eq:emp loss} and Theorem \ref{thm:popu append} we get the bound in Theorem \ref{thm:rade app}. We can also bound $M$ in \eqref{eq:bound_rade}.

Finally we will use Lemma \ref{lem:M to K} to bound $M$.
\begin{lemma}\label{lem:M to K}
    Let $M$ be defined as in \eqref{eq:bound_rade}.    
    With probability at least $1 - n^{-c+1}$, we have $M<caL(\sqrt{r} + \log(n))$.
\end{lemma}
Let $\vb_i$ be replaced by $\hat \Ub_r^\top\x_i$ in Lemma \ref{lemma:chi-sqr}, then this directly results from Lemma \ref{lemma:chi-sqr}. Lemma \ref{lem:M to K} bounds $M$, thus bounds $K$ (which is $L$ Lipschitz in $M$) in Lemma \ref{lem:rade known}. After we insert \eqref{eq:tilde Rc} together into Lemma \ref{lem:rade known}, we can get the result in  Theorem \ref{thm:rade}.
% By Lemma \ref{lemma:chi-sqr} we know that for a constant $c>2$, we have  $\max{\|\hat\Ub_r^\top\x_i\|} \le c(\sqrt{r} + \log(n))$ for all $i=1,..,n$ with probability $1 - n^{-c+1}$. So with probability at least $1 - n^{-c+1}$, we have $M<ac(\sqrt{r} + \log(n))$.
\end{proof}



==> Paper/s_main_nn.tex <==
\begin{lemma}\label{lem:mean nn}
We assume that the data are generated as in Defs. \ref{def:task dis} to \ref{def:data_gen} and Def. \ref{def:nn}, and we study the $j$-th task whose feature matrix is $\Theta^j$. 
%{\color{blue} To be finished}
Define
\begin{align*}
    \mtx{h}(\Theta): \R^{r\times d} \rightarrow \R^r = \mtx{E}_{\x\sim\Px} f(\Theta \x)  \x
\end{align*}
Then $\mtx{E}_{(\x,y)\sim\Pxy}(y \x) = (\Theta^j)^\top(\Theta^j(\Theta^j)^\top)^{-1}\Theta^j\mtx{h}(\Theta^j)$, and $\|y\x\|\le 1$ with probability $1$.
%{\color{blue} To be finished}
\end{lemma}

\noindent\textbf{Proof of Lemma \ref{lem:mean nn}} The boundedness is trivial and we study the expectation.
Denote
\begin{align*}
    \tilde \Theta^j = (\Theta^j)^\top (\Theta^j(\Theta^j)^\top)^{-1}\Theta^j
\end{align*}

We first write the expectation as
\begin{align*}
    &\mtx{E}_{(\x,y)\sim\Pxy}(y \x) \\
    &= \mtx{E}_{\x} f(\Theta^j \x) \x\\
    &= \mtx{E}_{\x\sim\Px} \left(f(\Theta^j \x)  \tilde \Theta^j \x + f(\Theta^j \x) (\x -  \tilde \Theta^j\x) \right).
\end{align*}
Now we prove that 
\begin{align*}
    \mtx{E}_{\x\sim\Px}f(\Theta^j \x) (\x -  \tilde \Theta^j\x) =0
\end{align*}
Denote 
\begin{align*}
    \bar \x &= \tilde \Theta^j\x - (\x -  \tilde \Theta^j\x)\\
    &= 2\tilde \Theta^j\x - \x.
\end{align*}
Then it is easy to see
\begin{align}
    \Theta^j \x  &= \Theta^j \bar \x,\label{eq:easy1 nn} \\
    \x -  \tilde \Theta^j\x &= - \left(\bar \x -  \tilde \Theta^j\bar \x\right),\label{eq:easy2 nn}\\
    \x &=2\tilde \Theta^j\bar \x - \bar \x.
\end{align}


Now we consider the density function of $\bar x$. Let the density of $\x$ be $p_{\x}$, which is uniform on the unit sphere, we have that 
{\color{blue} Need a better notation!}
\begin{align}
    p_{\bar \x} (\bar \x) &= p_{\x}(2\tilde \Theta^j\bar \x - \bar \x) \big|\nabla_{\bar \x} (2\tilde \Theta^j\bar \x - \bar \x \big| \label{eq:den2 nn}\\
    &= p_{\x}(\x) \big|\mathrm{det}(2\tilde \Theta^j - I) \big|\label{eq:den3}\\
    &= p_{\x}(\x).
\end{align}
Here \eqref{eq:den2} uses the fact that the density function $p_{\x}$ is uniform (thus is a constant everywhere), and \eqref{eq:den3} uses that the eigenvalues of $\frac{2\theta^j(\theta^j)^\top}{\|\theta^j\|^2} - I$ only consists of $\pm 1$. Now we can see that the distributions of $\x$ and $\bar \x$ are the same.

So we have that
\begin{align}
    &\quad \mtx{E}_{\x\sim\Px}f(\Theta^j\bar \x) (\bar \x - \tilde \Theta^j\bar \x)\notag\\
    &= \mtx{E}_{\x\sim\Px}f(\Theta^j \x) \left(- (\x -  \tilde \Theta^j\x)\right)\notag\\
    &= - \mtx{E}_{\x\sim\Px}f(\Theta^j \x) (\x -  \tilde \Theta^j\x).\label{eq:mns nn}
\end{align}
which uses \eqref{eq:easy1 nn}, \eqref{eq:easy2 nn}. Since the distributions of $\x$ and $\bar \x$ are the same, we compute via a simple change of variable
\begin{align}
    &\quad \mtx{E}_{\x\sim\Px}f(\Theta^j\bar \x) (\bar \x - \tilde \Theta^j\bar \x) \notag\\
    &= \mtx{E}_{\bar \x\sim\Px}f(\Theta^j\bar \x) (\bar \x - \tilde \Theta^j\bar \x)\notag\\
    &= \mtx{E}_{\x\sim\Px}f(\Theta^j \x) (\x -  \tilde \Theta^j\x).\label{eq:pls nn}
\end{align}

Comparing \eqref{eq:mns nn} and \eqref{eq:pls nn}, we have 
\begin{align*}
    &\quad \mtx{E}_{\x\sim\Px}f(\Theta^j \x) (\x -  \tilde \Theta^j\x)\\
    &= -\mtx{E}_{\x\sim\Px}f(\Theta^j \x) (\x -  \tilde \Theta^j\x)
\end{align*}
so $\mtx{E}_{\x\sim\Px}f(\Theta^j \x) (\x -  \tilde \Theta^j\x)=0$.

Going back to Lemma \ref{lem:mean nn}, we have 
\begin{align*}
    \mtx{E}_{(\x,y)\sim\Pxy}(y \x)
    &= \mtx{E}_{\x\sim\Px} f(\Theta^j \x)  \tilde \Theta^j \x
    \\&= \mtx{E}_{\x\sim\Px} f(\Theta^j \x)  (\Theta^j)^\top (\Theta^j(\Theta^j)^\top)^{-1}\Theta^j \x.
\end{align*}
%\Theta^j

{\color{blue} From here I'll prove using the fact that $y\x$ is subGaussian with $\|\mathbf{Cov}(y\x)\| \le \sigma^2$.}

First we study the concentration of data within the $j$-th class. 
\begin{lemma}
Let $\delta\in(0,1)$, with probability $1-\delta$, there exists a constant $c$ such that
\begin{align*}
    \|\frac{1}{t}\sum_{i=1}^t \yij\xij - \theta^j\| \le c\sigma\sqrt{\frac{d}{t}\log(\frac{kd}{\delta})} 
\end{align*}
for all $j=1,...,k$. 
\end{lemma}
\begin{lemma}
For all $\vb$ such that $\|\vb\| = 1$, there exists a constant $c$ such that
\begin{align*}
    \Eb\left( (\vb^T\cdot (\frac{1}{t}\sum_{i=1}^t \yij\xij - \theta^j))^2\right) \le c\sigma^2 / t. 
\end{align*}
\end{lemma}
\begin{lemma}
There exists a constant $c$ such that \begin{align*}
    \Eb \left(\|\frac{1}{t}\sum_{i=1}^t \yij\xij - \theta^j \|^2\right) \le c\sigma^2d/t. 
\end{align*}
\end{lemma}
\begin{lemma}
Define
\begin{align*}
    \Zb_j = (\frac{1}{t}\sum_{i=1}^t \yij\xij)(\frac{1}{t}\sum_{i=t+1}^{2t} \yij\xij)^\top - \theta^j(\theta^j)^\top,
\end{align*}
Then there exists a constant $c$ such that with probability $1-\delta$, for all $j=1,...,k$, 
\begin{align}
    \|\Zb_j \| \le \frac{c\sigma^2d}{t} \log(\frac{kd}{\delta}). \label{eq:evt}
\end{align}
\end{lemma}

\begin{lemma}
There exists a constant $c$ such that
\begin{align*}
   \|\Eb\sum_{j=1}^k\Zb_j\Zb_j^\top\| \le c\sigma^4dk/t
\end{align*}
\end{lemma}
\begin{lemma}
Let $\delta\in(0,1)$. There exists a constant $c$, such that for any $\epsilon\in(0,1)$, and 
\begin{align}
    k = \frac{cd}{t}\log^2(\frac{kd}{\delta}) \max\{\frac{1}{\epsilon^2}, \frac{1}{\epsilon} \log(\frac{kd}{\delta})\}, \label{eq:k lb}
\end{align}
with probability $1-\delta$, 
\begin{align*}
    \|\frac{1}{k} \sum_{j=1}^k \Zb_j\| \le \epsilon \sigma^2.
\end{align*}
\end{lemma}
This means that when \eqref{eq:k lb}, with probability $1-\delta$,
\begin{align*}
    \left\|\hat \bM - \frac{1}{k}\sum_{j=1}^k\left(\tilde \Theta^j \mtx{h}(\Theta^j)\mtx{h}^\top(\Theta^j)\tilde \Theta^j\right)\right\| \le \epsilon \sigma^2.
\end{align*}


==> Paper/s_main_proof.tex <==
\section{Proof of main theorems}
\SO{Clearly Theorem \ref{thm:hatM append} is a restatement of Theorem \ref{thm:hatM}. Why don't you say so? Reader is not expected to figure out this by himself. Let us make things clear.}

\SO{Similarly, where is proof of Lemma 3.1? Looks like Lemma \ref{lem:mean nn} is its restatement but again not clear at all for reader. They cannot find proof of Lemma 3.1 in the text.}

\SO{Here is the organization we need: In the appendix, proof of each technical result in the main text is supposed to have its own subsection. Just like this subsection that I added i.e.~Proof of Theorem \ref{thm:hatM}.}
\SO{Maybe briefly describe the outline. Right now, little confusing due to Lemmas within the proof so outline would help i.e.~we first prove Lemma ... which shows ...}
\subsection{Proof of Lemma \ref{lem:M exp} and Theorem \ref{thm:hatM}}
We sketch the proof at the beginning. First we compute the expectation of $y\x$ in Lemma \ref{lem:mean nn}. That leads to the proof of Lemma \ref{lem:M exp}. Then in Lemma \ref{lem:err_yx} we bound the difference between sum of $y\x$ and its mean using concentration. The concentration of covariance estimator is studied later in Lemma \ref{lem:Zj} and \ref{lem:Zj2}, which leads to Theorem \ref{thm:hatM}.

\subsubsection{Proof of Lemma \ref{lem:M exp}}
We first state Lemma \ref{lem:M exp} below.
\begin{lemma}\label{lem:M exp append}
Let 
\begin{subequations}\label{eq:hatM append}
\begin{align}
\hat\bM &= \mathop{\Scale[1.8]{\sum}}_{j=1}^k \frac{2}{n_j^2}\left[(\sum_{i=1}^{n_j/2} \yij\xij) (\sum_{i=n_j/2+1}^{n_j} \yij\xij)^\top \right.\\
&\quad\quad\quad\quad \left. +  ( \sum_{i=n_j/2+1}^{n_j} \yij\xij) ( \sum_{i=1}^{n_j/2} \yij\xij)^\top\right].\nonumber
\end{align}
\end{subequations}
And
\begin{align*}
    &\mtx{h}^j(\W): \R^{r\times d} \rightarrow \R^d = \mtx{E}_{\x}[f^j(\W \x)\x]\\
    &\bM := \W^\top\W\left(\frac{1}{k}\sum_{j=1}^k \mtx{h}^j(\W)( \mtx{h}^j(\W))^\top\right)\W^\top\W.
\end{align*}
Then $\bM,\hat{\bM}$ satisfies the following. (a) $\text{rank}(\bM)\leq r$. (b) $\text{range-space}(\bM)\subset \text{row-space}(\W)$. (c) $\mtx{E}[\hat{\M}]=\bM$. 
\end{lemma}
\begin{proof}
Part (a) and (b) are easy to see. $\W\in\R^{r\times d}$ so that $\text{rank}(\bM)\leq r$, and since $\bM$ is the product of $\W^\top$ and another matrix, then  $\text{range-space}(\bM)\subset \text{row-space}(\W)$.
Now we will prove Part (c). We first give the lemma for the mean of the random vector $y\x$.

\begin{lemma}\label{lem:mean nn}
We assume that the data is generated as in Def. \ref{def:task}, and we study the $j$-th task whose activation function is $f^j$. 
%{\color{blue} To be finished}
Define
\begin{align*}
    \mtx{h}^j(\W): \R^{r\times d} \rightarrow \R^d = \mtx{E}_{\x\sim\gauss} f^j(\W \x)  \x
\end{align*}
Denote the joint distribution of $(\x,y)$ as $\Pxy$.
Then $\mtx{E}_{(\x,y)\sim\Pxy}(y \x) = \W^\top\W \mtx{h}^j(\W)$.
\end{lemma}

\emph{Proof of Lemma \ref{lem:mean nn}.} The expectation can be expanded as
\begin{align*}
    &\mtx{E}_{(\x,y)\sim\Pxy}(y \x) \\
    &= \mtx{E}_{\x\sim\gauss} f^j(\W \x) \x\\
    &= \mtx{E}_{\x\sim\gauss} \left(f^j(\W \x)  \W^\top\W \x + f^j(\W \x) (I - \W^\top\W)\x \right).
\end{align*}
Note that, because $\x\sim\gauss$ so $\W \x$ and $(I - \W^\top\W)\x$ are Gaussian. $\W\W^\top = I$ implies 
\begin{align*}
    &\quad \Eb (\W \x)\x^\top((I - \W^\top\W))\\
    &= \W(I - \W^\top\W) = 0.
\end{align*}
So $\W \x$ and $(I - \W^\top\W)\x$ are independent, so 
\begin{align*}
    &\quad \mtx{E}_{\x\sim\gauss}  f^j(\W \x) (I - \W^\top\W)\x \\
    &= (\mtx{E}_{\x\sim\gauss}  f^j(\W \x)) (\mtx{E}_{\x\sim\gauss} (I - \W^\top\W)\x) = 0
\end{align*}
Then 
\begin{align*}
    \mtx{E}_{(\x,y)\sim\Pxy}(y \x) &= \W^\top\W(\mtx{E}_{\x\sim\gauss} f^j(\W \x) \x)\\
    &= \W^\top\W \h_j(\W).
\end{align*}

Denote 
\begin{align}\label{eq:Hj def}
    \Hb^j(\W) = \W^\top\W \mtx{h}^j(\W)
\end{align}
Because $\frac{2}{n_j}\sum_{i=1}^{n_j/2} \yij\xij$
and 
$\frac{2}{n_j}\sum_{i={n_j/2}+1}^{n_j} \yij\xij$ 
are independent, and their expectation are both $\Hb^j(\W)$, so that
\begin{align*}
    &\quad \mtx{E}(\frac{2}{n_j}\sum_{i=1}^{n_j/2} \yij\xij)(\frac{2}{n_j}\sum_{i={n_j/2}+1}^{n_j} \yij\xij)^\top \\
    &= \Hb^j(\W)(\Hb^j(\W))^\top.
\end{align*}
At then end
\begin{align*}
    \hat \bM &= \frac{1}{k}\sum_{j=1}^k \mtx{E}(\frac{2}{n_j}\sum_{i=1}^{n_j/2} \yij\xij)(\frac{2}{n_j}\sum_{i={n_j/2}+1}^{n_j} \yij\xij)^\top,\\
    \bM &= \frac{1}{k}\sum_{j=1}^k\Hb^j(\W)(\Hb^j(\W))^\top,
\end{align*}
so we can prove Part (c) that $\mtx{E}(\hat \bM) = \bM$.
\end{proof}


\subsubsection{Proof of Theorem \ref{thm:hatM}}
We restate Theorem \ref{thm:hatM append} below. 
\begin{theorem}\label{thm:hatM append}
Suppose the data is generated as Def. \ref{def:task}. Let $\delta\in(0,1)$, $\epsilon\in(0,1)$. Suppose $y\x$ is a subGaussian random vector with covariance upper bounded by
\begin{align}
   \| \mathbf{Cov}(y \x) \| \le \sigma^2. \label{eq:covyx append}
\end{align} 
Define
\begin{align*}
    \mtx{h}^j(\W): \R^{r\times d} \rightarrow \R^d = \mtx{E}_{\x\sim\gauss} f^j(\W \x)  \x
\end{align*}
And let %$\bM = \mtx{E}_{\theta\sim\mathcal{N}(0,\bSi)} (g(\theta))^2\frac{\theta\theta^\top}{\|\theta\|^2}$, then
\begin{align*}
    \bM = \W^\top\W\left(\frac{1}{k}\sum_{j=1}^k \mtx{h}^j(\W)( \mtx{h}^j(\W))^\top\right)\W^\top\W
\end{align*}
Then there exists a constant $c$, with probability at least $1-\delta$, let 
\begin{align*}
    k = \frac{cd}{n}\log^2(\frac{kd}{\delta}) \max\{\frac{1}{\epsilon^2}, \frac{1}{\epsilon} \log(\frac{kd}{\delta})\}
\end{align*}
we have 
\begin{align*}
    \|\hat \bM - \bM\| \le \epsilon\sigma^2.
\end{align*}
\end{theorem}
\begin{proof}
The following lemmas are similar to \cite{kong2020meta} Section A.1. We extend the concentration inequalities from bounded random vectors to Gaussian random vectors. For completeness we place the lemmas here.

\begin{lemma}\label{lem:err_yx}
(\cite{jin2019short} Cor. 7) 
Let $\|\mathbf{Cov}(y\x)\| \le \sigma^2$, $\delta\in(0,1)$, $t>0$, $\Hb^j(\W)$ be defined in \eqref{eq:Hj def}. With probability $1-\delta$, there exists a constant $c>0$ such that for every $j$,
\som{Remind the exact assumption on $\sigma$}
\begin{align}
   \|\frac{1}{t}\sum_{i=1}^t \yij\xij - \Hb^j(\W)\| \le c\sigma\sqrt{\frac{d}{t}\log(\frac{kd}{\delta})} \label{eq:gauss_bern}
\end{align}
\som{Call $\W^\top\W \mtx{h}^j(\W)$ something for simpler notation}
Denote this event as $\mathcal{E}$.
\iffalse
{\it\color{red} for every i,j pairs ? }Denote this event as $\mathcal{E}$.
{\it \color{red} if we dont say "for every i,j pairs" ,k should not appear in an inequality which holds for only one task. Also maybe it is better to  cite [21] A.5, because [28] Cor.7 says only the following
$$\|\frac{1}{t}\sum_{i=1}^t \yij\xij - \W^\top\W \mtx{h}^j(\W)\| \le c\sigma\sqrt{\frac{1}{t}\log(\frac{2d}{\delta})}$$}
\fi
\end{lemma}
With the covariance of $y\x$ being bounded by $\sigma^2$, the following inequalities are true \cite{kong2020meta}.
\begin{align*}
    \Eb\left( (\vb^T\cdot (\frac{1}{t}\sum_{i=1}^t \yij\xij - \theta^j))^2\right) &\le \sigma^2 / t,\mbox{~for~} \|\vb\|=1.\\
    \Eb \left(\|\frac{1}{t}\sum_{i=1}^t \yij\xij - \theta^j \|^2\right) &\le \sigma^2d/t.
\end{align*}


\begin{lemma}\label{lem:Zj}
Define
\begin{align*}
    \Zb_j &= (\frac{2}{n_j}\sum_{i=1}^{n_j/2} \yij\xij)(\frac{2}{n_j}\sum_{i={n_j/2}+1}^{n_j} \yij\xij)^\top \\
    &\quad - \Hb^j(\W)(\Hb^j(\W))^\top,
\end{align*}
Then there exists a constant $c$ such that on the event $\mathcal{E}$ (thus with probability $1-\delta$), for all $j=1,...,k$, 
\begin{align}
    \|\Zb_j \| \le \frac{c\sigma^2d}{n_j} \log(\frac{kd}{\delta}). \label{eq:evt}
\end{align}
\end{lemma}

% {\it \color{red} From my understanding we should have 
% $$\|\Zb_j \| \le (Eq A.1 Bound)(Eq. A.1 bound + 2\|\W^\top\W \mtx{h}^j(\W)\|)$$ choosing $t=\dfrac{n_j}{2}$ then we have $$\|\Zb_j \| \le (c\sigma\sqrt{\frac{2}{n_j}\log(\frac{2d}{\delta})})(c\sigma\sqrt{\frac{2}{n_j}\log(\frac{2d}{\delta})} + 2\|\W^\top\W \mtx{h}^j(\W)\|)$$
% This is more or less what you have found, but the difference is k in $\log$ term and d term }



The proof is almost same as \cite{kong2020meta}, the only difference is that we replace the bound in (\cite{kong2020meta} Prop A.1) by \eqref{eq:gauss_bern}. With the similar replacement, we propose the following lemma. 
\begin{lemma}\label{lem:Zj2}
Let $\delta\in(0,1)$. There exists a constant $c$, such that for any $\epsilon\in(0,1)$, and 
\begin{align}
    k = \frac{cd}{n_j}\log^2(\frac{kd}{\delta}) \max\{\frac{1}{\epsilon^2}, \frac{1}{\epsilon} \log(\frac{kd}{\delta})\}, \label{eq:k lb}
\end{align}
with probability $1-\delta$, 
\begin{align*}
    \|\frac{1}{k} \sum_{j=1}^k \Zb_j\| \le \epsilon \sigma^2.
\end{align*}
\end{lemma}
This means that when \eqref{eq:k lb} is true, with probability $1-\delta$,
\begin{align*}
    \left\|\hat \bM - \W^\top\W\left(\frac{1}{k}\sum_{j=1}^k \mtx{h}^j(\W)( \mtx{h}^j(\W))^\top\right)\W^\top\W\right\| \le \epsilon \sigma^2.
\end{align*}
Note that $\bM$ is defined as \[\bM=\W^\top\W\left(\frac{1}{k}\sum_{j=1}^k \mtx{h}^j(\W)( \mtx{h}^j(\W))^\top\right)\W^\top\W.\] So we have proven that with probability $1-\delta$,
\begin{align*}
    \left\|\hat \bM - \bM\right\| \le \epsilon \sigma^2.
\end{align*}

\som{Remind that this is $\hat \bM-\bM$ i.e. $\bM=\text{the messy sum}$}
\end{proof}

\SO{Create a subsection here!!! Reduce the confusion as much as possible, make transitions smooth.}
\subsection{Proof of Theorem \ref{thm:down}}
Now we will prove Theorem \ref{thm:down}. We first review the notations and assumptions mentioned in the theorem.

\subsubsection{Review of Notations and Assumptions}
We define the SVD of $\hat \bM$ as $\hat \Ub \hat\La \hat\Vb^\top$. Let the first $r$ columns of $\hat \Ub$ be $\Ub_r$. 

Let $\hat\W$ be defined as 
\begin{align}
    \hat \W &= \hat \Ub_r \hat \Qb, \label{eq:def W append}\\
    \hat \Qb &= \mathop{\mathrm{argmin}}_{\Qb\in\R^{r\times r}, \Qb\Qb^\top = I}\ \|\hat \Ub_r \Qb - \W\|.
\end{align}
The population cross entropy loss is defined as
\begin{align*}
    &\cLCE(f;\Pb) : \Fc\times \R^{r\times d}\rightarrow \R=\\
    &-\mtx{E}_{\x,y\sim\Pxy} (y\log f(\hat\Pb \x) + (1-y)\log (1 - f(\hat\Pb \x))).
\end{align*}
We will search for a function $f^* \in \Fc$ that minimizes the population cross entropy loss. $\Fc$ is a set of functions satisfying
\begin{enumerate}
    \item For any function $f\in\Fc$, any orthonormal matrix $\Qb\in\R^{r\times r}$ and any matrix $\Pb\in\R^{r\times d}$, there exists $g \in \Fc$ such that $f(\Pb \x) = g(\Qb\Pb \x)$.
    \item $\Fc \subseteq \{f\ |\ \log f,~ \log(1-f)\mathrm{~are~}L\mathrm{~Lipschitz}\}\bigcap \{f\ |\ 0<f(x)<1,\forall x\in\R^r\}$.
\end{enumerate}
We solve for $\hat f$, defined as \begin{align}
    \hat f &= \argmin_{f\in\Fc}\ \cLCE(f;\hat \Ub_r^\top). \label{eq:def f append}
\end{align}
\subsubsection{Proof of Theorem \ref{thm:down}}
Now we are ready to restate Theorem \ref{thm:down} and prove it.
\begin{theorem}\label{thm:popu append}
Based on the definition above, we have that
    \begin{align*}
        \cLCE(\hat f;\hat \Ub_r^\top)  - \cLCE(f^*;\Ub_r^\top) \lesssim L\sqrt{r}\|\hat \W - \W\|.
    \end{align*}
\end{theorem}

\begin{proof}
We learn the model from the following optimization algorithm.
\begin{align*}
    \hat f &= \argmin_{f\in\Fc}\ \cLCE(f;\hat \Ub_r^\top)\\
    &= \argmin_{f\in\Fc}\ -\mtx{E}_{\x,y\sim\Pxy} (y\log f(\hat\Ub_r^\top \x) \\
    &\quad + (1-y)\log (1 - f(\hat\Ub_r^\top \x)))\\
    &= \argmin_{f\in\Fc}\ -\mtx{E}_{\x\sim\gauss} \left(f^*(\W \x)\log f(\hat \Ub_r^\top \x)\right. \\
    & \quad \left. + (1-f^*(\W \x))\log (1 - f(\hat \Ub_r^\top \x)) \right).
\end{align*}
Denote $\tilde f\in\Fc$ as the function such that $\tilde f(\hat \W \x) = \hat f(\hat \Ub_r^\top \x)$. So that $\cLCE(\hat f;\hat \Ub_r^\top) = \cLCE(\tilde f;\hat \W)$. Since $\hat f$ minimizes the cross entropy loss, we have that $\cLCE(\tilde f;\hat \W) \le \cLCE(f^*;\hat \W)$. 

Now we have 
\begin{align*}
    &\quad \cLCE (\tilde f;\hat \W) - \cLCE (f;\W)\\
    &\le \cLCE (f^*;\hat \W) - \cLCE (f^*;\W)\\
    &\le -\mtx{E}_{\x\sim\gauss} \left(f^*(\W \x)(\log f^*(\hat\W \x) -\log f^*(\W \x))\right. \\
    & \quad \left. + (1-f^*(\W \x))(\log (1 - f^*(\hat \W \x)) - \log (1 - f^*(\W \x))) \right)\\
    &\le \mtx{E}_{\x\sim\gauss} L\|(\hat \W - \W)x\|\\
    &\lesssim L\sqrt{r}\|\hat \W - \W\|.
\end{align*}
\end{proof}

\subsection{Proof of Theorem \ref{thm:rade}}
%Now we prove that the upper bound of the error for few-shot learning with finite samples.
We first state Theorem \ref{thm:rade} below.
\begin{theorem}\label{thm:rade app}
    Suppose we generate $n$ sample data for few shot learning solve for $\hat \theta_e$ from \eqref{eq:fstar finite theta}. There exist constants $c>0$, $\delta\in(0,1)$, with probability at least $1 - n^{-c+1} - \delta$, the solution $\hat\theta_e$ and $\hat\Ub_r$ satisfy
    \begin{align*}
        &\quad \mathcal{L} (\hat\theta_e;\hat\Ub_r^\top) - \mathcal{L} (\theta^*;\W) \\
        &\lesssim \frac{ac(\sqrt{r}+\log(n)) (1+ \sqrt{\log(1/\delta)})}{\sqrt{n}} + \sqrt{r}\|\hat \W - \W\|. 
    \end{align*}
\end{theorem}
\begin{proof}
We sketch the proof of Theorem \ref{thm:rade app}. After reviewing the notations, we quote a standard generalization bound via Rademacher complexity in Lemma \ref{lem:rade known}. Then we use the smoothness of the loss function to link to the generalization error of linear functions \eqref{eq:lin rade}, and then use Lemma \ref{lemma:chi-sqr} to compute \eqref{eq:lin rade} and finish the proof.

In few-shot learning, the true parameter is $\theta^*$, and the empirical loss function with finite data is 
\begin{align}
    &\cL_e(\theta;\Pb) : \Fc\times \R^{r\times d}\rightarrow \R= \notag\\
    &-\frac{1}{n}\sum_{i=1}^n (y_i\log\phi (\theta^\top\Pb \x_i) + (1-y_i)\log (1 - \phi(\theta^\top\Pb \x_i))) \label{eq:cLCE finite theta app}
\end{align}
Denote each term in the summation as 
\begin{align*}
    &\quad \cL_e^i(\theta;\Pb) : \Fc\times \R^{r\times d}\rightarrow \R=\notag\\
    &- (y_i\log \phi (\theta^\top\Pb \x_i) + (1-y_i)\log (1 - \phi(\theta^\top\Pb \x_i)))
\end{align*}
We search for the solution by
\begin{align}
    \hat \theta_e &= \argmin_{\theta}\ \cL_e(\theta;\Ub_r^\top),\mbox{~such~that~} \|\theta\|\le a.\label{eq:fstar finite theta app}
\end{align}
In Theorem \ref{thm:popu append}, we know that
\begin{align*}
    \cLCE(\hat \theta;\hat \Ub_r^\top)  - \cLCE(\theta^*;\Ub_r^\top) \lesssim L\sqrt{r}\|\hat \W - \W\|.
\end{align*}
Denote 
    \begin{align}
        M = \max_{\|\theta\|\le a} |\theta^\top \hat\Ub_r^\top\x_i| \le a \max\|\hat\Ub_r^\top\x_i\|.\label{eq:bound_rade}
    \end{align}
We will bound the difference between $\cL$ and $\cL_e$ by Rademacher complexity theory.
\begin{lemma}\label{lem:rade known}
    \cite{mohri2018foundations}
 
    Let $\mscrU$ be the independent random variables uniformly chosen from $\{-1,1\}$.
    Let $\Rc$ be the Rademacher complexity of the logistic functionals defined on the data,
    \begin{align*}
        \Rc &= \frac{1}{n}\Eb_{\epsilon_i\in\mscrU} \sup_{\|\theta\|\le a} \sum_{i=1}^n\epsilon_i\cL_e^i(\theta;\hat\Ub_r^\top) \\
        K &= |\log(\phi(-M))|>\max_i\cL_e^i(\theta;\hat\Ub_r^\top)
    \end{align*}
    %We know $\cL_e^i(\theta;\hat\Ub_r^\top)<K$ with probability at least $1-n^{-c_1+1}$,
    %then for any $\theta$ such that $\|\theta\|\le a$, with probability $1-\delta-n^{-c_1+1}$, we have that 
    with probability $1-\delta$, we have that 
    \begin{align*}
        |\cL_e(\theta;\Ub_r^\top) - \cL(\theta;\Ub_r^\top)| \le \Rc + \frac{\sqrt{\log(1/\delta)}}{\sqrt{n}}K.
    \end{align*}
\end{lemma}
Thus we have that 
\begin{align*}
    |\mathcal{L} (\hat\theta_e;\hat\Ub_r^\top) - \mathcal{L}_e (\hat\theta_e;\hat\Ub_r^\top)| &\le \Rc + \frac{\sqrt{\log(1/\delta)}}{\sqrt{n}}K,\\
    |\mathcal{L} (\hat\theta;\hat\Ub_r^\top) - \mathcal{L}_e (\hat\theta;\hat\Ub_r^\top)| &\le \Rc + \frac{\sqrt{\log(1/\delta)}}{\sqrt{n}}K.
\end{align*}
Because $\hat\theta_e$ minimizes the empirical loss $\mathcal{L}_e$,
\begin{align*}
    \mathcal{L}_e (\hat\theta_e;\hat\Ub_r^\top) \le \mathcal{L}_e (\hat\theta;\hat\Ub_r^\top).
\end{align*}
Thus 
\begin{align}
    \mathcal{L} (\hat\theta_e;\hat\Ub_r^\top) - \mathcal{L} (\hat\theta;\hat\Ub_r^\top) \le 2\left(\Rc + \frac{\sqrt{\log(1/\delta)}}{\sqrt{n}}K\right).\label{eq:emp loss}
\end{align}
So the remaining target is to bound $\Rc$. 

We first denote $\vb_i = \hat\Ub_r^\top \x_i$, so $\vb_i\in\R^r$ and $\vb_i$ are jointly independent standard normal random variables. In binary classification, $\cL_e^i$ is always $1$ Lipschitz in $\theta^\top\vb_i$, the Rademacher complexity can be upper bounded by
\begin{align}\label{eq:lin rade}
    \Rc \le \tilde\Rc := \frac{1}{n}\Eb_{\epsilon_i\in\mscrU} \sup_{\|\theta\|\le a} \sum_{i=1}^n \epsilon_i\theta^\top\vb_i. 
\end{align}
We first refer to the following lemma.
\begin{lemma}\label{lemma:chi-sqr}
    \cite{laurent2000adaptive} Let $c>0$, $X$ follow $\chi_r^2$ distribution, then
    \begin{align*}
        \Pb(X - r \ge 2\sqrt{cr\log n} + 2c\log n) \le n^{-c}.
    \end{align*}
\end{lemma}

For a constant $c>1$, via union bound we have that $\max{\|\vb_i\|^2} \le r + 2\sqrt{cr\log n} + 2c\log n$ for all $i=1,..,n$ with probability $1 - n^{-c+1}$. We use $\max{\|\vb_i\|} \lesssim c(\sqrt{r} + \log(n))$ for simplicity.

Conditioned on this event, we apply the Rademacher complexity for linear model that 
\begin{align}
   \tilde \Rc &\le \frac{\max\|\theta\| \cdot \max\|\vb_i\|}{\sqrt{n}}\\
   &\le \frac{ca(\sqrt{r} + \log(n))}{\sqrt{n}}. \label{eq:tilde Rc}
\end{align}
Combining with \eqref{eq:emp loss} and Theorem \ref{thm:popu append} we get the bound in Theorem \ref{thm:rade app}. We can also bound $M$ in \eqref{eq:bound_rade}.

Finally we will use Lemma \ref{lem:M to K} to bound $M$.
\begin{lemma}\label{lem:M to K}
    Let $M$ be defined as in \eqref{eq:bound_rade}.    
    With probability at least $1 - n^{-c+1}$, we have $M<ac(\sqrt{r} + \log(n))$.
\end{lemma}
Let $\vb_i$ be replaced by $\hat \Ub_r^\top\x_i$ in Lemma \ref{lemma:chi-sqr}, then this directly results from Lemma \ref{lemma:chi-sqr}. Lemma \ref{lem:M to K} bounds $M$, thus bounds $K$ (which is $1$ Lipschitz in $M$) in Lemma \ref{lem:rade known}. After we insert \eqref{eq:tilde Rc} together into Lemma \ref{lem:rade known}, we can get the result in  Theorem \ref{thm:rade}.
% By Lemma \ref{lemma:chi-sqr} we know that for a constant $c>2$, we have  $\max{\|\hat\Ub_r^\top\x_i\|} \le c(\sqrt{r} + \log(n))$ for all $i=1,..,n$ with probability $1 - n^{-c+1}$. So with probability at least $1 - n^{-c+1}$, we have $M<ac(\sqrt{r} + \log(n))$.
\end{proof}



==> Paper/s_prob.tex <==
\setlength{\topsep}{0.25em}
\newcommand{\xij}{{\x_{i,j}}}
\newcommand{\xijt}{{\x_{i,j}^\top}}
\newcommand{\yij}{{y_{i,j}}}

\section{Problem Formulation}\label{s:prob}
% {\color{red} YS: a paragraph for notation?}
The meta-learning setup that will be considered in this work consists of two phases: (i) meta-training: prior tasks are used to learn a good representation and (ii) few-shot learning: the new task is learned with few samples.
%\som{Is meta-train/test standard and correct phrases?} 
%{\mf better not to use the meta-train and meta-test phrases if we don't need to} 
In the meta-training phase, we learn the low dimensional space spanned by parameters. In the few-shot learning phase, we use the subspace to learn the model of a new task ideally with few samples.

In the first phase, there are multiple tasks to infer from, each with its own distribution. We consider a realizable model where the input and label is associated via a labeling function. One accesses batches of data, each of whom is collected from a task, however we may not know which task it comes from. We make this setup more precise using the following definitions. Below, the ground-truth representation will be denoted by a matrix $\W\in\R^{r\times d}$ row space of which corresponds to the subspace of interest.

%\som{Use $n_j$ for sample size rather than $t_j$ (at least for training)}
\begin{definition} \label{def:task}
\textbf{Meta-training data.} Fix a matrix $\W\in\R^{r\times d}$ satisfying $\W\W^T=\Iden$. The $j$-th task is associated with function $f^j: \R^r\rightarrow \R$. Given input $\x$, the label $y$ is distributed as $p_j(y|\x)=p_j(y|\W\x)$\footnote{In words, the label only depends on the relevant features induced by $\W$.} and the expectation satisfies $\mtx{E}(y) = f^j(\W\x)$.
%{\mf give properties like domain and range of $f$ here, first time it appears.}
Suppose there are $n_j$ samples from the $j$-th task sampled i.i.d.~from this distribution and we denote the dataset $\Sc^j = (\xij, \yij)_{i=1}^{n_j}$. Define the full meta-training dataset to be $\Sc = \bigcup_{j=1}^k\Sc^j$.
\end{definition}
Here, $f^j$ is allowed to be any Lipschitz nonlinear function, i.e., a neural network\footnote{In our theoretical results, we treat $f$ as a general linear function, and in experiments we will use a neural network with a specific structure.}.


%In the multi-task problem, there are a collection of tasks in the meta-training phase, which is defined below.


\iffalse
\begin{definition}\label{def:task dis}\som{I don't think we should use a distribution early on.}
\textbf{Low rank task distribution.} There are in total $k$ tasks. Each training task is associated with a parameter vector $\bt^j\in\R^d$ for $j=1,...,k$.
{\mf right now we're just setting the notation---additional assumptions like definition 2.2 on random features should come later.}
These are generated i.i.d. from a Gaussian distribution $\mathcal{N}(0, \bSi)$. Let $\la_i$ be the $i$-th eigenvalue of $\bSi$ with decreasing order. For low rank parameters, we assume that $\la_{r+1} = 0$. We call $r$ as the effective dimension of parameters.
\end{definition}



\begin{definition} \label{def:task}
\textbf{Meta-training data.} The $j$-th task is associated with parameter $\bt^j\in\R^d$. 
%For any parameter $\bt$, one can collect data from it. 
Suppose there are $n_j$ data from the $j$-th task, we call the dataset $\Sc^j = \{(\xij, \yij)\ |\ i=1,...,n_j\}$. Here $\xij\in\R^d$, $\yij\in\R$. $\xij$, $\yij$ satisfy $\mtx{E}(\yij) = f(\xijt\bt^j)$ for some function $f$. Let the whole meta-training dataset be $\Sc = \bigcup_{j=1,...,k}\Sc^j$. {\mf repeated}
\end{definition}

%\noindent\textbf{:}

\begin{definition} \label{def:data_gen}
\textbf{Data generation.} We assume that there are $k$ binary classification tasks, the $j$-th associated with $\bt^j$. The data $\Sc^j$ is generated by $\xij = \bz / \|\bz\|$ and $\bz \sim \mathcal{N}(0, I)$, $\bz$ is generated independently. Denote the distribution of $\xij$ as $\mathscr{P}_x$.
%The labels $\yij$ satisfy
%$\mtx{E}(\yij|\xij, \bt^j) = f(\xijt\bt^j)$ for some Lipschitz function $f:\R\rightarrow \R$. We propose two examples below.
\end{definition}
%{\color{blue} Do we need to normalize $x$? Just for citing the result in \cite{kong2020meta}, they use Bernstein so they have to use bounded rv. In principle unbounded subGaussian works.}
\fi


\begin{definition} \label{def:bin_class}
\textbf{Binary classification.} Suppose $f^j$ takes values over $[0,1]$,
%{\it\color{red}{Is it [0,1] ?}}. The labels $\yij$ are generated as 
\begin{align*}
    \yij = 
     \begin{cases}
       \text{1,} &{\mbox{with probability } f^j(\W \xij),}\\
       \text{0,} &{\mbox{with probability } 1-f^j(\W\xij).}\\
     \end{cases}
\end{align*}
%Here $f^j(a)\in[0,1]$ for all $a\in[-1,1]$, and the event that $f(a) = 0$ is not true with probability $1$ with respect to Lebesgue measure on $[-1,1]$\footnote{In other words, $f$ is not a constant $0$ function.}.
\end{definition}

\begin{definition}\label{def:GLM}
\noindent\textbf{Generalized linear models (GLM)} (which include logistic/linear regression) can be modeled by choosing $f^j$ to be parameterized by a vector $\bt_j\in\R^r$ and a link function $\phi:\R\rightarrow\R$ as $f^j(\W \xij) := \phi(\bt_j^T\W\xij )$.

\end{definition}
%for $\bt_j\in\R^r$, $\phi$ is a function mapping from $\R$ to $(0,1)$.

% Denote the distribution of $\x,y$ as $\mathscr{P}_{x,y}$.
%\begin{definition}\label{def:nn}
%\textbf{Non-linear regression.} More generally, for $\bt^j\in\R^{r\times d}$, the labels $\yij$ are generated as
%\begin{align*}
%    \yij = f^j(\W\xij) + \epsilon,
%\end{align*}
%$\epsilon$ is a zero mean bounded random variable. 
%\end{definition}

When the dimension of the span of parameters is small, \cite{kong2020meta} performs a dimension reduction algorithm to find the low-dimensional subspace that the parameters span. This is done by selecting the top eigenvectors of the covariance estimate of the cross-correlation between input and labels.
\begin{definition}\label{def:mom}
\textbf{Moment estimator of covariance.} We define the covariance estimator as
\begin{subequations}\label{eq:hatM}
\begin{align}
\hat\bM &= \mathop{\Scale[1.8]{\sum}}_{j=1}^k \frac{2}{n_j^2}\left[(\sum_{i=1}^{n_j/2} \yij\xij) (\sum_{i=n_j/2+1}^{n_j} \yij\xij)^\top \right.\\
&\quad\quad\quad\quad \left. +  ( \sum_{i=n_j/2+1}^{n_j} \yij\xij) ( \sum_{i=1}^{n_j/2} \yij\xij)^\top\right].\nonumber
\end{align}
\end{subequations}
\end{definition}
\noindent\textbf{Subspace estimation.} 
To estimate the subspace $\W$, we use rank-$r$ approximation of $\hat \bM$ to retrieve its principal eigenvector subspace. 
Let $\hat\Ub \hat \La \hat \Ub^\top$ be the eigen-decomposition of $\hat \bM$. Denote $\hat \la_j$ as the $j$th eigenvalue of $\hat \La$. Let $\hat\Ub_r$ be the first $r$ columns of $\hat\Ub$, thus the rank-$r$ approximation is $\hat\bM_r = \hat\Ub_r \mathrm{diag}(\hat \la_{1},...,\hat\la_{r}) \hat \Ub_r^\top$. In the next section, we will prove that the range of $\hat \Ub$ is close to the row space of $\W$.

%{\color{blue} No need to put an algorithm here. If we have a bound for downstream task as well we can fill up the whole procedure.}

%Now we propose the algorithm that accomplishes the subspace retrieval process above. 

In Algorithm \ref{algo:1}, the output $\hat\Ub_r$ is the estimator of the task subspace $\W$. $\hat\Ub_r$ is used as a training step for the few-shot learning phase. For the new task, we search for the function $f^*$ that minimizes the population loss. We shall provide an instructive analysis for the cross-entropy loss, which is usually employed for classification tasks.

\so{Currently, cross-entropy comes out of nowhere. For using cross-ent, label has to be discrete. It cannot be an arbitrary nonlinear function. Overall, we need to do one of the followings:\\
 Option 1: Do the analysis for a Lipschitz loss function for which cross-entropy is a special case.\\
 Option 2: Let us just say that for few-shot phase, we focus on classification and study cross-entropy. Clearly state label is discrete 0-1.}
\begin{definition}\label{def: test}
\textbf{Few-shot classification (Population).} In the few-shot learning phase, suppose $\x,y\sim\Pxy$ satisfy $\mtx{E}(y|\x) = f^*(\W\x)$. Let $\Fc$ be a family of functions as the search space for few-shot learning model. 
Let $\cLCE: \Fc\times \R^{r\times d}\rightarrow \R$ be population cross-entropy loss, defined as 
\begin{align}
    \cLCE(f;\Pb)=-\mtx{E}_{\Pxy} (&y\log f(\Pb \x)\label{eq:cLCE}\\
   &+ (1-y)\log (1 - f(\Pb \x))) \nonumber.
\end{align}
\so{Following my comment above, for cross-ent, clearly $0\leq f\leq 1$. This has to be specified in the definition.}

We search for the solution induced by $\hat{\Ub}_r$ by
\begin{align}
    \hat f &= \argmin_{f\in\Fc}\ \cLCE(f;\hat{\Ub}_r^\top)\label{eq:fstar}
\end{align}
%If $\Pb$ is known, we use $\cLCE(f(\Pb x))$ as an equivalent way of representing $\cLCE(f;\Pb)$.
\end{definition}
Observe that, without representation learning, one has to search for both $f$ and $\Pb$. However with representation learning, we fix $\Pb=\hat{\Ub}_r$ and only search for $f$.
\begin{remark}\label{rem:logistic}
For the GLM Definition \ref{def:GLM}, we can choose $\Fc$ to be the $\ell_2$ norm constrained functions for some $a\leq\infty$% the set of functions $f$ satisfying
% {\color{red} YS: I want to say $\Fc = \phi\circ\bt\circ(\mathrm{variable})$}
\begin{align}
    \Fc = \{\x\rightarrow \phi(\bt^T\x)~\big|~\|\bt\|_2 \le a,~\bt\in\R^r\}, \label{eq:Fcbin}
\end{align}
Let the new data be generated with $f^*(\W\x) = \phi({\bt^*}^\top\W\x)$ for some ground-truth parameter $\bt^*$. We use $\cLCE(\bt;\Pb)$ to denote the cross-entropy loss in this setting. $\hat f$ (parameterized by $\hat{\bt}$) is given by
\begin{align}
    \hat \bt &= \argmin_{\bt}\ \cLCE(\bt;\hat \Ub_r^\top ),\mbox{~such~that~} \|\bt\| \le a. \label{eq:fstarbin}
\end{align}
\end{remark}


\iffalse
\begin{definition}\label{def: test finite}
\textbf{Finite sample few-shot learning.} In the few-shot learning phase, there are in total $n$ samples, and suppose 
$\x_i\in\R^d$ are generated independently, following standard normal distribution, $y_i\in\R$, for $i=1,...,n$. $\x_i$, $y_i$ satisfy $\mtx{E}(y_i|\x_i) = f^*(\W\x_i)$. Lef $\Fc$ be a family of functions as the search space for few-shot activation function. 
Let $\cL_e$ be empirical cross entropy loss, defined as 
\begin{align}
    &\cL_e(f;\Pb) : \Fc\times \R^{r\times d}\rightarrow \R= \notag\\
    &-\frac{1}{n}\sum_{i=1}^n (y_i\log f(\Pb \x_i) + (1-y_i)\log (1 - f(\Pb \x_i))) \label{eq:cLCE finite}
\end{align}
We search for the solution by
\begin{align}
    \hat f_e &= \argmin_{f\in\Fc}\ \cL_e(f;\Ub_r^\top)\label{eq:fstar finite}
\end{align}

\end{definition}
\fi
% and suppose $\x_i\in\R^d$ are generated independently, following standard normal distribution, $y_i\in\R$, for $i=1,...,n$.
\begin{definition}\label{def: test finite}
\textbf{Few-shot learning (Finite sample GLM).} Suppose there are in total $n$ samples for new task $(\x_i,y_i)_{i=1}^n$ and $(\x_i,y_i)$ satisfies $\mtx{E}(y_i|\x_i) = f^*(\W\x_i)$. Lef $\Fc$ be a family of functions for few-shot learning phase. We consider the setup of Remark \ref{rem:logistic}, where $\phi$ is the logistic function. 
%: \Fc\times \R^{r\times d}\rightarrow \R= \notag\\
\begin{align}
    \cL_e(\bt;\Pb)=-\frac{1}{n}\sum_{i=1}^n (&y_i\log(\phi (\bt^\top\Pb \x_i))\label{eq:cLCE finite theta}\\
    &+ (1-y_i)\log (1 - \phi(\bt^\top\Pb \x_i))).\nonumber 
\end{align}
Given an $\ell_2$-norm constraint $a\leq \infty$, the empirical risk minimizer (ERM) is defined as follows
\begin{align}
    \hat \bt_e &= \argmin_{\bt}\ \cL_e(\bt;\Ub_r^\top)\quad\text{such~that}\quad\|\bt\|_2\le a.\label{eq:fstar finite theta}
\end{align}
\end{definition}


\begin{algorithm}[t!]
\caption{Meta-training and Few-shot Learning}\label{algo:1}
\begin{algorithmic}
% with $k$ tasks, the size of data of the $j$-th task has size $n_j$. Dimension $d$. Effective dimension $r$. Set of functions $\Fc$.
\REQUIRE {Dataset $\mathcal{S}$, representation size $r$, function space $\Fc$}
\STATE{Compute $\hat \bM$ via method-of-moments \eqref{eq:hatM}.}
\STATE{Rank $r$ approximation:\\
$\quad\hat\bM_r \leftarrow \hat\Ub_r \mathrm{diag}(\hat \La_{1,1},...,\hat\La_{r,r}) \hat \Ub_r^\top$.}
\STATE{Either~$\hat f \leftarrow \argmin_{f\in\Fc}\ \cLCE(f;\Ub_r^\top) $. $\cLCE$ is defined as \eqref{eq:cLCE}.}
\STATE{Or~~~~~~$\hat f_e \leftarrow \argmin_{f\in\Fc}\ \cL_e(f;\Ub_r^\top) $. $\cL_e$ is defined as \eqref{eq:cLCE finite theta}}
\RETURN{$\hat\Ub_r$ and $\hat f$ or $\hat f_e$.}
\end{algorithmic}
\end{algorithm}%\vspace{-10pt}


==> notation.tex <==

\usepackage{hyperref,graphicx,amsmath,amsfonts,amssymb,bm,url,breakurl,epsfig,epsf,color,MnSymbol,mathbbol,fmtcount,semtrans,caption,subcaption,multirow,comment, boldline, enumitem}
%\usepackage[]{algorithm2e}
%\usepackage[noend]{algpseudocode}
\usepackage{wrapfig}
\usepackage{amssymb}

\usepackage[utf8]{inputenc} % allow utf-8 input
\usepackage[T1]{fontenc}    % use 8-bit T1 fonts
\usepackage{url}            % simple URL typesetting
\usepackage{booktabs}       % professional-quality tables
\usepackage{amsfonts}       % blackboard math symbols
\usepackage{nicefrac}       % compact symbols for 1/2, etc.
\usepackage{microtype}      % microtypography

\makeatletter
\providecommand*{\boxast}{%
  \mathbin{% as \boxplus and \boxtimes
    \mathpalette\@boxit{*}%
  }%
}
\newcommand*{\@boxit}[2]{%
  % #1: math style (\displaystyle, \textstyle, ...)
  % #2: symbol to be boxed that is centered around the math axis
  \sbox0{$\m@th#1\Box$}%
  % Manual correction for font bounding boxes:
  \ifx#1\displaystyle \ht0=\dimexpr\ht0+.05ex\relax \fi
  \ifx#1\textstyle \ht0=\dimexpr\ht0+.05ex\relax \fi
  \ifx#1\scriptstyle \ht0=\dimexpr\ht0+.04ex\relax \fi
  \ifx#1\scriptscriptstyle \ht0=\dimexpr\ht0+.065ex\relax \fi
  \sbox2{$#1\vcenter{}$}% \ht2 is positionn of math axis
  \rlap{%
    \hbox to \wd0{%
      \hfill
      \raisebox{%
        \dimexpr.5\dimexpr\ht0+\dp0\relax-\ht2\relax
      }{$\m@th#1#2$}%
      \hfill
    }%
  }%
  \Box
}
\makeatother

  \makeatletter
\def\BState{\State\hskip-\ALG@thistlm}
\makeatother


  \usepackage{mathtools}
\DeclarePairedDelimiter{\floor}{\lfloor}{\rfloor}

\usepackage{titlesec}

\usepackage{tikz}
\usepackage{pgfplots}
\usetikzlibrary{pgfplots.groupplots}

\setcounter{secnumdepth}{3}

\titleformat{\paragraph}
{\normalfont\normalsize\bfseries}{\theparagraph}{1em}{}
\titlespacing*{\paragraph}
{0pt}{3.25ex plus 1ex minus .2ex}{1.5ex plus .2ex}

\usepackage{movie15}

%\usepackage{caption}
\usepackage[bottom,hang,flushmargin]{footmisc} 

\setlength{\captionmargin}{30pt}

\newcommand{\tsn}[1]{{\left\vert\kern-0.25ex\left\vert\kern-0.25ex\left\vert #1 
    \right\vert\kern-0.25ex\right\vert\kern-0.25ex\right\vert}}

\definecolor{darkred}{RGB}{150,0,0}
\definecolor{darkgreen}{RGB}{0,150,0}
\definecolor{darkblue}{RGB}{0,0,200}
\hypersetup{colorlinks=true, linkcolor=darkred, citecolor=darkgreen, urlcolor=darkblue}

%--------------
\newtheorem{theorem}{Theorem}[section]
\newtheorem{result}{Result}
\newtheorem{problem}{Problem}
\newtheorem{claim}{Claim}
\newtheorem{assumption}{Assumption}
\newtheorem{question}{Question}
\newtheorem{lemma}[theorem]{Lemma}
\newtheorem{corollary}[theorem]{Corollary}
\newtheorem{propo}[theorem]{Proposition}
\newtheorem{definition}[theorem]{Definition}
\newtheorem{condition}[theorem]{Condition}
\newtheorem{conjecture}[theorem]{Conjecture}

\newtheorem{remark}[subsection]{Remark}
\newtheorem{remarks}[subsection]{Remarks}
\newtheorem{example}[subsection]{Example}

%% TT's definitions
\newcommand\tr{{{\operatorname{trace}}}}
\newcommand{\eps}{\varepsilon}
\newcommand{\epsr}{\varepsilon_R}
\newcommand{\mur}{\mu_R}
\newcommand{\bn}{\alpha}
\newcommand{\pp}{{\text{CL}}}
\newcommand{\distas}{\overset{\text{i.i.d.}}{\sim}}
\newcommand{\np}{{n\wedge p}}
\newcommand{\KB}{\bar{K}}
\newcommand{\bG}{\boldsymbol{\Gamma}}
\newcommand{\xw}{\x_{\w}}
\newcommand{\xv}{\x_{\vb}}
\newcommand{\xu}{\x_{\ub}}
\newcommand{\xvt}[1]{\x_{\vb_{#1}}}
\newcommand{\xvtt}[1]{\x_{\vb,#1}}
\newcommand{\xwt}[1]{\x_{#1,\w}}
\newcommand{\xws}[1]{\x_{#1,\ws}}
\newcommand{\xs}{\x_{\ws}}
\newcommand{\yst}{\hat{\y}}
\newcommand{\st}{\star}
\newcommand{\eig}{\text{eigvec}}
\newcommand{\hu}{h}
\newcommand{\ru}{r}
\newcommand{\pbar}{{{\bar{p}}}}
\newcommand{\pbd}{p}
\newcommand{\lay}[1]{{\vct{k}}^{(#1)}}
\newcommand{\lah}[1]{{\vct{\hat{k}}}^{(#1)}}
\newcommand{\lan}{\vct{k}}
\newcommand{\cmp}{P_{\text{nn}}}
\newcommand{\rest}{{\bf{r}}}
\newcommand{\dcp}{\vct{d}^{\text{cnn}}}
\newcommand{\fcp}{\vct{g}^{\text{CNN}}}
\newcommand{\beq}{\begin{equation}}
\newcommand{\nrest}{\bar{n}}
\newcommand{\eeq}{\end{equation}}
\newcommand{\prox}{{{\text{\bf{prox}}}}}
\newcommand{\cov}{{{\text{\bf{cov}}}}}
\newcommand{\ex}{{{\text{\bf{ex}}}}}
\newcommand{\modu}{{{\text{{mod}}}}}
\newcommand{\map}{{{\text{\bf{map}}}}}
\newcommand{\var}[1]{{{\text{\bf{var}}}}[#1]}
\newcommand{\vrn}{\nu}
\newcommand{\func}[1]{{f_{\text{CNN}}}(#1)}
\newcommand{\funh}[1]{{{\hat{f}}_{\text{CNN}}}(#1)}
\newcommand{\funcp}[1]{{f'_{\text{cnn}}}(#1)}
\newcommand{\funcw}[1]{{{{f}}'_{\text{cnn}}}(#1)}
\newcommand{\dev}{{{\text{\bf{dev}}}}}
\newcommand{\meas}{{{\text{\bf{mean}}(\sigma)}}}
\newcommand{\nn}{\nonumber}
\newcommand{\la}{\lambda}
\newcommand{\K}{{K}}
\newcommand{\A}{{\mtx{A}}}
\newcommand{\sfmx}[1]{\text{sfmx}(#1)}
\newcommand{\cat}[1]{\text{Cat}(#1)}
\newcommand{\amp}{\alpha_{\text{cnn}}}
\newcommand{\bOt}{\bigotimes}
\newcommand{\bt}{\boldsymbol{\theta}}
\newcommand{\Bt}{\boldsymbol{\Theta}}
%\newcommand{\nt}{\boldsymbol{n}}

%\newcommand{\bt}{\times}
\newcommand{\robt}[1]{\bigotimes_{\ell=1}^D{#1}_{\ell}}
\newcommand{\robtu}[1]{\bigotimes_{\ell=1}^D{#1}^{(\ell)}}
\newcommand{\bd}{\bigodot}
\newcommand{\kal}{\prod_{i=1}^{D-1}\tn{\lay{i}}}
%\newcommand{\kall}[1]{\prod_{i=1}^{#1}\tn{\lay{i}}}
\newcommand{\kall}[1]{1_{\lan #1}}
\newcommand{\lall}[1]{{\order{\lip_{\lan #1}}}}%{L^{#1}\prod_{i=1}^{#1}\tn{\lay{i}}}
\newcommand{\lell}[1]{{\lip}_{\lan #1}}
\newcommand{\bell}[1]{{{{\beta}}}_{\lan #1}}
\newcommand{\Ub}{{\mtx{U}}}
\newcommand{\Ubb}{{\mtx{U}}}
\newcommand{\V}{{\mtx{V}}}
\newcommand{\ten}{(\{\vb_\ell\}_{\ell=1}^D)}
\newcommand{\uten}{(\{\ub_\ell\}_{\ell=1}^D)}
\newcommand{\ken}{(\{\lay{i}\}_{i=1}^D)}
\newcommand{\B}{{{\mtx{B}}}}
\newcommand{\alx}{{{\alpha_\X}}}
\newcommand{\aly}[1]{{{\alpha_{\X_{#1}}}}}
\newcommand{\Ib}{{{\mtx{I}}}}
\newcommand{\Xbin}{{{\mtx{B}}}}
\newcommand{\Gbin}{{{\mtx{S}}}}
\newcommand{\xbin}{{{\mtx{b}}}}
\newcommand{\Sb}{{{\mtx{S}}}}
\newcommand{\Gb}{{\mtx{G}}}
\newcommand{\ymean}{{\bar{\y}(\w;\text{avg})}}
\newcommand{\yavg}{{{y}_{\text{avg}}}}
\newcommand{\ravg}[1]{{{r}_{{\text{avg}}}(#1)}}
\newcommand{\fmean}{{\funcw{\w;\text{avg}}}}
\newcommand{\diag}[1]{\text{diag}(#1)}
\newcommand{\out}{\text{out}}
\newcommand{\linest}{\text{lin}}
\newcommand{\inp}{\text{in}}
\newcommand{\inh}{\hat{\text{in}}}
\newcommand{\sexp}{subexponential }
\newcommand{\Lc}{{\cal{L}}}
\newcommand{\Nc}{{\cal{N}}}
\newcommand{\Jc}{{\cal{J}}}
\newcommand{\Jcb}{{\overline{\cal{J}}}}
\newcommand{\Dc}{{\cal{D}}}
\newcommand{\Dcg}[1]{{\cal{D}}^{#1}_{\text{subg}}}
\newcommand{\Dct}{{\tilde{\cal{D}}}}
\newcommand{\Sct}{{\tilde{\cal{S}}}}
%\newcommand{\smn}{\s_{\min}}
\newcommand{\btd}{{\bt_{\ell=1}^D d_\ell}}
\newcommand{\Ro}{{\cal{RO}}}
\newcommand{\PC}{{\cal{PC}}}
\newcommand{\Pb}{{\mtx{P}}}
\newcommand{\Tb}{{\mtx{T}}}
\newcommand{\Kba}{{\vct{k}}_{\text{all}}}
\newcommand{\Qb}{{\mtx{Q}}}
\newcommand{\rng}{\gamma}
\newcommand{\Cb}{{\mtx{C}}}
\newcommand{\Eb}{{\mtx{E}}}
\newcommand{\Hb}{{\mtx{H}}}
\newcommand{\Gc}{{\cal{G}}}
\newcommand{\F}{{\mtx{F}}}
\newcommand{\diff}{{\text{diff}}}
\newcommand{\La}{{\boldsymbol{{\Lambda}}}}
%\newcommand{\noresamp}[1]{{\textcolor{red}{#1}}}
\newcommand{\noresamp}[1]{{\textcolor{red}{#1}}}
\newcommand{\sigmap}{\phi'}
\newcommand{\sigmal}[1]{\sigma^{(#1)}}
\newcommand{\sigmalp}[1]{\sigma'^{(#1)}}
\newcommand{\sigmaa}{\sigma'_{\text{all}}}
\newcommand{\sigmai}[1]{\sigma'_{\text{all},#1}}
\newcommand{\bSi}{{\boldsymbol{{\Sigma}}}}
\newcommand{\bSit}{{\boldsymbol{{\tilde{\Sigma}}}}}
\newcommand{\bSih}{{\boldsymbol{{\hat{\Sigma}}}}}
\newcommand{\bmu}{{\boldsymbol{{\mu}}}}
\newcommand{\Db}{{\mtx{D}}}
\newcommand{\db}{{\vct{d}}}
\newcommand{\oneb}{{\mathbb{1}}}
\newcommand{\onebb}{{\mathbf{1}}}
\newcommand{\Iden}{{\mtx{I}}}
\newcommand{\M}{{\mtx{M}}}
\newcommand{\gm}{\gamma_m}
\newcommand{\order}[1]{{\cal{O}}(#1)}
\newcommand{\rmax}[1]{{\bf{r}_{\max}(#1)}}
\newcommand{\rbmax}[1]{{\bf{\bar{r}}_{\max}(#1)}}
\newcommand{\rmin}[1]{{\bf{r}_{\min}(#1)}}
\newcommand{\smn}[1]{{s_{\min}(#1)}}
\newcommand{\smx}[1]{{s_{\max}(#1)}}
\newcommand{\z}{{\vct{z}}}
\newcommand{\zb}{{\bar{\z}}}
\newcommand{\el}{{\ell}}
\newcommand{\tn}[1]{\|{#1}\|_{\ell_2}}
\newcommand{\tff}[1]{\|{#1}\|_{\ell_4}}
\newcommand{\tin}[1]{\|{#1}\|_{\ell_\infty}}
\newcommand{\trow}[1]{\|{#1}\|_{2,\infty}}
\newcommand{\bad}{{\bar{d}}}
\newcommand{\Dp}{{D^+}}
\newcommand{\tf}[1]{\|{#1}\|_{F}}
\newcommand{\te}[1]{\|{#1}\|_{\psi_1}}
\newcommand{\tsub}[1]{\|{#1}\|_{\psi_2}}
\newcommand{\tsut}[1]{\|{#1}\|_{\psi_{2/3}}}
\newcommand{\tsup}[1]{\|{#1}\|_{\psi_a}}
\newcommand{\dist}[1]{\text{dist}(#1)}
\newcommand{\upp}{{\cal{B}}_{\alpha,\Gamma}}
\newcommand{\upz}{{\cal{B}}_{\alpha_0,\Gamma}}
\newcommand{\dpz}{{\cal{D}}_{\alpha_0,\Gamma}}
\newcommand{\dpp}{{\cal{D}}_{\alpha,\Gamma}}
\newcommand{\mpp}{M_{\alpha,\Gamma}}
%\newcommand{\supp}[1]{\text{supp}(#1)}
\newcommand{\cone}[1]{{\text{cone}(#1)}}
\newcommand{\paf}{\partial f(\x)}
\newcommand{\Cc}{\mathcal{C}}
\newcommand{\Ac}{\mathcal{A}}
\newcommand{\Ccb}{\bar{\mathcal{C}}}
\newcommand{\Xc}{\mathcal{X}}
\newcommand{\xc}{{\text{excess}}}
\newcommand{\Rc}{\mathcal{R}}
\newcommand{\Rcp}{\mathcal{\bar{R}}'}
\newcommand{\Rcb}{\mathcal{N}}
\newcommand{\btrue}{\bbeta_{true}}
\newcommand{\bteta}{\boldsymbol{\theta}}
\newcommand{\bbteta}{\widetilde{\boldsymbol{\theta}}}
\newcommand{\brteta}{\overline{\boldsymbol{\theta}}}
\newcommand{\bbeta}{{\boldsymbol{\beta}}}
\newcommand{\ddelta}{{\boldsymbol{\delta}}}
\newcommand{\babeta}{{\bar{\beta}}}
\newcommand{\balpha}{{\bar{\alpha}}}
\newcommand{\bgamma}{{\bar{\gamma}}}
\newcommand{\Bc}{\mathcal{B}}
\newcommand{\Sc}{\mathcal{S}}
\newcommand{\Mc}{\mathcal{M}}
\newcommand{\pa}{{\partial}}
\newcommand{\Nn}{\mathcal{N}}
\newcommand{\pol}{^\circ}
\newcommand{\vb}{\vct{v}}
\newcommand{\Jb}{\mtx{J}}
\newcommand{\Jt}{\mtx{\tilde{J}}}
\newcommand{\vbl}{\vct{v}^{\text{lin}}}
\newcommand{\fb}{\vct{f}}
\newcommand{\ib}{{\bf{i}}}
\newcommand{\hib}{{\bf{\hat{i}}}}
\newcommand{\Ic}{{\mathcal{I}}}
\newcommand{\all}{{\text{all}}}
\newcommand{\vh}{\vct{\hat{v}}}
\newcommand{\vbb}{\vct{\bar{v}}}
\newcommand{\Xb}{\mtx{\bar{X}}}
\newcommand{\abb}{\mtx{\bar{a}}}
\newcommand{\cb}{\mtx{c}}
\newcommand{\bbb}{\mtx{\bar{b}}}
\newcommand{\w}{\vct{w}}
\newcommand{\err}[1]{\text{Err}_{\Dc}(#1)}
\newcommand{\Wp}{\mtx{W}^\dagger}
\newcommand{\tilW}{\widetilde{\mtx{W}}}
\newcommand{\tilw}{\widetilde{\vct{w}}}
\newcommand{\ob}{\mtx{o}}
\newcommand{\obh}{\mtx{\hat{o}}}
\newcommand{\wh}{{\hat{\mtx{w}}}}
\newcommand{\li}{\left<}
\newcommand{\ri}{\right>}
\newcommand{\s}{\vct{s}}
\newcommand{\sh}{\hat{\vct{s}}}
\newcommand{\ab}{\vct{a}}
\newcommand{\bb}{\vct{b}}
\newcommand{\ub}{{\vct{u}}}
\newcommand{\ubb}{\bar{\vct{u}}}
\newcommand{\h}{\vct{h}}
\newcommand{\hh}{{\vct{h}}}
\newcommand{\g}{{\vct{g}}}
\newcommand{\ii}{{\vct{i}}}
\newcommand{\zm}[1]{{\text{{\bf{zm}}}(#1)}}
\newcommand{\dd}{{\vct{d}}}
\newcommand{\ddt}{{\vct{d}}_\tau}
\newcommand{\Zb}{\mtx{Z}}
\newcommand{\hf}{\hat{f}}
\newcommand{\corrCA}{\rho_\Cc(\M)}
\newcommand{\corr}[1]{{\bf{cor}}(#1)}
\newcommand{\Tc}{\mathcal{T}}
\newcommand{\Fc}{\mathcal{F}}
\newcommand{\Hc}{\mathcal{H}}


%%YP's macros
\newcommand{\qqq}[1]{{\textcolor{red}{?{#1}?}}}
\newcommand{\ihere}{{\textcolor{red}{I AM HERE! }}}
\newcommand{\mat}[1]{{\text{mat}{#1}}}
\newcommand{\gb}{\bar{\g}}
\newcommand{\bs}{\bar{s}}
\newcommand{\cgain}{\alpha_{\text{CNN}}}
\newcommand{\cgainp}{\tn{\E_{\x\sim\Nn(0,\Iden)}[\gcnn{}]}}
\newcommand{\gcnn}[1]{{\vct{g}}_{\text{cnn}#1}}
\newcommand{\ccorr}{\rho_{\text{cnn}}}
\newcommand{\kb}{\vct{k}}
\newcommand{\xh}{\hat{\x}}
\newcommand{\yh}{\hat{\y}}
\newcommand{\xbr}{\bar{\h}}
\newcommand{\xdr}{\tilde{\x}}
\newcommand{\m}{\vct{m}}
\newcommand{\xt}{\tilde{\x}}
\newcommand{\nt}{\tilde{n}}
%\newcommand{\ht}{\tilde{h}}
\newcommand{\rt}{\tilde{r}}
\newcommand{\ft}{\tilde{f}}
\newcommand{\yt}{\tilde{\y}}
\newcommand{\gh}{\hat{\g}}
\newcommand{\gt}{\tilde{\g}}
\newcommand{\wb}{\bar{\w}}
\newcommand{\lip}{L}
\newcommand{\mipp}{L_{\max}}
\newcommand{\mupp}{\bar{\mu}_{\max}}
\newcommand{\mapp}{\mu}
\newcommand{\tcnn}{{\mtx{T}}_{\text{cnn}}}
\newcommand{\lcnn}{{\mtx{L}}_{\text{CNN}}}
\newcommand{\lipa}{{L}}
\newcommand{\smo}{S}
\newcommand{\SM}{{{\bf{S}}}_{L,\kb}}
\newcommand{\SMB}{{{\bf{\bar{S}}}}_{L,\kb}}
\newcommand{\Ws}{\W^\star}
\newcommand{\ws}{{\w^\star}}
\newcommand{\wss}{{\w^\star}}
\newcommand{\yp}[1]{\textcolor{red}{ #1}}
\newcommand{\zeronorm}[1]{\left\|#1 \right\|_0}
\newcommand{\unorm}[1]{\left\|#1 \right\|_u}
\newcommand{\ynorm}[1]{\left\|#1 \right\|_{\bar{y}}}
\newcommand{\onetwonorm}[1]{\left\|#1\right\|_{1,2}}
\newcommand{\opnorm}[1]{\left\|#1\right\|}
\newcommand{\fronorm}[1]{\left\|#1\right\|_{F}}
\newcommand{\onenorm}[1]{\left\|#1\right\|_{\ell_1}}
\newcommand{\twonorm}[1]{\left\|#1\right\|_{\ell_2}}
\newcommand{\wnorm}[2]{\left\|#1\right\|_{#2}}
\newcommand{\Dnorm}[1]{\left\|#1\right\|_{D}}
\newcommand{\oneinfnorm}[1]{\left\|#1\right\|_{1,\infty}}
\newcommand{\infnorm}[1]{\left\|#1\right\|_{\ell_\infty}}
\newcommand{\nucnorm}[1]{\left\|#1\right\|_*}
\newcommand{\abs}[1]{\left|#1\right|}
\newcommand{\avg}[1]{\left< #1 \right>}

\newcommand{\lipp}{\prod_{\ell=1}^D \twonorm{\vct{k}^{(\ell)}}}

\renewcommand{\d}{\mathrm{d}}

\newcommand{\cA}{\mathcal{A}}
\newcommand{\rotd}{\text{R1TD}}
\newcommand{\nntd}{\text{DeepTD}}
\newcommand{\x}{\vct{x}}
\newcommand{\rb}{\vct{r}}
\newcommand{\rbb}{\vct{\widetilde{r}}}
\newcommand{\y}{\vct{y}}
\newcommand{\ybh}{\vct{\hat{y}}}
\newcommand{\W}{\mtx{W}}
\newcommand{\Wc}{{\cal{W}}}
\newcommand{\Vc}{{\cal{V}}}
\newcommand{\bgl}{{~\big |~}}

%--------------

% EJC's macros

\definecolor{emmanuel}{RGB}{255,127,0}
\newcommand{\ejc}[1]{\textcolor{emmanuel}{EJC: #1}}

\newcommand{\p}{{\vct{p}}}
\newcommand{\Kb}{{\mtx{K}}}
\newcommand{\somelog}{16\Kb\log (\Kb)}
\newcommand{\somelg}{\Kb\log (\Kb)}
\newcommand{\pb}{{\vct{p}}}
\newcommand{\qb}{{\vct{q}}}
\newcommand{\R}{\mathbb{R}}
\newcommand{\Pro}{\mathbb{P}}
\newcommand{\C}{\mathbb{C}}
\newcommand{\Z}{\mathbb{Z}}
\newcommand{\<}{\langle}
\renewcommand{\>}{\rangle}
\newcommand{\Var}{\textrm{Var}}
\newcommand{\sgn}[1]{\textrm{sgn}(#1)}
\renewcommand{\P}{\operatorname{\mathbb{P}}}
%\newcommand{\E}{\operatorname{\mathbb{E}}}
\newcommand{\EE}{\operatorname{\mathbb{E}}}
%\newcommand{\var}{\operatorname{\mathbf{var}}}

\newcommand{\todo}[1]{{\bf TODO: #1}}
\newcommand{\grad}[1]{{\nabla\Lc(#1)}}
\newcommand{\gradf}[1]{{\nabla f(#1)}}
\newcommand{\hessf}[1]{{\nabla^2f(#1)}}
\newcommand{\gradw}[1]{{\nabla{\Lc}(#1)}}
\newcommand{\grd}[2]{{\nabla\Lc_{#1}(#2)}}
\newcommand{\e}{\mathrm{e}}
\newcommand{\eb}{\vct{e}}
\renewcommand{\i}{\imath}

\newcommand{\vct}[1]{\bm{#1}}
\newcommand{\mtx}[1]{\bm{#1}}

% MS's macros

\newcommand{\rank}{\operatorname{rank}}
\newcommand{\supp}[1]{\operatorname{supp}(#1)}
\newcommand{\restrict}[1]{\big\vert_{#1}}
\newcommand{\Id}{\text{\em I}}
\newcommand{\OpId}{\mathcal{I}}

\newcommand{\Real}{\operatorname{Re}}
\newcommand{\Imag}{\operatorname{Im}}

\newcommand{\piyp}{\pi'_1(\vct{y})}
\newcommand{\piy}{\pi_1(\vct{y})}
\newcommand{\piar}{\pi_1(\vct{a}_r)}
\newcommand{\piarp}{\pi'_1(\vct{a}_r)}
\newcommand{\set}{{\cal{F}}}
\newcommand{\des}{{\x_0}}

\newcommand{\Pc}{{\cal{P}}}
\newcommand{\X}{{\mtx{X}}}
\newcommand{\Y}{{\mtx{Y}}}
\newcommand{\Vb}{{\mtx{V}}}
\newcommand{\Vh}{\hat{{\mtx{V}}}}
\newcommand{\Vbd}{{\mtx{V}^\dagger}}
\newcommand{\Rb}{{\mtx{R}}}

\newcommand{\calF}{\mathcal{I}}
\newcommand{\calS}{\mathcal{N}}


\newcommand{\MS}[1]{\textcolor{blue}{MS: #1}}
\newcommand{\MST}[1]{\textcolor{red}{#1}}
\newcommand{\SO}[1]{\textcolor{darkgreen}{SO: #1}}


\numberwithin{equation}{section} 

\def \endprf{\hfill {\vrule height6pt width6pt depth0pt}\medskip}
%\newenvironment{proof}{\noindent {\bf Proof} }{\endprf\par}
\newenvironment{proofsk}{\noindent {\bf Proof sketch} }{\endprf\par}


%\newcommand{\qed}{{\unskip\nobreak\hfil\penalty50\hskip2em\vadjust{}
           %\nobreak\hfil$\Box$\parfillskip=0pt\finalhyphendemerits=0\par}}


\newcommand{\note}[1]{{\bf [{\em Note:} #1]}}

\newcommand{\iprod}[2]{\left\langle #1 , #2 \right\rangle}

\newcommand{\red}{\textcolor{red}}
\newcommand{\gi}{\ab_{\gamma_i}}
\newcommand{\ang}{\text{ang}}
\newcommand{\ham}[2]{{\|#1,#2\|_H}}

%\renewcommand{\algorithmicrequire}{\textbf{Input:}}
%\renewcommand{\algorithmicensure}{\textbf{Output:}}

%AJ's macros
\newcommand{\hth}{{\widehat{\boldsymbol{\theta}}}}
\newcommand{\bth}{{\boldsymbol{\theta}}}
\newcommand\cL{\mathcal{L}}
\newcommand\cD{\mathcal{D}}
\newcommand\hcD{\widehat{\cD}}
\newcommand\reals{\mathbb{R}}
\newcommand\bSigma{\boldsymbol{\Sigma}}
\newcommand\normal{{\sf N}}
\newcommand\bdelta{\boldsymbol{\delta}}
\newcommand\sign{{\rm sign}}
\newcommand\sT{{\sf T}}
\newcommand\I{\mtx{I}}
\newcommand\zero{\mtx{0}}
\newcommand\bA{\mtx{A}}
\newcommand\bv{\mtx{v}}
\newcommand\cI{\mathcal{I}}
\newcommand\bz{\boldsymbol{z}}
\newcommand\bg{\boldsymbol{g}}
\newcommand\ba{\boldsymbol{a}}
\def\cC{\mathcal{C}}
\def\de{{\rm d}}
\def\bM{\mtx{M}}
\def\cH{\mathcal{H}}
\def\bu{\boldsymbol{u}}
\def\by{\boldsymbol{y}}
\def\bw{\boldsymbol{w}}
\def\bX{\boldsymbol{X}}
\def\tbX{\tilde{\boldsymbol{X}}}
\def\tbx{\tilde{\boldsymbol{x}}}
\def\tbth{\tilde{\boldsymbol{\theta}}}
\def\hz{\widehat{z}}
\def\ind{\mathbf{1}}
\def\cS{\mathcal{S}}
\def\prob{\mathbb{P}}
\def\tx{\tilde{x}}
\def\reals{\mathbb{R}}
\newcommand{\aj}[1]{\noindent{\textcolor{blue}{\textbf{\#\#\# AJ:} \textsf{#1} \#\#\#}}}

\newcommand{\gauss}{\mathcal{N}(0,I)}
\newcommand{\gausscov}[1]{\mathcal{N}(0,{#1})}
\newcommand{\argmin}{\mathop{\mathrm{argmin}}}
%\newcommand{\cLCE}{\cL_{\mathrm{CE}}}
\newcommand{\cLCE}{\cL}
\newcommand{\mscrU}{{\mathscr{U}}}

==> s_exp.tex <==
\maketitle
\section{Numerical Experiments}\vspace{-5pt}
\label{s:exp}

% {\color{blue} Leave to Ibrahim}

% {\color{blue} I can roughly see what you did, but I'm not sure about a few details. Maybe I can mark down and talk to you on Mon, I'll have enough time to edit after that.}


We generate synthetic datasets with $k$ different tasks and $n$ samples for all tasks. As dimension of the data and dimension of the subspace we choose $d=50$ and $r=5$, respectively. %In all experiments we choose all $n_j$'s to be same i.e.~$n_j=n$. 

We study two different setups. In the first one data is generated according to Def.~\ref{def:GLM}. For the second setup, there is an underlying 3-layer neural network that fits the data. In both setups our only aim is to retrieve subspace representations of the data using Algorithm \ref{algo:1}.

\begin{figure}[t!]
\centering
\begin{subfigure}[htbp!]{0.23\textwidth}
\centering
\includegraphics[width = \linewidth]{Paper/Figures_in_Paper/11.png}
\subcaption{}\label{fig1a}
\end{subfigure}
\begin{subfigure}[htbp!]{0.23\textwidth}
\centering
\includegraphics[width =\linewidth]{Paper/Figures_in_Paper/21.png}
\subcaption{}\label{fig1b}
\end{subfigure}
\vspace{-0.35cm}
\captionsetup{width=\linewidth}{\caption{Subspace correlations with fixed number of tasks. \hspace{0.4cm}(a) Binary classification (b) Neural network.}  \label{fig1}} 
\end{figure} 

For neural network experiments, we assume that the data are generated from a ground truth neural network which has 3 layers, defined as  
$$ \yij = f^j(\xij) + \epsilon_{i,j} = \mtx{W}_{j3}(\mtx{W}_{j2}(\mtx{W}_{j1}(\mtx{W}\xij))_+)_+ + \epsilon_{i,j}$$ 
where  $\epsilon_{i,j}\sim\Nn(0,1)$ is gaussian noise, $(\cdot)_+$ is the ReLU activation function, $\mtx{W}\in\R^{5\times 50}$ is representation matrix which is same for all $j$'s. The weight matrices $\mtx{W}_{j1},\mtx{W}_{j2}$ and $\vct{W}_{j3}$ are different for each task and they are random gaussian matrices in $\R^{20\times 5},\R^{20\times 20},\R^{20}$ respectively.
\vspace{0cm}
\iffalse
\begin{figure}[htbp!]
\centering
\begin{subfigure}[htbp!]{0.23\textwidth}
\centering
\includegraphics[width = \linewidth]{Paper/Figures_in_Paper/12.png}
\subcaption{}\label{fig2a}
\end{subfigure}
\begin{subfigure}[htbp!]{0.23\textwidth}
\centering
\includegraphics[width =\linewidth]{Paper/Figures_in_Paper/22.png}
\subcaption{}\label{fig2b}
\end{subfigure}
\vspace{-0.2cm}
\captionsetup{width=\linewidth}{\caption{Subspace correlations with fixed number of samples per task and varying number of tasks. (a) Binary classification, (b) Neural network.}  \label{fig2}} 
\end{figure} 
\fi
%{\color{blue} Could you send me the data of the plots? I can work on the figure a bit. It would be better to set ``ylim'' so that the lines span the range of vertical direction. E.g., ylim=[0.4,1] in the first figure. And don't use colors, ICASSP requires grey-scale figures so we can't tell by color.}

In Fig.~\ref{fig1}
%, we apply Algorithm \ref{algo:1} to recover the $r$ dimensional subspace and get $\hat \Ub_r$, and check its distance to the true representation space $\Ub_r$ under different $n$'s and $k$'s. 
we use the subspace correlation as the metric for evaluating the accuracy of subspace recovery, which is defined by  $\frac{\|{\hat{\mtx{U}_r}^\top\mtx{U}_r}\|^2}{\|\mtx{U}_r\|^2}$.
In Fig.~\ref{fig1}, $k=100$ is fixed but $n$'s vary from $20$ to $200$. It can be seen from Fig.~\ref{fig1} that as $nk$ gets bigger, the subspace correlation becomes closer to $1$, which is compatible with Theorem \ref{thm:hatM}

In Fig.~\ref{fig3}(a), the downstream task accuracies for binary classification are depicted. For the new task, a new 1-layer neural network without any activation function is trained with and without the retrieved representations of the earlier tasks. We find the parameters of the neural network by minimizing the cross entropy loss via SGD. For this setup, during meta-training, we set $n=50$ for all tasks and $k=2000$, to have almost perfect representation. We evaluate the test error with $1000$ new samples.
%by generating $1000$ samples from the same task, 

\begin{figure}[t!]
\centering
\begin{subfigure}[htbp!]{0.24\textwidth}
\centering
\includegraphics[width =  \linewidth]{Paper/Figures_in_Paper/colorednewtaskacc.png}
\end{subfigure}
\hspace{-0.2em}
\begin{subfigure}[htbp!]{0.22\textwidth}
\centering
\includegraphics[width =  \linewidth]{Paper/Figures_in_Paper/alltogether.png}
\end{subfigure}
\captionsetup{width=.45\textwidth}{\caption{(a) Accuracy for downstream task, binary classification (b) Accuracy for downstream the task, MNIST} \label{fig3}}
\end{figure}


If the number of few-shot training samples is small, accuracy improves much faster when we use representation learning. This validates that dimension reduction reduces the degrees-of-freedom for few-shot learning, so the optimal model can be learned with fewer samples. As the sample size grows, the relative benefit of representation is smaller but still noticeable.

In Fig. \ref{fig3}(b), Algorithm \ref{algo:1} is also tested in MNIST dataset. $d=784$ and $r$ is not known. We assume that we have different binary classification tasks among pairs of digits such as 0-1;2-3;0-8;8-4 etc. There exist 15 meta-training tasks (i.e., $k=15$). For each task we have 500 samples in each classes. We choose a different pair of classes as few-shot learning task. We choose binary classification among images of 1 and 9, which is not included in the meta-learning phase. We tune the predicted subspace dimensions and number of samples to get Fig. \ref{fig3}(b).
\iffalse
\begin{figure}[htbp!]
\centering
\begin{subfigure}[htbp!]{0.37\textwidth}
\centering
\includegraphics[width =   \linewidth]{Paper/Figures_in_Paper/alltogether.png}
\end{subfigure}
\captionsetup{width=.45\textwidth}{\caption{Accuracy for downstream the task,MNIST} \label{figlast}}
\end{figure}
\vspace{-0.25cm}
\fi
It can be concluded that when $r=20$, 
%it does not serve a good representation 
The downstream task is not learnt well so we need to expand the subspace. For $r=50$ and $r=100$ subspace learning helps for few-shot learning, as when the number of training samples $n$ is between 8-56 they outperform the case without representation. When $r$ gets closer to $d$, the few-shot sample size has to be large to succeeed due to higher degree of freedom.
%When it comes to $r=400$ we deduce that we get results very similar to no representation case, as when $r$ is big and close to $d$, the model has huge degree of freedom so for good test accuracies $n$ must be big.
% \begin{figure}[htbp!]
% \centering
% \begin{subfigure}[htbp!]{0.35\textwidth}
% \centering
% \includegraphics[width =  \linewidth]{Paper/Figures_in_Paper/r15_1vs8_bluered_new_n.png}
% \end{subfigure}
% \captionsetup{width=.45\textwidth}{\caption{Accuracy for downstream task} \label{fig3}}
% \end{figure}
% \vspace{-0.25cm}


% \begin{figure}[htbp!]
% \centering
% \begin{subfigure}[htbp!]{0.35\textwidth}
% \centering
% \includegraphics[width =  \linewidth]{Paper/Figures_in_Paper/r15_1vs8_bluered_new_n.png}
% \end{subfigure}
% \captionsetup{width=.45\textwidth}{\caption{Accuracy for downstream task} \label{fig3}}
% \end{figure}
% \vspace{-0.25cm}
% \section{Conclusion and Future Work}
% In this work we showed that subspace-based representations can be efficiently learned for highly nonlinear tasks including GLMs and neural networks and help reduce sample complexity for future downstream tasks. A drawback of our results is that they are restricted to normally distributed data. It would be desirable to address such limitations by using distributional universality results such as \cite{oymak2018universality,abbasi2019universality}. Another direction is developing a more refined understanding for deep learning by restricting our nonlinear model space to deep neural nets.
%in contrast to more general purpose results developed here.
% {\color{red} YS: The blue curve is about 0.9, I feel it's already very accurate so we don't need this paragraph.}
% Additionally, we generate samples as defined in Def. \ref{def:bin_class}. $y$ conditioned on $\x$ is a random variable, yet not deterministic, so the data is implicitly noisy. Therefore the accuracy cannot reach $1$ empirically on the generated data.
% In Fig. \ref{fig1}, subspace correlations between the actual subspace and the predicted one using Algorithm \ref{algo:1}. Subspace correlations are calculated by  $\frac{\|{\hat{\mtx{U}_r}^\top\mtx{U}_r}\|^2}{\|\mtx{U}_r\|^2}$.It can be deduced that in both nonlinear setup subspace can be learned via moment estimator $t_j$ increases.
% \begin{figure}[htbp!]
% \centering
% \begin{subfigure}[htbp!]{0.4\textwidth}
% \centering
% \includegraphics[width = \linewidth]{Paper/Figures_in_Paper/GrayScale_NN_k100_subspace.png}
% \subcaption{}\label{fig1a}
% \end{subfigure}
% \begin{subfigure}[htbp!]{0.4\textwidth}
% \centering
% \includegraphics[width =\linewidth]{Paper/Figures_in_Paper/GrayScale_NN_nj30_subspace.png}
% \subcaption{}\label{fig1b}
% \end{subfigure}
% \captionsetup{width=.45\textwidth}{\caption{Subspace correlations, (a) for binary classification task whereas (b) stands for 3-layer Neural Net experiment.}  \label{fig1}} 
% \end{figure} 


==> s_gen_loss_proof.tex <==

\section{Proof of main theorems}

\iffalse
\SO{Clearly Theorem \ref{thm:hatM append} is a restatement of Theorem \ref{thm:hatM}. Why don't you say so? Reader is not expected to figure out this by himself. Let us make things clear.}

\SO{Similarly, where is proof of Lemma 3.1? Looks like Lemma \ref{lem:mean nn} is its restatement but again not clear at all for reader. They cannot find proof of Lemma 3.1 in the text.}

\SO{Here is the organization we need: In the appendix, proof of each technical result in the main text is supposed to have its own subsection. Just like this subsection that I added i.e.~Proof of Theorem \ref{thm:hatM}.}
\SO{Maybe briefly describe the outline. Right now, little confusing due to Lemmas within the proof so outline would help i.e.~we first prove Lemma ... which shows ...}
\subsection{Proof of Lemma \ref{lem:M exp} and Theorem \ref{thm:hatM}}
\fi
We sketch the proof at the beginning. First we compute the expectation of $y\x$ in Lemma \ref{lem:mean nn}. That leads to the proof of Lemma \ref{lem:M exp}. Then in Lemma \ref{lem:err_yx} we bound the difference between sum of $y\x$ and its mean using concentration. The concentration of covariance estimator is studied later in Lemma \ref{lem:Zj} and \ref{lem:Zj2}, which leads to Theorem \ref{thm:hatM}.

\subsubsection{Proof of Lemma \ref{lem:M exp}}
We first state Lemma \ref{lem:M exp} below.
\begin{lemma}\label{lem:M exp append}
Let 
\begin{subequations}\label{eq:hatM append}
\begin{align}
\hat\bM &= \mathop{\Scale[1.8]{\sum}}_{j=1}^k \frac{2}{n_j^2}\left[(\sum_{i=1}^{n_j/2} \yij\xij) (\sum_{i=n_j/2+1}^{n_j} \yij\xij)^\top \right.\\
&\quad\quad\quad\quad \left. +  ( \sum_{i=n_j/2+1}^{n_j} \yij\xij) ( \sum_{i=1}^{n_j/2} \yij\xij)^\top\right].\nonumber
\end{align}
\end{subequations}
And
\begin{align*}
    &\mtx{h}^j(\W): \R^{r\times d} \rightarrow \R^d = \mtx{E}_{\x}[f^j(\W \x)\x]\\
    &\bM := \W^\top\W\left(\frac{1}{k}\sum_{j=1}^k \mtx{h}^j(\W)( \mtx{h}^j(\W))^\top\right)\W^\top\W.
\end{align*}
Then $\bM,\hat{\bM}$ satisfies the following. (a) $\text{rank}(\bM)\leq r$. (b) $\text{range-space}(\bM)\subset \text{row-space}(\W)$. (c) $\mtx{E}[\hat{\M}]=\bM$. 
\end{lemma}
\begin{proof}
Part (a) and (b) are easy to see. $\W\in\R^{r\times d}$ so that $\text{rank}(\bM)\leq r$, and since $\bM$ is the product of $\W^\top$ and another matrix, then  $\text{range-space}(\bM)\subset \text{row-space}(\W)$.
Now we will prove Part (c). We first give the lemma for the mean of the random vector $y\x$.

\begin{lemma}\label{lem:mean nn}
We assume that the data is generated as in Def. \ref{def:task}, and we study the $j$-th task whose activation function is $f^j$. 
%{\color{blue} To be finished}
Define
\begin{align*}
    \mtx{h}^j(\W): \R^{r\times d} \rightarrow \R^d = \mtx{E}_{\x\sim\gauss} f^j(\W \x)  \x
\end{align*}
Denote the joint distribution of $(\x,y)$ as $\Pxy$.
Then $\mtx{E}_{(\x,y)\sim\Pxy}(y \x) = \W^\top\W \mtx{h}^j(\W)$.
\end{lemma}

\emph{Proof of Lemma \ref{lem:mean nn}.} The expectation can be expanded as
\begin{align*}
    &\mtx{E}_{(\x,y)\sim\Pxy}(y \x) \\
    &= \mtx{E}_{\x\sim\gauss} f^j(\W \x) \x\\
    &= \mtx{E}_{\x\sim\gauss} \left(f^j(\W \x)  \W^\top\W \x + f^j(\W \x) (I - \W^\top\W)\x \right).
\end{align*}
Note that, because $\x\sim\gauss$ so $\W \x$ and $(I - \W^\top\W)\x$ are Gaussian. $\W\W^\top = I$ implies 
\begin{align*}
    &\quad \Eb (\W \x)\x^\top((I - \W^\top\W))\\
    &= \W(I - \W^\top\W) = 0.
\end{align*}
So $\W \x$ and $(I - \W^\top\W)\x$ are independent, so 
\begin{align*}
    &\quad \mtx{E}_{\x\sim\gauss}  f^j(\W \x) (I - \W^\top\W)\x \\
    &= (\mtx{E}_{\x\sim\gauss}  f^j(\W \x)) (\mtx{E}_{\x\sim\gauss} (I - \W^\top\W)\x) = 0
\end{align*}
Then 
\begin{align*}
    \mtx{E}_{(\x,y)\sim\Pxy}(y \x) &= \W^\top\W(\mtx{E}_{\x\sim\gauss} f^j(\W \x) \x)\\
    &= \W^\top\W \h_j(\W).
\end{align*}

Denote 
\begin{align}\label{eq:Hj def}
    \Hb^j(\W) = \W^\top\W \mtx{h}^j(\W)
\end{align}
Because $\frac{2}{n_j}\sum_{i=1}^{n_j/2} \yij\xij$
and 
$\frac{2}{n_j}\sum_{i={n_j/2}+1}^{n_j} \yij\xij$ 
are independent, and their expectation are both $\Hb^j(\W)$, so that
\begin{align*}
    &\quad \mtx{E}(\frac{2}{n_j}\sum_{i=1}^{n_j/2} \yij\xij)(\frac{2}{n_j}\sum_{i={n_j/2}+1}^{n_j} \yij\xij)^\top \\
    &= \Hb^j(\W)(\Hb^j(\W))^\top.
\end{align*}
At then end
\begin{align*}
    \hat \bM &= \frac{1}{k}\sum_{j=1}^k \mtx{E}(\frac{2}{n_j}\sum_{i=1}^{n_j/2} \yij\xij)(\frac{2}{n_j}\sum_{i={n_j/2}+1}^{n_j} \yij\xij)^\top,\\
    \bM &= \frac{1}{k}\sum_{j=1}^k\Hb^j(\W)(\Hb^j(\W))^\top,
\end{align*}
so we can prove Part (c) that $\mtx{E}(\hat \bM) = \bM$.
\end{proof}


\subsubsection{Proof of Theorem \ref{thm:hatM}}
We restate Theorem \ref{thm:hatM append} below. 
\begin{theorem}\label{thm:hatM append}
Suppose the data is generated as Def. \ref{def:task}. Let $\delta\in(0,1)$, $\epsilon\in(0,1)$. Suppose $y\x$ is a subGaussian random vector with covariance upper bounded by
\begin{align}
   \| \mathbf{Cov}(y \x) \| \le \sigma^2. \label{eq:covyx append}
\end{align} 
Define
\begin{align*}
    \mtx{h}^j(\W): \R^{r\times d} \rightarrow \R^d = \mtx{E}_{\x\sim\gauss} f^j(\W \x)  \x
\end{align*}
And let %$\bM = \mtx{E}_{\theta\sim\mathcal{N}(0,\bSi)} (g(\theta))^2\frac{\theta\theta^\top}{\|\theta\|^2}$, then
\begin{align*}
    \bM = \W^\top\W\left(\frac{1}{k}\sum_{j=1}^k \mtx{h}^j(\W)( \mtx{h}^j(\W))^\top\right)\W^\top\W
\end{align*}
Then there exists a constant $c$, with probability at least $1-\delta$, let 
\begin{align*}
    k = \frac{cd}{n}\log^2(\frac{kd}{\delta}) \max\{\frac{1}{\epsilon^2}, \frac{1}{\epsilon} \log(\frac{kd}{\delta})\}
\end{align*}
we have 
\begin{align*}
    \|\hat \bM - \bM\| \le \epsilon\sigma^2.
\end{align*}
\end{theorem}
\begin{proof}
The following lemmas are similar to \cite{kong2020meta} Section A.1. We extend the concentration inequalities from bounded random vectors to Gaussian random vectors. For completeness we place the lemmas here.

\begin{lemma}\label{lem:err_yx}
(\cite{jin2019short} Cor. 7) 
Let $\|\mathbf{Cov}(y\x)\| \le \sigma^2$, $\delta\in(0,1)$, $t>0$, $\Hb^j(\W)$ be defined in \eqref{eq:Hj def}. With probability $1-\delta$, there exists a constant $c>0$ such that for every $j$,
%\som{Remind the exact assumption on $\sigma$}
\begin{align}
   \|\frac{1}{t}\sum_{i=1}^t \yij\xij - \Hb^j(\W)\| \le c\sigma\sqrt{\frac{d}{t}\log(\frac{kd}{\delta})} \label{eq:gauss_bern}
\end{align}
%\som{Call $\W^\top\W \mtx{h}^j(\W)$ something for simpler notation}
Denote this event as $\mathcal{E}$.
\iffalse
{\it\color{red} for every i,j pairs ? }Denote this event as $\mathcal{E}$.
{\it \color{red} if we dont say "for every i,j pairs" ,k should not appear in an inequality which holds for only one task. Also maybe it is better to  cite [21] A.5, because [28] Cor.7 says only the following
$$\|\frac{1}{t}\sum_{i=1}^t \yij\xij - \W^\top\W \mtx{h}^j(\W)\| \le c\sigma\sqrt{\frac{1}{t}\log(\frac{2d}{\delta})}$$}
\fi
\end{lemma}
With the covariance of $y\x$ being bounded by $\sigma^2$, the following inequalities are true \cite{kong2020meta}.
\begin{align*}
    \Eb\left( (\vb^T\cdot (\frac{1}{t}\sum_{i=1}^t \yij\xij - \theta^j))^2\right) &\le \sigma^2 / t,\mbox{~for~} \|\vb\|=1.\\
    \Eb \left(\|\frac{1}{t}\sum_{i=1}^t \yij\xij - \theta^j \|^2\right) &\le \sigma^2d/t.
\end{align*}


\begin{lemma}\label{lem:Zj}
Define
\begin{align*}
    \Zb_j &= (\frac{2}{n_j}\sum_{i=1}^{n_j/2} \yij\xij)(\frac{2}{n_j}\sum_{i={n_j/2}+1}^{n_j} \yij\xij)^\top \\
    &\quad - \Hb^j(\W)(\Hb^j(\W))^\top,
\end{align*}
Then there exists a constant $c$ such that on the event $\mathcal{E}$ (thus with probability $1-\delta$), for all $j=1,...,k$, 
\begin{align}
    \|\Zb_j \| \le \frac{c\sigma^2d}{n_j} \log(\frac{kd}{\delta}). \label{eq:evt}
\end{align}
\end{lemma}

% {\it \color{red} From my understanding we should have 
% $$\|\Zb_j \| \le (Eq A.1 Bound)(Eq. A.1 bound + 2\|\W^\top\W \mtx{h}^j(\W)\|)$$ choosing $t=\dfrac{n_j}{2}$ then we have $$\|\Zb_j \| \le (c\sigma\sqrt{\frac{2}{n_j}\log(\frac{2d}{\delta})})(c\sigma\sqrt{\frac{2}{n_j}\log(\frac{2d}{\delta})} + 2\|\W^\top\W \mtx{h}^j(\W)\|)$$
% This is more or less what you have found, but the difference is k in $\log$ term and d term }



The proof is almost same as \cite{kong2020meta}, the only difference is that we replace the bound in (\cite{kong2020meta} Prop A.1) by \eqref{eq:gauss_bern}. With the similar replacement, we propose the following lemma. 
\begin{lemma}\label{lem:Zj2}
Let $\delta\in(0,1)$. There exists a constant $c$, such that for any $\epsilon\in(0,1)$, and 
\begin{align}
    k = \frac{cd}{n_j}\log^2(\frac{kd}{\delta}) \max\{\frac{1}{\epsilon^2}, \frac{1}{\epsilon} \log(\frac{kd}{\delta})\}, \label{eq:k lb}
\end{align}
with probability $1-\delta$, 
\begin{align*}
    \|\frac{1}{k} \sum_{j=1}^k \Zb_j\| \le \epsilon \sigma^2.
\end{align*}
\end{lemma}
This means that when \eqref{eq:k lb} is true, with probability $1-\delta$,
\begin{align*}
    \left\|\hat \bM - \W^\top\W\left(\frac{1}{k}\sum_{j=1}^k \mtx{h}^j(\W)( \mtx{h}^j(\W))^\top\right)\W^\top\W\right\| \le \epsilon \sigma^2.
\end{align*}
Note that $\bM$ is defined as \[\bM=\W^\top\W\left(\frac{1}{k}\sum_{j=1}^k \mtx{h}^j(\W)( \mtx{h}^j(\W))^\top\right)\W^\top\W.\] So we have proven that with probability $1-\delta$,
\begin{align*}
    \left\|\hat \bM - \bM\right\| \le \epsilon \sigma^2.
\end{align*}

%\som{Remind that this is $\hat \bM-\bM$ i.e. $\bM=\text{the messy sum}$}
\end{proof}

%\SO{Create a subsection here!!! Reduce the confusion as much as possible, make transitions smooth.}
\subsection{Proof of Theorem \ref{thm:down}}
Now we will prove Theorem \ref{thm:down}. We first review the notations and assumptions mentioned in the theorem.

\subsubsection{Review of Notations and Assumptions}
We define the SVD of $\hat \bM$ as $\hat \Ub \hat\La \hat\Vb^\top$. Let the first $r$ columns of $\hat \Ub$ be $\Ub_r$. 

Let $\hat\W$ be defined as 
\begin{align}
    \hat \W &= \hat \Ub_r \hat \Qb, \label{eq:def W append}\\
    \hat \Qb &= \mathop{\mathrm{argmin}}_{\Qb\in\R^{r\times r}, \Qb\Qb^\top = I}\ \|\hat \Ub_r \Qb - \W\|.
\end{align}
The population cross entropy loss is defined as
\begin{align*}
    &\cLCE(f;\Pb) : \Fc\times \R^{r\times d}\rightarrow \R=\\
    &-\mtx{E}_{\x,y\sim\Pxy} (y\log f(\hat\Pb \x) + (1-y)\log (1 - f(\hat\Pb \x))).
\end{align*}
We will search for a function $f^* \in \Fc$.% that minimizes the population cross entropy loss. 
\begin{assumption}\label{append ass:F}
$\Fc$ is a set of functions satisfying: For any function $f\in\Fc$, any orthonormal matrix $\Qb\in\R^{r\times r}$ and any matrix $\Pb\in\R^{r\times d}$, there exists $g \in \Fc$ such that $f(\Pb \x) = g(\Qb\Pb \x)$.
%\begin{enumerate}
%    \item For any function $f\in\Fc$, any orthonormal matrix $\Qb\in\R^{r\times r}$ and any matrix $\Pb\in\R^{r\times d}$, there exists $g \in \Fc$ such that $f(\Pb \x) = g(\Qb\Pb \x)$.
%    \item $\Fc \subseteq \{f\ |\ \log f,~ \log(1-f)\mathrm{~are~}L\mathrm{~Lipschitz}\}\bigcap \{f\ |\ 0<f(x)<1,\forall x\in\R^r\}$.
%\end{enumerate}
\end{assumption}
Now we define a general loss function $\cL$ and $\cL_e$.
\begin{assumption}\label{append ass:L}
Suppose $\cL$ satisfies the following assumptions:
\begin{enumerate}
    \item %$\cL$ takes $f(\Pb x)$ as the argument, i.e., 
    $\cL$ has the form $\cL(f;\Pb) = \mtx{E}_{\Pxy}\Lcs(f(\Pb \x),y)$. $\cL_e$ has the form $\cL_e(f;\Pb) = \frac{1}{n}\sum_{i=1}^n\Lcs(f(\Pb \x_i),y_i)$.
    \item $\Lcs$ is $L$ Lipschitz in $\Pb \x$.
    \item $\min_{\Pb}\cL(f;\Pb) = \cL(f;\W)$.
\end{enumerate}
\end{assumption}
We solve for $\hat f$, defined as \begin{align}
    \hat f &= \argmin_{f\in\Fc}\ \cLCE(f;\hat \Ub_r^\top). \label{eq:def f append}
\end{align}
\subsubsection{Proof of Theorem \ref{thm:down}}
Now we are ready to restate Theorem \ref{thm:down} and prove it.

\begin{theorem}\label{thm:popu append}
With Assumptions \ref{append ass:F} and \ref{append ass:L}, we have that
    \begin{align*}
        \cLCE(\hat f;\hat \Ub_r^\top)  - \cLCE(f^*;\Ub_r^\top) \lesssim L\sqrt{r}\|\hat \W - \W\|.
    \end{align*}
\end{theorem}

\begin{proof}
We learn the model from the following optimization algorithm.
\begin{align*}
    \hat f &= \argmin_{f\in\Fc}\ \cLCE(f;\hat \Ub_r^\top)
    %\\
    %&= \argmin_{f\in\Fc}\ -\mtx{E}_{\x,y\sim\Pxy} (y\log f(\hat\Ub_r^\top \x) \\
    %&\quad + (1-y)\log (1 - f(\hat\Ub_r^\top \x)))\\
    %&= \argmin_{f\in\Fc}\ -\mtx{E}_{\x\sim\gauss} \left(f^*(\W \x)\log f(\hat \Ub_r^\top \x)\right. \\
    %& \quad \left. + (1-f^*(\W \x))\log (1 - f(\hat \Ub_r^\top \x)) \right).
\end{align*}
Denote $\tilde f\in\Fc$ as the function such that $\tilde f(\hat \W \x) = \hat f(\hat \Ub_r^\top \x)$. So that $\cLCE(\hat f;\hat \Ub_r^\top) = \cLCE(\tilde f;\hat \W)$. Since $\hat f$ minimizes the cross entropy loss, we have that $\cLCE(\tilde f;\hat \W) \le \cLCE(f^*;\hat \W)$. 

Now we have 
\begin{align*}
    &\quad \cLCE (\tilde f;\hat \W) - \cLCE (f^*;\W)\\
    &\le \cLCE (f^*;\hat \W) - \cLCE (f^*;\W)\\
    %&\le -\mtx{E}_{\x\sim\gauss} \left(f^*(\W \x)(\log f^*(\hat\W \x) -\log f^*(\W \x))\right. \\
    %& \quad \left. + (1-f^*(\W \x))(\log (1 - f^*(\hat \W \x)) - \log (1 - f^*(\W \x))) \right)\\
    &\le \mtx{E}_{\x\sim\gauss} L\|(\hat \W - \W)x\|\\
    &\lesssim L\sqrt{r}\|\hat \W - \W\|.
\end{align*}
The last step uses the fact that $\hat \W$ and $\W$ are rank $r$.
\end{proof}

\subsection{Proof of Theorem \ref{thm:rade}}
%Now we prove that the upper bound of the error for few-shot learning with finite samples.
We first state Theorem \ref{thm:rade} below.
\begin{theorem}\label{thm:rade app}
    Suppose we generate $n$ sample data for few shot learning solve for $\hat \theta_e$ from 
    \begin{align}
   	 \hat \bt_e &= \argmin_{\bt}\ \cL_e(\bt;\Ub_r^\top)\quad\text{such~that}\quad\|\bt\|_2\le a.\label{eq:fstar finite theta append}
	\end{align}
   Suppose Assumptions \ref{append ass:F} and \ref{append ass:L} hold.
    There exist constants $c>0$, $\delta\in(0,1)$, with probability at least $1 - n^{-c+1} - \delta$, the solution $\hat\theta_e$ and $\hat\Ub_r$ satisfy
    \begin{align*}
        &\quad \mathcal{L} (\hat\theta_e;\hat\Ub_r^\top) - \mathcal{L} (\theta^*;\W) \\
        &\lesssim \frac{caL(\sqrt{r}+\log(n)) (1+ \sqrt{\log(1/\delta)})}{\sqrt{n}} + L\sqrt{r}\|\hat \W - \W\|. 
    \end{align*}
\end{theorem}
\begin{proof}
We sketch the proof of Theorem \ref{thm:rade app}. After reviewing the notations, we quote a standard generalization bound via Rademacher complexity in Lemma \ref{lem:rade known}. Then we use the smoothness of the loss function to link to the generalization error of linear functions \eqref{eq:lin rade}, and then use Lemma \ref{lemma:chi-sqr} to compute \eqref{eq:lin rade} and finish the proof.

In few-shot learning, the true parameter is $\theta^*$, and the empirical loss function with finite data is 
\begin{align}
    &\cL_e(\theta;\Pb) : \Fc\times \R^{r\times d}\rightarrow \R= \frac{1}{n}\sum_{i=1}^n \Lcs(f(\Pb\x_i), y_i)
    %\notag\\
    %&-\frac{1}{n}\sum_{i=1}^n (y_i\log\phi (\theta^\top\Pb \x_i) + (1-y_i)\log (1 - \phi(\theta^\top\Pb \x_i))) \label{eq:cLCE finite theta app}
\end{align}
Denote each term in the summation as 
\begin{align*}
    &\quad \cL_e^i(\theta;\Pb) : \Fc\times \R^{r\times d}\rightarrow \R = \Lcs(f(\Pb\x_i), y_i).
    %=\notag\\
    %&- (y_i\log \phi (\theta^\top\Pb \x_i) + (1-y_i)\log (1 - \phi(\theta^\top\Pb \x_i)))
\end{align*}
We search for the solution by
\begin{align}
    \hat \theta_e &= \argmin_{\theta}\ \cL_e(\theta;\Ub_r^\top),\mbox{~such~that~} \|\theta\|\le a.\label{eq:fstar finite theta app}
\end{align}
In Theorem \ref{thm:popu append}, we know that
\begin{align*}
    \cLCE(\hat \theta;\hat \Ub_r^\top)  - \cLCE(\theta^*;\Ub_r^\top) \lesssim L\sqrt{r}\|\hat \W - \W\|.
\end{align*}
Denote 
    \begin{align}
        M = \max_{\|\theta\|\le a} |\theta^\top \hat\Ub_r^\top\x_i| \le a \max\|\hat\Ub_r^\top\x_i\|.\label{eq:bound_rade}
    \end{align}
We will bound the difference between $\cL$ and $\cL_e$ by Rademacher complexity theory.
\begin{lemma}\label{lem:rade known}
    \cite{mohri2018foundations}
 
    Let $\mscrU$ be the independent random variables uniformly chosen from $\{-1,1\}$.
    Let $\Rc$ be the Rademacher complexity of the logistic functionals defined on the data,
    \begin{align*}
        \Rc &= \frac{1}{n}\Eb_{\epsilon_i\in\mscrU} \sup_{\|\theta\|\le a} \sum_{i=1}^n\epsilon_i\cL_e^i(\theta;\hat\Ub_r^\top) \\
        %K &= |\log(\phi(-M))|>\max_i\cL_e^i(\theta;\hat\Ub_r^\top)
        K&= \max_i\cL_e^i(\theta;\hat\Ub_r^\top) \le M.
    \end{align*}
    %We know $\cL_e^i(\theta;\hat\Ub_r^\top)<K$ with probability at least $1-n^{-c_1+1}$,
    %then for any $\theta$ such that $\|\theta\|\le a$, with probability $1-\delta-n^{-c_1+1}$, we have that 
    with probability $1-\delta$, we have that 
    \begin{align*}
        |\cL_e(\theta;\Ub_r^\top) - \cL(\theta;\Ub_r^\top)| \le \Rc + \frac{\sqrt{\log(1/\delta)}}{\sqrt{n}}K.
    \end{align*}
\end{lemma}
Thus we have that 
\begin{align*}
    |\mathcal{L} (\hat\theta_e;\hat\Ub_r^\top) - \mathcal{L}_e (\hat\theta_e;\hat\Ub_r^\top)| &\le \Rc + \frac{\sqrt{\log(1/\delta)}}{\sqrt{n}}K,\\
    |\mathcal{L} (\hat\theta;\hat\Ub_r^\top) - \mathcal{L}_e (\hat\theta;\hat\Ub_r^\top)| &\le \Rc + \frac{\sqrt{\log(1/\delta)}}{\sqrt{n}}K.
\end{align*}
Because $\hat\theta_e$ minimizes the empirical loss $\mathcal{L}_e$,
\begin{align*}
    \mathcal{L}_e (\hat\theta_e;\hat\Ub_r^\top) \le \mathcal{L}_e (\hat\theta;\hat\Ub_r^\top).
\end{align*}
Thus 
\begin{align}
    \mathcal{L} (\hat\theta_e;\hat\Ub_r^\top) - \mathcal{L} (\hat\theta;\hat\Ub_r^\top) \le 2\left(\Rc + \frac{\sqrt{\log(1/\delta)}}{\sqrt{n}}K\right).\label{eq:emp loss}
\end{align}
So the remaining target is to bound $\Rc$. 

We first denote $\vb_i = \hat\Ub_r^\top \x_i$, so $\vb_i\in\R^r$ and $\vb_i$ are jointly independent standard normal random variables. %In binary classification, 
$\cL_e^i$ is always $L$ Lipschitz in $\theta^\top\vb_i$, the Rademacher complexity can be upper bounded by
\begin{align}\label{eq:lin rade}
    \Rc \le \tilde\Rc := \frac{L}{n}\Eb_{\epsilon_i\in\mscrU} \sup_{\|\theta\|\le a} \sum_{i=1}^n \epsilon_i\theta^\top\vb_i. 
\end{align}
We first refer to the following lemma.
\begin{lemma}\label{lemma:chi-sqr}
    \cite{laurent2000adaptive} Let $c>0$, $X$ follow $\chi_r^2$ distribution, then
    \begin{align*}
        \Pb(X - r \ge 2\sqrt{cr\log n} + 2c\log n) \le n^{-c}.
    \end{align*}
\end{lemma}

For a constant $c>1$, via union bound we have that $\max{\|\vb_i\|^2} \le r + 2\sqrt{cr\log n} + 2c\log n$ for all $i=1,..,n$ with probability $1 - n^{-c+1}$. We use $\max{\|\vb_i\|} \lesssim c(\sqrt{r} + \log(n))$ for simplicity.

Conditioned on this event, we apply the Rademacher complexity for linear model that 
\begin{align}
   \tilde \Rc &\le \frac{L\max\|\theta\| \cdot \max\|\vb_i\|}{\sqrt{n}}\\
   &\le \frac{caL(\sqrt{r} + \log(n))}{\sqrt{n}}. \label{eq:tilde Rc}
\end{align}
Combining with \eqref{eq:emp loss} and Theorem \ref{thm:popu append} we get the bound in Theorem \ref{thm:rade app}. We can also bound $M$ in \eqref{eq:bound_rade}.

Finally we will use Lemma \ref{lem:M to K} to bound $M$.
\begin{lemma}\label{lem:M to K}
    Let $M$ be defined as in \eqref{eq:bound_rade}.    
    With probability at least $1 - n^{-c+1}$, we have $M<caL(\sqrt{r} + \log(n))$.
\end{lemma}
Let $\vb_i$ be replaced by $\hat \Ub_r^\top\x_i$ in Lemma \ref{lemma:chi-sqr}, then this directly results from Lemma \ref{lemma:chi-sqr}. Lemma \ref{lem:M to K} bounds $M$, thus bounds $K$ (which is $L$ Lipschitz in $M$) in Lemma \ref{lem:rade known}. After we insert \eqref{eq:tilde Rc} together into Lemma \ref{lem:rade known}, we can get the result in  Theorem \ref{thm:rade}.
% By Lemma \ref{lemma:chi-sqr} we know that for a constant $c>2$, we have  $\max{\|\hat\Ub_r^\top\x_i\|} \le c(\sqrt{r} + \log(n))$ for all $i=1,..,n$ with probability $1 - n^{-c+1}$. So with probability at least $1 - n^{-c+1}$, we have $M<ac(\sqrt{r} + \log(n))$.
\end{proof}



==> s_intro.tex <==
\section{Introduction}\label{s:intro}
Meta-learning (and multi-task learning) has proved to be a efficient when available training data is limited. The central idea is exploiting the information (e.g.~training data) provided by earlier related tasks to quickly adapt a new task using few samples.
This idea has a rich history \cite{caruana1997multitask,baxter2000model} and has shown promise in modern machine learning tasks, e.g., in image classification \cite{deng2009imagenet}, machine translation \cite{bojar2014findings} and reinforcement learning \cite{finn2017model}, all of which may involve numerous tasks to be learned with limited data per task.
% between thousands of English and French sentences



 \mf{where? give citation}
  \mf{should we use the term meta-learning or multitask learning? It's better to pick one for consistency}
Modern deep learning algorithms typically exploit the shared information between tasks by learning useful representations \cite{schmidhuber1987evolutionary, thrun2012learning}. The multi-task system was studied by \cite{caruana1997multitask}, and the idea of meta-learning or transfer learning is investigated empirically in modern machine learning framework, showing that the shared representation benefits for training on the new tasks \cite{bengio2013representation, hospedales2020meta, yosinski2014transferable}.  %\cite{bengio2013representation, hospedales2020meta, yosinski2014transferable, raghu2019rapid}. 
An instructive and well-studied problem for meta-learning is mixed linear regression,
for which efficient algorithms and sample complexity bounds are discussed in 
\cite{zhong2016mixed, li2018learning, chen2020learning}. If the tasks lie on a shared low-dimensional subspace, learning this subspace would serve as an efficient representation which helps reduce the search space for future tasks. Once the search space is low dimensional, in order to get the same accuracy, the amount of data required for training is reduced compared to training over the full parameter space. \cite{lounici2011oracle,cavallanti2010linear,maurer2016benefit} propose sample complexity bounds for representation learning for linear multi-task systems. There are study of mixed linear tasks combined with other structures, such as boolean combination of features \cite{balcan2015efficient}, half-spaces \cite{rish2008closed} and sparse representations \cite{argyriou2008convex}.
% \mf{main point: low-dimensional approximation of the feature space makes learning easier in a new task, with fewer samples. Thus in many ML applications one seeks such a representation. can omit 'learned by mixed linear regression'. rewrite parag.}

% The low dimensional subspace of the features, learned by mixed linear regression, is utilized as the search space for training on new tasks.
% \mf{swap the order with next paragraph} 

The recent papers \cite{kong2020meta,kong2020robust} propose meta-learning procedures that involve dimension reduction, clustering and few-shot learning. Here a low-dimensional task subspace is used as the search space for few-shot learning for the new task. 
Another related approach
\cite{du2020few,tripuraneni2020provable}
sets up a nonconvex optimization problem with matrix factors of appropriate sizes, which captures the low dimensional structure. One can apply gradient descent to this nonconvex problem, and studying its behavior requires a nontrivial landscape analysis of the matrix factorization problem.  

However, existing provable algorithms for representation learning are restricted to linear-regression tasks, whereas typical machine learning tasks involve nonlinearity. This can arise from the use of nonlinear models as well as nonlinear label link function (e.g.~generalized linear models).
%. The setup is restrictive compared with the variant types of nonlinear tasks. 
\mf{what does 'objective' mean here? do you mean there are different tasks to be performed with different goals, with the same data?}
A good example is classification problems 
%which represent much of the machine learning applications 
including computer vision and natural language processing \cite{deng2009imagenet, bojar2014findings}. 
In classification tasks, the model is a map from images/text to labels, and the labels are discrete and not linear with respect to the input (i.e.~logistic link function). Another example is the use of nonlinear models such as deep networks
%, which contain many nonlinear activation functions within their layers. 
The existing results for representation learning for the linear-regression setting cannot be easily extended to the nonlinear case. 

\noindent\emph{Can we learn efficient subspace representations for nonlinear tasks such as generalized linear models and neural nets?}
%If one can learn a representation that help classify across several tasks, this representation can be used in this model can be retrieved and transferred to a classifier for other objectives.
%\som{Redundant sentence: In these datasets, there are images of different types of objectives, and the task is to classify which categories each image comes from.}

We consider a realizable setup where the input data is high-dimensional, the \emph{relevant features} lie in a low dimensional subspace and the labels depend only on the \emph{relevant features}. These assumptions are the same as in the existing literature, however we additionally allow for the scenario where labels are possibly an arbitrary nonlinear function of the relevant features. We make the following contributions.

\noindent$\bullet$ \textbf{Efficient representations for nonlinear tasks:} We show that subspace found via method-of-moments (MOM) leads to a consistent estimate of the ground-truth subspace despite arbitrary task nonlinearities, when the data is normally distributed.  We combine this with non-asymptotic learning results to establish sample complexity bounds for representation learning.

% \som{emphasize generalized linear model?}
\noindent$\bullet$ \textbf{Few-shot learning and Applications:} We specialize our results to practical settings with tasks involving binary classification and neural nets. We theoretically and empirically show that subspace-based representation can greatly improve sample efficiency of future tasks.
% \som{More citations are needed! Consider adding a related work (sub)section!}

%that, can we still retrieve the subspace with the same amount of training data?

%{\color{blue}Contribution here}




==> s_main.tex <==
\section{Main Results}
% {\color{red} YS: Commented some text for space limitation}
\vspace{-.1cm}
In this section, we shall establish error bounds for Algorithm \ref{algo:1}. This involves three parts. Theorem \ref{thm:hatM} establishes the quality of the moment estimator $\hat\bM$. %The estimator is then used for few-shot learning, and 
Theorem \ref{thm:down} upper bounds the population cross-entropy risk of $\hat f$ in the few-shot learning stage. Theorem \ref{thm:rade} upper bounds the population risk of the ERM estimator $\hat f_e$, which is learned from finite data.

\subsection{Results on Meta-training}
\begin{lemma}\label{lem:M exp}
$\bM,\hat{\bM}$ satisfies the following. (a) $\text{rank}(\bM)\leq r$. (b) $\text{range-space}(\bM)\subset \text{row-space}(\W)$. (c) $\mtx{E}[\hat{\M}]=\bM$. 
\end{lemma}
In words, $\bM$ returns a consistent estimate of the representation space in the sense that its range is guaranteed to be the subspace of the representation. Observe that to fully recover representation, $\bM$ should contain a diverse set of tasks that can \emph{cover} the representation subspace. For GLM, one needs at least $k\geq r$ tasks to ensure range of $\bM$ is equal to the row-space of $\W$. Additionally, $\hat{\M}$ estimator is also consistent. %All missing proofs can be found in \cite{paperurl}.



% notation (any well-conditioned can be accomplished by estimating the covariance of the inputs and then whitening the data. Such normalization procedures are common e.g.~batch normalization. 
We next present the error on the estimator $\hat \bM$. This theorem applies to standard normal data $\x\sim\Nn(0,\Iden)$. %This is mostly used for notational convenience. In machine learning subGaussian distributions often behave very similar in sufficiently high-dimensions \cite{oymak2018universality,abbasi2019universality}. We leave such generalizations to more general distributions as a future work. 
While this may initially seem restrictive, we remark that identity covariance is mostly used for notational convenience. Additionally, in similar spirit to Central Limit Theorem, machine learning and signal processing algorithms often exhibit distributional universality: For instance, subgaussian distributions often behave very similar or even identical to gaussian distributions in sufficiently high-dimensions \cite{oymak2018universality,abbasi2019universality}. We leave such generalizations to more general distributions as a future work. 
\begin{theorem}[Moment Estimator]\label{thm:hatM}
Suppose the data is generated as in Def.~\ref{def:task}, $n_j\geq N$ for all $j$ and $\xij\distas\Nn(0,\Iden)$. Suppose for some $\sigma>0$ and for all tasks, the label-input product $y\x$ is a subGaussian random vector with covariance upper bounded by $\| \mathbf{Cov}(y \x) \| \le \sigma^2$. (These conditions hold when $|f^j(\x)|<\sigma$.) Let $\delta\in(0,1)$ and $\epsilon\in(0,1)$. Then there exists a constant $c>0$ such that if
\begin{align*}
    k \ge \frac{cd}{N}\log^2(\frac{kd}{\delta}) \max\{\frac{1}{\epsilon^2}, \frac{1}{\epsilon} \log(\frac{kd}{\delta})\},
\end{align*}
$\|\hat \bM - \bM\| \le \epsilon\sigma^2$ with probability at least $1-\delta$.
\end{theorem}
%In essense, this shows that subspace $\M$ can be estimated with $O(kd) samples$
\iffalse
Theorem \ref{thm:hatM} proposes an upper bound for the estimation error of $\bM$. The subspace spanned by $\hat \bM$ is used for few-shot learning. In the context of binary classification, we will show how this error affects the cross entropy loss for the few-shot learning stage. 
\fi
%Downstream task

Recall that $\hat \bM=\hat \Ub \hat\La \hat\Ub^\top$ and $\hat \Ub_r$ is the first $r$ columns of $\hat \Ub$. Denote the estimate of $\W$ via $\hat \W$ given by adjusting $\hat\Ub_r$
\begin{align}
    \hat \W &= (\hat \Ub_r \hat \Qb)^\top,\
    \hat \Qb = \mathop{\mathrm{argmin}}_{\Qb\in\R^{r\times r}, \Qb\Qb^\top = I}\ \|\hat \Ub_r \Qb - \W^\top\|\label{eq:def W}
\end{align}
With the definition of $\hat\W$, $\|\hat \W - \W\|$ defines a distance between the row space of $\W$ and the column space of $\hat \Ub_r$. If the span of the two subspaces are the same, then there exists an orthonormal matrix $\Qb$ such that $\hat \Ub_r \Qb = \W^\top$.

The previous lemma builds upon the assumption that $\|\hat \W - \W\|$ is small. 
%We quote the following lemma first. 
In Theorem \ref{thm:hatM}, we have got $\|\hat \bM - \bM\| \le \epsilon\sigma^2$, then with the extra assumption that $\bM$ is rank $r$, we have the following result from \cite{davis1970rotation}.
\begin{lemma}
If $\|\hat \bM - \bM\| \le \epsilon\sigma^2$, $\lambda_r(\bM) > \epsilon\sigma^2$, then \[\|\hat \W - \W\| \le \epsilon\sigma^2(\lambda_r(\bM) -\epsilon\sigma^2)^{-1}.
%\le \frac{\|\hat \bM - \bM\|}{\lambda_r(\bM) - \|\hat \bM - \bM\|} \le \frac{\epsilon\sigma^2}{\lambda_r(\bM) -\epsilon\sigma^2}.
\]
\end{lemma}



% I think it's better to keep this as \Qb is used in assumption 1 of \Fc

%Another definition of the distance between two subspaces is the difference of projection, defined as 
%\begin{align*}
%    \|\hat \Ub_r\hat \Ub_r^\top - \W^\top\W\|
%\end{align*}
%Note that, with \eqref{eq:def W}, if 

\iffalse
{\color{red} can remove the text, just to keep the assumption on $\Fc$}
Now we use $\hat\Ub_r$ for the downstream task, and we study the population loss of training caused by the error of the estimator $\hat \bM$. We consider the binary classification case, where the data in the new task is generated as Def. \ref{def:bin_class}, with the non-linear function being $f$ and the true subspace being $\W$. The loss we consider, is cross-entropy loss, which is defined as \eqref{eq:cLCE}.
%\begin{align*}
%    &\cLCE(f;\Pb) : \Fc\times \R^{r\times d}\rightarrow \R=\\
%    &-\mtx{E}_{\x,y\sim\Pxy} (y\log f(\hat\Pb \x) + (1-y)\log (1 - f(\hat\Pb \x))) 
%\end{align*}

To train on the data, we need to find the optimal function $f$ that minimizes the population loss. Define the search space of $f$ as $\Fc$. For binary classification, we assume that, 
\begin{enumerate}
    \item For any function $f\in\Fc$, any orthonormal matrix $\Qb\in\R^{r\times r}$ and any matrix $\Pb\in\R^{r\times d}$, there exists $g \in \Fc$ such that $f(\Pb \x) = g(\Qb\Pb \x)$.
    \item $\Fc \subseteq \{f\ |\ \log f,~ \log(1-f)\mathrm{~are~}L\mathrm{~Lipschitz}\}\bigcap \{f\ |\ 0<f(x)<1,\forall x\in\R^r\}$.
\end{enumerate}
We can see that, if we adopt the logistic regression for binary classification example in \eqref{eq:Fcbin}, then both assumptions are true with $L = a$.  

We learn the model from the optimization algorithm \eqref{eq:fstar} (also works for logistic regression in \eqref{eq:fstarbin}). Now we will bound the cross-entropy loss of this model.
\fi

%\so{There is a serious issue here. It seems, we never stated a bound on $\hat{\W}-\W$, we only prove a bound on $\hat{M}-\M$. Thm 3.2 should ideally state bound for the subspace as well. This bound should be in terms of the spectrum of $\M$ i.e. its $r$'th largest singular (e.g.~via davis-kahan thm). If you look at the few-shot learning results, they are in terms of $\|\hat{\W}-\W\|$. This is fine but we should also add an end-to-end learning result where $\|\hat{\W}-\W\|$ is bounded in terms of meta-training sample size. This should be addressed before arXiv submission.}
\subsection{Results on Few-shot Learning}
\vspace{-0.1cm}
In the next step, we will use $\hat\Ub_r$ for few shot learning and find $\hat f$ that minimize the population loss. 
%Recall that the search space for $\hat f$ is $\Fc$. For binary classification, we assume 
%\begin{enumerate}
%Only row-space (representation) matters
%    \item \textbf{Rotation invariance:} For any function $f\in\Fc$, any orthonormal matrix $\Qb\in\R^{r\times r}$ and any matrix $\Pb\in\R^{r\times d}$, there exists $g \in \Fc$ such that $f(\Pb \x) = g(\Qb\Pb \x)$.
%    \item \textbf{Lipschitz:} $\Fc \subseteq \{f\ |\ \log f,~ \log(1-f)\mathrm{~are~}L\mathrm{~Lipschitz}\}$ $~\bigcap~ \{f\ |\ 0<f(x)<1,\forall x\in\R^r\}$.
%\end{enumerate}

\begin{theorem}\label{thm:down}
    Let Assumptions \ref{ass:F} and \ref{ass:L} hold. Let $\hat\W$ be the same as in \eqref{eq:def W} and $\hat f$ be the same as in \eqref{eq:fstar}. Then we have 
    \begin{align*}
        \cLCE(\hat f;\hat \Ub_r^\top) - \cLCE(f^*;\W)\lesssim L\sqrt{r}\|\hat \W - \W\|.
    \end{align*}
\end{theorem}
$\cLCE (f^*;\W)$ assumes the knowledge of the true function $f^*$ and the representation $\W$. This shows that the inaccuracy of the moment estimator $\hat M$ costs us $O(L\sqrt{r}\|\hat \W - \W\|)$. 

Theorem \ref{thm:down} bounds the population risk of $\hat f$, when we use $\hat\Ub_r^\top$ as the representation subspace. Next we discuss the population risk of the finite sample solution $\hat f_e$, which should be worse than $\hat f$ due to the limited samples.
%deviating from true data distribution of the new task. Theorem \ref{thm:rade} bounds the risk in terms of the sample size $n$.

\iffalse
For a concrete example, we apply the logistic regression model for \eqref{eq:cLCE finite}, where $f(\vb) = \phi(\bt^\top\vb)$, $\vb \in \R^r$ and $\phi$ is logistic function. Let the ground truth parameter for generating few-shot learning data be $\bt^*$ and we assume $\|\bt^*\| \le a$. In few-shot learning, we train by solving for $\hat \bt_e$ in the set $\{\bt\ |\ \|\bt\| \le a\}$. The objective is {\color{red} can move this to def 2.6}
\begin{align}
    &\cL_e(\bt;\Pb) : \Fc\times \R^{r\times d}\rightarrow \R= \notag\\
    &-\frac{1}{n}\sum_{i=1}^n (y_i\phi (\bt^\top\Pb \x_i) + (1-y_i)\log (1 - \phi(\bt^\top\Pb \x_i))) \label{eq:cLCE finite theta}
\end{align}
The empirical minimizer is defined by
\begin{align}
    \hat \bt_e &= \argmin_{\bt}\ \cL_e(\bt;\Ub_r^\top),\mbox{~such~that~} \|\bt\|\le a.\label{eq:fstar finite theta}
\end{align}
\fi
\begin{theorem}\label{thm:rade}
    Consider the setup in Def.~\ref{def: test finite} with $n$ i.i.d.~examples with ground-truth model $\bt^*$. Solve for $\hat \bt_e$ via \eqref{eq:fstar finite theta}. There exist constants $c>1$, $\delta\in(0,1)$, with probability at least $1 - n^{-c+1} - \delta$, the solution pair $(\hat\bt_e,\hat\Ub_r)$ satisfies
    \begin{align*}
        \quad \mathcal{L}(&\hat\bt_e;\hat\Ub_r^\top) - \mathcal{L} (\bt^*;\W) \\
        &\leq \frac{caL(\sqrt{r}+\log(n)) (1+ \sqrt{\log(1/\delta)})}{\sqrt{n}} + L\sqrt{r}\|\hat \W - \W\|. 
    \end{align*}
\end{theorem}
Note that the first term grows as $\sqrt{r/n}$. This means the amount of data $n$ we request for few-shot learning is $n\approx r$,  as compared to $n\approx d$ if representation learning is not excecuted. 
%If we do not run representation learning before few-shot learning, the error would instead be proportional to $\sqrt{d/n}$ where $d$ is the ambient dimension and we would need $n\approx d$ examples to learn the new task.
% {\color{red} YS:  No math justification for $n\ge d$ here since I only have upper bound but no lower bound, so it's just an intuition}
%In \eqref{eq:fstar}, we solve for the minimizer of population loss function. Now we will study the finite sample case. In few-shot learning phase, suppose we have the dataset $(\x_i, y_i)$, $i=1,...,n$ and the data is generated as Def. \ref{def: test}. Now we consider the 

==> s_main_nn.tex <==
\begin{lemma}\label{lem:mean nn}
We assume that the data are generated as in Defs. \ref{def:task dis} to \ref{def:data_gen} and Def. \ref{def:nn}, and we study the $j$-th task whose feature matrix is $\Theta^j$. 
%{\color{blue} To be finished}
Define
\begin{align*}
    \mtx{h}(\Theta): \R^{r\times d} \rightarrow \R^r = \mtx{E}_{\x\sim\Px} f(\Theta \x)  \x
\end{align*}
Then $\mtx{E}_{(\x,y)\sim\Pxy}(y \x) = (\Theta^j)^\top(\Theta^j(\Theta^j)^\top)^{-1}\Theta^j\mtx{h}(\Theta^j)$, and $\|y\x\|\le 1$ with probability $1$.
%{\color{blue} To be finished}
\end{lemma}

\noindent\textbf{Proof of Lemma \ref{lem:mean nn}} The boundedness is trivial and we study the expectation.
Denote
\begin{align*}
    \tilde \Theta^j = (\Theta^j)^\top (\Theta^j(\Theta^j)^\top)^{-1}\Theta^j
\end{align*}

We first write the expectation as
\begin{align*}
    &\mtx{E}_{(\x,y)\sim\Pxy}(y \x) \\
    &= \mtx{E}_{\x} f(\Theta^j \x) \x\\
    &= \mtx{E}_{\x\sim\Px} \left(f(\Theta^j \x)  \tilde \Theta^j \x + f(\Theta^j \x) (\x -  \tilde \Theta^j\x) \right).
\end{align*}
Now we prove that 
\begin{align*}
    \mtx{E}_{\x\sim\Px}f(\Theta^j \x) (\x -  \tilde \Theta^j\x) =0
\end{align*}
Denote 
\begin{align*}
    \bar \x &= \tilde \Theta^j\x - (\x -  \tilde \Theta^j\x)\\
    &= 2\tilde \Theta^j\x - \x.
\end{align*}
Then it is easy to see
\begin{align}
    \Theta^j \x  &= \Theta^j \bar \x,\label{eq:easy1 nn} \\
    \x -  \tilde \Theta^j\x &= - \left(\bar \x -  \tilde \Theta^j\bar \x\right),\label{eq:easy2 nn}\\
    \x &=2\tilde \Theta^j\bar \x - \bar \x.
\end{align}


Now we consider the density function of $\bar x$. Let the density of $\x$ be $p_{\x}$, which is uniform on the unit sphere, we have that 
{\color{blue} Need a better notation!}
\begin{align}
    p_{\bar \x} (\bar \x) &= p_{\x}(2\tilde \Theta^j\bar \x - \bar \x) \big|\nabla_{\bar \x} (2\tilde \Theta^j\bar \x - \bar \x \big| \label{eq:den2 nn}\\
    &= p_{\x}(\x) \big|\mathrm{det}(2\tilde \Theta^j - I) \big|\label{eq:den3}\\
    &= p_{\x}(\x).
\end{align}
Here \eqref{eq:den2} uses the fact that the density function $p_{\x}$ is uniform (thus is a constant everywhere), and \eqref{eq:den3} uses that the eigenvalues of $\frac{2\theta^j(\theta^j)^\top}{\|\theta^j\|^2} - I$ only consists of $\pm 1$. Now we can see that the distributions of $\x$ and $\bar \x$ are the same.

So we have that
\begin{align}
    &\quad \mtx{E}_{\x\sim\Px}f(\Theta^j\bar \x) (\bar \x - \tilde \Theta^j\bar \x)\notag\\
    &= \mtx{E}_{\x\sim\Px}f(\Theta^j \x) \left(- (\x -  \tilde \Theta^j\x)\right)\notag\\
    &= - \mtx{E}_{\x\sim\Px}f(\Theta^j \x) (\x -  \tilde \Theta^j\x).\label{eq:mns nn}
\end{align}
which uses \eqref{eq:easy1 nn}, \eqref{eq:easy2 nn}. Since the distributions of $\x$ and $\bar \x$ are the same, we compute via a simple change of variable
\begin{align}
    &\quad \mtx{E}_{\x\sim\Px}f(\Theta^j\bar \x) (\bar \x - \tilde \Theta^j\bar \x) \notag\\
    &= \mtx{E}_{\bar \x\sim\Px}f(\Theta^j\bar \x) (\bar \x - \tilde \Theta^j\bar \x)\notag\\
    &= \mtx{E}_{\x\sim\Px}f(\Theta^j \x) (\x -  \tilde \Theta^j\x).\label{eq:pls nn}
\end{align}

Comparing \eqref{eq:mns nn} and \eqref{eq:pls nn}, we have 
\begin{align*}
    &\quad \mtx{E}_{\x\sim\Px}f(\Theta^j \x) (\x -  \tilde \Theta^j\x)\\
    &= -\mtx{E}_{\x\sim\Px}f(\Theta^j \x) (\x -  \tilde \Theta^j\x)
\end{align*}
so $\mtx{E}_{\x\sim\Px}f(\Theta^j \x) (\x -  \tilde \Theta^j\x)=0$.

Going back to Lemma \ref{lem:mean nn}, we have 
\begin{align*}
    \mtx{E}_{(\x,y)\sim\Pxy}(y \x)
    &= \mtx{E}_{\x\sim\Px} f(\Theta^j \x)  \tilde \Theta^j \x
    \\&= \mtx{E}_{\x\sim\Px} f(\Theta^j \x)  (\Theta^j)^\top (\Theta^j(\Theta^j)^\top)^{-1}\Theta^j \x.
\end{align*}
%\Theta^j

{\color{blue} From here I'll prove using the fact that $y\x$ is subGaussian with $\|\mathbf{Cov}(y\x)\| \le \sigma^2$.}

First we study the concentration of data within the $j$-th class. 
\begin{lemma}
Let $\delta\in(0,1)$, with probability $1-\delta$, there exists a constant $c$ such that
\begin{align*}
    \|\frac{1}{t}\sum_{i=1}^t \yij\xij - \theta^j\| \le c\sigma\sqrt{\frac{d}{t}\log(\frac{kd}{\delta})} 
\end{align*}
for all $j=1,...,k$. 
\end{lemma}
\begin{lemma}
For all $\vb$ such that $\|\vb\| = 1$, there exists a constant $c$ such that
\begin{align*}
    \Eb\left( (\vb^T\cdot (\frac{1}{t}\sum_{i=1}^t \yij\xij - \theta^j))^2\right) \le c\sigma^2 / t. 
\end{align*}
\end{lemma}
\begin{lemma}
There exists a constant $c$ such that \begin{align*}
    \Eb \left(\|\frac{1}{t}\sum_{i=1}^t \yij\xij - \theta^j \|^2\right) \le c\sigma^2d/t. 
\end{align*}
\end{lemma}
\begin{lemma}
Define
\begin{align*}
    \Zb_j = (\frac{1}{t}\sum_{i=1}^t \yij\xij)(\frac{1}{t}\sum_{i=t+1}^{2t} \yij\xij)^\top - \theta^j(\theta^j)^\top,
\end{align*}
Then there exists a constant $c$ such that with probability $1-\delta$, for all $j=1,...,k$, 
\begin{align}
    \|\Zb_j \| \le \frac{c\sigma^2d}{t} \log(\frac{kd}{\delta}). \label{eq:evt}
\end{align}
\end{lemma}

\begin{lemma}
There exists a constant $c$ such that
\begin{align*}
   \|\Eb\sum_{j=1}^k\Zb_j\Zb_j^\top\| \le c\sigma^4dk/t
\end{align*}
\end{lemma}
\begin{lemma}
Let $\delta\in(0,1)$. There exists a constant $c$, such that for any $\epsilon\in(0,1)$, and 
\begin{align}
    k = \frac{cd}{t}\log^2(\frac{kd}{\delta}) \max\{\frac{1}{\epsilon^2}, \frac{1}{\epsilon} \log(\frac{kd}{\delta})\}, \label{eq:k lb}
\end{align}
with probability $1-\delta$, 
\begin{align*}
    \|\frac{1}{k} \sum_{j=1}^k \Zb_j\| \le \epsilon \sigma^2.
\end{align*}
\end{lemma}
This means that when \eqref{eq:k lb}, with probability $1-\delta$,
\begin{align*}
    \left\|\hat \bM - \frac{1}{k}\sum_{j=1}^k\left(\tilde \Theta^j \mtx{h}(\Theta^j)\mtx{h}^\top(\Theta^j)\tilde \Theta^j\right)\right\| \le \epsilon \sigma^2.
\end{align*}


==> s_main_proof.tex <==
\section{Proof of main theorems}
\SO{Clearly Theorem \ref{thm:hatM append} is a restatement of Theorem \ref{thm:hatM}. Why don't you say so? Reader is not expected to figure out this by himself. Let us make things clear.}

\SO{Similarly, where is proof of Lemma 3.1? Looks like Lemma \ref{lem:mean nn} is its restatement but again not clear at all for reader. They cannot find proof of Lemma 3.1 in the text.}

\SO{Here is the organization we need: In the appendix, proof of each technical result in the main text is supposed to have its own subsection. Just like this subsection that I added i.e.~Proof of Theorem \ref{thm:hatM}.}
\SO{Maybe briefly describe the outline. Right now, little confusing due to Lemmas within the proof so outline would help i.e.~we first prove Lemma ... which shows ...}
\subsection{Proof of Lemma \ref{lem:M exp} and Theorem \ref{thm:hatM}}
We sketch the proof at the beginning. First we compute the expectation of $y\x$ in Lemma \ref{lem:mean nn}. That leads to the proof of Lemma \ref{lem:M exp}. Then in Lemma \ref{lem:err_yx} we bound the difference between sum of $y\x$ and its mean using concentration. The concentration of covariance estimator is studied later in Lemma \ref{lem:Zj} and \ref{lem:Zj2}, which leads to Theorem \ref{thm:hatM}.

\subsubsection{Proof of Lemma \ref{lem:M exp}}
We first state Lemma \ref{lem:M exp} below.
\begin{lemma}\label{lem:M exp append}
Let 
\begin{subequations}\label{eq:hatM append}
\begin{align}
\hat\bM &= \mathop{\Scale[1.8]{\sum}}_{j=1}^k \frac{2}{n_j^2}\left[(\sum_{i=1}^{n_j/2} \yij\xij) (\sum_{i=n_j/2+1}^{n_j} \yij\xij)^\top \right.\\
&\quad\quad\quad\quad \left. +  ( \sum_{i=n_j/2+1}^{n_j} \yij\xij) ( \sum_{i=1}^{n_j/2} \yij\xij)^\top\right].\nonumber
\end{align}
\end{subequations}
And
\begin{align*}
    &\mtx{h}^j(\W): \R^{r\times d} \rightarrow \R^d = \mtx{E}_{\x}[f^j(\W \x)\x]\\
    &\bM := \W^\top\W\left(\frac{1}{k}\sum_{j=1}^k \mtx{h}^j(\W)( \mtx{h}^j(\W))^\top\right)\W^\top\W.
\end{align*}
Then $\bM,\hat{\bM}$ satisfies the following. (a) $\text{rank}(\bM)\leq r$. (b) $\text{range-space}(\bM)\subset \text{row-space}(\W)$. (c) $\mtx{E}[\hat{\M}]=\bM$. 
\end{lemma}
\begin{proof}
Part (a) and (b) are easy to see. $\W\in\R^{r\times d}$ so that $\text{rank}(\bM)\leq r$, and since $\bM$ is the product of $\W^\top$ and another matrix, then  $\text{range-space}(\bM)\subset \text{row-space}(\W)$.
Now we will prove Part (c). We first give the lemma for the mean of the random vector $y\x$.

\begin{lemma}\label{lem:mean nn}
We assume that the data is generated as in Def. \ref{def:task}, and we study the $j$-th task whose activation function is $f^j$. 
%{\color{blue} To be finished}
Define
\begin{align*}
    \mtx{h}^j(\W): \R^{r\times d} \rightarrow \R^d = \mtx{E}_{\x\sim\gauss} f^j(\W \x)  \x
\end{align*}
Denote the joint distribution of $(\x,y)$ as $\Pxy$.
Then $\mtx{E}_{(\x,y)\sim\Pxy}(y \x) = \W^\top\W \mtx{h}^j(\W)$.
\end{lemma}

\emph{Proof of Lemma \ref{lem:mean nn}.} The expectation can be expanded as
\begin{align*}
    &\mtx{E}_{(\x,y)\sim\Pxy}(y \x) \\
    &= \mtx{E}_{\x\sim\gauss} f^j(\W \x) \x\\
    &= \mtx{E}_{\x\sim\gauss} \left(f^j(\W \x)  \W^\top\W \x + f^j(\W \x) (I - \W^\top\W)\x \right).
\end{align*}
Note that, because $\x\sim\gauss$ so $\W \x$ and $(I - \W^\top\W)\x$ are Gaussian. $\W\W^\top = I$ implies 
\begin{align*}
    &\quad \Eb (\W \x)\x^\top((I - \W^\top\W))\\
    &= \W(I - \W^\top\W) = 0.
\end{align*}
So $\W \x$ and $(I - \W^\top\W)\x$ are independent, so 
\begin{align*}
    &\quad \mtx{E}_{\x\sim\gauss}  f^j(\W \x) (I - \W^\top\W)\x \\
    &= (\mtx{E}_{\x\sim\gauss}  f^j(\W \x)) (\mtx{E}_{\x\sim\gauss} (I - \W^\top\W)\x) = 0
\end{align*}
Then 
\begin{align*}
    \mtx{E}_{(\x,y)\sim\Pxy}(y \x) &= \W^\top\W(\mtx{E}_{\x\sim\gauss} f^j(\W \x) \x)\\
    &= \W^\top\W \h_j(\W).
\end{align*}

Denote 
\begin{align}\label{eq:Hj def}
    \Hb^j(\W) = \W^\top\W \mtx{h}^j(\W)
\end{align}
Because $\frac{2}{n_j}\sum_{i=1}^{n_j/2} \yij\xij$
and 
$\frac{2}{n_j}\sum_{i={n_j/2}+1}^{n_j} \yij\xij$ 
are independent, and their expectation are both $\Hb^j(\W)$, so that
\begin{align*}
    &\quad \mtx{E}(\frac{2}{n_j}\sum_{i=1}^{n_j/2} \yij\xij)(\frac{2}{n_j}\sum_{i={n_j/2}+1}^{n_j} \yij\xij)^\top \\
    &= \Hb^j(\W)(\Hb^j(\W))^\top.
\end{align*}
At then end
\begin{align*}
    \hat \bM &= \frac{1}{k}\sum_{j=1}^k \mtx{E}(\frac{2}{n_j}\sum_{i=1}^{n_j/2} \yij\xij)(\frac{2}{n_j}\sum_{i={n_j/2}+1}^{n_j} \yij\xij)^\top,\\
    \bM &= \frac{1}{k}\sum_{j=1}^k\Hb^j(\W)(\Hb^j(\W))^\top,
\end{align*}
so we can prove Part (c) that $\mtx{E}(\hat \bM) = \bM$.
\end{proof}


\subsubsection{Proof of Theorem \ref{thm:hatM}}
We restate Theorem \ref{thm:hatM append} below. 
\begin{theorem}\label{thm:hatM append}
Suppose the data is generated as Def. \ref{def:task}. Let $\delta\in(0,1)$, $\epsilon\in(0,1)$. Suppose $y\x$ is a subGaussian random vector with covariance upper bounded by
\begin{align}
   \| \mathbf{Cov}(y \x) \| \le \sigma^2. \label{eq:covyx append}
\end{align} 
Define
\begin{align*}
    \mtx{h}^j(\W): \R^{r\times d} \rightarrow \R^d = \mtx{E}_{\x\sim\gauss} f^j(\W \x)  \x
\end{align*}
And let %$\bM = \mtx{E}_{\theta\sim\mathcal{N}(0,\bSi)} (g(\theta))^2\frac{\theta\theta^\top}{\|\theta\|^2}$, then
\begin{align*}
    \bM = \W^\top\W\left(\frac{1}{k}\sum_{j=1}^k \mtx{h}^j(\W)( \mtx{h}^j(\W))^\top\right)\W^\top\W
\end{align*}
Then there exists a constant $c$, with probability at least $1-\delta$, let 
\begin{align*}
    k = \frac{cd}{n}\log^2(\frac{kd}{\delta}) \max\{\frac{1}{\epsilon^2}, \frac{1}{\epsilon} \log(\frac{kd}{\delta})\}
\end{align*}
we have 
\begin{align*}
    \|\hat \bM - \bM\| \le \epsilon\sigma^2.
\end{align*}
\end{theorem}
\begin{proof}
The following lemmas are similar to \cite{kong2020meta} Section A.1. We extend the concentration inequalities from bounded random vectors to Gaussian random vectors. For completeness we place the lemmas here.

\begin{lemma}\label{lem:err_yx}
(\cite{jin2019short} Cor. 7) 
Let $\|\mathbf{Cov}(y\x)\| \le \sigma^2$, $\delta\in(0,1)$, $t>0$, $\Hb^j(\W)$ be defined in \eqref{eq:Hj def}. With probability $1-\delta$, there exists a constant $c>0$ such that for every $j$,
\som{Remind the exact assumption on $\sigma$}
\begin{align}
   \|\frac{1}{t}\sum_{i=1}^t \yij\xij - \Hb^j(\W)\| \le c\sigma\sqrt{\frac{d}{t}\log(\frac{kd}{\delta})} \label{eq:gauss_bern}
\end{align}
\som{Call $\W^\top\W \mtx{h}^j(\W)$ something for simpler notation}
Denote this event as $\mathcal{E}$.
\iffalse
{\it\color{red} for every i,j pairs ? }Denote this event as $\mathcal{E}$.
{\it \color{red} if we dont say "for every i,j pairs" ,k should not appear in an inequality which holds for only one task. Also maybe it is better to  cite [21] A.5, because [28] Cor.7 says only the following
$$\|\frac{1}{t}\sum_{i=1}^t \yij\xij - \W^\top\W \mtx{h}^j(\W)\| \le c\sigma\sqrt{\frac{1}{t}\log(\frac{2d}{\delta})}$$}
\fi
\end{lemma}
With the covariance of $y\x$ being bounded by $\sigma^2$, the following inequalities are true \cite{kong2020meta}.
\begin{align*}
    \Eb\left( (\vb^T\cdot (\frac{1}{t}\sum_{i=1}^t \yij\xij - \theta^j))^2\right) &\le \sigma^2 / t,\mbox{~for~} \|\vb\|=1.\\
    \Eb \left(\|\frac{1}{t}\sum_{i=1}^t \yij\xij - \theta^j \|^2\right) &\le \sigma^2d/t.
\end{align*}


\begin{lemma}\label{lem:Zj}
Define
\begin{align*}
    \Zb_j &= (\frac{2}{n_j}\sum_{i=1}^{n_j/2} \yij\xij)(\frac{2}{n_j}\sum_{i={n_j/2}+1}^{n_j} \yij\xij)^\top \\
    &\quad - \Hb^j(\W)(\Hb^j(\W))^\top,
\end{align*}
Then there exists a constant $c$ such that on the event $\mathcal{E}$ (thus with probability $1-\delta$), for all $j=1,...,k$, 
\begin{align}
    \|\Zb_j \| \le \frac{c\sigma^2d}{n_j} \log(\frac{kd}{\delta}). \label{eq:evt}
\end{align}
\end{lemma}

% {\it \color{red} From my understanding we should have 
% $$\|\Zb_j \| \le (Eq A.1 Bound)(Eq. A.1 bound + 2\|\W^\top\W \mtx{h}^j(\W)\|)$$ choosing $t=\dfrac{n_j}{2}$ then we have $$\|\Zb_j \| \le (c\sigma\sqrt{\frac{2}{n_j}\log(\frac{2d}{\delta})})(c\sigma\sqrt{\frac{2}{n_j}\log(\frac{2d}{\delta})} + 2\|\W^\top\W \mtx{h}^j(\W)\|)$$
% This is more or less what you have found, but the difference is k in $\log$ term and d term }



The proof is almost same as \cite{kong2020meta}, the only difference is that we replace the bound in (\cite{kong2020meta} Prop A.1) by \eqref{eq:gauss_bern}. With the similar replacement, we propose the following lemma. 
\begin{lemma}\label{lem:Zj2}
Let $\delta\in(0,1)$. There exists a constant $c$, such that for any $\epsilon\in(0,1)$, and 
\begin{align}
    k = \frac{cd}{n_j}\log^2(\frac{kd}{\delta}) \max\{\frac{1}{\epsilon^2}, \frac{1}{\epsilon} \log(\frac{kd}{\delta})\}, \label{eq:k lb}
\end{align}
with probability $1-\delta$, 
\begin{align*}
    \|\frac{1}{k} \sum_{j=1}^k \Zb_j\| \le \epsilon \sigma^2.
\end{align*}
\end{lemma}
This means that when \eqref{eq:k lb} is true, with probability $1-\delta$,
\begin{align*}
    \left\|\hat \bM - \W^\top\W\left(\frac{1}{k}\sum_{j=1}^k \mtx{h}^j(\W)( \mtx{h}^j(\W))^\top\right)\W^\top\W\right\| \le \epsilon \sigma^2.
\end{align*}
Note that $\bM$ is defined as \[\bM=\W^\top\W\left(\frac{1}{k}\sum_{j=1}^k \mtx{h}^j(\W)( \mtx{h}^j(\W))^\top\right)\W^\top\W.\] So we have proven that with probability $1-\delta$,
\begin{align*}
    \left\|\hat \bM - \bM\right\| \le \epsilon \sigma^2.
\end{align*}

\som{Remind that this is $\hat \bM-\bM$ i.e. $\bM=\text{the messy sum}$}
\end{proof}

\SO{Create a subsection here!!! Reduce the confusion as much as possible, make transitions smooth.}
\subsection{Proof of Theorem \ref{thm:down}}
Now we will prove Theorem \ref{thm:down}. We first review the notations and assumptions mentioned in the theorem.

\subsubsection{Review of Notations and Assumptions}
We define the SVD of $\hat \bM$ as $\hat \Ub \hat\La \hat\Vb^\top$. Let the first $r$ columns of $\hat \Ub$ be $\Ub_r$. 

Let $\hat\W$ be defined as 
\begin{align}
    \hat \W &= \hat \Ub_r \hat \Qb, \label{eq:def W append}\\
    \hat \Qb &= \mathop{\mathrm{argmin}}_{\Qb\in\R^{r\times r}, \Qb\Qb^\top = I}\ \|\hat \Ub_r \Qb - \W\|.
\end{align}
The population cross entropy loss is defined as
\begin{align*}
    &\cLCE(f;\Pb) : \Fc\times \R^{r\times d}\rightarrow \R=\\
    &-\mtx{E}_{\x,y\sim\Pxy} (y\log f(\hat\Pb \x) + (1-y)\log (1 - f(\hat\Pb \x))).
\end{align*}
We will search for a function $f^* \in \Fc$ that minimizes the population cross entropy loss. $\Fc$ is a set of functions satisfying
\begin{enumerate}
    \item For any function $f\in\Fc$, any orthonormal matrix $\Qb\in\R^{r\times r}$ and any matrix $\Pb\in\R^{r\times d}$, there exists $g \in \Fc$ such that $f(\Pb \x) = g(\Qb\Pb \x)$.
    \item $\Fc \subseteq \{f\ |\ \log f,~ \log(1-f)\mathrm{~are~}L\mathrm{~Lipschitz}\}\bigcap \{f\ |\ 0<f(x)<1,\forall x\in\R^r\}$.
\end{enumerate}
We solve for $\hat f$, defined as \begin{align}
    \hat f &= \argmin_{f\in\Fc}\ \cLCE(f;\hat \Ub_r^\top). \label{eq:def f append}
\end{align}
\subsubsection{Proof of Theorem \ref{thm:down}}
Now we are ready to restate Theorem \ref{thm:down} and prove it.
\begin{theorem}\label{thm:popu append}
Based on the definition above, we have that
    \begin{align*}
        \cLCE(\hat f;\hat \Ub_r^\top)  - \cLCE(f^*;\Ub_r^\top) \lesssim L\sqrt{r}\|\hat \W - \W\|.
    \end{align*}
\end{theorem}

\begin{proof}
We learn the model from the following optimization algorithm.
\begin{align*}
    \hat f &= \argmin_{f\in\Fc}\ \cLCE(f;\hat \Ub_r^\top)\\
    &= \argmin_{f\in\Fc}\ -\mtx{E}_{\x,y\sim\Pxy} (y\log f(\hat\Ub_r^\top \x) \\
    &\quad + (1-y)\log (1 - f(\hat\Ub_r^\top \x)))\\
    &= \argmin_{f\in\Fc}\ -\mtx{E}_{\x\sim\gauss} \left(f^*(\W \x)\log f(\hat \Ub_r^\top \x)\right. \\
    & \quad \left. + (1-f^*(\W \x))\log (1 - f(\hat \Ub_r^\top \x)) \right).
\end{align*}
Denote $\tilde f\in\Fc$ as the function such that $\tilde f(\hat \W \x) = \hat f(\hat \Ub_r^\top \x)$. So that $\cLCE(\hat f;\hat \Ub_r^\top) = \cLCE(\tilde f;\hat \W)$. Since $\hat f$ minimizes the cross entropy loss, we have that $\cLCE(\tilde f;\hat \W) \le \cLCE(f^*;\hat \W)$. 

Now we have 
\begin{align*}
    &\quad \cLCE (\tilde f;\hat \W) - \cLCE (f;\W)\\
    &\le \cLCE (f^*;\hat \W) - \cLCE (f^*;\W)\\
    &\le -\mtx{E}_{\x\sim\gauss} \left(f^*(\W \x)(\log f^*(\hat\W \x) -\log f^*(\W \x))\right. \\
    & \quad \left. + (1-f^*(\W \x))(\log (1 - f^*(\hat \W \x)) - \log (1 - f^*(\W \x))) \right)\\
    &\le \mtx{E}_{\x\sim\gauss} L\|(\hat \W - \W)x\|\\
    &\lesssim L\sqrt{r}\|\hat \W - \W\|.
\end{align*}
\end{proof}

\subsection{Proof of Theorem \ref{thm:rade}}
%Now we prove that the upper bound of the error for few-shot learning with finite samples.
We first state Theorem \ref{thm:rade} below.
\begin{theorem}\label{thm:rade app}
    Suppose we generate $n$ sample data for few shot learning solve for $\hat \theta_e$ from \eqref{eq:fstar finite theta}. There exist constants $c>0$, $\delta\in(0,1)$, with probability at least $1 - n^{-c+1} - \delta$, the solution $\hat\theta_e$ and $\hat\Ub_r$ satisfy
    \begin{align*}
        &\quad \mathcal{L} (\hat\theta_e;\hat\Ub_r^\top) - \mathcal{L} (\theta^*;\W) \\
        &\lesssim \frac{ac(\sqrt{r}+\log(n)) (1+ \sqrt{\log(1/\delta)})}{\sqrt{n}} + \sqrt{r}\|\hat \W - \W\|. 
    \end{align*}
\end{theorem}
\begin{proof}
We sketch the proof of Theorem \ref{thm:rade app}. After reviewing the notations, we quote a standard generalization bound via Rademacher complexity in Lemma \ref{lem:rade known}. Then we use the smoothness of the loss function to link to the generalization error of linear functions \eqref{eq:lin rade}, and then use Lemma \ref{lemma:chi-sqr} to compute \eqref{eq:lin rade} and finish the proof.

In few-shot learning, the true parameter is $\theta^*$, and the empirical loss function with finite data is 
\begin{align}
    &\cL_e(\theta;\Pb) : \Fc\times \R^{r\times d}\rightarrow \R= \notag\\
    &-\frac{1}{n}\sum_{i=1}^n (y_i\log\phi (\theta^\top\Pb \x_i) + (1-y_i)\log (1 - \phi(\theta^\top\Pb \x_i))) \label{eq:cLCE finite theta app}
\end{align}
Denote each term in the summation as 
\begin{align*}
    &\quad \cL_e^i(\theta;\Pb) : \Fc\times \R^{r\times d}\rightarrow \R=\notag\\
    &- (y_i\log \phi (\theta^\top\Pb \x_i) + (1-y_i)\log (1 - \phi(\theta^\top\Pb \x_i)))
\end{align*}
We search for the solution by
\begin{align}
    \hat \theta_e &= \argmin_{\theta}\ \cL_e(\theta;\Ub_r^\top),\mbox{~such~that~} \|\theta\|\le a.\label{eq:fstar finite theta app}
\end{align}
In Theorem \ref{thm:popu append}, we know that
\begin{align*}
    \cLCE(\hat \theta;\hat \Ub_r^\top)  - \cLCE(\theta^*;\Ub_r^\top) \lesssim L\sqrt{r}\|\hat \W - \W\|.
\end{align*}
Denote 
    \begin{align}
        M = \max_{\|\theta\|\le a} |\theta^\top \hat\Ub_r^\top\x_i| \le a \max\|\hat\Ub_r^\top\x_i\|.\label{eq:bound_rade}
    \end{align}
We will bound the difference between $\cL$ and $\cL_e$ by Rademacher complexity theory.
\begin{lemma}\label{lem:rade known}
    \cite{mohri2018foundations}
 
    Let $\mscrU$ be the independent random variables uniformly chosen from $\{-1,1\}$.
    Let $\Rc$ be the Rademacher complexity of the logistic functionals defined on the data,
    \begin{align*}
        \Rc &= \frac{1}{n}\Eb_{\epsilon_i\in\mscrU} \sup_{\|\theta\|\le a} \sum_{i=1}^n\epsilon_i\cL_e^i(\theta;\hat\Ub_r^\top) \\
        K &= |\log(\phi(-M))|>\max_i\cL_e^i(\theta;\hat\Ub_r^\top)
    \end{align*}
    %We know $\cL_e^i(\theta;\hat\Ub_r^\top)<K$ with probability at least $1-n^{-c_1+1}$,
    %then for any $\theta$ such that $\|\theta\|\le a$, with probability $1-\delta-n^{-c_1+1}$, we have that 
    with probability $1-\delta$, we have that 
    \begin{align*}
        |\cL_e(\theta;\Ub_r^\top) - \cL(\theta;\Ub_r^\top)| \le \Rc + \frac{\sqrt{\log(1/\delta)}}{\sqrt{n}}K.
    \end{align*}
\end{lemma}
Thus we have that 
\begin{align*}
    |\mathcal{L} (\hat\theta_e;\hat\Ub_r^\top) - \mathcal{L}_e (\hat\theta_e;\hat\Ub_r^\top)| &\le \Rc + \frac{\sqrt{\log(1/\delta)}}{\sqrt{n}}K,\\
    |\mathcal{L} (\hat\theta;\hat\Ub_r^\top) - \mathcal{L}_e (\hat\theta;\hat\Ub_r^\top)| &\le \Rc + \frac{\sqrt{\log(1/\delta)}}{\sqrt{n}}K.
\end{align*}
Because $\hat\theta_e$ minimizes the empirical loss $\mathcal{L}_e$,
\begin{align*}
    \mathcal{L}_e (\hat\theta_e;\hat\Ub_r^\top) \le \mathcal{L}_e (\hat\theta;\hat\Ub_r^\top).
\end{align*}
Thus 
\begin{align}
    \mathcal{L} (\hat\theta_e;\hat\Ub_r^\top) - \mathcal{L} (\hat\theta;\hat\Ub_r^\top) \le 2\left(\Rc + \frac{\sqrt{\log(1/\delta)}}{\sqrt{n}}K\right).\label{eq:emp loss}
\end{align}
So the remaining target is to bound $\Rc$. 

We first denote $\vb_i = \hat\Ub_r^\top \x_i$, so $\vb_i\in\R^r$ and $\vb_i$ are jointly independent standard normal random variables. In binary classification, $\cL_e^i$ is always $1$ Lipschitz in $\theta^\top\vb_i$, the Rademacher complexity can be upper bounded by
\begin{align}\label{eq:lin rade}
    \Rc \le \tilde\Rc := \frac{1}{n}\Eb_{\epsilon_i\in\mscrU} \sup_{\|\theta\|\le a} \sum_{i=1}^n \epsilon_i\theta^\top\vb_i. 
\end{align}
We first refer to the following lemma.
\begin{lemma}\label{lemma:chi-sqr}
    \cite{laurent2000adaptive} Let $c>0$, $X$ follow $\chi_r^2$ distribution, then
    \begin{align*}
        \Pb(X - r \ge 2\sqrt{cr\log n} + 2c\log n) \le n^{-c}.
    \end{align*}
\end{lemma}

For a constant $c>1$, via union bound we have that $\max{\|\vb_i\|^2} \le r + 2\sqrt{cr\log n} + 2c\log n$ for all $i=1,..,n$ with probability $1 - n^{-c+1}$. We use $\max{\|\vb_i\|} \lesssim c(\sqrt{r} + \log(n))$ for simplicity.

Conditioned on this event, we apply the Rademacher complexity for linear model that 
\begin{align}
   \tilde \Rc &\le \frac{\max\|\theta\| \cdot \max\|\vb_i\|}{\sqrt{n}}\\
   &\le \frac{ca(\sqrt{r} + \log(n))}{\sqrt{n}}. \label{eq:tilde Rc}
\end{align}
Combining with \eqref{eq:emp loss} and Theorem \ref{thm:popu append} we get the bound in Theorem \ref{thm:rade app}. We can also bound $M$ in \eqref{eq:bound_rade}.

Finally we will use Lemma \ref{lem:M to K} to bound $M$.
\begin{lemma}\label{lem:M to K}
    Let $M$ be defined as in \eqref{eq:bound_rade}.    
    With probability at least $1 - n^{-c+1}$, we have $M<ac(\sqrt{r} + \log(n))$.
\end{lemma}
Let $\vb_i$ be replaced by $\hat \Ub_r^\top\x_i$ in Lemma \ref{lemma:chi-sqr}, then this directly results from Lemma \ref{lemma:chi-sqr}. Lemma \ref{lem:M to K} bounds $M$, thus bounds $K$ (which is $1$ Lipschitz in $M$) in Lemma \ref{lem:rade known}. After we insert \eqref{eq:tilde Rc} together into Lemma \ref{lem:rade known}, we can get the result in  Theorem \ref{thm:rade}.
% By Lemma \ref{lemma:chi-sqr} we know that for a constant $c>2$, we have  $\max{\|\hat\Ub_r^\top\x_i\|} \le c(\sqrt{r} + \log(n))$ for all $i=1,..,n$ with probability $1 - n^{-c+1}$. So with probability at least $1 - n^{-c+1}$, we have $M<ac(\sqrt{r} + \log(n))$.
\end{proof}



==> s_prob.tex <==
\setlength{\topsep}{0.25em}
\newcommand{\xij}{{\x_{i,j}}}
\newcommand{\xijt}{{\x_{i,j}^\top}}
\newcommand{\yij}{{y_{i,j}}}

\section{Problem Formulation}\label{s:prob}
% {\color{red} YS: a paragraph for notation?}
The meta-learning setup that will be considered in this work consists of two phases: (i) meta-training: prior tasks are used to learn a good representation and (ii) few-shot learning: the new task is learned with few samples.
%\som{Is meta-train/test standard and correct phrases?} 
%{\mf better not to use the meta-train and meta-test phrases if we don't need to} 
In the meta-training phase, we learn the low dimensional space spanned by parameters. In the few-shot learning phase, we use the subspace to learn the model of a new task ideally with few samples.

In the first phase, there are multiple tasks to infer from, each with its own distribution. We consider a realizable model where the input and label is associated via a labeling function. One accesses batches of data, each of whom is collected from a task, however we may not know which task it comes from. We make this setup more precise using the following definitions. Below, the ground-truth representation will be denoted by a matrix $\W\in\R^{r\times d}$ row space of which corresponds to the subspace of interest.

%\som{Use $n_j$ for sample size rather than $t_j$ (at least for training)}
\begin{definition} \label{def:task}
\textbf{Meta-training data.} Fix a matrix $\W\in\R^{r\times d}$ satisfying $\W\W^T=\Iden$. The $j$-th task is associated with function $f^j: \R^r\rightarrow \R$. Given input $\x$, the label $y$ is distributed as $p_j(y|\x)=p_j(y|\W\x)$\footnote{In words, the label only depends on the relevant features induced by $\W$.} and the expectation satisfies $\mtx{E}(y) = f^j(\W\x)$.
%{\mf give properties like domain and range of $f$ here, first time it appears.}
Suppose there are $n_j$ samples from the $j$-th task sampled i.i.d.~from this distribution and we denote the dataset $\Sc^j = (\xij, \yij)_{i=1}^{n_j}$. Define the full meta-training dataset to be $\Sc = \bigcup_{j=1}^k\Sc^j$.
\end{definition}
Here, $f^j$ is allowed to be any Lipschitz nonlinear function, i.e., a neural network\footnote{In our theoretical results, we treat $f$ as a general linear function, and in experiments we will use a neural network with a specific structure.}.


%In the multi-task problem, there are a collection of tasks in the meta-training phase, which is defined below.


\iffalse
\begin{definition}\label{def:task dis}\som{I don't think we should use a distribution early on.}
\textbf{Low rank task distribution.} There are in total $k$ tasks. Each training task is associated with a parameter vector $\bt^j\in\R^d$ for $j=1,...,k$.
{\mf right now we're just setting the notation---additional assumptions like definition 2.2 on random features should come later.}
These are generated i.i.d. from a Gaussian distribution $\mathcal{N}(0, \bSi)$. Let $\la_i$ be the $i$-th eigenvalue of $\bSi$ with decreasing order. For low rank parameters, we assume that $\la_{r+1} = 0$. We call $r$ as the effective dimension of parameters.
\end{definition}



\begin{definition} \label{def:task}
\textbf{Meta-training data.} The $j$-th task is associated with parameter $\bt^j\in\R^d$. 
%For any parameter $\bt$, one can collect data from it. 
Suppose there are $n_j$ data from the $j$-th task, we call the dataset $\Sc^j = \{(\xij, \yij)\ |\ i=1,...,n_j\}$. Here $\xij\in\R^d$, $\yij\in\R$. $\xij$, $\yij$ satisfy $\mtx{E}(\yij) = f(\xijt\bt^j)$ for some function $f$. Let the whole meta-training dataset be $\Sc = \bigcup_{j=1,...,k}\Sc^j$. {\mf repeated}
\end{definition}

%\noindent\textbf{:}

\begin{definition} \label{def:data_gen}
\textbf{Data generation.} We assume that there are $k$ binary classification tasks, the $j$-th associated with $\bt^j$. The data $\Sc^j$ is generated by $\xij = \bz / \|\bz\|$ and $\bz \sim \mathcal{N}(0, I)$, $\bz$ is generated independently. Denote the distribution of $\xij$ as $\mathscr{P}_x$.
%The labels $\yij$ satisfy
%$\mtx{E}(\yij|\xij, \bt^j) = f(\xijt\bt^j)$ for some Lipschitz function $f:\R\rightarrow \R$. We propose two examples below.
\end{definition}
%{\color{blue} Do we need to normalize $x$? Just for citing the result in \cite{kong2020meta}, they use Bernstein so they have to use bounded rv. In principle unbounded subGaussian works.}
\fi


\begin{definition} \label{def:bin_class}
\textbf{Binary classification.} Suppose $f^j$ takes values over $[0,1]$,
%{\it\color{red}{Is it [0,1] ?}}. The labels $\yij$ are generated as 
\begin{align*}
    \yij = 
     \begin{cases}
       \text{1,} &{\mbox{with probability } f^j(\W \xij),}\\
       \text{0,} &{\mbox{with probability } 1-f^j(\W\xij).}\\
     \end{cases}
\end{align*}
%Here $f^j(a)\in[0,1]$ for all $a\in[-1,1]$, and the event that $f(a) = 0$ is not true with probability $1$ with respect to Lebesgue measure on $[-1,1]$\footnote{In other words, $f$ is not a constant $0$ function.}.
\end{definition}

\begin{definition}\label{def:GLM}
\noindent\textbf{Generalized linear models (GLM)} (which include logistic/linear regression) can be modeled by choosing $f^j$ to be parameterized by a vector $\bt_j\in\R^r$ and a link function $\phi:\R\rightarrow\R$ as $f^j(\W \xij) := \phi(\bt_j^T\W\xij )$.

\end{definition}
%for $\bt_j\in\R^r$, $\phi$ is a function mapping from $\R$ to $(0,1)$.

% Denote the distribution of $\x,y$ as $\mathscr{P}_{x,y}$.
%\begin{definition}\label{def:nn}
%\textbf{Non-linear regression.} More generally, for $\bt^j\in\R^{r\times d}$, the labels $\yij$ are generated as
%\begin{align*}
%    \yij = f^j(\W\xij) + \epsilon,
%\end{align*}
%$\epsilon$ is a zero mean bounded random variable. 
%\end{definition}

When the dimension of the span of parameters is small, \cite{kong2020meta} performs a dimension reduction algorithm to find the low-dimensional subspace that the parameters span. This is done by selecting the top eigenvectors of the covariance estimate of the cross-correlation between input and labels.
\begin{definition}\label{def:mom}
\textbf{Moment estimator of covariance.} We define the covariance estimator as
\begin{subequations}\label{eq:hatM}
\begin{align}
\hat\bM &= \mathop{\Scale[1.8]{\sum}}_{j=1}^k \frac{2}{n_j^2}\left[(\sum_{i=1}^{n_j/2} \yij\xij) (\sum_{i=n_j/2+1}^{n_j} \yij\xij)^\top \right.\\
&\quad\quad\quad\quad \left. +  ( \sum_{i=n_j/2+1}^{n_j} \yij\xij) ( \sum_{i=1}^{n_j/2} \yij\xij)^\top\right].\nonumber
\end{align}
\end{subequations}
\end{definition}
\noindent\textbf{Subspace estimation.} 
To estimate the subspace $\W$, we use rank-$r$ approximation of $\hat \bM$ to retrieve its principal eigenvector subspace. 
Let $\hat\Ub \hat \La \hat \Ub^\top$ be the eigen-decomposition of $\hat \bM$. Denote $\hat \la_j$ as the $j$th eigenvalue of $\hat \La$. Let $\hat\Ub_r$ be the first $r$ columns of $\hat\Ub$, thus the rank-$r$ approximation is $\hat\bM_r = \hat\Ub_r \mathrm{diag}(\hat \la_{1},...,\hat\la_{r}) \hat \Ub_r^\top$. In the next section, we will prove that the range of $\hat \Ub$ is close to the row space of $\W$.

%{\color{blue} No need to put an algorithm here. If we have a bound for downstream task as well we can fill up the whole procedure.}

%Now we propose the algorithm that accomplishes the subspace retrieval process above. 

In Algorithm \ref{algo:1}, the output $\hat\Ub_r$ is the estimator of the task subspace $\W$. $\hat\Ub_r$ is used as a training step for the few-shot learning phase. For the new task, we search for the function $f^*$ that minimizes the population loss. We shall provide an instructive analysis for the cross-entropy loss, which is usually employed for classification tasks.

\so{Currently, cross-entropy comes out of nowhere. For using cross-ent, label has to be discrete. It cannot be an arbitrary nonlinear function. Overall, we need to do one of the followings:\\
 Option 1: Do the analysis for a Lipschitz loss function for which cross-entropy is a special case.\\
 Option 2: Let us just say that for few-shot phase, we focus on classification and study cross-entropy. Clearly state label is discrete 0-1.}
\begin{definition}\label{def: test}
\textbf{Few-shot classification (Population).} In the few-shot learning phase, suppose $\x,y\sim\Pxy$ satisfy $\mtx{E}(y|\x) = f^*(\W\x)$. Let $\Fc$ be a family of functions as the search space for few-shot learning model. 
Let $\cLCE: \Fc\times \R^{r\times d}\rightarrow \R$ be population cross-entropy loss, defined as 
\begin{align}
    \cLCE(f;\Pb)=-\mtx{E}_{\Pxy} (&y\log f(\Pb \x)\label{eq:cLCE}\\
   &+ (1-y)\log (1 - f(\Pb \x))) \nonumber.
\end{align}
\so{Following my comment above, for cross-ent, clearly $0\leq f\leq 1$. This has to be specified in the definition.}

We search for the solution induced by $\hat{\Ub}_r$ by
\begin{align}
    \hat f &= \argmin_{f\in\Fc}\ \cLCE(f;\hat{\Ub}_r^\top)\label{eq:fstar}
\end{align}
%If $\Pb$ is known, we use $\cLCE(f(\Pb x))$ as an equivalent way of representing $\cLCE(f;\Pb)$.
\end{definition}
Observe that, without representation learning, one has to search for both $f$ and $\Pb$. However with representation learning, we fix $\Pb=\hat{\Ub}_r$ and only search for $f$.
\begin{remark}\label{rem:logistic}
For the GLM Definition \ref{def:GLM}, we can choose $\Fc$ to be the $\ell_2$ norm constrained functions for some $a\leq\infty$% the set of functions $f$ satisfying
% {\color{red} YS: I want to say $\Fc = \phi\circ\bt\circ(\mathrm{variable})$}
\begin{align}
    \Fc = \{\x\rightarrow \phi(\bt^T\x)~\big|~\|\bt\|_2 \le a,~\bt\in\R^r\}, \label{eq:Fcbin}
\end{align}
Let the new data be generated with $f^*(\W\x) = \phi({\bt^*}^\top\W\x)$ for some ground-truth parameter $\bt^*$. We use $\cLCE(\bt;\Pb)$ to denote the cross-entropy loss in this setting. $\hat f$ (parameterized by $\hat{\bt}$) is given by
\begin{align}
    \hat \bt &= \argmin_{\bt}\ \cLCE(\bt;\hat \Ub_r^\top ),\mbox{~such~that~} \|\bt\| \le a. \label{eq:fstarbin}
\end{align}
\end{remark}


\iffalse
\begin{definition}\label{def: test finite}
\textbf{Finite sample few-shot learning.} In the few-shot learning phase, there are in total $n$ samples, and suppose 
$\x_i\in\R^d$ are generated independently, following standard normal distribution, $y_i\in\R$, for $i=1,...,n$. $\x_i$, $y_i$ satisfy $\mtx{E}(y_i|\x_i) = f^*(\W\x_i)$. Lef $\Fc$ be a family of functions as the search space for few-shot activation function. 
Let $\cL_e$ be empirical cross entropy loss, defined as 
\begin{align}
    &\cL_e(f;\Pb) : \Fc\times \R^{r\times d}\rightarrow \R= \notag\\
    &-\frac{1}{n}\sum_{i=1}^n (y_i\log f(\Pb \x_i) + (1-y_i)\log (1 - f(\Pb \x_i))) \label{eq:cLCE finite}
\end{align}
We search for the solution by
\begin{align}
    \hat f_e &= \argmin_{f\in\Fc}\ \cL_e(f;\Ub_r^\top)\label{eq:fstar finite}
\end{align}

\end{definition}
\fi
% and suppose $\x_i\in\R^d$ are generated independently, following standard normal distribution, $y_i\in\R$, for $i=1,...,n$.
\begin{definition}\label{def: test finite}
\textbf{Few-shot learning (Finite sample GLM).} Suppose there are in total $n$ samples for new task $(\x_i,y_i)_{i=1}^n$ and $(\x_i,y_i)$ satisfies $\mtx{E}(y_i|\x_i) = f^*(\W\x_i)$. Lef $\Fc$ be a family of functions for few-shot learning phase. We consider the setup of Remark \ref{rem:logistic}, where $\phi$ is the logistic function. 
%: \Fc\times \R^{r\times d}\rightarrow \R= \notag\\
\begin{align}
    \cL_e(\bt;\Pb)=-\frac{1}{n}\sum_{i=1}^n (&y_i\log(\phi (\bt^\top\Pb \x_i))\label{eq:cLCE finite theta}\\
    &+ (1-y_i)\log (1 - \phi(\bt^\top\Pb \x_i))).\nonumber 
\end{align}
Given an $\ell_2$-norm constraint $a\leq \infty$, the empirical risk minimizer (ERM) is defined as follows
\begin{align}
    \hat \bt_e &= \argmin_{\bt}\ \cL_e(\bt;\Ub_r^\top)\quad\text{such~that}\quad\|\bt\|_2\le a.\label{eq:fstar finite theta}
\end{align}
\end{definition}


\begin{algorithm}[t!]
\caption{Meta-training and Few-shot Learning}\label{algo:1}
\begin{algorithmic}
% with $k$ tasks, the size of data of the $j$-th task has size $n_j$. Dimension $d$. Effective dimension $r$. Set of functions $\Fc$.
\REQUIRE {Dataset $\mathcal{S}$, representation size $r$, function space $\Fc$}
\STATE{Compute $\hat \bM$ via method-of-moments \eqref{eq:hatM}.}
\STATE{Rank $r$ approximation:\\
$\quad\hat\bM_r \leftarrow \hat\Ub_r \mathrm{diag}(\hat \La_{1,1},...,\hat\La_{r,r}) \hat \Ub_r^\top$.}
\STATE{Either~$\hat f \leftarrow \argmin_{f\in\Fc}\ \cLCE(f;\Ub_r^\top) $. $\cLCE$ is defined as \eqref{eq:cLCE}.}
\STATE{Or~~~~~~$\hat f_e \leftarrow \argmin_{f\in\Fc}\ \cL_e(f;\Ub_r^\top) $. $\cL_e$ is defined as \eqref{eq:cLCE finite theta}}
\RETURN{$\hat\Ub_r$ and $\hat f$ or $\hat f_e$.}
\end{algorithmic}
\end{algorithm}%\vspace{-10pt}


==> s_prob_2.tex <==
\setlength{\topsep}{0.25em}
\newcommand{\xij}{{\x_{i,j}}}
\newcommand{\xijt}{{\x_{i,j}^\top}}
\newcommand{\yij}{{y_{i,j}}}

\section{Problem Formulation}\label{s:prob}
% {\color{red} YS: a paragraph for notation?}
\vspace{-0.1cm}
The meta-learning setup that will be considered in this work consists of two phases: (i) meta-training: prior tasks are used to learn a good representation and (ii) few-shot learning: the new task is learned with few samples.
%\som{Is meta-train/test standard and correct phrases?} 
%{\mf better not to use the meta-train and meta-test phrases if we don't need to} 
In the meta-training phase, we learn the low dimensional space spanned by parameters. In the few-shot learning phase, we use the subspace to learn the model of a new task ideally with few samples.

In the first phase, there are multiple task vectors to infer from.%, each with its own distribution. 
We consider a realizable model where the input and label is associated via a labeling function. One accesses batches of data, each of whom is collected from a task.
%, however we may not know which task it comes from. 
%We make this setup more precise using the following definitions. 
Below, we denote the ground-truth representation by a matrix $\W\in\R^{r\times d}$ whose row space corresponds to the subspace of interest.

%\som{Use $n_j$ for sample size rather than $t_j$ (at least for training)}
\begin{definition} \label{def:task}
\textbf{Meta-training data.} Fix a matrix $\W\in\R^{r\times d}$ satisfying $\W\W^T=\Iden$. The $j$-th task is associated with function $f^j: \R^r\rightarrow \R$. Given input $\x\in\R^{d}$, the label $y$ is distributed as $p_j(y|\x)=p_j(y|\W\x)$\footnote{In words, the label only depends on the relevant features induced by $\W$.} and the expectation satisfies $\mtx{E}(y) = f^j(\W\x)$.
%{\mf give properties like domain and range of $f$ here, first time it appears.}
Suppose there are $n_j$ samples from the $j$-th task sampled i.i.d.~from this distribution and we denote the dataset $\Sc^j = (\xij, \yij)_{i=1}^{n_j}$. Define the full meta-training dataset to be $\Sc = \bigcup_{j=1}^k\Sc^j$.
\end{definition}
Here, $f^j$ is allowed to be any Lipschitz nonlinear function, i.e., a neural network\footnote{In our theoretical results, we treat $f$ as a general linear function, and in experiments we will use a neural network with a specific structure.}.


%In the multi-task problem, there are a collection of tasks in the meta-training phase, which is defined below.


\iffalse
\begin{definition}\label{def:task dis}
%\som{I don't think we should use a distribution early on.}
\textbf{Low rank task distribution.} There are in total $k$ tasks. Each training task is associated with a parameter vector $\bt^j\in\R^d$ for $j=1,...,k$.
{\mf right now we're just setting the notation---additional assumptions like definition 2.2 on random features should come later.}
These are generated i.i.d. from a Gaussian distribution $\mathcal{N}(0, \bSi)$. Let $\la_i$ be the $i$-th eigenvalue of $\bSi$ with decreasing order. For low rank parameters, we assume that $\la_{r+1} = 0$. We call $r$ as the effective dimension of parameters.
\end{definition}



\begin{definition} \label{def:task}
\textbf{Meta-training data.} The $j$-th task is associated with parameter $\bt^j\in\R^d$. 
%For any parameter $\bt$, one can collect data from it. 
Suppose there are $n_j$ data from the $j$-th task, we call the dataset $\Sc^j = \{(\xij, \yij)\ |\ i=1,...,n_j\}$. Here $\xij\in\R^d$, $\yij\in\R$. $\xij$, $\yij$ satisfy $\mtx{E}(\yij) = f(\xijt\bt^j)$ for some function $f$. Let the whole meta-training dataset be $\Sc = \bigcup_{j=1,...,k}\Sc^j$. {\mf repeated}
\end{definition}

%\noindent\textbf{:}

\begin{definition} \label{def:data_gen}
\textbf{Data generation.} We assume that there are $k$ binary classification tasks, the $j$-th associated with $\bt^j$. The data $\Sc^j$ is generated by $\xij = \bz / \|\bz\|$ and $\bz \sim \mathcal{N}(0, I)$, $\bz$ is generated independently. Denote the distribution of $\xij$ as $\mathscr{P}_x$.
%The labels $\yij$ satisfy
%$\mtx{E}(\yij|\xij, \bt^j) = f(\xijt\bt^j)$ for some Lipschitz function $f:\R\rightarrow \R$. We propose two examples below.
\end{definition}
%{\color{blue} Do we need to normalize $x$? Just for citing the result in \cite{kong2020meta}, they use Bernstein so they have to use bounded rv. In principle unbounded subGaussian works.}
\fi


\begin{definition} \label{def:bin_class}
\textbf{Binary classification.} Suppose $f^j$ takes values over $[0,1]$,
%{\it\color{red}{Is it [0,1] ?}}. The labels $\yij$ are generated as 
\begin{align*}
    \yij = 
     \begin{cases}
       \text{1,} &{\mbox{with probability } f^j(\W \xij),}\\
       \text{0,} &{\mbox{with probability } 1-f^j(\W\xij).}\\
     \end{cases}
\end{align*}
%Here $f^j(a)\in[0,1]$ for all $a\in[-1,1]$, and the event that $f(a) = 0$ is not true with probability $1$ with respect to Lebesgue measure on $[-1,1]$\footnote{In other words, $f$ is not a constant $0$ function.}.
\end{definition}

\begin{definition}\label{def:GLM}
\noindent\textbf{Generalized linear models (GLM)} (which include logistic/linear regression) can be modeled by choosing $f^j$ to be parameterized by a vector $\bt_j\in\R^r$ and a link function $\phi:\R\rightarrow\R$ as $f^j(\W \xij) := \phi(\bt_j^T\W\xij )$.

\end{definition}
%for $\bt_j\in\R^r$, $\phi$ is a function mapping from $\R$ to $(0,1)$.

% Denote the distribution of $\x,y$ as $\mathscr{P}_{x,y}$.
%\begin{definition}\label{def:nn}
%\textbf{Non-linear regression.} More generally, for $\bt^j\in\R^{r\times d}$, the labels $\yij$ are generated as
%\begin{align*}
%    \yij = f^j(\W\xij) + \epsilon,
%\end{align*}
%$\epsilon$ is a zero mean bounded random variable. 
%\end{definition}

When the dimension of the span of parameters is small, \cite{kong2020meta} performs a dimension reduction algorithm to find the low-dimensional subspace that the parameters span. This is done by selecting the top eigenvectors of the covariance estimate of the cross-correlation between input and labels.
\begin{definition}\label{def:mom}
\textbf{Moment estimator of covariance.} We define the covariance estimator as
\begin{equation}\label{eq:hatM}
\begin{split}
\hat\bM &= \mathop{\Scale[1.8]{\sum}}_{j=1}^k \frac{2}{n_j^2}\left[(\sum_{i=1}^{n_j/2} \yij\xij) (\sum_{i=n_j/2+1}^{n_j} \yij\xij)^\top \right.\\
&\quad\quad\quad\quad \left. +  ( \sum_{i=n_j/2+1}^{n_j} \yij\xij) ( \sum_{i=1}^{n_j/2} \yij\xij)^\top\right].
\end{split}
\end{equation}
Define
\begin{align*}
    &\mtx{h}^j(\W): \R^{r\times d} \rightarrow \R^d = \mtx{E}_{\x}[f^j(\W \x)\x]\\
    &\bM := \W^\top\W\left(\frac{1}{k}\sum_{j=1}^k \mtx{h}^j(\W)( \mtx{h}^j(\W))^\top\right)\W^\top\W.
\end{align*}
\end{definition}
We will prove that $\hat\bM$ is a finite sample estimate of $\bM$.
\noindent\textbf{Subspace estimation.} 
To estimate the subspace $\W$, we use rank-$r$ approximation of $\hat \bM$ to retrieve its principal eigenvector subspace. 
Let $\hat\Ub \hat \La \hat \Ub^\top$ be the eigen-decomposition of $\hat \bM$. Denote $\hat \la_j$ as the $j$th eigenvalue of $\hat \La$. Let $\hat\Ub_r$ be the first $r$ columns of $\hat\Ub$, thus the rank-$r$ approximation is $\hat\bM_r = \hat\Ub_r \mathrm{diag}(\hat \la_{1},...,\hat\la_{r}) \hat \Ub_r^\top$. In the next section, we will prove that the range of $\hat \Ub$ is close to the row space of $\W$.

%{\color{blue} No need to put an algorithm here. If we have a bound for downstream task as well we can fill up the whole procedure.}

%Now we propose the algorithm that accomplishes the subspace retrieval process above. 

In Algorithm \ref{algo:1}, the output $\hat\Ub_r$ is the estimator of the task subspace $\W$. $\hat\Ub_r$ is used as a training step for the few-shot learning phase. For the new task, we search for the function $f^*$ that minimizes the population loss. We shall provide an instructive analysis for a general class of functional family and loss.
\begin{assumption}\label{ass:F}
$\Fc$ is a set of functions satisfying: For any function $f\in\Fc$, any orthonormal matrix $\Qb\in\R^{r\times r}$ and any representation matrix $\Pb\in\R^{r\times d}$, there exists $g \in \Fc$ such that $f(\Pb \x) = g(\Qb\Pb \x)$.
%\begin{enumerate}
%    \item For any function $f\in\Fc$, any orthonormal matrix $\Qb\in\R^{r\times r}$ and any matrix $\Pb\in\R^{r\times d}$, there exists $g \in \Fc$ such that $f(\Pb \x) = g(\Qb\Pb \x)$.
%    \item $\Fc \subseteq \{f\ |\ \log f,~ \log(1-f)\mathrm{~are~}L\mathrm{~Lipschitz}\}\bigcap \{f\ |\ 0<f(x)<1,\forall x\in\R^r\}$.
%\end{enumerate}
\end{assumption}
\ys{In this assumption, we basically mean that the $\Fc$ is invariant with orthonormal rotation $\Qb$. In other words, we only need to find the $r$ dimensional row space $\mathrm{row}(\Pb)$ (to project the features onto it as a low dimensional representation), and don't worry the exact matrix $\Pb$ itself.

Let us introduce population risk $\cL$ and empirical risk $\cL_e$ based on any single loss function between model prediction and true label.}
\begin{align*}
&\cL(f;\Pb) = \mtx{E}_{\Pxy}\cLoss(f(\Pb \x),y)\\
&\cL_e(f;\Pb) = \frac{1}{n}\sum_{i=1}^n\cLoss(f(\Pb \x_i),y_i).
\end{align*}
We make the following assumption on the population risk.
\begin{assumption}\label{ass:L}
Suppose population loss $\cL$ and empirical loss $\cL_e$ satisfy the following assumptions:
\begin{enumerate}[itemsep=-0.1em,topsep=0.3em]
    %\item $\cL$ has the form $\cL(f;\Pb) = \mtx{E}_{\Pxy}\cL(f(\Pb \x),y)$.
    %$\cL_e$ has the form $\cL_e(f;\Pb) = \frac{1}{n}\sum_{i=1}^n\cL(f(\Pb \x_i),y_i)$.
    \item $\cL$ is $L$ Lipschitz in $\Pb \x$.
    \item $\min_{\Pb}\cL(f;\Pb) = \cL(f;\W)$.
\end{enumerate}
\end{assumption}
\noindent\textbf{Example:} Suppose $f$ is an $L$-Lipschitz function with range in $(0,1)$ \ys{and the true labels $y_i$ are from $\{0,1\}$.} The cross entropy function satisfies the assumptions.
\begin{align}
    \cLCE(f;\Pb)=-\mtx{E}_{\Pxy} (&y\log f(\Pb \x)\label{eq:cLCE}\\
   &+ (1-y)\log (1 - f(\Pb \x))) \nonumber.\\
   \cL_e(f;\Pb)=-\frac{1}{n}\sum_{i=1}^n (&y_i\log(f(\Pb \x_i))\label{eq:cLCE finite theta}\\
    &+ (1-y_i)\log (1 - f(\Pb \x_i))).\nonumber 
   %\cL_e(\bt;\Pb)=-\frac{1}{n}\sum_{i=1}^n (&y_i\log(\phi (\bt^\top\Pb \x_i))\label{eq:cLCE finite theta}\\
    %&+ (1-y_i)\log (1 - \phi(\bt^\top\Pb \x_i))).\nonumber 
\end{align}
\ys{With an abuse of notation, we can define the loss with respect to parameterization of the function $f$. For example, if we use the model in Def. \ref{def:GLM}, then we can write the empirical loss as 
\begin{align}
    \cL_e(\bt;\Pb)=-\frac{1}{n}\sum_{i=1}^n (&y_i\log(\phi (\bt^\top\Pb \x_i))\\%\label{eq:cLCE finite theta}\\
    &+ (1-y_i)\log (1 - \phi(\bt^\top\Pb \x_i))).\nonumber
\end{align}
}

% the cross-entropy loss, which is usually employed for classification tasks.
\iffalse
\so{Currently, cross-entropy comes out of nowhere. For using cross-ent, label has to be discrete. It cannot be an arbitrary nonlinear function. Overall, we need to do one of the followings:\\
 Option 1: Do the analysis for a Lipschitz loss function for which cross-entropy is a special case.\\
 Option 2: Let us just say that for few-shot phase, we focus on classification and study cross-entropy. Clearly state label is discrete 0-1.}
 \fi
\begin{definition}\label{def: test}
\textbf{Few-shot classification (Population).} In the few-shot learning phase, suppose $\x,y\sim\Pxy$ satisfy $\mtx{E}[y~|~\x] = f^*(\W\x)$. Let $\Fc$ be a family of functions as the search space for few-shot learning model. 
Let Assumptions \ref{ass:F} and \ref{ass:L} hold. We search for the solution induced by $\hat{\Ub}_r$ by
\begin{align}
    \hat f &= \argmin_{f\in\Fc}\ \cLCE(f;\hat{\Ub}_r^\top)\label{eq:fstar}
\end{align}
%$\cLCE: \Fc\times \R^{r\times d}\rightarrow \R$ be population cross-entropy loss, defined as 
%\begin{align}
%    \cLCE(f;\Pb)=-\mtx{E}_{\Pxy} (&y\log f(\Pb \x)\label{eq:cLCE}\\
%   &+ (1-y)\log (1 - f(\Pb \x))) \nonumber.
%\end{align}

\iffalse
\so{Following my comment above, for cross-ent, clearly $0\leq f\leq 1$. This has to be specified in the definition.}
\fi


%If $\Pb$ is known, we use $\cLCE(f(\Pb x))$ as an equivalent way of representing $\cLCE(f;\Pb)$.
\end{definition}
Observe that, without representation learning, one has to search for both $f$ and $\W$. However with representation learning, we use $\hat{\Ub}_r^\top$ as the representation matrix and only search for $f$.
\begin{remark}\label{rem:logistic}
For the GLM Definition \ref{def:GLM}, we can choose $\Fc$ to be the $\ell_2$ norm constrained functions for some $a\leq\infty$% the set of functions $f$ satisfying
% {\color{red} YS: I want to say $\Fc = \phi\circ\bt\circ(\mathrm{variable})$}
\begin{align}
    \Fc = \{\x\rightarrow \phi(\bt^T\x)~\big|~\|\bt\|_2 \le a,~\bt\in\R^r\}, \label{eq:Fcbin}
\end{align}
Let the new data be generated with $f^*(\W\x) = \phi({\bt^*}^\top\W\x)$ for some ground-truth parameter $\bt^*$. We use $\cLCE(\bt;\Pb)$ to denote the cross-entropy loss in this setting. $\hat f$ (parameterized by $\hat{\bt}$) is given by
\begin{align}
    \hat \bt &= \argmin_{\bt}\ \cLCE(\bt;\hat \Ub_r^\top ),\mbox{~such~that~} \|\bt\| \le a. \label{eq:fstarbin}
\end{align}
\end{remark}


\iffalse
\begin{definition}\label{def: test finite}
\textbf{Finite sample few-shot learning.} In the few-shot learning phase, there are in total $n$ samples, and suppose 
$\x_i\in\R^d$ are generated independently, following standard normal distribution, $y_i\in\R$, for $i=1,...,n$. $\x_i$, $y_i$ satisfy $\mtx{E}(y_i|\x_i) = f^*(\W\x_i)$. Lef $\Fc$ be a family of functions as the search space for few-shot activation function. 
Let $\cL_e$ be empirical loss, satisfying Assumptions \ref{ass:F} and \ref{ass:L}.

%defined as 
%\begin{align}
%    &\cL_e(f;\Pb) : \Fc\times \R^{r\times d}\rightarrow \R= \notag\\
%    &-\frac{1}{n}\sum_{i=1}^n (y_i\log f(\Pb \x_i) + (1-y_i)\log (1 - f(\Pb \x_i))) \label{eq:cLCE finite}
%\end{align}
We search for the solution by
\begin{align}
    \hat f_e &= \argmin_{f\in\Fc}\ \cL_e(f;\Ub_r^\top)\label{eq:fstar finite}
\end{align}

\end{definition}
\fi
% and suppose $\x_i\in\R^d$ are generated independently, following standard normal distribution, $y_i\in\R$, for $i=1,...,n$.
\begin{definition}\label{def: test finite}
\textbf{Few-shot learning (Finite sample GLM).} Suppose there are $n$ samples for new task $(\x_i,y_i)_{i=1}^n$ and $(\x_i,y_i)$ satisfies $\mtx{E}(y_i|\x_i) = f^*(\W\x_i)$. 
%Let $\Fc$ be a family of functions for few-shot learning phase. 
Let $\cL_e$ be empirical loss, satisfying Assumptions \ref{ass:F} and \ref{ass:L}.
%We consider the setup of Remark \ref{rem:logistic}, where $\phi$ is the logistic function. 
%: \Fc\times \R^{r\times d}\rightarrow \R= \notag\\
%\begin{align}
%    \cL_e(\bt;\Pb)=-\frac{1}{n}\sum_{i=1}^n (&y_i\log(\phi (\bt^\top\Pb \x_i))\label{eq:cLCE finite theta}\\
%    &+ (1-y_i)\log (1 - \phi(\bt^\top\Pb \x_i))).\nonumber 
%\end{align}
Given norm constraint $a\leq \infty$, the empirical risk minimizer (ERM) is defined as
\begin{align}
    \hat \bt_e &= \argmin_{\bt}\ \cL_e(\bt;\hat\Ub_r^\top)\quad\text{such~that}\quad\|\bt\|_2\le a.\label{eq:fstar finite theta}
\end{align}
\end{definition}


\setlength{\textfloatsep}{.5em}
\begin{algorithm}[t!]
\caption{Meta-training and Few-shot Learning}\label{algo:1}
\begin{algorithmic}
% with $k$ tasks, the size of data of the $j$-th task has size $n_j$. Dimension $d$. Effective dimension $r$. Set of functions $\Fc$.
\REQUIRE {Dataset $\mathcal{S}$, representation size $r$, function space $\Fc$}
\STATE{Compute $\hat \bM$ via method-of-moments \eqref{eq:hatM}.}
\STATE{Rank $r$ approximation:\\
$\quad\hat\bM_r \leftarrow \hat\Ub_r \mathrm{diag}(\hat \La_{1,1},...,\hat\La_{r,r}) \hat \Ub_r^\top$.}
\STATE{Either~$\hat f \leftarrow \argmin_{f\in\Fc}\ \cLCE(f;\Ub_r^\top) $.
%$\cLCE$ is defined as \eqref{eq:cLCE}.
}
\STATE{Or~~~~~~$\hat f_e \leftarrow \argmin_{f\in\Fc}\ \cL_e(f;\Ub_r^\top) $.
%$\cL_e$ is defined as \eqref{eq:cLCE finite theta}
}
\RETURN{$\hat\Ub_r$ and $\hat f$ or $\hat f_e$.}
\end{algorithmic}
\end{algorithm}%\vspace{-10pt}

